Parameterised Multiparty Session Types

For many application-level distributed protocols and parallel algorithms, the set of participants, the number of messages or the interaction structure are only known at run-time. This paper proposes a dependent type theory for multiparty sessions which can statically guarantee type-safe, deadlock-free multiparty interactions among processes whose specifications are parameterised by indices. We use the primitive recursion operator from G\"odel's System T to express a wide range of communication patterns while keeping type checking decidable. To type individual distributed processes, a parameterised global type is projected onto a generic generator which represents a class of all possible end-point types. We prove the termination of the type-checking algorithm in the full system with both multiparty session types and recursive types. We illustrate our type theory through non-trivial programming and verification examples taken from parallel algorithms and Web services usecases.

==> all_syntax.tex <==
\subsection{Process syntax}
\label{sec:usersyntax}

\input{fig_all_syntax}

%\paragraph{\bf Syntax}
The syntax of expressions and processes is given in Figure~\ref{fig:syntax},
extended from \cite{BettiniCDLDY08LONG}, adding the primitive recursion operator and
a new request process.  Identifiers $\Iu$ can be variables $\x$ or
channel names $\Ia$. Values $\Iv$ are either channels $\Ia$ or natural numbers $\n$.
% or boolean $\true,\false$.
Expressions $e$ are built out of indices
$\tii$, values $\Iv$, variables $\x$, session end points (for delegation) and
operations over expressions.
Participants $\pp$ can include indices which 
are substituted by values and evaluated during reductions (see 
the next subsection). 
%constants (\Alice, \Bob, ...) that can
%be indexed by one or more parameters, \eg $\Worker[5][\i+1]$.
%Processes follow a standard syntax for multiparty session-based
% calculi.  
In processes, sessions are asynchronously initiated by $\sr\uu{\p_0,..,\p_\n}\y\PP$. 
It spawns, for each of the $\{\p_0,..,\p_\n\}$, 
\footnote{Since the set of principals is parameterised, we allow some syntactic
sugar to express ranges of participants that depend on parameters.}
a request that is accepted by the participant through $\ssa\uu\p\y\PP$. 
Messages
are sent by $\Pout{\ccc}{\p}{\e}{\PP}$ to the participant $\p$ 
and received by $\Pin{\ccc}{\q}{\x}{\PP}$ from the participant $\q$.  
% Delegation, $\Pdel{\ccc}{\p}{\ccc'}{\PP}$, allows the end point of a running
% session to be sent to $\p$. Delegated sessions
% are received by $\q$ using $\Prec{\ccc}{\p}{\y}{\PP}$.  
Selection $\Psel{\ccc}{\p}{l}{\PP}$, and branching $\Pbranch{\ccc}{\q}$, allow a
participant to choose a branch from those supported by another.  Standard
language constructs include recursive processes $\mu \X.P$, restriction
$\nuc{\Ia}{\PP}$ and
$\nuc{s}{\PP}$,  and
% the local definition of recursive processes
% $\defIn{\Ddef}\PP$ and their use $\proccall{\XX}{\e}{\y}$,
parallel composition $\PP \pc \QQ$.
% conditionals $\ifthenelse{\e}{\PP}{\QQ}$ and the null process $\inact$.  
The primitive recursion operator $\RECSEQP{\PP}{\ii}{\X}{\QQ}$ takes as
parameters a process $\PP$, a function taking an index parameter $\ii$ and a
recursion variable $\X$. A queue $\s:\h$ stores the asynchronous messages in
transit.

%  Note the distinction between $\proccall{\XX}{\e}{\y}$
% (infinite repeat) and $\X$ (finite repeat).  

\label{par:annotated}
An {\em annotated} $P$ is the result of annotating $P$'s bound names and
variables by their types or ranges as in e.g.~$(\nu a\!:\!\ENCan{G})Q$ or
$s?(\pp,x\!:\! U);Q$ or 
$\RECSEQP{\QQ}{\ii\!:\!\II}{\X}{\QQ'}$.
% $\lambda \AT{\ii}{\II}.P$.
We omit the annotations 
unless needed.  We often omit $\inact$ and the participant $\p$ from the session
primitives.  Requests, session restriction and channel queues appear only at
runtime, as explained below.




==> app_fft.tex <==
\section{The Fast Fourier Transform algorithm and proofs of Theorem \ref{theorem:fft}}
\label{app:fft}
%Figure~\ref{fig:fft}(d) gives the end-point (local) type that each of the machines has to
%satisfy in order to comply with the global type. 
% We first give more detailed explanations of the FFT algorithm, 
% its global type and end-point  processes in the FFT example in
% \S~\ref{subsec:fft}.
% Then 
We prove Theorem \ref{theorem:fft} -- the processes
are typable against the given global type. Their termination
(i.e.~deadlock-freedom) is then obtained as a corollary.

% \subsection{More on the FFT}
% We start by a quick reminder of the discrete fourier transform definition,
% followed by the description of an FFT algorithm that implements it over a
% butterfly network. We then give the corresponding global session type. From the
% diagram in (b) and the session type from (c), it is finally straightforward to
% implement the FFT as simple interacting processes.

% \paragraph{The Discrete Fourier Transform}  
% The goal of the FFT is to compute the Discrete Fourier Transform
% (DFT) of a vector of complex numbers.
% Assume the input consists in $N$ complex numbers $\vec{x}=x_0, \ldots,
% x_{N-1}$ that can be interpreted as the coefficients of a polynomial
% $f(y)=\sum_{j=0}^{N-1}x_j\,y^j$.  The DFT transforms $\vec{x}$ in a vector
% $\vec{X}=X_0, \ldots, X_{N-1}$ defined by
% $$
% X_k = f(\omega_N^k) 
% $$\\[-3ex]
% \noindent
% with $\omega_N^k=\e^{ \imath\frac{ 2 k\pi }{N}}$ a primitive root of unity. The
% DFT can be seen as a polynomial interpolation on the primitive roots of unity or
% as the application of the square matrix $(\omega_N^{ij})_{i,j}$ to the vector
% $\vec{x}$.

% %We first summarise FFT over the butterfly network \cite[\S~3.7]{FThomson}. 

% \paragraph{FFT and the butterfly network} 
% We present here the radix-2 variant of the Cooley-Tukey FFT
% algorithm~\cite{CT65}. Assuming that $N$ is a power of $2$, this FFT algorithm
% uses a divide-and-conquer strategy based on the following equation (we use the
% fact that $\omega_N^{2k}=\omega_{N/2}^k$):

% $
% \begin{array}{rcl}
%   X_k& = & \sum_{j=0}^{N-1}x_j\,\omega_N^{jk} \\[1mm]
% %        & = & \sum_{j=0}^{N/2-1}x_{2j}\,\omega_N^{2jk}
% %   + \sum_{j=0}^{N/2-1}x_{2j+1}\,\omega_N^{(2j+1)k}\\[1mm]
%   & = &\sum_{j=0}^{N/2-1}x_{2j}\,\omega_{N/2}^{jk}
%   + \omega_N^k\sum_{j=0}^{N/2-1}x_{2j+1}\,\omega_{N/2}^{jk}
% \end{array}
% $\\[1mm]
% Each of the two separate sums are DFT of half of the original vector members,
% separated into even and odd indices. Recursive calls can then divide the input
% set further based on the value of the next binary bits. The good complexity of
% this FFT algorithm comes from the lower periodicity of $\omega_{N/2}$: we have
% $\omega_{N/2}^{jk}=\omega_{N/2}^{j(k-N/2)}$ and thus computations of $X_k$ and
% $X_{k-N/2}$ only differ by the multiplicative factor affecting one of the two
% recursive calls. Figure~\ref{fig:fft}(a) illustrates this recursive
% principle, called {\em butterfly}, where two different outputs can be computed
% in constant time from the results of the same two recursive calls.

% The complete algorithm is illustrated by the diagram from
% figure~\ref{fig:fft}(b).  It features the application of the FFT on a network of
% $N=2^3=8$ machines computing the DFT of vector $x_0, \ldots, x_7$.  Each row
% represents a single machine at each step of the algorithm. Each edge represents
% a value sent to another machine. The dotted edges represent the particular
% messages that a machine sends to itself to remember a value for the next step.
% When reading the diagram from right to left, each step consists in merging the
% results from half of the inputs, following in this the butterfly pattern: each
% machine is successively involved in a butterfly with a machine whose number
% differs by only one bit. Note that the recursive partition over the value of a
% different bit at each step requires a particular bit-reversed ordering of the
% input vector: the machine number $\pp$ initially receives $x_{\overline{\pp}}$
% where $\overline{\pp}$ denotes the bit-reversal of $\pp$.

% % The FFT algorithm relies on the mathematical relations that exist within the
% % group of primitive roots to avoid recomputing twice the same value. For a vector
% % of $N=2^n$ numbers, the sequential complexity is $N\log{N}$ and it benefits from
% % an excellent $O(N)$ speedup on a butterfly network of $N$ machine to reach a
% % complexity of $\log{N}$.

% % Figure~\ref{fig:fft} illustrates the butterfly network topology for $N=2^3=8$.

% This parallel version of the FFT algorithm gives an excellent $O(N)$ speedup on
% a butterfly network of $N$ machines when applied on a vector of size $N$. It has
% also the advantage of being able to compute the DFT inverse by just changing the
% multiplication factors of each butterfly. Finally, this algorithm can be
% implemented easily on common network topologies such as the hypercube.
% %Variants of the
% %butterfly topology include changing the degree ($2$ in our case) which means
% %recursing on a bigger number of smaller instances.

% \paragraph{Global Types}
% Figure~\ref{fig:fft}(c) gives the global session type corresponding to the
% execution of the FFT.  The size of the network is specified by the index
% parameter $n$: for a given $n$, $2^n$ machines compute the DFT of a vector of
% size $2^n$. The first iteration 
% concerns the initialisation:
% each of the machines sends the $x_\pp$ value to themselves. Then we have an
% iteration over variable $l$ for the $n$ successive steps of the algorithm. The
% iterators over variables $i,j$ work in a more complex way: at each step, the
% algorithm applies the butterfly pattern between pairs of machines whose numbers
% differ by only one bit (at step $l$, bit number $n-l$ is concerned). Iterators
% over variables $i$ and $j$ thus generate all the values of the other bits: for
% each $l$, $i*2^{n-l}+j$ and $i*2^{n-l}+2^{n-l-1}+j$ range over all pairs of
% integers from $2^n-1$ to $0$ that differ on the $(n-l)$th bit. The four repeated
% messages within the loops then correspond exactly to the four edges of the
% butterfly pattern.



% % Integers from $2^n-1$ to $0$ are generated using their binary
% % representation: $i$ corresponds to the $l-1$ first bits, variables $k$ or $k'$
% % represent the $l$-th bit and $j$ gives the $n-l-1$ last bits. This way, the
% % integers $i*2^{n-l}+k*2^{n-l-1}+j$ and $i*2^{n-l}+k'*2^{n-l-1}+j$ range over all
% % integers from $2^n-1$ to $0$ and only differ (if they differ) on their $l$-th
% % bit. This test on the $l$-th bit is the direct translation of the even/odd
% % partition featured in the FFT algorithm. 
% % Note that the inner most two recursors 
% % $(\RECSEQ{z}{k}{u}{(\RECSEQ{u}{k'}{v}{ \cdots }})2)2$ 
% % %%Moreover, the schema:
% % %{\small\begin{align*}
% % %   \ldots   &  (\RECSEQ{z}{k}{u}{  \\
% % %        &  \quad (\RECSEQ{u}{k'}{v}{  \\
% % %          & \qquad \GS{\W[i*2^{n-l}+k*2^{n-l-1}+j] \\
% % %            & \quad \qquad }{\W[i*2^{n-l}+k'*2^{n-l-1}+j]}{\Nat}.u}\\
% % %        & \quad)\APP  2} \\
% % %      &)\APP  2\ \ldots\\
% % %    \end{align*}
% % %}
% % %\noindent 
% % exactly represents the $4$ edges of the butterfly pattern from
% % figure~\ref{fig:fft}(a).

% %Figure~\ref{fig:fft}(d) gives the local type that each of the machines has to
% %satisfy in order to comply with the global type. Index $n$ is still a
% %parameter. The main loop is an iteration over the $n$ steps of the
% %algorithm. The natural projection would be:
% %{\small
% %\begin{align*}
% % \T_{\pp} = &\ \Pi n.\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{}} \\
% % & \quad (\LR{\End}{\l}{\xx} {\\
% %   & \qquad
% %   \ifthenelse{\bit{n-l}(\pp)=0\\
% %     & \qquad} {\Lout{\pp+2^{n-l-1}}{\Nat}{\Lin{\pp+2^{n-l-1}}{\Nat}{\\
% %         & \qquad \qquad\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}\\
% %     & \qquad} {\Lout{\pp-2^{n-l-1}}{\Nat}{\Lin{\pp-2^{n-l-1}}{\Nat}{\\
% %         & \qquad \qquad\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}}})\\
% %& \APP n
% %\end{align*}} The test $\bit{n-l}(\pp)=0$ corresponds to testing the value of
% %the $k$ and $k'$ index from the global type. Each of the branches of the test
% %have the two sends and two receives corresponding to the butterfly pattern.  For
% %programming reasons (as seen in the processes), we have here shifted the
% %self-receive $\Lin{\pp}\Nat{}$ from the initialization to the beginning of the
% %loop iteration at the price of adding the last self-receive to the end:
% %$\Lin{\pp}\Nat{\End}$. The lting type is in
% %figure~\ref{fig:fft}(d).

% \paragraph{Processes}
% The processes that are run on each machine to execute the FFT algorithm are
% presented in figure~\ref{fig:fft}(d). % We give the runtime syntax 
% % which are annotated by the destinations for giving more information 
% % to the reader.  
% When $\pp$ is the machine number, $x_{\overline{\pp}}$ the initial value, and
% $\y$ the session channel, the machine starts by sending $x_{\overline{\pp}}$ to
% itself: $\outS{\y}{\x_{\overline{\pp}}}{}$. The main loop corresponds to the
% iteration over the $n$ steps of the algorithm. At step $l$, each machine is
% involved in a butterfly corresponding to bit number $n-l$, i.e. whose number
% differs on the $(n-l)$th bit. In the process, we thus distinguish the two cases
% corresponding to each value of the $(n-l)$th bit (test on $\bit{n-l}(\pp)$). In
% the two branches, we receive the previously computed value $\inpS{\y}\x{..}$,
% then we send to and receive from the other machine (of number $\p+2^{n-l-1}$ or
% $\p-2^{n-l-1}$, i.e. whose $(n-l)$th bit was flipped). We finally compute the
% new value and send it to ourselves: respectively by
% $\outS{\y}{\x+\z\,\omega_N^{g(l,\pp)}}{\X}$ or
% $\outS{\y}{\z+\x\,\omega_N^{g(l,\pp)}}{\X}$. Note that the two branches do not
% present the same order of send and receive as the global session type specifies
% that the diagonal up arrow of the butterfly comes first. At the end of the
% algorithm, the calculated values are sent to some external channels:
% $\Poutend{r_\pp}{0}{\x}$.

% % The content of the loop consists of the
% % following actions: we receive the previously computed value $\inpS{\y}\x{..}$,
% % we then send it to the other machine involved in the current butterfly
% % $\outS{\y}{\x}{}$, we next receive the value this other machine sent
% % $\inpS{y}{\z}{}$, we finally compute the new value and send it to ourselves
% % $\outS{\y}{\x+\z\,\omega_N^{g(l,\pp)}}{\X}$ or
% % $\outS{\y}{\z+\x\,\omega_N^{g(l,\pp)}}{\X}$, depending on our position (up or
% % down) in the butterfly pattern (given by $\bit{n-l}(\pp)$). 

% We show our static type-checking can guarantee communication-safety 
% and deadlock-freedom for a whole group of $N$-processes 
% over this complex butterfly topology. 

% % More concretely, we start from a polynomial $f$ defined by
% % $f(X)=\sum_{i=0}^{N-1}x_iX^i$ and we want its values over the primitive roots of
% % unity: $\omega_N^0,\omega_N^1, \ldots, \omega_N^{N-1}$.

% % The figure~\ref{fig:fft} presents the butterfly topology used by the
% % algorithm. The principle is that a message is exchanged at step $l$ between
% % participants whose index only differ by the $l$-th bit. 
% % %
% % \begin{align*}
% %   &\lambda n.\RECSEQP{\End}{\l}{\X}{\lambda \x.\inpS{\y}\z\\
% %     & \quad
% %     \ifthenelse{\bit{n-l}(\pp)=0}{\outS{\y}{\x+\y\omega_N^{g(l,\pp)}}{\X(\x+\y\omega_N^{g(l,\pp)})}\\
% %     &\qquad }{\outS{\y}{\y+\x\omega_N^{g(l,\pp)}}{\X(\y+\x\omega_N^{g(l,\pp)})}}}
% % \end{align*}


% %\noindent where $g(l,\pp)=\pp \mod 2^l$
% % We describe here a global session type specifying the messages involved in a
% % butterfly topology. As a first approximation, we 

% % \begin{align*}
% % & \Pi d.\Pi n.  \\
% % & (\RECSEQ{\End}{l}{x}{\\
% %   & \quad (\RECSEQ{x}{i}{y}{ \\
% %     & \qquad (\RECSEQ{y}{j}{z}{ \\
% %       &  \quad \qquad (\RECSEQ{z}{k_1}{u}{  \\
% %         &  \qquad \qquad (\RECSEQ{u}{k_2}{v}{  \\
% %           & \quad \qquad \qquad \GS{W[l+1][i*d^{n-l}+k_1*d^{n-l-1}+j] \\
% %             & \qquad \qquad \qquad }{W[l][i*d^{n-l}+k_2*d^{n-l-1}+j]}{\Nat}.v}\\
% %         & \qquad \qquad)\APP  d} \\
% %       & \quad \qquad)\APP  d} \\
% %     & \qquad)\APP  d^{n-l-1}} \\
% %   & \quad) \APP d^l } \\
% % &) \APP n \\
% % \end{align*}

% % Let's describe an Omega network of degree $d$ with number of nodes $N=d*m=d^n$.
% %   \begin{align*}
% %     \Pi d.\Pi m.\Pi n. & (\RECSEQ{\End}{u}{l}{\\
% %       & \quad (\RECSEQ{u}{i}{x}{ \\
% %       & \qquad (\RECSEQ{x}{j}{y}{ \\
% %       & \quad \qquad (\RECSEQ{y}{k}{z}{  \\
% %         & \qquad \qquad  \GS{W[l+1][i*d+j]}{W[l][j*m+k]}{\Nat}.z})\\
% %       & \quad \qquad\APP  d}) \\
% %       & \qquad\APP  m}) \\
% %       & \quad\APP  d}) \\
% %       & \APP  n
% %    \end{align*}

% % The algorithm works in the following way:

% % \begin{enumerate}
% % \item The worker $W[l][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$
% %   receives $x_1$ from $W[l+1][i*d^{n-l}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$ and
% %   $x_2$ from $W[l+1][i*d^{n-l}+d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$. It
% %   sends $x_1+
% %   \omega_N^{d^{(n-l)}(k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j)}x_2$ to
% %   $W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+j]$ and
% %   $W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+d^{n-l-3}+j$.
% % \item We start from the polynomial $\sum_{p=0}^{n-1} x_p X^p$ we want to
% %   interpolate.
% % \item The worker $W[d][p]$ initially holds the value $x_p$. The worker $W[0][p]$
% %   finishes the session with $X_{\over{p}}$ (bit-reverse position).
% % \item The base case worker $W[l][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$ has local
% %   session type
% %   ($i\in[0..d^l-1],j\in[0..d^{n-l-3}-1],k_1\in[0,d-1],k_2\in[0,d-1],k_3\in[0,d-1]$):
% % {\small
% % \begin{align*}
% %   &
% %   (\RECSEQ{\\
% %     & \quad (\RECSEQ{\End
% %   }{k_3'}{v}{ \\
% %   & \qquad \qquad \Lout{W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3'*d^{n-l-3}+j]}{\Nat}{v}} \\
% %   & \qquad\APP d)\\
% %   & \quad
% %   }{k_1'}{u}{ \\
% %   & \qquad\Lin{W[l+1][i*d^{n-l}+k_1'*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]}{\Nat}{u}} \\
% %   & \quad\APP d)\\
% % %   & \Lin{W[l+1][i*d^{n-l}+d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]}{\Nat}{} \\
% % %   & \Lout{W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+j]}{\Nat}{} \\
% % %   & \Lout{W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+d^{n-l-3}+j]}{\Nat}{} \\
% % \end{align*}
% % }
% % \item The first column of workers $W[n][i*d+k_1]$ has local
% %   session type ($i\in[0..d^{n-1}-1],k_1\in[0,d-1]$):
% % \begin{align*}
% %   & (\RECSEQ{\End}{k_1'}{u}{\Lout{W[n-1][i*d+k_1']}{\Nat}{u}}\APP d)\\
% % %   & \Lout{W[n-1][i*d]}{\Nat}{} \\
% % %   & \Lout{W[n-1][i*d+1]}{\Nat}{\End} \\
% % \end{align*}
% % \item The last column of workers $W[0][k_1*d^{n-1}+j]$ has local
% %   session type ($j\in[0..d^{n-1}-1],k_1\in[0,d-1]$):
% % \begin{align*}
% %   & (\RECSEQ{\End}{k_1'}{u}{\Lin{W[0][k_1'*d^{n-1}+j]}{\Nat}{u}}\APP d)\\
% % %   & \Lin{W[1][j]}{\Nat}{} \\
% % %   & \Lin{W[1][d^{n-1}+j]}{\Nat}{\End} \\
% % \end{align*}

% % \item The worker $W[l][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$
% %   receives $x_1$ from $W[l+1][i*d^{n-l}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$ and
% %   $x_2$ from $W[l+1][i*d^{n-l}+d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$. It
% %   sends $x_1+
% %   \omega_N^{d^{(n-l)}(k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j)}x_2$ to
% %   $W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+j]$ and
% %   $W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+d^{n-l-3}+j$.
% % \end{enumerate}

% \subsection{Proofs of Theorem \ref{theorem:fft}}
We assume index $n$ to be a parameter as in figure~\ref{fig:fft}. 
The main loop is an iteration over the $n$ steps of the
algorithm. Forgetting for now the content of the main loop, the generic
projection for machine $\pp$ has the following skeleton:\\[1mm]
{\small
$\begin{array}{ll}
& \Pi n.(\RECSEQ{(\RECSEQ{\End}{l}{\xx}{(\ldots)}\APP n) \\
& }{k}{\uuu}{\\
& \quad \ifthenelse{\pp=k}{\Lout{k}{\U}{\Lin{k}{\U}{\uuu}}}{\uuu}})\\
& ~ 2^n\\
\end{array}$} 
\\[1mm]
A simple induction gives us through \tftrule{WfRecExt} the equivalent type:\\[1mm]
{\small
$\begin{array}{ll}
& \Pi n.\Lout{\pp}{\U}{\Lin{\pp}{\U}{(\RECSEQ{\End}{l}{\xx}{(\ldots)}\APP n)}} \APP 2^n\\
\end{array}$} 
\\[1mm]
We now consider the inner loops. The generic projection gives:\\[1mm]
{\small
$\begin{array}{@{}l@{}l}
& \ldots \\
& \quad (\RECSEQ{\xx}{i}{\yy}{ \\
    & \qquad (\RECSEQ{\yy}{j}{\zz}{ \\
          & \quad \qquad \ifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j=i*2^{n-l}+j}{\ldots\\
          & \quad \qquad }{\ifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j}{\Lout{i*2^{n-l}+j}{\U}{\ldots}\\
          & \quad \qquad }{\ifthenelse{\pp=i*2^{n-l}+j}{\Lin{i*2^{n-l}+2^{n-l-1}+j}{\U}{\ldots}\\
          & \quad \qquad }{\ifthenelse{\ldots}{\ldots}{\ldots}}}}}\\
    & \qquad)\APP  2^{n-l-1}} \\
  & \quad) \APP 2^l \\
& \ldots \\
\end{array}$}
\\[1mm]
An induction over $\pp$ and some simple arithmetic over binary numbers gives us
through \tftrule{WfRecExt} the only two branches that can be taken:\\[1mm]
{\small
$\begin{array}{@{}l@{}l}
& \ldots \\
&\ifthenelse{\bit{n-l}(\pp)=0 \\
& }{\Lin{\pp+2^{n-l-1}}{\U}{\Lout{\pp+2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\Lin{\pp}\U{\xx}}}}\\
& }{\Lout{\pp-2^{n-l-1}}{\U}{\Lin{\pp-2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\Lin{\pp}\U{\xx}}}}}\\
% & \quad (\RECSEQ{\xx}{i}{\yy}{ \\
%     & \qquad (\RECSEQ{\yy}{j}{\zz}{ \\
%           & \quad \qquad \ifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j=i*2^{n-l}+j}{\ldots\\
%           & \quad \qquad }{\ifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j}{\Lout{i*2^{n-l}+j}{\U}{\ldots}\\
%           & \quad \qquad }{\ifthenelse{\pp=i*2^{n-l}+j}{\Lin{i*2^{n-l}+2^{n-l-1}+j}{\U}{\ldots}\\
%           & \quad \qquad }{\ifthenelse{\ldots}{\ldots}{\ldots}}}}\\
% %          & \quad \qquad \GS{i*2^{n-l}+2^{n-l-1}+j}{i*2^{n-l}+j}{\Nat}.\\
% %          & \quad \qquad \GS{i*2^{n-l}+j}{i*2^{n-l}+2^{n-l-1}+j}{\Nat}.\\
% %          & \quad \qquad \GS{i*2^{n-l}+2^{n-l-1}+j}{i*2^{n-l}+2^{n-l-1}+j}{\Nat}.\\
% %          & \quad \qquad \GS{i*2^{n-l}+j}{i*2^{n-l}+j}{\Nat}.\zz}\\
%     & \qquad)\APP  2^{n-l-1}} \\
%   & \quad) \APP 2^l \\
& \ldots \\
\end{array}$} 
\\[1mm]
The first branch corresponds to the upper part of the butterfly while the second
one corresponds to the lower part.
% The natural projection would be:\\[1mm]
% {\small
% $
% \begin{array}{lll}
% \Pi n.\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{}} \\[1mm]
%   \ (\LR{\End}{\l}{\xx} {\\[1mm]
%     \ 
%    \ifthenelse{\bit{n-l}(\pp)=0\\
%       \ } {\Lin{\pp+2^{n-l-1}}{\Nat}{\Lout{\pp+2^{n-l-1}}{\Nat}{
%           \Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}\\[1mm]
%       \ } {\Lout{\pp-2^{n-l-1}}{\Nat}{\Lin{\pp-2^{n-l-1}}{\Nat}{
%          \Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}}}) \APP n
% \end{array}
% $
% } 
% \\[1mm]
% The test $\bit{n-l}(\pp)=0$ corresponds to testing the value of
% the $k$ and $k'$ index from the global type. 
% Each of the branches of the test
% have the two sends and two receives corresponding to the butterfly pattern.  
For programming reasons (as seen in the processes, the natural implementation
include sending a first initialisation message with the $x_k$ value), we want to
shift the self-receive $\Lin{\pp}\U{}$ from the initialisation to the beginning
of the loop iteration at the price of adding the last self-receive to the end:
$\Lin{\pp}\U{\End}$. 
The resulting equivalent type up to $\equiv$ is: \\[2mm]
{\small
$
\begin{array}{ll}
\Pi n.\Lout{\pp}{\U}{} \\
 \ (\LR{\Lin{\pp}\U{\End}}{\l}{\xx} {\\[1mm]
 \  \ifthenelse{\bit{n-l}(\pp)=0\\[1mm]
    \ } {\Lin{\pp}\U{\Lin{\pp+2^{n-l-1}}{\U}{\Lout{\pp+2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\xx}}}}\\[1mm]
    \ } {\Lin{\pp}\U{\Lout{\pp-2^{n-l-1}}{\U}{\Lin{\pp-2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\xx}}}}}}) \APP n
\end{array}
$
}\\[1mm]
From this end-point type, it is straightforward to type 
and implement the processes defined in 
figure~\ref{fig:fft}(d) in \S~\ref{subsec:fft}. 


==> app_runtime.tex <==
\section{Typing system for runtime processes}
\label{app:runtime}
This appendix defines a typing system for runtime processes
(which contain queues).   
Most of the definitions are from \cite{BettiniCDLDY08LONG}. 


\begin{center}
\begin{tabular}{c}
\begin{tabular}{lrclr}
  Message & $\TQ$ & ::= &
         \oT\UT{\pv} & \emph{message send}\\
         &     & \sep  & \seltypes &\emph{message selection}\\
         &     & \sep  & $\TQ;\TQ'$ &\emph{message sequence}\\
\\
  Generalised \quad\quad\quad & $\TG$ & ::= &
         \T
  & \emph{session}\\
         &     & \sep & \TQ &\ \emph{message}\\
         &     & \sep & $\TQ;\T$ &\ \emph{continuation}\\[0.5mm]
\end{tabular}
\end{tabular}
\end{center}

\noindent
{\em Message types} are the types for queues: they
represent the messages contained in the queues. The {\em message
send type} \oT\UT{\pv}\ expresses the communication to $\pv$ 
of a value or of a channel of type \UT. The {\em
message selection type} \seltypes{} represents the communication to
participant $\pv$ of the label $l$ and $\TQ;\TQ'$
represents sequencing of message types (we assume associativity for $;$). For
example $\oplus\anglep{1}{\kf{ok}}$ is the message type for the
message $(2,1,\kf{ok})$. A {\em generalised type} is either
a session type, or a message type, or a message type followed by a
session type. Type $\TQ;\T$ represents the continuation of the type $\TQ$
associated to a queue with the type $\T$ associated to a pure process. An
example of generalised type is
$\oplus\anglep{1}{\kf{ok}};!\langle
3,\kf{string}\rangle; ?\langle 3,\kf{date}\rangle; \End$.

In order to take into account the structural congruence between
queues (see Figure~\ref{tab:structcong}) we consider message types
modulo the equivalence relation \equivT{}{}\ induced by the
rules shown as follows 
(with $\natural\in\set{!,\oplus}$ and $Z\in\set{\UT,l}$): 
\begin{center}
$\equivT{\oTG{Z}{\pv};\oTGp{Z}{\qv};\TQ}{\oTGp{Z}{\qv};\oTG{Z}{\pv};\TQ}$
\quad if $\pv\not = \qv$
\end{center}
The equivalence relation on message types extends to generalised types by:
\[\equivT{\TQ}{\TQ'}\text{ implies }\equivT{\TQ;\TG}{\TQ';\TG}\]
\indent 
We say that two session environments 
$\D$ and $\D'$ are equivalent (notation $\equivT{\D}{\D'}$) if
$\ccc:\TG\in\D$ and $\TG\not=\End$ imply $\ccc:\TG'\in\D'$ with $\equivT{\TG}{\TG'}$ and vice versa. This equivalence relation is used in rule \trule{Equiv} (see Figure~\ref{fig:runtime-process-typing}).

\input{fig_runtime}

We start by defining the typing rules for single queues, in which the turnstile
$\vdash$ is decorated with \set\s\ (where \s\ is the session name of the current
queue) and the session environments are mappings from channels to message types.
The empty queue has empty session environment. Each message adds an
output type to the current type of the channel which has the role of
the message sender.  Figure~\ref{fig:queue-typing} lists the typing rules for
queues, where \Tcomp\ is defined by:

\begin{center}
$\D \Tcomp\set{s[\qv]: \TQ} = \begin{cases}
 \D' ,s[\qv]: \TQ';\TQ     & \text{if }\D=\D',  s[\qv]:\TQ', \\
 \D,s[\qv]: \TQ    & \text{otherwise}.
\end{cases}$
\end{center}
For example we can derive $\derq{}{\s:(3,1,\kf{ok})}{\set{\si\s 1:\oplus\anglep{1}{\kf{ok}}}}$.

In order to type pure processes in parallel with queues,
we need to use generalised types in session environments and
further typing rules. Figure~\ref{fig:runtime-process-typing}
lists the typing rules for processes containing queues.
The judgement $\derqq{\Ga}{\Sigma}{\PP}{\D}$ means that
$\PP$ contains the queues whose session names are in $\Sigma$.
Rule \trule{GInit} promotes the typing of a pure process
to the typing of an arbitrary process, since a pure process does not
contain queues. When two arbitrary processes are put in parallel (rule
\trule{GPar}) we need to require that each session name is associated
to at most one queue (condition $\Sigma\cap\Sigma'=\emptyset$). In
composing the two session environments we want to put in sequence a
message type and a session type for the same channel with role. 
For this reason we define the composition \Dcomp\ between 
generalised types as:

\begin{center}
$\TG \Dcomp \TG'=\begin{cases}
  \TG \Tcomp \TG'    & \text{if $\TG$ is a message type}, \\[-.2em]
    \TG'\Tcomp \TG   & \text{if $\TG'$ is a message type}, \\[-.2em]
    \bot  & \text{otherwise}\\
\end{cases}$
\end{center}

\noindent
where $\bot$ represents failure of typing.

We extend \Dcomp\ to session environments as expected:

\begin{center}
$\D \Dcomp \D' = \D\backslash \dom{\D'} \cup \D' \backslash \dom{\D}
\cup \set{\ccc: \TG \Dcomp \TG' \sep
  \ccc:\TG \in \D~\&~\ccc:\TG' \in \D'}$.
\end{center}

\noindent Note that \Dcomp\ is commutative, i.e., $\D \Dcomp
\D'=\D' \Dcomp \D$. Also if we can derive message types only for
channels with roles, we consider the channel variables in the
definition of \Dcomp\ for session environments since we want to
get for example $\set{y:\End}\Dcomp\set{y:\End}=\bot$ (message
types do not contains $\End$). 

%An example of derivable judgement is:

%$
%\derq{}{\PP\pc\s:(3,\set{1,2},\kf{ok})}{\set{\si\s
%3:\oplus\anglep{\set{1,2}}{\kf{ok}};!\langle \{1\},\kf{string}\rangle; ?\langle
%1,\kf{date}\rangle; \End}}
%$

%\noindent
%where $\PP=\si\s 3!\langle\set{1},
%\texttt{"Address"}\rangle;\si\s 3?(1,\textit{date}); \inact$.

In rule \trule{GSRes} we require the coherence of the session 
environment \D\ with respect to the session name \s\
to be restricted (notation \coe\D\s). This coherence 
is defined in Definition~\ref{cd} using the notions of projection 
of generalised types and of duality, 
introduced respectively in Definitions~\ref{def:genproj} and~\ref{dd}. 

\begin{DEFINITION}\label{def:genproj} 
\rm 
The {\em projection
of the generalised local type \TG\ onto \q}, denoted by $\pro\TG\q$,
is defined by:
\[
\begin{array}{rcl}
\pro{(\oT\UT{\pv};\TG')}\q&=&\begin{cases}
  !\UT;\pro{\TG'}\q  & \text{if }\q = \pv, \\
   \pro{\TG'}\q & \text{otherwise}.
\end{cases}\\
\pro{(\seltypes;\TG')}\q&=&\begin{cases}
  \oplus l;\pro{\TG'}\q  & \text{if }\q=\pv, \\
   \pro{\TG'}\q & \text{otherwise}.
\end{cases}\\
\pro{(\iT\UT{\p};\T)}\q&=&\begin{cases}
  ?\UT;\pro{\T}\q  & \text{if }\q=\p, \\
   \pro{\T}\q & \text{otherwise.}
\end{cases}\\
\pro{(\seltype)}\q&=&\begin{cases}
  \seltypeT  & \text{if }\q = \p, \\
  \sqcup_{i\in I}\pro{\T_i}\q & \text{otherwise.}
\end{cases}\\
\pro{(\branchtype)}\q&=&\begin{cases}
  \branchtypeT  & \text{if }\q=\p, \\
\sqcup_{i\in I}\pro{\T_i}\q 
&  \text{otherwise.}
\end{cases}\\
\pro{(\mu \xx.\T)}\q&=& \mu \xx.(\pro{\T}\q) \quad
\pro\xx\q=\xx\quad\pro\End\q=
         \End\\
       \end{array}
       \]

\noindent where $\sqcup_{i\in I}\pro{\T_i}\q$ is defined as $\sqcup_{i\in I}
T_i$ in Definition~\ref{def:mergeability} replacing by:  

\[ 
\begin{array}{lll}
\&\langle\{l_k:T_k\}_{i\in I}\rangle \ \mergecup 
\&\langle\{l_j:T_j'\}_{j\in J}\rangle \ = \\ 
\quad \&\langle\{l_k:T_k\mergecup T_k'\}_{k\in K\cap J}
\cup \{l_k:T_k\}_{k\in K\setminus J}
\cup \{l_j:T_j'\}_{j\in J\setminus K}\rangle\\[1mm]
\end{array}
\]
\end{DEFINITION}

\begin{DEFINITION}\label{dd}
The {\em duality relation} between projections of generalised
types is the minimal symmetric relation which satisfies:

\begin{center}
$\dual\End\End\qquad \dual\xx\xx\qquad \dual\T{\T'}\implies
\dual{\mu \xx.\T}{\mu \xx.\T'}$ 

$\dual\TG{\T}\implies\dual{!\UT;\TG}{?\UT;\T}$

$\forall i\in I ~\dual{\T_i}{\T_i'}\implies \dual \seltypeTp
\branchtypeTp $

$\exists i\in I ~l=l_i~\&~\dual{\TG}{\T_i}\implies \dual {\oplus
l;\TG} \branchtypes $

\end{center}
\end{DEFINITION}















==> app_sr.tex <==
\subsection{}

\begin{THM}[Subject Congruence and Reduction]
(cf \ref{thm:sr})\mbox{}\\[-3ex]
\begin{itemize}
\item
If $\derqq\Ga{}\PP\D$ and $\PP\equiv{\PP'}$, then
\derqq\Ga{}{\PP'}{\D}. 
\item 
If \derqq\Ga{}\PP\Ty\ and \redM\PP{\PP'}, then
\derqq\Ga{}{\PP'}{\Ty'}\ for some $\Ty'$ such that
$\seredstar\Ty\Ty'$.
\end{itemize}
\end{THM}
\begin{proof} 
  We only list the crucial cases of the proof of subject reduction: the recursor
  (where mathematical induction is required) and the initialisation. Our proof
  works by induction on the length of the derivation \redM\PP{\PP'}. The base
  case is trivial. We then proceed by a case analysis on the reduction
  \red\PP{\PP'}. We omit the hat from principal values for readability.
% The most interesting case 
% is the recursor where we use
% mathematical induction in addition to induction on the derivation. 
% Also the initialisation uses the mergeability lemma. 
%We omit 
%$\Sigma$ from the turnstile since it is fixed for these cases. 
%The session initialisation uses the property of the subtyping 
%for the mergeability. 
%\\[1mm]
%{\bf Case Beta:}  Suppose 
%$\derqq\Ga{}{(\lambda \ii.\PP)\n}{\Ty}$  
%and $\red{(\lambda \ii.\PP)\n}{\PP\subst{\n}{\ii}}$. 
%Then there exists $\Ty'$ such that 
%$\derqq\Ga{}{\lambda \ii.\PP}{\Pi\AT{\ii}{\II}.\Ty'}$ 
%and $\Ty \equiv (\Pi\AT{\ii}{\II}.\Ty') \n \equiv \Ty'\subst{\n}{\ii}$
%and $\Ga{\models}{n: \II}$. The first judgement must have been 
%derived with \trule{TApp}, thus we have the derivations such that 
%$\Gamma, \AT{\ii}{\II}\vdash \PP\rhd \Ty'$. By applying the
%Substitution Lemma (Lemma \ref{lem:substitution} (\ref{subs01})), we obtain
%$\Gamma\vdash \PP\subst{\n}{\ii}\rhd \Ty'\subst{\n}{\ii}$, 
%as required. 
\\[1mm]
{\bf Case ZeroR:}  Trivial. \\[1mm]
{\bf Case SuccR:}  Suppose 
$\derqq\Ga{}{\GR{P}{\ii}{X}{Q}\APP \n+1}{\tau}$
and 
$\red{\GR{P}{\ii}{X}{Q}\APP \n+1}
{P\sub{\n}{\ii}\sub{\GR{P}{\ii}{X}{Q}\APP \n}{X}}$. 
Then there exists $\Ty'$ such that 
\begin{eqnarray}
& 
\label{eq:rec1}
\Gamma, \ii : \minus{\II},\X:\Ty\sub{\ii}{\jj}  \vdash \QQ  \rhd
  \Ty'\sub{\ii+1}{\jj} \\
& 
\label{eq:rec2}
\derqq\Ga{}{P}{\Ty'\subst{0}{\ii}}\\ 
& 
\label{eq:rec3}
\Gamma\vdash \Pi \AT{\jj}{\II}.\Ty \RHD \Pi\AT{\jj}{\II}.\K
\end{eqnarray}
with 
$\Ty \equiv (\Pi\AT{\ii}{\II}.\Ty') \n+1 \equiv \Ty'\subst{\n+1}{\ii}$
and $\Ga{\models}{\n+1:\II}$. 
By Substitution Lemma (Lemma \ref{lem:substitution} (\ref{subs01})), 
noting $\Ga{\models}{\n: \minus{\II}}$,  
we have: 
$\Gamma, \X:\Ty\sub{\ii}{\jj}\sub{\n}{\ii}  \vdash \QQ\sub{\n}{\ii}  \rhd
  \Ty'\sub{\ii+1}{\jj}\sub{\n}{\ii}$, 
which means that 
\begin{eqnarray}
\label{eq:subs}
\Gamma, \X:\Ty\sub{\n}{\jj}  \vdash \QQ\sub{\n}{\ii}  \rhd
  \Ty'\sub{\n+1}{\jj} 
\end{eqnarray}
Then there are two cases. \\[1mm]
{\em Base Case $\n=0$:} 
By applying Substitution Lemma (Lemma \ref{lem:substitution}
(\ref{subs02})) to  (\ref{eq:subs}) with (\ref{eq:rec2}), we have 
$\Gamma  \vdash \QQ\sub{1}{\ii}\sub{P}{X}  \rhd
  \Ty'\sub{1}{\jj}$.  \\[1mm]
{\em Inductive Case $\n\geq 1$:} 
By the inductive hypothesis on $\n$, 
we assume: 
$\derqq\Ga{}{\GR{P}{\ii}{X}{Q}\APP \n}{\Ty'\sub{\n}{\jj}}$. 
Then by applying Substitution Lemma (Lemma \ref{lem:substitution}) to
(\ref{eq:subs}) with this hypothesis, 
we obtain
$\Gamma\vdash \QQ\sub{\n}{\ii}\sub{\GR{P}{\ii}{X}{Q}\ \n}{X}  \rhd
 \Ty'\sub{\n+1}{\jj}$. \\[1mm]
\\[1mm]
{\bf Case [Init]}
$$
\sr\Ia{\p_0,..,\p_\n}{\y}{\PP}\redsym (\nu \s)(
        \PP\sub{\si\s {\p_0}}{\y} \pc s : \qbot \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
        \sj{\Ia}{\p_\n}{\s})
$$
We assume that
$\derqq{\Ga}{\emptyset}{\sr\Ia{\p_0,..,\p_\n}{\y}{\PP}}{\D}$. Inversion of
\trule{TInit} and \trule{TSub} gives that $\D'\leq\D$ and:
\begin{eqnarray}
& \forall i\neq 0, & \Gamma \proves \p_i\rhd \Nat\label{case-pi}\\
& & \Gamma \vdash \Ia:\mar{\G} \label{case-Ia}\\
& & \Gamma \models \pid(\G)=\{\p_0..\p_\n\} \label{case-pid}\\
& & \Gamma \vdash \PP \rhd \D', \y:\G \proj{\p_0} \label{case-PP}\\
\text{From~(\ref{case-PP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}),}
& & \derqq{\Ga}{}{\PP\sub{\si\s {\p_0}}{\y}}{\D, \si\s {\p_0}:\G \proj{\p_0}} \label{case-sub}\\
\text{\hspace{-3ex}From Lemma~\ref{lem:basic}~(\ref{lem:agreeEnv}) and \trule{QInit},}
& & \derqq{\Ga}{s}{s : \qbot}{\emptyset} \label{case-sbot}\\
\text{From (\ref{case-pi}), (\ref{case-Ia}), (\ref{case-pid}) and
  \trule{TReq},}
& \forall i\neq 0, & \Gamma \vdash \sj{\Ia}{\pp_i}{\s} \rhd \s[\pp_i]:\G \proj{\pp_i} \label{case-sppi}
\end{eqnarray}

% From~(\ref{case-PP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}), we have
% $\derqq{\Ga}{}{\PP\sub{\si\s {\p_0}}{\y}}{\D, \si\s {\p_0}:\G \proj{\p_0}}$ 

% From Lemma~\ref{lem:basic}~(\ref{lem:agreeEnv}) and \trule{QInit}, we
% have $\derqq{\Ga}{s}{s : \qbot}{\emptyset}$.

% From (\ref{case-pi}) and (\ref{case-Ia}) and (\ref{case-pid}), \trule{TJoin}
% gives us $\Gamma \vdash \sj{\Ia}{\pp_i}{\s} \rhd \s[\pp_i]:\G \proj{\pp_i}$ for
% $i$ between $1$ and $n$. 

Then \trule{TPar} on (\ref{case-sub}), (\ref{case-sbot}) and (\ref{case-sppi}) gives:
$$\Gamma \vdash \PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} %
\rhd \D', \s[\pp_0]:\G \proj{\pp_0}, ... , \s[\pp_n]:\G
\proj{\pp_n}
$$
From \trule{GInit} and \trule{GPar}, we have:
$$\Gamma \vdash _ s \PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} \pc s : \qbot%
\rhd \D', \s[\pp_0]:\G \proj{\pp_0}, ... , \s[\pp_n]:\G
\proj{\pp_n}
$$
From Lemma \ref{lem:mergeability} we know that $\coe{(\s[\pp_0]:\G \proj{\pp_0},
  ... , \s[\pp_n]:\G\proj{\pp_n})}{\s}$. We can then use \trule{GSRes} to get:
$$\Gamma \vdash _ \emptyset (\nu \s)(\PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} \pc s : \qbot) \rhd \D'
$$
We conclude from % \trule{GInit}, \trule{GPar}, \trule{GSRes} and 
\trule{TSub}.
\\[1mm]
{\bf Case [Join]} 
$$
\sj{\Ia}{\pp}{\s} \pc \sa\Ia{\pp}{\y}{\PP}\redsym 
        \PP\sub{\si \s {\p}}{\y}
$$
We assume that $\Gamma \vdash _{} \sj{\Ia}{\p}{\s} \pc \sa\Ia{\p}{\y}{\PP}\rhd
\D$. Inversion of \trule{TPar} and \trule{TSub} gives that $\D=\D',\s[\pp]:\T$ and :
\begin{eqnarray}
& & \Gamma \vdash \sj{\Ia}{\pp}{\s} \rhd \s[\pp]:\G \proj{\pp}\label{case-Join-spp}\\
& & \T\geq\G\proj{\pp}\label{case-Join-subt}\\
& & \Gamma \vdash \sa\uu\pp\y\PP \rhd \D'\label{case-Join-PP}\\
\text{By inversion of \trule{TAcc} from~(\ref{case-Join-PP})}
& & \Gamma \vdash \PP \rhd \D', \y:\G \proj{\pp}\label{case-Join-projPP}\\
\text{From~(\ref{case-Join-projPP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}),}
& & \derqq{\Ga}{}{\PP\sub{\si\s {\p}}{\y}}{\D', \si\s {\p}:\G \proj{\p}} \label{case-Join-sub}
\end{eqnarray}

We conclude by \trule{TSub} from (\ref{case-Join-sub}) and (\ref{case-Join-subt}).
% \\[1mm]
% {\bf Case [Branch]} 

% $$\lbranch{\sii}{\q} \Par \qpop{\labheap{l_{i_0
%     }}{\p}{\q}} \redsym \PP_{i_0 } \Par \mqueue{\s}{\queue} \quad (i_0
%   \in I)
% $$
% We assume $\Gamma \vdash _{}\lbranch{\sii}{\q} \Par
% \qpop{\labheap{l_{i_0}}{\p}{\q}}\rhd \D $. Inversion of \trule{TPar} and
% \trule{TSub} gives that $\D=(\D',\s[\pp]:\T_\pp) \Dcomp (\D'',\s[\qq]:\T_\qq)$ and :
% \begin{eqnarray}
% & & \Gamma \vdash \Pbranch{\si\s {\p}}{\q}\rhd \D',\si\s{\p}:\LbranchI{\q}{\T_i}{i}{I}
% \label{case-Branch-bra}\\
% & & \T_\pp\geq\LbranchI{\q}{\T_i}{i}{I}\label{case-Branch-bra-sub}\\
% & & \derq{\Ga}{\qpop{\labheap{l_{i_0}}{\p}{\q}}}{\D'',\siq :\LselI{\p}{\T'_j}{j}{J}}\label{case-Branch-sel}\\
% & & \T_\qq\geq\LselI{\p}{\T'_j}{j}{J}\label{case-Branch-sel-sub}\\
% \text{From \ref{}}
% \end{eqnarray}


% We use Lemma \ref{lem:mergeability} to get the existence of a global type
% $G$ such that $\Gamma \vdash T_i\geq\G \proj{\pp_i}$ and $\coe{(\D,
%   \s[\pp_0]:\T_o, ... , \s[\pp_n]:\T_n)}{\s}$. 



% \mbox{} \\[1mm]
% {\bf Case Link} We omit the hat from principals for a readability. 
% {\small
% \begin{center}
%          $\sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}
%         \pc..\pc\sa\Ia{\p_1}{\y_1}{\PP_1}
%          \redsym (\nu \s)(\PP_{0}\sub{\si\s {\p_0}}{\y_{0}} \pc ...\pc
%         \PP_\n\sub{\si \s {\p_\n}}{\y_\n}\pc s : \emptyset)$.  
% \end{center}
% }
% \noindent Assume
% $\derqq{\Ga}{\Sigma}{
% \sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}\pc
% \sa\Ia{\p_1}{\y_1}{\PP_1}\pc...\pc\sa\Ia{\p_\n}{\y_\n}{\PP_\n}}{\D}$,
% then $\Sigma=\emptyset$ and
% \begin{eqnarray}
% & \der{\Ga}{\sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}}{\D_0'}\\
% & \der{\Ga}{\sr\Ia {\p_i}{\y_i}{\PP_i}}{\D_i'}\quad (1\leq i\leq \n)
% \label{L3}
% \end{eqnarray}
% where $\D =\bigcup_{i=0}^{\n} \D_i$ with $\D_i\geq \D_i'$.
% Then we have, by Lemma \ref{lem:mergeability}, 
% \begin{eqnarray}
% & & \nonumber \de\Ga \Ia{\an \G}\label{L4}\\
% & & \der{\Ga}{\PP_0}{\D_0',\y_0:T_0\quad \quad T_0\subT \pro{\G}{\p_0}\label{L5}}	
% \end{eqnarray}
% and  $\Gamma\proves \pid(G)=\{\p_0,...,\p_\n\}$.
% Next we have, again by Lemma \ref{lem:mergeability},  
% \begin{eqnarray}
% & & \nonumber \de\Ga \Ia{\an \G}\label{L6}\\
% & & \der\Ga{\PP_i}{\D_i',\y_i\ins T_i} \quad \quad T_i \leq \pro{\G}{\p_i} 
% \quad \quad (1\leq i\leq \n). 
% \label{L7}\end{eqnarray}
% Using Substation Lemma (Lemma \ref{lem:substitution} (4)) on (\ref{L5}) and (\ref{L7})
% \begin{eqnarray}
% \derq\Ga{\PP_i\sub{\si\s i}{\y_i}}{\D_i',\si{\s}{i}:T_i} \quad (1\leq
% i\leq n). \label{L8}\end{eqnarray}
% Using \trule{Conc} more times on (\ref{L8}) we have
% \begin{eqnarray}
% \der{\Ga}{\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}}{\bigcup_{i=0}^{\n} (\D_i',\si{\s}{i}:T_i
%         )}.\label{L9}\end{eqnarray}
% Note that
% \begin{eqnarray*}
% \bigcup_{i=0}^{\n} (\D'_i,\si{\s}{i}\ins T_i) \leq \D,\si{\s}{0}\ins\pro{\G}{\p_0},\ldots,\si{\s}{n}\ins\pro{\G}{\p_\n}\end{eqnarray*}
% Using \trule{GInit}, \trule{QInit}, \trule{GPar} and \trule{Subs} on (\ref{L9}) we have
% \begin{eqnarray}
% \derqq{\Ga}{\{\s\}}{\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}\pc s :
% \eq}{\D,\si{\s}{1}\ins\pro{\G}{\p_0},
% \ldots,\si{\s}{\n}\ins\pro{\G}{\p_\n}} \quad \quad \label{L10}
% \end{eqnarray}
% Using \trule{QScope} on (\ref{L10}) we have
% \begin{eqnarray}
% \derqq{\Ga}{\emptyset}{(\nu \s)(\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}\pc s : \eq)}{\D}\label{L11}
% \end{eqnarray}
% since 
% \[
% (\D,\si{\s}{0}\ins\pro{\G}{\p_0},\ldots,\si{\s}{\n}\ins
% \pro{\G}{\p_{\n}})\setminus {\s} = \D. 
% \]
%The proof of the communication rules uses the subtyping relation
%and the Substitution Lemma (\ref{lem:substitution} (\ref{subs1}),
%(\ref{subs2})), together with the subtyping rule for the extended mergeability
%(Lemma \ref{lem:mergeability}).
\end{proof}

The proof of the progress is a corollary from this theorem. 
The detailed definitions (simple and well-linked) can be found in a full version 
of \cite{CHY07}. 


==> basicproperties.tex <==
%\section{Formal results}
\section{Properties of typing}
\label{sec:property}
\noindent 
We study the two main properties of the typing system: one is the
termination of type-checking and another is type-soundness. The proofs
require a careful analysis due to the subtle interplay between
dependent types, recursors, recursive types and branching types.
\subsection{Basic properties}
\label{sec:basic}
%\noindent 
\noindent We prove here a series of consistency lemmas concerning permutations
and weakening.
% of judgements .
They are invariably deduced by induction on the derivations in the
standard manner.  

We use the following additional notations: $\Ga
\subseteq \Ga'$ iff $\AT{u}{S}\in \Ga$ implies $\AT{u}{S}\in \Ga'$ and
similarly for other mappings. In other words, $\Ga \subseteq \Ga'$
means that $\Ga'$ is a permutation of an extension of $\Gamma$.

\begin{LEM} \label{lem:basic}
\begin{enumerate}
\item (Permutation and Weakening)\ 
\label{lem:per}
Suppose $\Ga \subseteq \Ga'$ and $\Ga'\proves \Env$. Then 
$\Gamma \proves \judg$ 
implies
$\Gamma' \proves \judg$.  

\item (Strengthening)\ 
\label{lem:st}
$\Gamma,\AT{u}{U},\Gamma' \proves \judg$ 
and $u\not\in \fv(\Gamma', \judg)\cup \fn(\Gamma', \judg)$. Then $\Gamma,\Gamma' \proves \judg$.
Similarly for other mapping. 

\item (Agreement)
\label{lem:agree}
\begin{enumerate}
\item 
\label{lem:agreeEnv}
$\Gamma \proves J$ implies $\Gamma \proves \Env$. 
\item 
\label{lem:agreeK}
$\Gamma \proves \G \RHD \K$ implies 
$\Gamma \proves \K$. Similarly for other judgements. 

\item 
\label{lem:agreeEq}
$\Gamma \proves \G \equiv \G'$ implies 
$\Gamma \proves G \RHD \K$. Similarly for other judgements. 

\item 
\label{lem:agreeTy}
$\Gamma \proves P \rhd \Ty$ implies $\Gamma \proves \Ty \RHD \K$.
Similarly for other judgements. 
\end{enumerate}
\item (Exchange) 
\label{lem:agreeEx}
\begin{enumerate} 
\item 
\label{lem:ExT}
$\Gamma,\AT{u}{U},\Gamma' \proves \judg$ and $\Gamma \proves U\equiv
U'$. Then $\Gamma,\AT{u}{U'},\Gamma' \proves \judg$. 
Similarly for other mappings. 
\item 
\label{lem:ExI}
$\Gamma,\AT{\ii}{\II},\Gamma' \proves \judg$ and $\Gamma\models
\AT{\ii}{\II}=
\AT{\ii}{\II'}$. Then 
$\Gamma,\AT{\ii}{\II'},\Gamma' \proves \judg$. 

\item 
\label{lem:ExP}
$\Gamma,\PRED,\Gamma' \proves \judg$ and $\Gamma\models
\PRED=\PRED'$. Then 
$\Gamma,\PRED',\Gamma' \proves \judg$. 
\end{enumerate}
\end{enumerate}
\end{LEM}
\begin{proof}
By induction on the derivations. We note that the proofs are 
done simultaneously.  For the rules which use substitutions 
in the conclusion of the rule, such as \tftrule{TApp} in
Figure~\ref{fig:process-typing1}, 
we require to use the next substitution lemma simultaneously. 
We only show the most interesting case 
with a recursor. \\[1mm]
{\bf Proof of (3)(b). Case \trule{KRcr}:}  Suppose 
$\Gamma \vdash \GR{\G}{\AT{\ii}{\II^-}}{\xx}{\G'}  
\RHD \Pi\AT{\jj}{\II}. \K$ is derived by \trule{KRcr} in 
Figure~\ref{fig:kindsystembase}.  We prove $\Gamma \vdash  
\Pi\AT{\jj}{\II}. \K$. 
From $\Gamma, \ii:\II^- \vdash \G' \RHD \K\subst{i+1}{j}$ in the
premise of \trule{KRcr}, 
we have $\Gamma, \ii:\II^- \vdash \K\subst{i+1}{j}$ by inductive
hypothesis.  By definition of $\II^-$, this implies 
$\Gamma, \jj:\II \vdash \K$. Now by  \trule{KSeq}, 
we have $\Gamma\vdash \Pi\AT{\jj}{\II}.\K$, as desired. 
\end{proof}
The following lemma which states that well-typedness is
preserved by substitution of appropriate values for variables, is the
key result underlying Subject Reduction. This also guarantees that 
the substitution for the index which affects to a shared environment and
a type of a term, and the substitution for a process variable are
always well-defined.  
Note that 
%shows that, under certain circumstances, a variable can be replaced
%% by an index or a term throughout a judgement, although this
%% 
substitutions may change session types and environments in the index case.
%% The application of (1) to process judgements is especially useful for the
%% Subject Reduction Theorem:  
%% if \derqq{\Ga,\ptilde{\ii}:\II,\Ga'}{\Sigma}{\PP}{\Ty} and 
%% \der{\Ga}{\n}{\Nat} with $\Ga\models \n: \II$, then 
%% $\derqq{\Ga,(\Ga'\subst{\n}{\ii})}{\Sigma}{\PP\subst{\n}{\ii}}{\Ty\subst{\n}{\ii}}$. 

\begin{LEM}[Substitution lemma]\label{lem:substitution}
\begin{enumerate}
\item \labelx{subs01} 
If ${\Ga,\ptilde{\ii}:\II,\Ga'}\proves_\Sigma {\judg}$ and 
$\Ga\models \n: \II$, then 
${\Ga,(\Ga'\subst{\n}{\ii})}\proves_\Sigma \judg\subst{\n}{\ii}$.
%If \der{\Ga,\ptilde{\ii}:\II,\Ga'}{\PP}{\Ty} and 
%\de\Ga{\n}{\Nat} with $\Ga\models \n: \II$, then 
%\der{\Ga,\Ga'\subst{\n}{\ii}}{\PP\subst{\n}{\ii}}{\Ty\subst{\n}{\ii}}.
\item \labelx{subs02} 
If \derqq{\Ga,\ptilde{\X}:\ptilde{\D_0}}{\Sigma}{\PP}{\Ty} and 
\de\Ga{\ptilde{\QQ}}{\D_0}, then
\derqq{\Ga}{\Sigma}{\PP\subst{\QQ}{\ptilde{X}}}{\Ty}.
\item \label{subs1} 
If \derqq{\Ga,\ptilde{\x}:\ptilde{\ST}}{\Sigma}{\PP}{\D} and \de\Ga{\ptilde{v}}{\ptilde{\ST}}, then
\derqq{\Ga}{\Sigma}{\PP\subst{\ptilde{\va}}{\ptilde{\x}}}{\D}.
\item \labelx{subs2} If
\derqq{\Ga}{\Sigma}{\PP}{\D,\y:\T}, then
\derqq{\Ga}{\Sigma}{\PP\sub{\si\s \pv}{\y}}{\D,\si\s \pv:\T}.
\end{enumerate}
\end{LEM}
\begin{proof}
By induction on the derivations.
We prove the most interesting case: 
if \derqq{\Ga,\ptilde{\ii}:\II,\Ga'}{\Sigma}{\PP}{\Ty} and 
\der{\Ga}{\n}{\Nat} with $\Ga\models \n: \II$, then 
$\derqq{\Ga,(\Ga'\subst{\n}{\ii})}{\Sigma}{\PP\subst{\n}{\ii}}{\Ty\subst{\n}{\ii}}$
when the last applied rule is \tftrule{TPRec}. 
Assume 
\[
\Gamma,k:J, \Gamma' \vdash \RECSEQP{\PP}{\ii}{\X}{\QQ} \rhd \Pi
\AT{\jj}{\II}.\Ty 
\quad \mbox{with} \quad \Ga\models \n: J
\]
is derived from \tftrule{TPRec}. This is derived by: 
{\small
\begin{eqnarray}
& & 
\Gamma,k:J, \Gamma', \ii : \minus{\II},\X:\Ty\sub{\ii}{\jj}  \vdash \QQ  \rhd
\Ty\sub{\ii+1}{\jj} \label{sub:q-1}\\
& & 
\Gamma, k:J, \Gamma'\vdash \PP  \rhd\Ty\sub{0}{\jj} 
\label{sub:p-1}\\
& & \Gamma, k:J, \Gamma',\AT{\jj}{\II} \vdash \Ty \RHD \K \label{sub:ty-1}\\
\text{From (\ref{sub:q-1})}
& & 
\Gamma,\Gamma'\sub{\n}{k}, \ii : \minus{\II}\sub{\n}{k},\X:\Ty\sub{\ii}{\jj}\sub{\n}{k}  \vdash \QQ\sub{\n}{k}  \rhd
\Ty\sub{\ii+1}{\jj}\sub{\n}{k} \label{sub:q-2}\\
\text{From (\ref{sub:p-1})}
& & \Gamma, \Gamma'\sub{\n}{k} \vdash 
\PP\sub{\n}{k}  \rhd\Ty\sub{0}{\jj}\sub{\n}{k} 
\label{sub:p-2}\\
\text{From (\ref{sub:ty-1})}
& & 
\Gamma,\Gamma'\sub{\n}{k},\AT{\jj}{\II}\sub{\n}{k} \vdash
\Ty\sub{\n}{k} \RHD 
\K\sub{\n}{k} 
\label{sub:ty-2}
\end{eqnarray}
}
From (\ref{sub:q-2}), (\ref{sub:p-2})
and (\ref{sub:ty-2}), by \tftrule{TPRec}, we obtain 
$\Gamma,\Gamma'\sub{\n}{k} \vdash
(\RECSEQP{\PP}{\ii}{\X}{\QQ})\sub{\n}{k} \rhd 
(\Pi \AT{\jj}{\II}.\Ty)\sub{\n}{k}$ as required.
\end{proof}


%We also use the following lemma for the branching 
%local types whose projections are extended by the mergeability operator  
%$\mergeop$. Below, $\subT$ denotes the standard 
%branching subtyping \cite{GH05,CHY07} 
%(the full definitions can be found in Figure~\ref{fig:subtyping} 
%in Appendix).   
%%congruwith the 
%%selection rule and its dual branching rules:
%\begin{center}
%{\small
%$
%\begin{array}{llll}
%\begin{prooftree}
%{\forall \ii\in I\subseteq J,\ \Gamma \vdash \T_\ii \subT \T_\ii'}
%\justifies
%{ \Gamma \vdash \LselI{\p}{\T_\ii'}{\ii}{I}\subT  \LselI{\p}{\T_\jj'}{\jj}{J}} \using\using\trule{Sel${}_\subT$}
%\end{prooftree}\\
%%\\
%%\begin{prooftree}
%%{\forall \ii\in J\subseteq I,\ \Gamma \vdash \T_\ii \subT \T_\ii'}
%%\justifies
%%{ \Gamma \vdash \LbranchI{\p}{\T_\ii'}{\ii}{I} \subT \LbranchI{\p}{\T_\jj'}{\jj}{J}} \using\trule{Bra${}_\subT$}
%%\end{prooftree}\\
%\end{array}
%$
%}
%\end{center} 
%%whose typability is extended by mergeability. 



==> basicproperties_tmp.tex <==
%\section{Formal results}
\section{Properties of typing}
\label{sec:property}
\noindent 
We study the two main properties of the typing system: one is the
termination of type-checking and another is type-soundness. The proofs
require a careful analysis due to the subtle interplay between
dependent types, recursors, recursive types and branching types.
\subsection{Basic properties}
\label{sec:basic}
%\noindent 
\noindent We prove here a series of consistency lemmas concerning permutations
and weakening
of judgements follow.
They are invariably deduced by induction on the derivations in the
standard manner.  

We use the following additional notations: $\Ga
\subseteq \Ga'$ iff $\AT{u}{S}\in \Ga$ implies $\AT{u}{S}\in \Ga'$ and
similarly for other mappings. In other words, $\Ga \subseteq \Ga'$
means that $\Ga'$ is a permutation of an extension of $\Gamma$.

\begin{LEM} \label{lem:basic}
\begin{enumerate}
\item (Permutation and Weakening)\ 
\label{lem:per}
Suppose $\Ga \subseteq \Ga'$ and $\Ga'\proves \Env$. Then 
$\Gamma \proves \judg$ 
implies
$\Gamma' \proves \judg$.  

\item (Strengthening)\ 
\label{lem:st}
$\Gamma,\AT{u}{U},\Gamma' \proves \judg$ 
and $u\not\in \fv(\Gamma', \judg)\cup \fn(\Gamma', \judg)$. Then $\Gamma,\Gamma' \proves \judg$.
Similarly for other mapping. 

\item (Agreement)
\label{lem:agree}
\begin{enumerate}
\item 
\label{lem:agreeEnv}
$\Gamma \proves J$ implies $\Gamma \proves \Env$. 
\item 
\label{lem:agreeK}
$\Gamma \proves \G \RHD \K$ implies 
$\Gamma \proves \K$. Similarly for other judgements. 

\item 
\label{lem:agreeEq}
$\Gamma \proves \G \equiv \G'$ implies 
$\Gamma \proves G \RHD \K$. Similarly for other judgements. 

\item 
\label{lem:agreeTy}
$\Gamma \proves P \rhd \Ty$ implies $\Gamma \proves \Ty \RHD \K$.
Similarly for other judgements. 
\end{enumerate}
\item (Exchange) 
\label{lem:agreeEx}
\begin{enumerate} 
\item 
\label{lem:ExT}
$\Gamma,\AT{u}{U},\Gamma' \proves \judg$ and $\Gamma \proves U\equiv
U'$. Then $\Gamma,\AT{u}{U'},\Gamma' \proves \judg$. 
Similarly for other mappings. 
\item 
\label{lem:ExI}
$\Gamma,\AT{\ii}{\II},\Gamma' \proves \judg$ and $\Gamma\models
\AT{\ii}{\II}=
\AT{\ii}{\II'}$. Then 
$\Gamma,\AT{\ii}{\II'},\Gamma' \proves \judg$. 

\item 
\label{lem:ExP}
$\Gamma,\PRED,\Gamma' \proves \judg$ and $\Gamma\models
\PRED=\PRED'$. Then 
$\Gamma,\PRED',\Gamma' \proves \judg$. 
\end{enumerate}
\end{enumerate}
\end{LEM}
\begin{proof}
By induction on the derivations. We note that the proofs are 
done simultaniously.  For the rules which use substitutions 
in the conclusion of the rule, such as \tfrule{TApp} in
Figure~\ref{fig:process-typing1}, 
we require to use the next substitution lemma simultaniously. 
We only show the most interesting case 
with a recursor. \\[1mm]
{\bf Proof of (3)(b). Case \trule{KRcr}:}  Suppose 
$\Gamma \vdash \GR{\G}{\AT{\ii}{\II^-}}{\xx}{\G'}  
\RHD \Pi\AT{\jj}{\II}. \K$ is derived by \trule{KRcr} in 
Figure~\ref{fig:kindsystembase}.  We prove $\Gamma \vdash  
\Pi\AT{\jj}{\II}. \K$. 
From $\Gamma, \ii:\II^- \vdash \G' \RHD \K\subst{i+1}{j}$ in the
premise of \trule{KRcr}, 
we have $\Gamma, \ii:\II^- \vdash \K\subst{i+1}{j}$ by inductive
hypothesis.  By definition of $\II^-$, this implies 
$\Gamma, \jj:\II \vdash \K$. Now by  \tfrule{KSeq}, 
we have $\Gamma\vdash \Pi\AT{\jj}{\II}.\K$, as desired. 
\qed
\end{proof}
The following lemma which states that well-typedness is
preserved by substitution of appropriate values for variables, is the
key result underlying Subject Reduction. This also guarantees that 
the substitution for the index which affects to a shared environment and
a type of a term, and the substitution for a process variable are
always well-defined.  
Note that 
%shows that, under certain circumstances, a variable can be replaced
%% by an index or a term throughout a judgement, although this
%% 
substitutions may change session types and environments in the index case.
%% The application of (1) to process judgements is especially useful for the
%% Subject Reduction Theorem:  
%% if \derqq{\Ga,\ptilde{\ii}:\II,\Ga'}{\Sigma}{\PP}{\Ty} and 
%% \der{\Ga}{\n}{\Nat} with $\Ga\models \n: \II$, then 
%% $\derqq{\Ga,(\Ga'\subst{\n}{\ii})}{\Sigma}{\PP\subst{\n}{\ii}}{\Ty\subst{\n}{\ii}}$. 

\begin{LEM}[Substitution Lemma]\label{lem:substitution}
\begin{enumerate}
\item \labelx{subs01} 
If ${\Ga,\ptilde{\ii}:\II,\Ga'}\proves_\Sigma {\judg}$ and 
$\Ga\models \n: \II$, then 
${\Ga,(\Ga'\subst{\n}{\ii})}\proves_\Sigma \judg\subst{\n}{\ii}$.
%If \der{\Ga,\ptilde{\ii}:\II,\Ga'}{\PP}{\Ty} and 
%\de\Ga{\n}{\Nat} with $\Ga\models \n: \II$, then 
%\der{\Ga,\Ga'\subst{\n}{\ii}}{\PP\subst{\n}{\ii}}{\Ty\subst{\n}{\ii}}.
\item \labelx{subs02} 
If \derqq{\Ga,\ptilde{\X}:\ptilde{\D_0}}{\Sigma}{\PP}{\Ty} and 
\de\Ga{\ptilde{\QQ}}{\D_0}, then
\derqq{\Ga}{\Sigma}{\PP\subst{\QQ}{\ptilde{X}}}{\Ty}.
\item \label{subs1} 
If \derqq{\Ga,\ptilde{\x}:\ptilde{\ST}}{\Sigma}{\PP}{\D} and \de\Ga{\ptilde{v}}{\ptilde{\ST}}, then
\derqq{\Ga}{\Sigma}{\PP\subst{\ptilde{\va}}{\ptilde{\x}}}{\D}.
\item \labelx{subs2} If
\derqq{\Ga}{\Sigma}{\PP}{\D,\y:\T}, then
\derqq{\Ga}{\Sigma}{\PP\sub{\si\s \pv}{\y}}{\D,\si\s \pv:\T}.
\end{enumerate}
\end{LEM}
\begin{proof}
By induction on the derivations.
We prove the most interesting case: 
if \derqq{\Ga,\ptilde{\ii}:\II,\Ga'}{\Sigma}{\PP}{\Ty} and 
\der{\Ga}{\n}{\Nat} with $\Ga\models \n: \II$, then 
$\derqq{\Ga,(\Ga'\subst{\n}{\ii})}{\Sigma}{\PP\subst{\n}{\ii}}{\Ty\subst{\n}{\ii}}$
when the last applied rule is \tfrule{TPRec}. 
Assume 
\[
\Gamma,k:J, \Gamma' \vdash \RECSEQP{\PP}{\ii}{\X}{\QQ} \rhd \Pi
\AT{\jj}{\II}.\Ty 
\quad \mbox{with} \quad \Ga\models \n: J
\]
is derived from \tfrule{TPRec}. This is derived by: 
{\small
\begin{eqnarray}
& & 
\Gamma,k:J, \Gamma', \ii : \minus{\II},\X:\Ty\sub{\ii}{\jj}  \vdash \QQ  \rhd
\Ty\sub{\ii+1}{\jj} \label{sub:q-1}\\
& & 
\Gamma, k:J, \Gamma'\vdash \PP  \rhd\Ty\sub{0}{\jj} 
\label{sub:p-1}\\
& & \Gamma, k:J, \Gamma',\AT{\jj}{\II} \vdash \Ty \RHD \K \label{sub:ty-1}\\
\text{From (\ref{sub:q-1})}
& & 
\Gamma,\Gamma'\sub{\n}{k}, \ii : \minus{\II}\sub{\n}{k},\X:\Ty\sub{\ii}{\jj}\sub{\n}{k}  \vdash \QQ\sub{\n}{k}  \rhd
\Ty\sub{\ii+1}{\jj}\sub{\n}{k} \label{sub:q-2}\\
\text{From (\ref{sub:p-1})}
& & \Gamma, \Gamma'\sub{\n}{k} \vdash 
\PP\sub{\n}{k}  \rhd\Ty\sub{0}{\jj}\sub{\n}{k} 
\label{sub:p-2}\\
\text{From (\ref{sub:ty-1})}
& & 
\Gamma,\Gamma'\sub{\n}{k},\AT{\jj}{\II}\sub{\n}{k} \vdash
\Ty\sub{\n}{k} \RHD 
\K\sub{\n}{k} 
\label{sub:ty-2}
\end{eqnarray}
}
From (\ref{sub:q-2}), (\ref{sub:p-2})
and (\ref{sub:ty-2}), by \tfrule{TPRec}, we obtain 
$\Gamma,\Gamma'\sub{\n}{k} \vdash
(\RECSEQP{\PP}{\ii}{\X}{\QQ})\sub{\n}{k} \rhd 
(\Pi \AT{\jj}{\II}.\Ty)\sub{\n}{k}$ as required. \qed 
\end{proof}


%We also use the following lemma for the branching 
%local types whose projections are extended by the mergeability operator  
%$\mergeop$. Below, $\subT$ denotes the standard 
%branching subtyping \cite{GH05,CHY07} 
%(the full definitions can be found in Figure~\ref{fig:subtyping} 
%in Appendix).   
%%congruwith the 
%%selection rule and its dual branching rules:
%\begin{center}
%{\small
%$
%\begin{array}{llll}
%\begin{prooftree}
%{\forall \ii\in I\subseteq J,\ \Gamma \vdash \T_\ii \subT \T_\ii'}
%\justifies
%{ \Gamma \vdash \LselI{\p}{\T_\ii'}{\ii}{I}\subT  \LselI{\p}{\T_\jj'}{\jj}{J}} \using\using\trule{Sel${}_\subT$}
%\end{prooftree}\\
%%\\
%%\begin{prooftree}
%%{\forall \ii\in J\subseteq I,\ \Gamma \vdash \T_\ii \subT \T_\ii'}
%%\justifies
%%{ \Gamma \vdash \LbranchI{\p}{\T_\ii'}{\ii}{I} \subT \LbranchI{\p}{\T_\jj'}{\jj}{J}} \using\trule{Bra${}_\subT$}
%%\end{prooftree}\\
%\end{array}
%$
%}
%\end{center} 
%%whose typability is extended by mergeability. 



==> bmarks.tex <==
%\subsection{Implementation Experience}
\label{subsec:bmarks}
\paragraph{Implementation experience}
%
We discuss some preliminary benchmark results that demonstrate how the greater expressiveness of dependent multiparty types in comparison to binary sessions permits significant performance improvement.
An overview of parallel algorithm implementation using SJ, \cite{HU07TYPE-SAFE,SJwebsite}, an extension of Java for 
%type-safe, 
\textit{binary} session programming with multicast constructs, was discussed in \cite{BHY09}. The features of SJ make it a suitable target language for (an adapted) dependent global type projection, giving the main interaction structures for concrete, executable end-point implementations. 

One of the algorithms implemented in \cite{BHY09} is a parallel simulation of the $n$-Body Problem \cite{GLSkjellum}. The $n$-Body simulation features an advanced interaction structure based on the ring topology, for which the projection algorithm has been outlined above. (\cite{BHY09} also presents session-typed implementations of algorithms featuring other topologies, such as mesh-based Jacobi iteration.) 
%The basic idea is to divide the particles being modelled between a group of processes. A simulation step involves update packets forwarded from each process around the ring until each process has seen all updates from the others. Processes perform a partial calculation as each update is received; the full calculation for the simulation step is completed after all updates have been seen.
Due to the restrictions of binary session typing, the direct SJ implementation 
%requires three distinct roles for (Starter, Middle and Final workers), and also 
involves the creation of one fresh session per simulation step between
Starter and Final (the final ring link) in addition to the main
sessions between each of the other neighbouring nodes
\cite{BHY09}. Without transport-specific runtime support for reusing
old connections, this can become a costly overhead. \ny{However, with
%dependent global types,  we can clearly design how 
%each role realises a whole protocol with multicast
%primitives,  completely avoiding this nested session problem.
dependent global types, we can design the behaviour of 
each role clearly within the construction of the whole multiparty protocol, 
%with multicast primitives, 
completely avoiding this nested session problem.  
%whilst reducing the number of distinct roles to two: as described above, the Master $\W[n]$ (who bootstraps the simulation) and the general Workers $\W[i]$ ($0 \leq i < n$). (The dependent typing aspect is of course required to specify a general global type for $n$ parties.) 
Communication-safety and deadlock-freedom for the resulting implementation are ensured
for any configuration of $m > 1$ parties.}
%we omit the details here, see \cite{fullversion} for the full types and implementations.

In the experiment, we compared the performance of the original binary
session version against the implementations derived from projection
(for the purposes of practical benchmarks, we also make use of
asynchronous communication subtyping \cite{esop09} after projection).
%\textit{after} projection, which is fully compatible with the dependent typing presented in this paper). 
The benchmark was executed in a low latency cluster environment (TCP
over gigabit Ethernet), varying the number of processes, simulations
steps and particles (distributed evenly). As expected, the latter,
without the nested session overhead, performs significantly better
across all parameter combinations; for instance, with 10 processes
performing 100 simulations steps on 100 particles each, the direct SJ
implementation took on average 180s whilst the projected
implementation took 103s, an improvement of 43\%. The full source code
for the benchmark applications, exact benchmark environment details
and the complete results can be found at \cite{fullversion}.


==> conclusions.tex <==
%\input{shortprotocol}

\section{Conclusion and related work}
\label{sec:related}
This paper studies a parameterised multiparty session type theory
which combines three well-known theories: indexed dependent types
\cite{DBLP:conf/popl/XiP99}, dependent types with
recursors \cite{DBLP:conf/mfps/Nelson91}
and multiparty session types \cite{BettiniCDLDY08LONG,CHY07}.
The resulting typing system is decidable (under
an appropriate assumption about the index arithmetic).
It offers great expressive power
for describing complex communication topologies
and guarantees safety properties of processes running under
such topologies.
We have explored the impact of
parameterised type structures for
communications
through implementations of the above web service usecases and of several parallel
algorithms in Java and C with session
types~\cite{HU07TYPE-SAFE,HKOYH10}, including
the N-body (with a ring topology),
the Jacobi method
(with sequence and mesh topologies)
and the FFT \cite{NYPHK11,NYH12}.
We observe (1) a clear coordination
of the communication behaviour of each party with the
construction of the whole multiparty protocol, thus reducing
programming errors and ensuring deadlock-freedom; and (2)
a performance benefit against the original binary session version,
reducing the overhead of multiple binary session
establishments (see also \cite{NYPHK11,NYH12}).
Full implementation and integration of our theory
into~\cite{HU07TYPE-SAFE,CorinDFBL09,HKOYH10} is on-going work.

% \paragraph{Extensions to Web Services and Experiments}
%\paragraph{Programming experiments}
%%We further examine the expressiveness of our type theory by program
%%and type a real-world Web service usecase: Quote Request (C-U-002) is
%%the most complex scenario described in \cite{CDLRequirements}, the
%%public document authored by the W3C Choreography Description Language
%%Working Group. Due to the space limitation, we leave the full
%%descriptions in Appendix \ref{sec:protocol}. In this usecase, a buyer
%%interacts with multiple suppliers who in turn interact with multiple
%%manufacturers (independently from others)
%%in order to obtain quotes for some goods or services;
%%after a supplier build their quotes from manufactures, the eventual
%%best quote is sent back to the buyer concurrently, then the buyer
%%chooses whether he agrees, requests the modified quote,
%%retries the loop or quits.
%%The specification is challenging, requiring the abilities to
%%repeat the set of interactions
%%between different participators,
%%and to refer a global description from within a
%%global description to support recursive behaviour, which
%%needs to go back to the different points depending
%%on the values of the quotes.
%%The full parameterised multiparty session types
%%can modularly construct
%%the whole protocol from a piece of the protocols,
%%and meet the Requirements
%%in \cite[Section 3.1.2.2]{CDLRequirements}.
%%In addition, by our asynchronous join primitive,
%%a pair can start and interact
%%independently without waiting for others, but all parties
%%can correctly synchronise at the necessary
%%points, and ensure the deadlock-freedom.

%We have explored the impact of the
%parametrised type structures for
%communications
%%% leads to
%%% clearer prospects regarding safety and resource usage.
%through implementation of the above use case as well as a few parallel
%algorithms with parameterised topologies in Java with session
%types~\cite{HU07TYPE-SAFE}, including
%%the $n$-Body Problem  (with a ring topology),
%the Jacobi method
%(with a sequence and a mesh)
%%, a linear
%%equation solver (using a toric mesh) and
%and the FFT (a butterfly network on an
%hypercube).
%We observe two immediate benefits: (1) a clear coordination
%of the communication behaviour of each party with the
%construction of the whole multiparty protocol, thus reducing the
%programming errors and ensuring deadlock-freedom; (2)
%a performance benefit against the original binary session version,
%reducing the overhead of multiple binary session
%establishments (see \cite{fullversion}).


\subsection{Related work}
We focus on the works on dependent types and other typed process
calculi which are related to multiparty session types; for further
comparisons of session types with other service-oriented calculi and
behaviour typing systems, see \cite{DL10} for a wide ranging survey of
the related literature.

\paragraph*{\bf Dependent types}
\noindent
The first use of primitive recursive functionals for dependent types
is in Nelson's $\mathcal{T}^\pi$~\cite{DBLP:conf/mfps/Nelson91}
for the $\lambda$-calculus, which is %% (as he stated)
a finite
representation of $\mathcal{T}^\infty$ by Tait and Martin L\"of
\cite{Tait,PerMartin}.
% for forming infinite sequences of terms and types.
$\mathcal{T}^\pi$ % The system \cite{DBLP:conf/mfps/Nelson91}
can type functions previously untypable in ML, and the finite
representability of dependent types makes it possible to have a
type-reconstruction algorithm. We also use the ideas from DML's
dependent typing system in \cite{DBLP:conf/popl/XiP99,DependentBook}
where type dependency is only allowed for index sorts, so that
type-checking can be reduced to a constraint-solving problem over
indices.
%over them.
Our design choice to combine both systems %are for
gives (1) the simplest formulation of sequences of global and end-point types and
processes described by the primitive recursor; (2) a precise specification
for parameters appearing in the participants based on index sorts; and (3) a
clear
%combination
integration with the full session types
%with
and general recursion, whilst ensuring decidability of type-checking (if the
constraint-solving problem is decidable).
%Based on these work,
From the basis of these works,
our type equivalence
does not have to rely on
behavioural equivalence between processes, but only on the strongly
normalising {\em types} represented by recursors.

Dependent types have been also studied in the context
of process calculi, where the dependency centres
on locations (e.g.~\cite{Hennessy07}),
and channels (e.g.~\cite{Yoshida04}) for mobile agents or
higher-order processes.
An effect-based session typing system
for corresponding assertions to specify fine-grained
communication specifications is studied
in \cite{BAG05} where effects can appear both in types and
processes.
None of these works investigate families of global specifications using
dependent types.
Our main typing rules require a careful treatment for type
soundness not found in the previous works, due to the simultaneous instantiation
of terms and indices by the recursor, with reasoning by mathematical induction
(note that type soundness was left open in \cite{DBLP:conf/mfps/Nelson91}).

\paragraph*{\bf Types and contracts for multiparty interactions}
The first papers on multiparty session types were \cite{BC07} and
\cite{CHY07}. The former uses a distributed calculus where
each channel connects a master end-point to one or more slave
endpoints; instead of global types, they use only
local types.
% %a few work on its extension is
Since the first
work \cite{CHY07} was proposed, this theory has been used in the
different contexts such as distributed protocol implementation and
optimisation~\cite{SivaramakrishnanNZE10},
security~\cite{CorinDFBL09,ccdr10},
design by contract~\cite{BHTY10},
parallel algorithms~\cite{NYPHK11,NYH12}, web services~\cite{YDBH10},
multicore programming~\cite{YoshidaVPH08},
an advanced progress guarantee~\cite{BettiniCDLDY08LONG},
messaging optimisation~\cite{esop09},
structured exceptions~\cite{CGY10},
buffer and channel size analysis for multiparty
interactions~\cite{Bufferfull},
medical guidelines~\cite{NYH09} and
communicating automata \cite{DY12},
some of which initiated industrial collaborations, cf.~\cite{HondaMBCY11}.
%\NY
Our typing system can be smoothly integrated
with other works as no changes to the runtime typing components have been made
while expressiveness has been greatly improved.

%
%
%In type checking, local types are projected to binary
%sessions, so that type safety is ensured using duality, but it loses
%sequencing information: hence progress in a session interleaved with
%other sessions is not guaranteed.
%One of the benefits of our typing system is extendibility
%to other previously developed multiparty session typing systems, such as
%synchronous multiparty
%with multicasting \cite{BY08}, global progress for multiparty
%interleaved session types \cite{BettiniCDLDY08},
%asynchronous subtyping which allows
%for commutativity of actions,
%and sum types for symmetric synchronisations since in our approach,
%the runtime typing system does not have to be modified.

The work \cite{carbone.honda.yoshida:esop07}
presented an {\emph{executable global processes}}
for web interactions
based on binary session types.
Our work provides flexible, programmable  global descriptions
as {\em types}, offering a progress for parameterised multiparty
session, which is not ensured in \cite{carbone.honda.yoshida:esop07}.

% the type disciplines for the two global and local process calculi
% in \cite{carbone.honda.yoshida:esop07}
% are based on {\em binary} session types;
% hence safety and progress for multiparty interactions were
% not considered, while the current paper offers
% safe, parameterised multiparty interactions
% towards enriching the facility of global types.

The work \cite{B10} provides a programming idiom of roles, defining
different classes of participants, and a different type system for
parameterised session types. There is no investigation of the system
expressivity for the 3D-Mesh pattern as we have presented in this
paper through the Fast Fourier Transformation example.  The static
type system follows the typing strategy and programming methodology of
multiparty session types: programmers first define the global type of
the intended pattern and then define each of the roles; the roles are then
validated through projection of the global type onto the principals by
type-checking.

%A work \cite{B10} aims to find a way to automatically extract
%different classes of participants (called ``roles'') from
%parameterised global types.  Although not as general (it cannot treat
%3D-meshes or butterfly topologies such as the Fast Fourier Transformation
%example presented in this paper), this technique can remove the need for some
%local type equivalences when the global types are limited to certain classes of
%rings, trees and 2D-meshes.
%"Recently, the idea of parameterised session types has been studied
%also in \cite{DBLP:conf/icfem/Bejleri10}, introducing a programming
%idiom of roles and a new type system. Roles provide a similar concept
%to classes in class-based languages and so, offer a design on how to
%incorporate parameterised session types into a mainstream language
%such as Java and C#. The static type system follows the typing
%strategy and programming methodology of multiparty session types
%\cite{CHY07}: programmers first define the global type of the intended
%pattern and then define each role of it; roles are validated through
%projection of the global type onto the principals by type-checking.
%Strict global type annotations and efficient type-checking are
%achieved by extending the multiparty~s projection algorithm to
%parameterised principals. Values of parameters range over infinite
%sets of natural numbers, providing full computation power to correct
%programs that implement parameterised sessions. However, the examples
%in that paper are limited to patterns such as Ring, Tree and Mesh.
%There is no investigation of the system expressivity for the 3D-Mesh
%pattern as we have presented in this paper through the Fast Fourier
%Transformation example."

Recent formalisms for typing multiparty interactions include
\cite{CP09,CairesV09}.
%Contracts are more abstract (for example, they allow mixed choice)
%and focus on the local point of view.
These works treat different aspects of dynamic session structures.
{\em Contracts} \cite{CP09} % use a process-based specification of
% protocols, where conformance means Must-preorder (so that we can
% ensure liveness). The system in \cite{CP09}
can type more processes
than session types, thanks to the flexibility of process syntax
for describing protocols.
However, typable processes themselves in \cite{CP09} may
not always satisfy the properties of session types such as progress: it is
proved later by checking whether the type meets a certain form.  Hence
proving progress with contracts effectively
requires an exploration of all possible paths (interleaving, choices)
of a protocol.  The most complex example of~\cite[\S~3]{CP09} (a group
key agreement protocol from~\cite{AST98}), which is typed as
$\pi$-processes with delegations, can be specified and articulated
by a single parameterised
global session type as:
{\small
\begin{align*}
\label{group}
 \Pi \AT{n}{I}.(& \FOREACH{i}{<n}{\GS{\W[n-i]}{\W[n-i+1]}{\Nat}};\\
               & \FOREACH{i}{<n}{\GS{\W[n-i]}{\W[n+1]}{\Nat}.\GS{\W[n+1]}{\W[n-i]}{\Nat}})
\end{align*}
}
%
%If
Once the end-point process conforms to this specification, we can
automatically guarantee communication safety and progress.
% Another
% merit of using (dependent) types is a clearly articulated,
% programs which clarify interaction structures, in correspondence with
% the type description such as above.
%via end-point projection.
%%The example highlight the difference between two
%approaches: our parameterised session type to start from
%the global specification automatically guarantee
%the properties, while they start local specifications
%and check the properties later.
%In fact, The meaningful global specification of choreographies ensured in the
%multiparty case is left for future work in \cite{CP09}.
%
%Parameterised session types, on the other hand, do not support a change
%in the number of participants once the parameters have been instantiated.
%They however support the execution of a session whose parameters have only been
%chosen at run-time. The main example of~\cite{CP09} (a group key agreement
%protocol taken from~\cite{AST98}) can be easily written in our framework:
%%
%{\small
%\begin{align*}
% \Pi \AT{n}{I}.(& \FOREACH{i}{<n}{\GS{\W[n-i]}{\W[n-i+1]}{\Nat}};\\
%               & \FOREACH{i}{<n}{\GS{\W[n-i]}{\W[n]}{\Nat}.\GS{\W[n]}{\W[n-i]}{\Nat}})
%\end{align*}}
%%
%Such behaviour can be achieved in our framework by the dynamic
%choice of new session parameters. The goal of our work is to improve the
%expressiveness of global interaction specifications thanks to the parametrised
%global types and, more importantly, to feature a static type system that works
%from this global specification.

% We believe that most of these ideas and mechanisms are still to be combined and
% simplified in order to have, first, a core calculus on which theoretical results
% can be proved, then an expressive enough language that can specify both web
% services and distributed algorithms, and finally an effective verification
% mechanism that can, statically or dynamically, ensure the safety and progress of
% communications.

%%Another aspect of dynamic interaction structures is treated in


{\em  Conversation Calculus} \cite{CairesV09} supports the dynamic
joining and leaving of participants.
We also introduced a dynamic role-based multiparty session type
discipline in previous work \cite{DY11}, where an arbitrary number of participants can
interact in a running session via a universal polling operator. This
work was extended with simple relations between roles
in \cite{Poon11} to dynamically handle
the complex topologies presented in this paper.
Although the formalism in \S~\ref{subsec:semantics} can operationally capture some dynamic
features, the aim of the present work is
%{\em not}
not
the type-abstraction
of dynamic interaction patterns. Our purpose is
to capture, in a single type description, a family
of protocols over arbitrary numbers of participants,
to be instantiated at runtime.
Parameterisation gives freedom not possible with previous session
types: once typed, a parametric process is ensured that its arbitrary
well-typed instantiations, in terms of both topologies and process
behaviours, satisfy the safety and progress properties of typed
processes, without the cost of complex runtime support (as in \cite{DY11}).
Parameterisation, composition and repetition are common idioms in
parallel algorithms and choreographic/conversational interactions, all
of which are uniformly treatable in our dependent type theory. Here
types offer a rigorous structuring principle which can economically
abstract rich interaction structures, including parameterised ones.
% , whose
% effectiveness has been demonstrated
% through the description and typing of a wide range of practical multiparty
% protocols.
%
% where while preserving all properties of typable processes in the original
% first-order type discipline \cite{CHY07}.
% enable a rigorous type abstraction of
% parameterised multiparty protocols, capturing in a single
%
% do not change
% the number of participants once the parameters have been instantiated,
% but support the execution of a session whose parameters have only been
% chosen at runtime. Based on this facility, the dynamic choice of new
% session parameters (i.e. a new participant can join to a
% sub-multiparty session) can be simulated by creating a sub-session
% through passing a new name with indices which depend on that name (more
% exactly, we would use channel dependent types from \cite{Yoshida04}).
% Formal theories of contracts using multiparty interaction
% structures other than multiparty session types are studied in
% \cite{CastagnaGP08} using CCS-like processes as a type
% representation. The recent work \cite{CP09} extends
% \cite{CastagnaGP08} with the treatment of mobile and forwarding channels,
% comparing its expressiveness with session types. Another recent
% work~\cite{CairesV09} presents a typed calculus for service
% orientation by extending the $\pi$-calculus with context-sensitive
% interactions, equipped with service and request primitives. Our
% method differs from these approaches since we start from programming
% general topologies as global specifications, hence various dynamic,
% parameterised communications can be explicitly described for a shared
% agreement among multiple peers. Our system allows
% participant identities to change during program execution by index
% instantiation, which is effective, in particular, for data exchange
% across complex %but programmable
% structures such as the butterfly topology.
% The work~\cite{SOCK08C} proposes a distributed calculus with sessions that
% incorporates the merging of running sessions; however, type-safety for
% interleaved sessions is left as an open problem. Parameterisation and repetition
% are widely appearing idioms in most parallel algorithms and choreographic
% interactions, and with session delegations, they can represent a mechanism for
% merging conversations with progress combining with \cite{GProgress08};
% %however,
% dynamic features such as late joining
% and a service discovery facility are complementary with our
% work, but the extensions to these features
% are interesting research topics. The
% preceding works do not treat the main technical problems addressed in
% the present work ---
% %programming and treating
% programming methodology and a formal system for dynamically changing global
% specifications and type-safety via a general projection method in a dependent
% type format, backed-up by efficient type-checking and resource usage, and
% ensuring strong safety properties for complex topologies based on the
% parameterised multiparty session type discipline.
%
%A calculus of service-oriented computing is introduced in
%\cite{VieiraCS08}, where a conversation models the interactions
%between a client and various services. New primitives of communication
%are introduced such as conversation context (shared interaction point)
%communication and communication inside an end-point.
%
%Different approaches to the description of service-oriented multiparty
%communications are considered in \cite{SCBravettiZ07,SOCK08C}.  In
%\cite{SCBravettiZ07}, the global and local views of protocols are
%described in two different calculi and the agreement between these
%views becomes a bisimulation between processes; \cite{SOCK08C}
%proposes a distributed calculus which provides communications either
%inside sessions or inside locations, modelling merging running
%sessions. The type-safety and progress in interleaved sessions are
%left as an open problem in \cite{SOCK08C}.
%
%\begin{itemize}
%\item All multiparty session types papers.
%%\item Conversation Calculus
%\item More recent paper of contracts from Beppe's home page.
%\item Mergeability (ESOP'07 by Carbone et al, Tutorial Paper by
%  Carbone et al, Lasse's new paper(from his home page))
%
%\end{itemize}
%
%\paragraph*{Web Services.}
%We are currently designing and implementing a modelling and
%specification language with multiparty session types \cite{scribble}
%for the standards of business and financial protocols with our
%industry collaborators \cite{UNIFI,CDL}.
%
%This language consists of three layers: the first layer is a global type which
%corresponds to a signature of class models in UML; the second one is
%for conversation models where signatures and variables for multiple
%conversations are integrated; and the third layer includes extensions
%of the existing languages (such as Java \cite{HU07TYPE-AFE}) which
%implement conversation models.  We are currently considering to extend
%this modelling framework with our type discipline so that we can
%specify and ensure progress for executable conversations.
%This paper presents a language of contracts to capture the behaviour of
%mobile processes that dynamically generate and forward channels.
%Unlike session types, which equip channels with types and processes
%with type environments, contracts give behavioural types to processes
%themselves.  The authors show that their contracts can be used to
%prove progress (deadlock freedom) for a wider range of processes than
%session types (and with less complicated restrictions.)  On the other
%hand, proving progress with contracts is not compositional: it
%effectively requires an exploration of all possible paths
%(interleavings, choices) in a process.


%\paragraph{\bf Acknowledgements.}
%%\noindent{\bf Acknowledgements.}
\section*{Acknowledgements}

We thank the reviewers,
Lasse Nielsen and Dimitris Mostrous for their useful comments for the
paper and  Kohei Honda for discussions, and
Michael Emmanuel, Yiannos Kryftis, Nicholas Ng, Olivier Pernet and Hok Shun Poon
for their implementation work of the examples presented
in this paper.
The work is partially supported by EPSRC EP/G015635/1 and EP/F003757/1, and the NSF Ocean Observatories Initiative. The last author was also supported by EPSRC PhD Plus and EPSRC Knowledge Transfer Secondment.



==> fft.tex <==
%\subsection{FFT on a butterfly network}

\input{fig_fft}

%\paragraph{\bf FFT} %in figure~\ref{fig:fft}}
\subsection{Fast Fourier Transform}
\label{subsec:fft}
\noindent 
% As an expressiveness test for our global specification language,
We describe a
parallel implementation of the Fast Fourier Transform algorithm (more
precisely the radix-2 variant of the Cooley-Tukey % FFT
algorithm~\cite{CT65}).
% 
% his subsection attests the expressiveness of our global specification language
% by describing the Fast Fourier Transform (FFT) algorithm over a butterfly network.
% The FFT
% % is an algorithm that computes the Discrete
% % Fourier Transform (DFT) of a discrete function. It
% is one of the most widely used algorithms in computer science and
% engineering. Its application range from signal processing to big integer
% multiplication. It is also easily parallelisable and fast in the
% parallel domain. % : the butterfly is chosen since one of the most 
% % widely used topologies for FFT with complex, dynamic connections
% 
We start by a quick reminder of the discrete fourier transform definition,
followed by the description of an FFT algorithm that implements it over a
butterfly network. We then give the corresponding global session type. From the
diagram in (b) and the session type from (c), it is finally straightforward to
implement the FFT as simple interacting processes.

\paragraph{\bf The Discrete Fourier Transform}  
The goal of the FFT is to compute the Discrete Fourier Transform
(DFT) of a vector of complex numbers.
Assume the input consists in $N$ complex numbers $\vec{x}=x_0, \ldots,
x_{N-1}$ that can be interpreted as the coefficients of a polynomial
$f(y)=\sum_{j=0}^{N-1}x_j\,y^j$.  The DFT transforms $\vec{x}$ in a vector
$\vec{X}=X_0, \ldots, X_{N-1}$ defined by:
$$
X_k = f(\omega_N^k) 
$$\\[-3ex]
\noindent
with $\omega_N^k=\e^{ \imath\frac{ 2 k\pi }{N}}$ one of the $n$-th primitive
roots of unity. The DFT can be seen as a polynomial interpolation on the
primitive roots of unity or as the application of the square matrix
$(\omega_N^{ij})_{i,j}$ to the vector $\vec{x}$.
% 
% %We first summarise FFT over the butterfly network \cite[\S~3.7]{FThomson}. 

\paragraph{\bf FFT and the butterfly network} 
We present % here 
the radix-2 variant of the Cooley-Tukey % FFT
algorithm~\cite{CT65}. % Assuming that $N$ is a power of $2$, this FFT algorithm
It uses a divide-and-conquer strategy based on the following equation (we use
the fact that $\omega_N^{2k}=\omega_{N/2}^k$):

\[
\begin{array}{rcl}
  X_k& = & \sum_{j=0}^{N-1}x_j\,\omega_N^{jk} \\[1mm]
%        & = & \sum_{j=0}^{N/2-1}x_{2j}\,\omega_N^{2jk}
%   + \sum_{j=0}^{N/2-1}x_{2j+1}\,\omega_N^{(2j+1)k}\\[1mm]
  & = &\sum_{j=0}^{N/2-1}x_{2j}\,\omega_{N/2}^{jk}
  + \omega_N^k\sum_{j=0}^{N/2-1}x_{2j+1}\,\omega_{N/2}^{jk}
\end{array}
\]
Each of the two separate sums are DFT of half of the original vector members,
separated into even and odd. Recursive calls can then divide the input set
further based on the value of the next binary bits. The good complexity of this
FFT algorithm comes from the lower periodicity of $\omega_{N/2}$: we have
$\omega_{N/2}^{jk}=\omega_{N/2}^{j(k-N/2)}$ and thus computations of $X_k$ and
$X_{k-N/2}$ only differ by the multiplicative factor affecting one of the two
recursive calls.

Figure~\ref{fig:fft}(a) illustrates this
recursive principle, called {\em butterfly}, where two
different intermediary values can be computed in constant time from the results
of the same two recursive calls. % ($\omega_N$ is the $N$th primitive root of
                                % unity). 

The complete algorithm is illustrated by the diagram from
Figure~\ref{fig:fft}(b).  It features the application of the FFT on a network of
$N=2^3$ machines on an hypercube network computing the discrete Fourier
transform of vector $x_0, \ldots, x_7$.  Each row represents a single machine at
each step of the algorithm. Each edge represents a value sent to another
machine. The dotted edges represent the particular messages that a machine sends
to itself to remember a value for the next step.  Each machine is successively
involved in a butterfly with a machine whose number differs by only one
bit. Note that the recursive partition over the value of a different bit at each
step requires a particular bit-reversed ordering of the input vector: the
machine number $\pp$ initially receives $x_{\overline{\pp}}$ where
$\overline{\pp}$ denotes the bit-reversal of $\pp$.

% Figure~\ref{fig:fft}(c) gives the global session type describing the
% interactions between $2^n$ machines. The first iterator is the initialisation
% step. Then we have an iteration over variable $l$ for the $n$ successive steps
% of the algorithm.  Figure~\ref{fig:fft}(d) defines the processes that each of
% the machines runs.  Each process returns the final answer at
% $r_{\p}$.% executes to run the algorithm.

% The FFT algorithm relies on the mathematical relations that exist within the
% group of primitive roots to avoid recomputing twice the same value. For a vector
% of $N=2^n$ numbers, the sequential complexity is $N\log{N}$ and it benefits from
% an excellent $O(N)$ speedup on a butterfly network of $N$ machine to reach a
% complexity of $\log{N}$.

% Figure~\ref{fig:fft} illustrates the butterfly network topology for $N=2^3=8$.

% This parallel version of the FFT algorithm gives an excellent $O(N)$ speedup on
% a butterfly network of $N$ machines when applied on a vector of size $N$. It has
% also the advantage of being able to compute the DFT inverse by just changing the
% multiplication factors of each butterfly. Finally, this algorithm can be
% implemented easily on common network topologies such as the hypercube.
% %Variants of the
% %butterfly topology include changing the degree ($2$ in our case) which means
% %recursing on a bigger number of smaller instances.

\paragraph{\bf Global Types}
Figure~\ref{fig:fft}(c) gives the global session type corresponding to the
execution of the FFT.  The size of the network is specified by the index
parameter $n$: for a given $n$, $2^n$ machines compute the DFT of a vector of
size $2^n$. The first iterator
$\FOREACH{\ii}{<2^n}{\GS{i}{i}{\Nat}};$
% $\RECSEQ{(\ldots)}{k}{\uuu}{\GS{k}{k}{\Nat}.\uuu}$ 
concerns the initialisation:
each of the machines sends the $x_\pp$ value to themselves. Then we have an
iteration over variable $l$ for the $n$ successive steps of the algorithm. The
iterators over variables $i,j$ work in a more complex way: at each step, the
algorithm applies the butterfly pattern between pairs of machines whose numbers
differ by only one bit (at step $l$, bit number $n-l$ is concerned). The iterators
over variables $i$ and $j$ thus generate all the values of the other bits: for
each $l$, $i*2^{n-l}+j$ and $i*2^{n-l}+2^{n-l-1}+j$ range over all pairs of
integers from $2^n-1$ to $0$ that differ on the $(n-l)$th bit. The four repeated
messages within the loops correspond to the four edges of the
butterfly pattern.



% Integers from $2^n-1$ to $0$ are generated using their binary
% representation: $i$ corresponds to the $l-1$ first bits, variables $k$ or $k'$
% represent the $l$-th bit and $j$ gives the $n-l-1$ last bits. This way, the
% integers $i*2^{n-l}+k*2^{n-l-1}+j$ and $i*2^{n-l}+k'*2^{n-l-1}+j$ range over all
% integers from $2^n-1$ to $0$ and only differ (if they differ) on their $l$-th
% bit. This test on the $l$-th bit is the direct translation of the even/odd
% partition featured in the FFT algorithm. 
% Note that the inner most two recursors 
% $(\RECSEQ{z}{k}{u}{(\RECSEQ{u}{k'}{v}{ \cdots }})2)2$ 
% %%Moreover, the schema:
% %{\small\begin{align*}
% %   \ldots   &  (\RECSEQ{z}{k}{u}{  \\
% %        &  \quad (\RECSEQ{u}{k'}{v}{  \\
% %          & \qquad \GS{\W[i*2^{n-l}+k*2^{n-l-1}+j] \\
% %            & \quad \qquad }{\W[i*2^{n-l}+k'*2^{n-l-1}+j]}{\Nat}.u}\\
% %        & \quad)\APP  2} \\
% %      &)\APP  2\ \ldots\\
% %    \end{align*}
% %}
% %\noindent 
% exactly represents the $4$ edges of the butterfly pattern from
% figure~\ref{fig:fft}(a).

%Figure~\ref{fig:fft}(d) gives the end-point type that each of the machines has to
%satisfy in order to comply with the global type. Index $n$ is still a
%parameter. The main loop is an iteration over the $n$ steps of the
%algorithm. The natural projection would be:
%{\small
%\begin{align*}
% \T_{\pp} = &\ \Pi n.\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{}} \\
% & \quad (\LR{\End}{\l}{\xx} {\\
%   & \qquad
%   \ifthenelse{\bit{n-l}(\pp)=0\\
%     & \qquad} {\Lout{\pp+2^{n-l-1}}{\Nat}{\Lin{\pp+2^{n-l-1}}{\Nat}{\\
%         & \qquad \qquad\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}\\
%     & \qquad} {\Lout{\pp-2^{n-l-1}}{\Nat}{\Lin{\pp-2^{n-l-1}}{\Nat}{\\
%         & \qquad \qquad\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}}})\\
%& \APP n
%\end{align*}} The test $\bit{n-l}(\pp)=0$ corresponds to testing the value of
%the $k$ and $k'$ index from the global type. Each of the branches of the test
%have the two sends and two receives corresponding to the butterfly pattern.  For
%programming reasons (as seen in the processes), we have here shifted the
%self-receive $\Lin{\pp}\Nat{}$ from the initialization to the beginning of the
%loop iteration at the price of adding the last self-receive to the end:
%$\Lin{\pp}\Nat{\End}$. The lting type is in
%figure~\ref{fig:fft}(d).

\paragraph{\bf Processes}
The processes that are run on each machine to execute the FFT algorithm are
presented in Figure~\ref{fig:fft}(d). % We give the runtime syntax 
% which are annotated by the destinations for giving more information 
% to the reader.  
When $\pp$ is the machine number, $x_{\overline{\pp}}$ the initial value, and
$\y$ the session channel, the machine starts by sending $x_{\overline{\pp}}$ to
itself: $\y!\langle\x_{\overline{\pp}}\rangle$. The main loop corresponds to the
iteration over the $n$ steps of the algorithm. At step $l$, each machine is
involved in a butterfly corresponding to bit number $n-l$, i.e. whose number
differs on the $(n-l)$th bit. In the process, we thus distinguish the two cases
corresponding to each value of the $(n-l)$th bit (test on $\bit{n-l}(\pp)$). In
the two branches, we receive the previously computed value $\inpS{\y}\x{..}$,
then we send to and receive from the other machine (of number $\p+2^{n-l-1}$ or
$\p-2^{n-l-1}$, i.e. whose $(n-l)$th bit was flipped). We finally compute the
new value and send it to ourselves: respectively by
$\outS{\y}{\x+\z\,\omega_N^{g(l,\pp)}}{\X}$ or
$\outS{\y}{\z+\x\,\omega_N^{g(l,\pp)}}{\X}$. Note that the two branches do not
present the same order of send and receive as the global session type specifies
that the diagonal up arrow of the butterfly comes first. At the end of the
algorithm, the calculated values are sent to some external channels:
$\Poutend{r_\pp}{0}{\x}$.

% % The content of the loop consists of the
% % following actions: we receive the previously computed value $\inpS{\y}\x{..}$,
% % we then send it to the other machine involved in the current butterfly
% % $\outS{\y}{\x}{}$, we next receive the value this other machine sent
% % $\inpS{y}{\z}{}$, we finally compute the new value and send it to ourselves
% % $\outS{\y}{\x+\z\,\omega_N^{g(l,\pp)}}{\X}$ or
% % $\outS{\y}{\z+\x\,\omega_N^{g(l,\pp)}}{\X}$, depending on our position (up or
% % down) in the butterfly pattern (given by $\bit{n-l}(\pp)$). 

% We show our static type-checking can guarantee communication-safety 
% and deadlock-freedom for a whole group of $N$-processes 
% over this complex butterfly topology. 

% More concretely, we start from a polynomial $f$ defined by
% $f(X)=\sum_{i=0}^{N-1}x_iX^i$ and we want its values over the primitive roots of
% unity: $\omega_N^0,\omega_N^1, \ldots, \omega_N^{N-1}$.

% The figure~\ref{fig:fft} presents the butterfly topology used by the
% algorithm. The principle is that a message is exchanged at step $l$ between
% participants whose index only differ by the $l$-th bit. 
% %
% \begin{align*}
%   &\lambda n.\RECSEQP{\End}{\l}{\X}{\lambda \x.\inpS{\y}\z\\
%     & \quad
%     \ifthenelse{\bit{n-l}(\pp)=0}{\outS{\y}{\x+\y\omega_N^{g(l,\pp)}}{\X(\x+\y\omega_N^{g(l,\pp)})}\\
%     &\qquad }{\outS{\y}{\y+\x\omega_N^{g(l,\pp)}}{\X(\y+\x\omega_N^{g(l,\pp)})}}}
% \end{align*}


%\noindent where $g(l,\pp)=\pp \mod 2^l$
% We describe here a global session type specifying the messages involved in a
% butterfly topology. As a first approximation, we 

% \begin{align*}
% & \Pi d.\Pi n.  \\
% & (\RECSEQ{\End}{l}{x}{\\
%   & \quad (\RECSEQ{x}{i}{y}{ \\
%     & \qquad (\RECSEQ{y}{j}{z}{ \\
%       &  \quad \qquad (\RECSEQ{z}{k_1}{u}{  \\
%         &  \qquad \qquad (\RECSEQ{u}{k_2}{v}{  \\
%           & \quad \qquad \qquad \GS{W[l+1][i*d^{n-l}+k_1*d^{n-l-1}+j] \\
%             & \qquad \qquad \qquad }{W[l][i*d^{n-l}+k_2*d^{n-l-1}+j]}{\Nat}.v}\\
%         & \qquad \qquad)\APP  d} \\
%       & \quad \qquad)\APP  d} \\
%     & \qquad)\APP  d^{n-l-1}} \\
%   & \quad) \APP d^l } \\
% &) \APP n \\
% \end{align*}

% Let's describe an Omega network of degree $d$ with number of nodes $N=d*m=d^n$.
%   \begin{align*}
%     \Pi d.\Pi m.\Pi n. & (\RECSEQ{\End}{u}{l}{\\
%       & \quad (\RECSEQ{u}{i}{x}{ \\
%       & \qquad (\RECSEQ{x}{j}{y}{ \\
%       & \quad \qquad (\RECSEQ{y}{k}{z}{  \\
%         & \qquad \qquad  \GS{W[l+1][i*d+j]}{W[l][j*m+k]}{\Nat}.z})\\
%       & \quad \qquad\APP  d}) \\
%       & \qquad\APP  m}) \\
%       & \quad\APP  d}) \\
%       & \APP  n
%    \end{align*}

% The algorithm works in the following way:

% \begin{enumerate}
% \item The worker $W[l][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$
%   receives $x_1$ from $W[l+1][i*d^{n-l}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$ and
%   $x_2$ from $W[l+1][i*d^{n-l}+d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$. It
%   sends $x_1+
%   \omega_N^{d^{(n-l)}(k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j)}x_2$ to
%   $W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+j]$ and
%   $W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+d^{n-l-3}+j$.
% \item We start from the polynomial $\sum_{p=0}^{n-1} x_p X^p$ we want to
%   interpolate.
% \item The worker $W[d][p]$ initially holds the value $x_p$. The worker $W[0][p]$
%   finishes the session with $X_{\over{p}}$ (bit-reverse position).
% \item The base case worker $W[l][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$ has end-point
%   session type
%   ($i\in[0..d^l-1],j\in[0..d^{n-l-3}-1],k_1\in[0,d-1],k_2\in[0,d-1],k_3\in[0,d-1]$):
% {\small
% \begin{align*}
%   &
%   (\RECSEQ{\\
%     & \quad (\RECSEQ{\End
%   }{k_3'}{v}{ \\
%   & \qquad \qquad \Lout{W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3'*d^{n-l-3}+j]}{\Nat}{v}} \\
%   & \qquad\APP d)\\
%   & \quad
%   }{k_1'}{u}{ \\
%   & \qquad\Lin{W[l+1][i*d^{n-l}+k_1'*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]}{\Nat}{u}} \\
%   & \quad\APP d)\\
% %   & \Lin{W[l+1][i*d^{n-l}+d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]}{\Nat}{} \\
% %   & \Lout{W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+j]}{\Nat}{} \\
% %   & \Lout{W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+d^{n-l-3}+j]}{\Nat}{} \\
% \end{align*}
% }
% \item The first column of workers $W[n][i*d+k_1]$ has end-point
%   session type ($i\in[0..d^{n-1}-1],k_1\in[0,d-1]$):
% \begin{align*}
%   & (\RECSEQ{\End}{k_1'}{u}{\Lout{W[n-1][i*d+k_1']}{\Nat}{u}}\APP d)\\
% %   & \Lout{W[n-1][i*d]}{\Nat}{} \\
% %   & \Lout{W[n-1][i*d+1]}{\Nat}{\End} \\
% \end{align*}
% \item The last column of workers $W[0][k_1*d^{n-1}+j]$ has end-point
%   session type ($j\in[0..d^{n-1}-1],k_1\in[0,d-1]$):
% \begin{align*}
%   & (\RECSEQ{\End}{k_1'}{u}{\Lin{W[0][k_1'*d^{n-1}+j]}{\Nat}{u}}\APP d)\\
% %   & \Lin{W[1][j]}{\Nat}{} \\
% %   & \Lin{W[1][d^{n-1}+j]}{\Nat}{\End} \\
% \end{align*}

% \item The worker $W[l][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$
%   receives $x_1$ from $W[l+1][i*d^{n-l}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$ and
%   $x_2$ from $W[l+1][i*d^{n-l}+d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j]$. It
%   sends $x_1+
%   \omega_N^{d^{(n-l)}(k_1*d^{n-l-1}+k_2*d^{n-l-2}+k_3*d^{n-l-3}+j)}x_2$ to
%   $W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+j]$ and
%   $W[l-1][i*d^{n-l}+k_1*d^{n-l-1}+k_2*d^{n-l-2}+d^{n-l-3}+j$.
% \end{enumerate}


==> fig_global_kind.tex <==
\begin{figure}[h]
\small
\centering
\begin{tabular}{c}
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash \p \rhd \Nat, \p' \rhd \Nat \quad 
\Gamma   \vdash G' \RHD \Type\\[1mm]
\Gamma \vdash \U  \RHD \Type\quad \ftv(\U)=\emptyset\\[1mm]
\end{array}
}
\justifies
{\Gamma \vdash \GS{\p}{\p'}{\U}.\G' \RHD \Type} \using\trule{KIO}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \p \rhd \Nat, \p' \rhd \Nat \quad %\Gamma \vdash \p' \rhd \Nat \quad
  \forall \ii \in \II,\ \Gamma \vdash \G_i \RHD \Type}
\justifies
{\Gamma \vdash \GB{\p}{\p'} \RHD \Type} \using\trule{KBra}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \G \RHD \Type}
\justifies
{\Gamma \vdash \GM{\ty}{\G} \RHD \Type} \using\trule{KRec}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \G \RHD \K\subst{0}{j} \quad \Gamma, \ii:\II^- \vdash \G' \RHD \Type}
\justifies
{\Gamma \vdash \GR{\G}{\AT{\ii}{\II^-}}{\xx}{\G'}  
\RHD \Pi\AT{\jj}{\II}. \K} \using\trule{KRcr}
\end{prooftree}\\
\\ 
\begin{prooftree}
{\Gamma \vdash \Env}
\justifies
{\Gamma \vdash \ty \RHD \Type} \using\trule{KTVar}
\end{prooftree}\quad 
\begin{prooftree}
{\Gamma \vdash \Env}
\justifies
{\Gamma \vdash \xx \RHD \Type} \using\trule{KVar}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma, \ii:\II \vdash \G \RHD \K}
\justifies
{\Gamma \vdash \Pi\AT{\ii}{\II}.\G \RHD \Pi\AT{\ii}{\II}.\K} 
\using\trule{KPi}
\end{prooftree}
\begin{prooftree}
{\Gamma \vdash \G \RHD  \Pi\AT{\ii}{\II}.\K \quad \Gamma \models \tii : I}
\justifies
{\Gamma \vdash \G\APP\tii \RHD \K\sub{\tii}{\ii}} \using\trule{KApp}
\end{prooftree}
\end{tabular}
\caption{Kinding rules for global types} \label{fig:kindsystembase}
\end{figure}


==> fig_intro.tex <==

\begin{figure}[t]\centering
\begin{tabular}{lc}
{\bf \textsf Sequence topology}\\[-3ex]
\begin{minipage}{10em}
\xymatrix@C=10pt{
  *+[F]{\small \n}\ar[r]
  &*+[F]\txt{\small \n-1}\ar[r]
  &{\ldots}\ar[r]
  &*+[F]\txt{\small 0}}
\end{minipage} &
\quad \quad \quad \quad 
\begin{minipage}{5em}{\small\begin{align*}
      \Pi n.(& \RECSEQ{\End\\
        &\quad }{i}{\xx}{\GS{\W[i+1]}{\W[i]}{\Nat}.\xx}\APP \\
      &n)\\
    \end{align*}}
\end{minipage}
\\[-5ex]
% {\bf \textsf (b) Ring topology}\\[-3ex]
% \begin{minipage}{10em}
% \xymatrix@C=10pt{
%   *+[F]{\small \n}\ar[r]
%   &*+[F]\txt{\small \n-1}\ar[r]
%   &{\ldots}\ar[r]
%   &*+[F]\txt{\small 0}\ar@/^1.5pc/[lll]}
% \end{minipage} &
% \begin{minipage}{5em}{\small\begin{align*}
%       \Pi n.(& \RECSEQ{\GS{\W[0]}{\W[n]}{\Nat}.\End\\
%         &\quad }{i}{\xx}{\GS{\W[i+1]}{\W[i]}{\Nat}.\xx}\APP \\
%       &n)\\
%     \end{align*}}
% \end{minipage} \\
\end{tabular}
\caption{Simple multiparty network topology}\label{fig:ex-intro}
\end{figure}
%\noindent 


==> fig_process_typing_communication.tex <==
\begin{figure}[h]
\begin{center}
\begin{tabular}{c}
% \begin{prooftree}
% {
% \begin{array}{c}
% \Gamma \vdash \uu:\mar{\G} \quad \Gamma \vdash \PP \rhd \D, \y:\G \proj{\p_0}\\[1mm]
% \Gamma \proves \p_i\rhd \Nat \quad \Gamma \models \pid(\G)=\{\p_0..\p_\n\}\\[1mm]
% \end{array}
% }
% \justifies
% {\Gamma \vdash \sr\uu{\p_0..\p_\n} \y\PP \rhd \D} 
% \using\trule{TReq}
% \end{prooftree}
% \quad
% \begin{prooftree}
% {
% \begin{array}{c}
% \Gamma \vdash \uu:\mar{\G} \quad 
% \Gamma \vdash \PP \rhd \D, \y:\G \proj{\pp}\\[1mm]
% \Gamma \proves \pp\rhd \Nat \quad 
% \Gamma \models \pp\in\pid(\G)\\[1mm]
% \end{array}
% }
% \justifies
% {\Gamma \vdash \sa\uu\pp\y\PP \rhd \D } \using\trule{TAcc}
% \end{prooftree}\\
% \\
% \begin{prooftree}
% {\Gamma \vdash \Ia:\mar{\G} \quad \Gamma \proves \pp\rhd \Nat \quad \Gamma \models
%   \pp\in\pid(\G)} 
% \justifies
% {\Gamma \vdash \sj{\Ia}{\pp}{\s} \rhd \s[\pp]:\G \proj{\pp}} \using\trule{TJoin}
% \end{prooftree}\\
% \\
% \begin{prooftree}
% {\Gamma \vdash \e \rhd \ST \quad \Gamma \vdash \PP\rhd \D,\cc:\T}
% \justifies
% {\Gamma \vdash \Pout{\cc}{\p}{\e}{\PP} \rhd \D,\cc:\Lout{\p}{\ST}{\T}} \using\trule{TOut}
% \end{prooftree}
% \quad
%% \\
%% \\
%%  \begin{prooftree}
%%  {\Gamma,\x:\ST \vdash \PP\rhd \D,\cc:\T}
%%  \justifies
%%  {\Gamma \vdash \Pin{\cc}{\p}{\x}{\PP} \rhd \D,\cc:\Lin{\p}{\ST}{\T}} \using\trule{TIn}
%%  \end{prooftree}\\
%% \\
% \\
% \begin{prooftree}
% {\Gamma \vdash \PP\rhd \D,\cc:\T}
% \justifies
% {\Gamma \vdash \Pdel{\cc}{\p}{\cc'}{\PP}\rhd \D,\cc:\Lout{\p}{\T'}{\T},\cc':\T'} \using\trule{TDeleg}
% \end{prooftree}
% \quad
% \begin{prooftree}
% {\Gamma \vdash \PP\rhd \D,\cc:\T,\y:\T'}
% \justifies
% {\Gamma \vdash \Prec{\cc}{\p}{\y}{\PP}\rhd \D,\cc:\Lin{\p}{\T'}{\T}} \using\trule{TRecep}
% \end{prooftree}
\begin{prooftree}
{\Gamma \vdash \PP\rhd \D,\cc:\T_\jj\quad \jj\in K}
\justifies
{\Gamma \vdash \Psel{\cc}{\p}{l_\jj}{\PP}\rhd \D,\cc:\Lsel{\p}{\T_k}} 
\using\tfrule{TSel}
\end{prooftree}\\
\\
\begin{prooftree}
{\forall k\in K,\Gamma \vdash \PP_k\rhd \D,\cc:\T_k}
\justifies
{\Gamma \vdash \Pbranch{\cc}{\p}\rhd \D,\cc:\Lbranch{\p}{\T_k} } \using\tfrule{TBra}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma, \Ia:\U \vdash \PP \rhd \Delta}
\justifies
{\Gamma \vdash \nuc{\Ia}{\PP} \rhd \Delta} \using\tfrule{TNu}
\end{prooftree}
\quad
% \begin{prooftree}
% {\Gamma \vdash \e \rhd \ST \quad \Gamma \vdash \inact \rhd \D }
% \justifies
% {\Gamma, \XX:\ST\APP\T \vdash \proccall{\XX}{\e}{\cc} \rhd \D,\cc:\T} \using\trule{TDVar}
% \end{prooftree}\\
% \\
% \begin{prooftree}
% {\Gamma, \XX:\ST\APP\T,\x:\ST \vdash \PP\rhd \y:\T
%   \quad \Gamma, \XX:\ST\APP\T\vdash \QQ\rhd \D}
% \justifies {\Gamma \vdash \DEF\ \XX(\x,\y)=\PP\ \IN\ \QQ\ \rhd \D}
% \using\trule{TDef}
% \end{prooftree}\\
% \\
\begin{prooftree}
{\Gamma \vdash \D \quad \D\ \End\text{ only}}
\justifies
{\Gamma \vdash \inact \rhd \D } \using\tfrule{TNull}
\end{prooftree}
\quad
\begin{prooftree}
{\Gamma \vdash \PP \rhd \D \quad \Gamma \vdash \QQ \rhd \D'}
\justifies
{\Gamma \vdash \PP \pc \QQ \rhd \D,\D' } \using\tfrule{TPar}
\end{prooftree}\\
\\
%\begin{prooftree}
%{\Gamma \vdash \PP \rhd \Delta \quad \Delta \leq \Delta'}
%\justifies
%{\Gamma vdash \PP \rhd \Delta'}\using\trule{TSub}
%\end{prooftree}
%\\
\\
% \begin{prooftree}
% {\Gamma \vdash \PP\rhd \Delta\quad \Gamma \vdash \QQ \rhd \Delta
% \quad \Gamma \vdash \e\rhd \Bool}
% \justifies
% {\Gamma \vdash \ifthenelse{\e}{\PP}{\QQ}\rhd \Delta} \using\trule{TIf}
% \end{prooftree}\\
% \\
\end{tabular}
\end{center}
\caption{Process typing (Part 2)} \label{fig:process-typing2}
\end{figure}

%\begin{figure}[h]
%\centering
%{\small
%\begin{tabular}{c}
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash \uu:\mar{\G} \quad \Gamma \vdash \PP \rhd \D, \y:\G \proj{\p_0}\\[1mm]
%\Gamma \proves \p_i\rhd \Nat \quad \Gamma \models \pid(\G)=\{\p_0..\p_\n\}\\[1mm]
%\end{array}
%}
%\justifies
%{\Gamma \vdash \sr\uu{\p_0..\p_\n} \y\PP \rhd \D} 
%\using\trule{TReq}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash \uu:\mar{\G} \quad 
%\Gamma \vdash \PP \rhd \D, \y:\G \proj{\pp}\\[1mm]
%\Gamma \proves \pp\rhd \Nat \quad 
%\Gamma \models \pp\in\pid(\G)\\[1mm] 
%\end{array}
%}
%\justifies
%{\Gamma \vdash \sa\uu\pp\y\PP \rhd \D } \using\trule{TAcc}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \e \rhd \ST \quad \Gamma \vdash \PP\rhd \D,\cc:\T}
%\justifies
%{\Gamma \vdash \Pout{\cc}{\p}{\e}{\PP} \rhd \D,\cc:\Lout{\p}{\ST}{\T}} \using\trule{TOut}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma,\x:\ST \vdash \PP\rhd \D,\cc:\T}
%\justifies
%{\Gamma \vdash \Pin{\cc}{\p}{\x}{\PP} \rhd \D,\cc:\Lin{\p}{\ST}{\T}} \using\trule{TIn}
%\end{prooftree}\\
%%\begin{prooftree}
%%{\Gamma \vdash \PP\rhd \D,\cc:\T}
%%\justifies
%%{\Gamma \vdash \Pdel{\cc}{\p}{\cc'}{\PP}\rhd \D,\cc:\Lout{\p}{\T'}{\T},\cc':\T'} \using\trule{TDeleg}
%%\end{prooftree}\\
%%\\
%%\begin{prooftree}
%%{\Gamma \vdash \PP\rhd \D,\cc:\T,\y:\T'}
%%\justifies
%%{\Gamma \vdash \Prec{\cc}{\p}{\y}{\PP}\rhd \D,\cc:\Lin{\p}{\T'}{\T}} \using\trule{TRecep}
%%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \PP\rhd \D,\cc:\T_\jj\quad \jj\in I}
%\justifies
%{\Gamma \vdash \Psel{\cc}{\p}{l_\jj}{\PP}\rhd \D,\cc:\Lsel{\p}{\T_i}} \using\trule{TSel}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\forall \ii\in I,\Gamma \vdash \PP_\ii\rhd \D,\cc:\T_\ii}
%\justifies
%{\Gamma \vdash \Pbranch{\cc}{\p}\rhd \D,\cc:\Lbranch{\p}{\T_i} } \using\trule{TBra}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma, \Ia:\U \vdash \PP \rhd \Delta}
%\justifies
%{\Gamma \vdash \nuc{\Ia}{\PP} \rhd \Delta} \using\trule{TNu}
%\end{prooftree}
%%\\
%%\\
%%\begin{prooftree}
%%{\Gamma \vdash \e \rhd \ST \quad \Gamma \vdash \inact \rhd \D }
%%\justifies
%%{\Gamma, \XX:\ST\APP\T \vdash \proccall{\XX}{\e}{\cc} \rhd \D,\cc:\T} \using\trule{TDVar}
%%\end{prooftree}\\
%%\\
%%\begin{prooftree}
%%{\Gamma, \XX:\ST\APP\T,\x:\ST \vdash \PP\rhd \y:\T
%%  \quad \Gamma, \XX:\ST\APP\T\vdash \QQ\rhd \D}
%%\justifies {\Gamma \vdash \DEF\ \XX(\x,\y)=\PP\ \IN\ \QQ\ \rhd \D}
%%\using\trule{TDef}
%%\end{prooftree}\\
%%\\
%\begin{prooftree}
%{\Gamma \vdash \D \quad \D\ \End\text{ only}}
%\justifies
%{\Gamma \vdash \inact \rhd \D } \using\trule{TNull}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \PP \rhd \D \quad \Gamma \vdash \QQ \rhd \D'}
%\justifies
%{\Gamma \vdash \PP \pc \QQ \rhd \D,\D' } \using\trule{TPar}
%\end{prooftree}
%%\\
%%\\
%%\begin{prooftree}
%%{\Gamma \vdash \PP\rhd \Ty\quad \Gamma \vdash \QQ \rhd \Ty
%%\quad \Gamma \vdash \e\rhd \Bool}
%%\justifies
%%{\Gamma \vdash \ifthenelse{\e}{\PP}{\QQ}\rhd \Ty} \using\trule{TIf}
%%\end{prooftree}\\
%%\\
%\end{tabular}
%}
%\caption{Process typing (Part 2)} \label{fig:process-typing2}
%\end{figure}


==> fig_runtime_syntax.tex <==
\begin{figure}[ht!]
\begin{tabular}{r@{\ }c@{\ }l@{\quad}l}
 \cc & ::=  & \y \sep \s[\p] & Channels \\
 \pv, \qv & ::=  & $\pv[\n] \sep \Names$ & Principal values\\
 \mm & ::=  & (\qv,\pv,\va) 
      \sep  (\qv,\pv,\s[\pv'])  
      \sep  (\qv,\pv,\Ll) & Messages in transit \\
 \h  & ::=  & $\qbot \sep \qcomp{\mm}{\h}$ & Queues \\
 \PP & ::=  & \etc & \hspace{-2em} Run-time processes \\
     & \sep & \Pout{\cc}{\p}{\e}{\PP}& Output \\
     & \sep & \Pin{\cc}{\p}{\x}{\PP}& Input \\
     & \sep & \Pdel{\cc}{\p}{\cc'}{\PP}& Session delegation \\
     & \sep & \Prec{\cc}{\p}{\y}{\PP}& Session reception \\
     & \sep & \Psel{\cc}{\p}{l}{\PP}& Selection \\
     & \sep & \Pbranch{\cc}{\p}& Branching \\
     & \sep & \nuc{\s} \PP & Restriction \\
     & \sep & \s:\h & Queues \\
\end{tabular}
\caption{Run-time processes (with the user-defined processes) }\label{fig:runtime-syntax}
\end{figure}
 


==> fig_simple_size.tex <==
\begin{figure}
\centering
\begin{tabular}{l@{\ }l@{\ }l@{\quad}l}
{\bf Judgements} &  
\ 
$\judgementsize{\Gamma \proves G_1 \gequivwf G_2}=
\judgementsize{\Gamma \proves G_1 \equivwf G_2}+1$
\\[1mm]
& 
$\judgementsize{\Gamma \proves G_1 \equivwf G_2}=$\\
& 
\quad $\begin{cases}
\Sigma_{0\leq \n \leq \m} \ 
\judgementsize{\Gamma \proves (G_1 \n) \equiv (G_2 \n)}+1\\[1mm]
%\Sigma_{0\leq \n \leq \m} \ \omega\cdot(\reductionsize{G_1\, \n}+
%\reductionsize{G_2\, \n})+\termsize{G_1 \n}+\termsize{G_2 \n}+1\\[1mm]
\quad (\text{if $G_i = 
\GR{\G_i'}{\AT{\ii}{\II}}{\xx}{\G_i''}$ and 
$\Gamma\models \II=[0..\m]\quad 0\leq \n
\leq \m$})\\[1mm]
\judgementsize{\Gamma \proves G_1' \equiv G_2'}
+ \judgementsize{\Gamma \proves G_1'' \equiv G_2''}
+ \termsize{G_1}+\termsize{G_2}+1
\\[1mm]
\quad (\text{if $G_i = 
\GR{\G_i'}{\AT{\ii}{\II}}{\xx}{\G_i''}$ and 
$\II$ infinite})\\[1mm]
\judgementsize{\Gamma \proves G_1' \equiv G_2'}
+ \termsize{G_1}+\termsize{G_2}+1
\\[1mm]
\quad (\text{if $G_i = G_i'\tii_i$ and $G_1' \tii_1$ 
or $G_2' \tii_2$ is a head normal form})\\[1mm]
%\judgementsize{\Gamma \proves G_{01} \equivwf G_{02}}+
%\termsize{G_1}+\termsize{G_2}+1 
%\quad (\text{if $G_{i} = G_{0i} \tii_i$})
% and $G_{0i} = 
%\GR{\G_i'}{\AT{\ii}{\II}}{\xx}{\G_i''}$ and 
%$\Gamma\models \II=[0..\m]\quad 0\leq \n
%\leq \m$})
%\\[1mm]
\omega\cdot(\reductionsize{G_1}+\reductionsize{G_2})+
\termsize{G_1}+\termsize{G_2}+1 \quad (\mbox{otherwise}) 
\end{cases}
$
\\[1mm]
{\bf Types} \\[2mm]
Value \quad& $\termsize{\Bool}={\Nat}=1$, 
             $\termsize{\mar\G}= \termsize{G}+1$\\[1mm]
Global \quad & $\termsize{\GS{\p}{\p'}{\U}.\G}=
   2+\termsize{\U}+\termsize{\G}$\\[1mm]
& $\termsize{\GB{\p}{\p'}}=2+\Sigma_{k\in K} (1+ \termsize{G_k})$\\[1mm]
& $\termsize{\GM{\xx}{\G}}=\termsize{\G}+2$, \quad 
  $\termsize{\xx}=\termsize{\n}=\termsize{\End}=1$\\[1mm]
&  
%$\termsize{\Pi \AT{\ii}{\II}.\G}=1+\termsize{G}$, \quad   
  $\termsize{\G\APP \tii}=\termsize{G}+2$, \quad 
  $\termsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}=
   4+\termsize{G}+\termsize{G'}$\\[1mm]
Local\quad &
  $\termsize{\Lout{\p}{\U}{\T}}=3+\termsize{\U}+\termsize{\T}$, 
  \quad 
  $\termsize{\Lin{\p}{\U}{\T}}=3+\termsize{\U}+\termsize{\T}$\\[1mm] 
  & $\termsize{\Lsel{\p}{\T_k}}= \termsize{\Lbranch{\p}{\T_k}}
     =2+\Sigma_{k\in K}(1+\termsize{T_k})$\\ 
   & $\termsize{\LM{\xx}{\T}} =\termsize{\T}+2$, 
\quad $\termsize{\xx}=\termsize{\n}=\termsize{\End}=1$\\[1mm]
& %$\termsize{\Pi \AT{\ii}{\II}.\T}=1+\termsize{T}$, \quad   
  $\termsize{\T\APP \tii}=\termsize{T}+2$,\quad 
$\termsize{\GR{\T}{\AT{\ii}{\II}}{\xx}{\T'}}=
   4+\termsize{T}+\termsize{T'}$\\[1mm]
Principals & 
$\termsize{\Pi\AT{\ii}{\II}.{U_p}}= 2 + \termsize{U_p}$\\[1mm]
Processes  & 
$\termsize{\emptyset}=0$, 
$\termsize{\Delta,\AT{c}{\T}}=\termsize{\Delta}+\termsize{\T}+1$,
$\termsize{\Pi\AT{\ii}{\II}.\tau}= 2 + \termsize{\tau}$ 
%$\termsize{\tau\APP \tii}= 1 + \termsize{\tau}$ 
\\[1mm]
\end{tabular}\\[2mm]
\caption{Size of types and judgements} \label{fig:size}
\end{figure}

%\begin{figure}
%\centering
%\begin{tabular}{l@{\ }l@{\ }l@{\quad}l}
%$\reductionsize{\GS{\p}{\p'}{\U}.\G}=
%\reductionsize{\U}+\reductionsize{\G}$,\quad 
%   $\reductionsize{\GB{\p}{\p'}}=\Sigma_{k\in K}
%    \reductionsize{G_k}$\\[1mm]
%$\reductionsize{\GM{\ty}{\G}}=\reductionsize{\G}$, \quad 
%$\reductionsize{\ty}=\reductionsize{\xx}=\reductionsize{\End}=0$\\[1mm]
%%$\reductionsize{\Pi \AT{\ii}{\II}.\G}=\reductionsize{G}$\\[1mm]
%$\reductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}=
%\reductionsize{G}+\reductionsize{G'}$\\[1mm]
%$\reductionsize{G\APP\m}=
%\headreductionsize{G \APP \m}+\reductionsize{\WHNF{G \APP \m}}$\\[1mm]
%$\reductionsize{G\APP\ii}=\inductionreductionsize{G}$\\[1mm]
%%$\inductionreductionsize{\Pi \AT{\ii}{\II}.\G}=\Sigma_{0\leq \tjj\leq \n+1}
%% \ (\reductionsize{G\APP \tjj}+1)+1$ \quad ($\II=[0..\n]$)\\[1mm] 
%%$\inductionreductionsize{\Pi \AT{\ii}{\II}.\G}=
%%\reductionsize{\Pi \AT{\ii}{\II}.\G}$ \quad ($\II=\Nat$)\\[1mm] 
%$\inductionreductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}
%=\Sigma_{0\leq \tjj\leq \n+1}
%\ (\reductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}{\tjj}}+1)+1$ 
%\quad ($\II=[0..\n]$)\\[1mm] 
%$\inductionreductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}
%=\reductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}$ 
%\quad ($\II=\Nat$)\\[1mm]
%$\headreductionsize{\G}=\nn \quad \text{if}\    \G\redsym^\nn G'\not\redsym$
%\end{tabular}\\[2mm]

%\caption{Number of reductions} \label{fig:reduction-size}
%\end{figure}



==> fig_type_equivalence.tex <==
\begin{figure}
\centering
\begin{tabular}{c}
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash \U_1 \WB \U_2 
\quad 
\Gamma \vdash \G_1 \WB \G_2 \quad %\\[1mm]
\Gamma \vdash \GS{\p}{\p'}{\U_i}.\G_i \RHD \GType\\
\end{array}
}
\justifies
{\Gamma \vdash 
\Gamma \vdash \GS{\p}{\p'}{\U_1}.\G_1\WB 
\Gamma \vdash \GS{\p}{\p'}{\U_2}.\G_2
} \using\trule{IsoIO}
\end{prooftree}\\
\\
\begin{prooftree}
{
\begin{array}{c}
\forall i\in I.\ \Gamma \vdash \G_{1i} \WB \G_{2i} \quad % \\[1mm]
\Gamma \vdash 
\TO{\p}{\q}\colon \{l_i: \G_{ji}\}_{i\in I}\RHD \GType \ 
\ (j=1,2)
\end{array}
}
\justifies
{\Gamma \vdash \TO{\p}{\q}\colon \{l_i: \G_{1i}\}_{i\in I}\WB 
\TO{\p}{\q}\colon \{l_i: \G_{2i}\}_{i\in I}} 
\using\trule{IsoBra}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \G_1 \WB  \GM{\xx}{\G_2}\RHD \K}
\justifies
{\Gamma \vdash \G_1 \WB \G_2\subst{\GM{\xx}{\G_2}}{\xx}} \using\trule{LRec}
\end{prooftree}
\quad
\begin{prooftree}
{\Gamma \vdash \GM{\xx}{\G_1} \WB \G_2 \RHD \K}
\justifies
{\Gamma \vdash \G_1\subst{\GM{\xx}{\G_1}}{\xx}}\WB \GM{\xx}{\G_2}  
\using\trule{RRec}
\end{prooftree}
\\
\\
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash G_1 \WB G_2
\quad 
\Gamma,\AT{\ii}{\II} \vdash G_1' \WB G_2' \quad %\\[1mm]
\Gamma \vdash
\GR{\G_i}{\AT{\ii}{\II}}{\xx}{\G_i'}\RHD \kappa 
\quad (i=1,2)\\[1mm]
\end{array}
}
\justifies
{
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
\WB 
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}
}
\using\trule{IsoR}
\end{prooftree}
\\
\\
% \begin{prooftree}
% {\Gamma \vdash \Env}
% \justifies
% {\Gamma \vdash \ty \WB \ty} \using\trule{IsoTVar}
% \end{prooftree}\\
% \\
\begin{prooftree}
{\Gamma \vdash \Env}
\justifies
{\Gamma \vdash \xx \WB \xx} \using\trule{IsoRVar}
\end{prooftree}
\quad
\begin{prooftree}
{\Gamma \vdash \Env}
\justifies
{\Gamma \vdash \End \WB \End} \using\trule{IsoEnd}
\end{prooftree}\\
\\
% \begin{prooftree}
% {\Gamma,\AT{\ii}{\II}\vdash \G_1\WB \G_2}
% \justifies
% {\Gamma \vdash \Pi \AT{\ii}{\II}.\G_1\WB \Pi \AT{\ii}{\II}.\G_2}
% \using\trule{IsoProd}
% \end{prooftree}\\
% \\
\begin{prooftree}
{\begin{array}{c}
\Gamma\vdash \G_1\WB \G_2 \quad 
\Gamma\models \tii_1:I = \tii_2:I \quad %\\[1mm]
\Gamma\vdash \G_i\tii_i \RHD \kappa 
\quad 
(i=1,2)\\[1mm]
\end{array}
}
\justifies
{\Gamma \vdash \G_1 \tii_1 \WB \G_2 \tii_2}
\using\trule{IsoApp}
\end{prooftree}\\
\\

%\\
%\begin{prooftree}
%{\Gamma\vdash \WHNF{\G_1}\WB \WHNF{\G_2}}
%\justifies
%{\Gamma \vdash \G_1\equiv \G_2}
%\using\trule{GTypeEq}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G' \equiv \G}
%\justifies
%{\Gamma \vdash \G \equiv \G'} \using\trule{EqSym}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G \equiv \G''
%  \quad \Gamma \vdash \G'' \equiv \G'}
%\justifies
%{\Gamma \vdash \G \equiv \G'} \using\trule{EqTrans}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma, \AT{\ii}{\II}\vdash \G \equiv G'
%}
%\justifies
%{
%\Gamma\vdash  \Pi\AT{\ii}{\II}.\G \equiv  \Pi\AT{\ii}{\II}.G'
%} \using\trule{EqAbs}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G \equiv G'\RHD \Pi\AT{\ii}{\II}.\K 
%\quad \Gamma \models \AT{\tii}{\II}=\AT{\tii'}{\II}
%}
%\justifies
%{\Gamma \vdash \G\tii \equiv \G'\tii'} \using\trule{EqApp}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G \RHD \K 
%  \quad \G \redsym  \G'}
%\justifies
%{\Gamma \vdash \G \equiv \G'} \using\trule{EqBeta}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma,\AT{\ii}{\II} \vdash \G \ii \equiv \G'}
%\justifies
%{\Gamma \vdash \G\equiv \lambda \AT{\ii}{\II}.G' } \using\trule{EqEta}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash \G,\G' \RHD \Pi\AT{\VEC{\ii}}{\VEC{I}}.\K\quad 
%\Gamma\proves \n_i:I_i\\[1mm]
%\G\VEC{\n} \longrightarrow^\ast G_0 \quad 
%\G'\VEC{\n} \longrightarrow^\ast G_0
%\end{array}
%}
%\justifies
%{\Gamma \vdash \G \equiv \G'} \using\trule{Eq}
%\end{prooftree}
%\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G \RHD \K}
%\justifies
%{\Gamma \vdash \GM{\ty}{\G} \equiv \G\subst{\GM{\ty}{\G}}{\ty}} \using\trule{EqRec}
%\end{prooftree}
%\\
%\\
\end{tabular}
\caption{Global type isomorphism and type equivalence} \label{fig:type-equivalence}
\end{figure}


==> fig_type_reduction.tex <==
\begin{figure}
\begin{center}
\begin{tabular}{rcl}
  $\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}\APP 0$  & \redsym & \G \\
  $\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}\APP \n$ & \redsym & 
    $\G'\sub{\tii}{\ii}\sub{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}\APP \n -1}{\xx}$ \\
%  $(\Pi \AT{\ii}{\II}.\G)\APP \nn$          & \redsym & \G\sub{\tii}{\nn}\\
\end{tabular}
\end{center}
\caption{Type reduction}\label{fig:typereduction}
\end{figure}


==> fig_type_syntax.tex <==
\begin{figure}
\begin{tabular}{r@{\ }c@{\ }l@{\quad}l}
\ST & ::= & \Bool \sep \Nat \sep .. \sep \mar \G & Value type\\
\U & ::= & \ST \sep \T & Payload type \\
$\tii$ & ::= & $\ii \bnfor \n \bnfor \tii + \tii' 
\bnfor \tii -\tii' \bnfor \tii\times\tii' $ & Indexes\\ 
\PRED & ::= & $\PRED\andl \PRED \sep \tii\leq \tii$& Propositions\\ 
\II & ::= & \Nat \sep \CONSTRAINT{\ii}{\II}{\PRED} & Index sorts \\ 
\Names & ::= & \Alice \sep \Bob \sep \Worker \sep \etc & Participants \\
\p & ::= & $\p[\tii] \sep \Names$ & Principals\\
%\p & ::= & \p[\e] \sep \Alice \sep \Bob \sep \W \sep \etc & Participants\\
\G & ::= & & \hspace{-2em} Global types \\ 
   & \sep & $\GS{\p}{\p'}{\U}.\G$ & Message \\
   & \sep & $\GB{\p}{\p'}$  & Branching \\
   & \sep & $\GM{\ty}{\G}$ & Recursion \\
   & \sep & $\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}$  & Primitive Recursion \\
   & \sep & \ty \sep \xx & Type variables \\
   & \sep &  $\Pi \AT{\ii}{\II}.\G$ & Dependent type\\
   & \sep & \G\APP \tii   & Application\\
   & \sep & \End & Null \\
\T & ::= &  & \hspace{-2em} Local types \\ 
   & \sep & \Lout{\p}{\U}{\T} & Output \\
   & \sep & \Lin{\p}{\U}{\T} & Input \\
   & \sep & \Lsel{\p}{\T_i} & Selection \\
   & \sep & \Lbranch{\p}{\T_i} & Branching \\
   & \sep & \LM{\ty}{\T} & Recursion \\
   & \sep & $\LR{\T}{\AT{\ii}{\II}}{\xx}{\T'}$  & Primitive Recursion \\
   & \sep & \ty \sep \xx & Type variables \\
   & \sep & $\Pi \AT{\ii}{\II}.\T$ & Dependent type\\
   & \sep & \T\APP \tii   & Application\\
   & \sep & \End & Null \\ 
\end{tabular}
\caption{Global and Local Types}\label{fig:global}
\end{figure}
 



==> fig_type_system.tex <==
\begin{figure}
\centering
$
\begin{array}{c}
\begin{prooftree}
{}
\justifies
{\emptyset \vdash  \Env}  \using\trule{EnvEmp}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \T \RHD \LType \quad \Gamma \vdash \ST \RHD \SType \quad \XX\not\in\dom{\Gamma}}
\justifies
{\Gamma, \XX:\ST\APP\T \vdash  \Env}  \using\trule{EnvRecVar}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \U \RHD \SType \quad \x\not\in\dom{\Gamma}}
\justifies
{\Gamma, u:\ST \vdash  \Env}  \using\trule{Envx}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \II \quad \ii\not\in\dom{\Gamma}}
\justifies
{\Gamma, \ii:\II \vdash  \Env}  \using\trule{Envii}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \Ty \RHD \PType \quad \X\not\in\dom{\Gamma}}
\justifies
{\Gamma, \X:\Ty \vdash  \Env}  \using\trule{EnvX}
\end{prooftree}\\
\\
\end{array}
$
\caption{Environment} \label{fig:environment}
\end{figure}


\begin{figure}[h]
\centering
{\small
\begin{tabular}{@{\,}c}
\begin{prooftree}
{\Gamma \vdash \Env}
\justifies
{\Gamma \vdash \n \rhd \Nat} 
\using\trule{TNat}
\end{prooftree}
\begin{prooftree}
{\Gamma \vdash \e\rhd \Bool \quad \Gamma \vdash \e'\rhd \Bool}
\justifies
{\Gamma \vdash \e \ \mathsf{and}\ \e' \rhd \Bool} \using\trule{TAnd}
\end{prooftree}\\
\\
%\begin{prooftree}
%{\Gamma, \ii : \II  \vdash \Env}
%\justifies
%{\Gamma, \ii : \II \vdash \ii \rhd \Nat} \using\trule{TVari}
%\end{prooftree}\\
%\\
\begin{prooftree}
{\Gamma  \vdash \U_p}
\justifies
{\Gamma\vdash \Alice\rhd \U_p} \using\trule{TId}
\end{prooftree}
\begin{prooftree}
{\Gamma  \vdash \p\rhd\Pi\AT{\ii}{\II}.\U_p\quad \Gamma\models \AT{\tii}{\II}}
\justifies
{\Gamma\vdash \p[\tii]\rhd \U_p\sub{\tii}{\ii}} \using\trule{TP}
\end{prooftree}\\
\\
%\begin{prooftree}
%{\Gamma \models 0\leq \tii \op \tii' }
%\justifies
%{\Gamma \vdash \tii \op \tii' \rhd \Nat} \using\trule{TIOp}
%\end{prooftree}\\
%\\
%\end{prooftree}\\
%%\\
\begin{prooftree}
{
\begin{array}{c}
{\Gamma, \ii : \minus{\II},\X:\Ty\sub{\ii}{\jj}  \vdash \QQ  \rhd
 \Ty\sub{\ii+1}{\jj}}
\\[2mm]
{\Gamma\vdash \PP  \rhd\Ty\sub{0}{\jj}  \qquad
  \Gamma\vdash \Pi \AT{\jj}{\II}.\Ty \RHD \Pi \AT{\jj}{\II}.\K
}
\end{array}
}
\justifies
{\Gamma \vdash \RECSEQP{\PP}{\ii}{\X}{\QQ} \rhd \Pi \AT{\jj}{\II}.\Ty}
\using\trule{TPRec}
\end{prooftree}\\
\\
\begin{prooftree}
{
{\Ga \vdash \PP  \rhd \tau \quad \Ga \vdash \tau \equiv \tau'}
}
\justifies
{  
\Ga \vdash \PP  \rhd \tau'
}
\using\trule{TEq}
\end{prooftree}\qquad
\begin{prooftree}
{\Gamma, \X:\Ty \vdash \Env}
\justifies
{\Gamma, \X:\Ty \vdash \X \rhd \Ty} \using\trule{TVar}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma, \ii : \II  \vdash \Ty}
\justifies
{\Gamma \vdash \lambda \ii.\PP \rhd \Pi \AT{\ii}{\II}.\Ty} \using\trule{TFun}
\end{prooftree}\qquad
\begin{prooftree}
{\Gamma \vdash \PP\rhd \Pi \AT{\ii}{\II}.\Ty 
\quad \Gamma \models {\tii}\in{\II} 
}
\justifies
{\Gamma \vdash \PP\APP\tii \rhd \Ty\sub{\tii}{\ii}} \using\trule{TApp}
\end{prooftree}\\[1ex]
\end{tabular}
}
\caption{Process typing (Part 1)} \label{fig:process-typing1}
\end{figure}

\begin{figure}[h]
\centering
{\small
\begin{tabular}{c}
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash \uu:\mar{\G} \quad \Gamma \vdash \PP \rhd \D, \y:\G \proj{\p_0}\\[1mm]
\Gamma \proves \p_i\rhd \Nat \quad \Gamma \models \pid(\G)=\{\p_0..\p_\n\}\\[1mm]
\end{array}
}
\justifies
{\Gamma \vdash \sr\uu{\p_0..\p_\n} \y\PP \rhd \D} 
\using\trule{TReq}
\end{prooftree}\\
\\
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash \uu:\mar{\G} \quad 
\Gamma \vdash \PP \rhd \D, \y:\G \proj{\pp}\\[1mm]
\Gamma \proves \pp\rhd \Nat \quad 
\Gamma \models \pp\in\pid(\G)\\[1mm] 
\end{array}
}
\justifies
{\Gamma \vdash \sa\uu\pp\y\PP \rhd \D } \using\trule{TAcc}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \e \rhd \ST \quad \Gamma \vdash \PP\rhd \D,\cc:\T}
\justifies
{\Gamma \vdash \Pout{\cc}{\p}{\e}{\PP} \rhd \D,\cc:\Lout{\p}{\ST}{\T}} \using\trule{TOut}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma,\x:\ST \vdash \PP\rhd \D,\cc:\T}
\justifies
{\Gamma \vdash \Pin{\cc}{\p}{\x}{\PP} \rhd \D,\cc:\Lin{\p}{\ST}{\T}} \using\trule{TIn}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \PP\rhd \D,\cc:\T}
\justifies
{\Gamma \vdash \Pdel{\cc}{\p}{\cc'}{\PP}\rhd \D,\cc:\Lout{\p}{\T'}{\T},\cc':\T'} \using\trule{TDeleg}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \PP\rhd \D,\cc:\T,\y:\T'}
\justifies
{\Gamma \vdash \Prec{\cc}{\p}{\y}{\PP}\rhd \D,\cc:\Lin{\p}{\T'}{\T}} \using\trule{TRecep}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \PP\rhd \D,\cc:\T_\jj\quad \jj\in I}
\justifies
{\Gamma \vdash \Psel{\cc}{\p}{l_\jj}{\PP}\rhd \D,\cc:\Lsel{\p}{\T_i}} \using\trule{TSel}
\end{prooftree}\\
\\
\begin{prooftree}
{\forall \ii\in I,\Gamma \vdash \PP_\ii\rhd \D,\cc:\T_\ii}
\justifies
{\Gamma \vdash \Pbranch{\cc}{\p}\rhd \D,\cc:\Lbranch{\p}{\T_i} } \using\trule{TBra}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma, \Ia:\U \vdash \PP \rhd \Delta}
\justifies
{\Gamma \vdash \nuc{\Ia}{\PP} \rhd \Delta} \using\trule{TNu}
\end{prooftree}
\\
\\
\begin{prooftree}
{\Gamma \vdash \e \rhd \ST \quad \Gamma \vdash \inact \rhd \D }
\justifies
{\Gamma, \XX:\ST\APP\T \vdash \proccall{\XX}{\e}{\cc} \rhd \D,\cc:\T} \using\trule{TDVar}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma, \XX:\ST\APP\T,\x:\ST \vdash \PP\rhd \y:\T
  \quad \Gamma, \XX:\ST\APP\T\vdash \QQ\rhd \D}
\justifies {\Gamma \vdash \DEF\ \XX(\x,\y)=\PP\ \IN\ \QQ\ \rhd \D}
\using\trule{TDef}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \D \quad \D\ \End\text{ only}}
\justifies
{\Gamma \vdash \inact \rhd \D } \using\trule{TNull}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma \vdash \PP \rhd \D \quad \Gamma \vdash \QQ \rhd \D'}
\justifies
{\Gamma \vdash \PP \pc \QQ \rhd \D,\D' } \using\trule{TPar}
\end{prooftree}
\\
\\
\begin{prooftree}
{\Gamma \vdash \PP\rhd \Delta\quad \Gamma \vdash \QQ \rhd \Delta
\quad \Gamma \vdash \e\rhd \Bool}
\justifies
{\Gamma \vdash \ifthenelse{\e}{\PP}{\QQ}\rhd \Delta} \using\trule{TIf}
\end{prooftree}\\
\\
\end{tabular}
}
\caption{Process typing (Part 2)} \label{fig:process-typing2}
\end{figure}






==> fig_user_syntax.tex <==
\begin{figure}
\centering
\begin{tabular}{r@{\;}c@{\;}l@{\quad}l}
\Iu & ::= & \x \bnfor \Ia & Identifiers\\
\Iv & ::= & $\Ia \bnfor \n \bnfor \true \bnfor \false$ & Values\\
%$e$  & ::= & $v \bnfor \x \bnfor \ii \bnfor 
%e  \op e' \bnfor \AND{e}{e'} \bnfor \NOT{e}$ & Expressions\\
$e$  & ::= & $\tii \bnfor v \bnfor \x \bnfor \e\op\e'$
% \AND{e}{e'} \bnfor \NOT{e}
 & Expressions\\

% \end{tabular}
% \begin{tabular}{ll}
% \begin{tabular}{rcl@{\quad}l}
 \PP & ::=  & &  Processes \\
     & \sep & \sr\uu{\p_0..\p_\n} \y\PP   &   {Multicast Request}\\
     & \sep & \sa\uu\p\y\PP   &   {Accept}\\
     & \sep & \outS{\y}\e\PP &    {Value sending}\\
     & \sep & \inpS{\y}\z\PP &    {Value reception}\\
     & \sep & \sdS{\y}{\y'} \PP & {Session delegation}\\
     & \sep & \rdS{\y}{\y'}\PP &  {Session reception}\\
     & \sep & \lselS{\y}{\l}{\PP} & {Selection}\\
     & \sep & \lbranchS{\y} & {Branching}\\
     & \sep & \nuc{\Ia}{\PP} & {Hiding}\\
% \end{tabular} \\
% \begin{tabular}{rcl@{\quad}l}
%      &  & & \\
     & \sep & \defIn{\Ddef}\PP & Recursive definition \\
     & \sep & \proccall{\XX}{\e}{\y} & {Process call}\\
     & \sep & \inact & {Inaction}\\
     & \sep & \PP \pc \QQ  &{Parallel}\\
     & \sep & \ifthenelse{\e}{\PP}{\QQ} &{Conditional}\\
     & \sep & $\RECSEQP{\PP}{\ii}{\X}{\QQ}$ & {Parallel Recursion}\\
     & \sep & \X &{Process Variable}\\
     & \sep & $\lambda \ii$.\PP & {Abstraction}\\
     & \sep & (\PP\APP\tii) &{Application}
% \end{tabular}
\end{tabular}
\caption{Syntax for user-defined processes}\label{fig:syntax}
\end{figure}



==> fig_wf_global_equivalence.tex <==
\begin{figure}
\centering
\begin{tabular}{c}
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash \U_1 \gequivwf \U_2 
\quad 
\Gamma \vdash \G_1 \gequivwf \G_2 \quad %\\[1mm]
\Gamma \vdash \GS{\p}{\p'}{\U_i}.\G_i \RHD \GType\\
\end{array}
}
\justifies
{\Gamma \vdash \GS{\p}{\p'}{\U_1}.\G_1\equivwf 
\Gamma \vdash \GS{\p}{\p'}{\U_2}.\G_2
} \using\trule{WfIO}
\end{prooftree}\\
\\
\begin{prooftree}
{
\begin{array}{c}
\forall k\in K.\ \Gamma \vdash \G_{1k} \gequivwf \G_{2k}  \quad %\\[1mm]
\Gamma \vdash 
\TO{\p}{\q}\colon \{l_k: \G_{jk}\}_{k\in K}\RHD \GType \ 
\ (j=1,2)
\end{array}
}
\justifies
{\Gamma \vdash \TO{\p}{\q}\colon \{l_k: \G_{1k}\}_{k\in K}\equivwf  
\TO{\p}{\q}\colon \{l_k: \G_{2k}\}_{k\in K}} 
\using\trule{WfBra}
\end{prooftree}
\\
\\
\begin{prooftree}
{\Gamma \vdash \G_1 \gequivwf \G_2}
\justifies
{\Gamma \vdash \GM{\xx}{\G_1} \equivwf \GM{\xx}{\G_2}}  
\using\trule{WfPRec}
\end{prooftree}
\\
\\
%% \begin{prooftree}
%% {
%%  \begin{array}{c}
%%  \Gamma \vdash G_1 \gequivwf G_2
%%  \quad 
%%  \Gamma \vdash G_1' \gequivwf G_2'\\[1mm]
%%  \Gamma \vdash
%%  \GR{\G_i}{\AT{\ii}{\II}}{\xx}{\G_i'}\RHD \kappa 
%%  \quad (i=1,2)\\[1mm]
%%  \end{array}
%% }
%% \justifies
%% {
%% \Gamma \vdash
%%  \GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
%%  \equivwf
%% \GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}
%% }
%% \using\trule{Wf}
%% \end{prooftree}
% \begin{prooftree}
% {\Gamma \vdash \Env}
% \justifies
% {\Gamma \vdash \ty \equivwf \ty} \using\trule{WfTVar}
% \end{prooftree}
\quad
\begin{prooftree}
{\Gamma \vdash \Env}
\justifies
{\Gamma \vdash \xx \equivwf \xx} \using\trule{WfRVar}
\end{prooftree}
\quad
\begin{prooftree}
{\Gamma \vdash \Env}
\justifies
{\Gamma \vdash \End \equivwf \End} \using\trule{WfEnd}
\end{prooftree}\\
\\
\begin{prooftree}
{\Gamma,\AT{\ii}{\II}\vdash \G_1\gequivwf \G_2}
\justifies
{\Gamma \vdash \Pi \AT{\ii}{\II}.\G_1\equivwf \Pi \AT{\ii}{\II}.\G_2}
\using\trule{WfProd}
\end{prooftree}
\\
\\
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash
\G_1
\gequivwf
\G_2
\quad 
\Gamma,\AT{\ii}{\II} \vdash
\G_1'
\gequivwf
\G_2'
\end{array}
}
\justifies
{
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
\equivwf
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}
}
\using\trule{WfRec}
\end{prooftree}
\\
\\
\begin{prooftree}
{\begin{array}{c}
\Gamma\vdash \G_1\equivwf \G_2 \quad 
\Gamma\models \tii_1:I = \tii_2:I \quad %\\[1mm]
\Gamma\vdash \G_i\tii_i \RHD \kappa 
\quad 
(i=1,2)\\[1mm]
\end{array}
}
\justifies
{\Gamma \vdash \G_1 \tii_1 \equivwf \G_2 \tii_2}
\using\trule{WfApp}
\end{prooftree}
%\\
%\begin{prooftree}
%{\Gamma\vdash \WHNF{\G_1}\WB \WHNF{\G_2}}
%\justifies
%{\Gamma \vdash \G_1\equiv \G_2}
%\using\trule{GTypeEq}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G' \equiv \G}
%\justifies
%{\Gamma \vdash \G \equiv \G'} \using\trule{EqSym}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G \equiv \G''
%  \quad \Gamma \vdash \G'' \equiv \G'}
%\justifies
%{\Gamma \vdash \G \equiv \G'} \using\trule{EqTrans}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma, \AT{\ii}{\II}\vdash \G \equiv G'
%}
%\justifies
%{
%\Gamma\vdash  \Pi\AT{\ii}{\II}.\G \equiv  \Pi\AT{\ii}{\II}.G'
%} \using\trule{EqAbs}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G \equiv G'\RHD \Pi\AT{\ii}{\II}.\K 
%\quad \Gamma \models \AT{\tii}{\II}=\AT{\tii'}{\II}
%}
%\justifies
%{\Gamma \vdash \G\tii \equiv \G'\tii'} \using\trule{EqApp}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G \RHD \K 
%  \quad \G \redsym  \G'}
%\justifies
%{\Gamma \vdash \G \equiv \G'} \using\trule{EqBeta}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma,\AT{\ii}{\II} \vdash \G \ii \equiv \G'}
%\justifies
%{\Gamma \vdash \G\equiv \lambda \AT{\ii}{\II}.G' } \using\trule{EqEta}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash \G,\G' \RHD \Pi\AT{\VEC{\ii}}{\VEC{I}}.\K\quad 
%\Gamma\proves \n_i:I_i\\[1mm]
%\G\VEC{\n} \longrightarrow^\ast G_0 \quad 
%\G'\VEC{\n} \longrightarrow^\ast G_0
%\end{array}
%}
%\justifies
%{\Gamma \vdash \G \equiv \G'} \using\trule{Eq}
%\end{prooftree}
%\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G \RHD \K}
%\justifies
%{\Gamma \vdash \GM{\ty}{\G} \equiv \G\subst{\GM{\ty}{\G}}{\ty}} \using\trule{EqRec}
%\end{prooftree}
%\\
%\\
\end{tabular}\\[2mm]
\caption{Global type weak head-normal form equivalence: Context rules} 
\label{fig:type-wf-context}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{c}
\begin{prooftree}
{
\Gamma \vdash \WHNF{G_1}\equivwf  \WHNF{G_2}
}
\justifies
{\Gamma \vdash G_1 \gequivwf G_2} 
\using\trule{WfBase}
\end{prooftree}
\\
\\ 
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}\ \n
\gequivwf
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}\ \n\quad \Gamma\models \II=[0..\m]\quad 0\leq \n
\leq \m 
\end{array}
}
\justifies
{
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
\equivwf
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}
}
\using\trule{WfRecF}
\end{prooftree}
\\
\\
\begin{prooftree}
{
\begin{array}{c}
%\Gamma \vdash G_1 \gequivwf G_2
%\quad 
%\Gamma \vdash \GR{\G_1}{\AT{\ii}{\II^-}}{\xx}{\G_1'}
%\equivwf
%\GR{\G_2}{\AT{\ii}{\II^-}}{\xx}{\G_2'}\\
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}\ \n
\gequivwf
\Pi \AT{\ii}{\II}.G_2 \ \n 
\quad \Gamma\models \II=[0..\m]\quad 0\leq \n
\leq \m 
\end{array}
}
\justifies
{
\Gamma \vdash
\GR{\G_0}{\AT{\ii}{\II}}{\xx}{\G_1}
\equivwf
\Pi \AT{\ii}{\II}.G_2
}
\using\trule{WfRL}
\end{prooftree}
\\
\\ 
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}\ \n
\gequivwf
\Pi \AT{\ii}{\II}.G_2 \ \n 
\quad \Gamma\models \II=[0..\m]\quad 0\leq \n
\leq \m 
\end{array}
}
\justifies
{
\Gamma \vdash
\Pi \AT{\ii}{\II}.G_2
\equivwf
\GR{\G_0}{\AT{\ii}{\II}}{\xx}{\G_1}
}
\using\trule{WfLR}
\end{prooftree}
\\
\\
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash
\Pi \AT{\ii}{\II}.G_1 \ \n 
\gequivwf
\Pi \AT{\ii}{\II}.G_2 \ \n 
\quad \Gamma\models \II=[0..\m]\quad 0\leq \n
\leq \m 
\end{array}
}
\justifies
{
\Gamma \vdash
\Pi \AT{\ii}{\II}.G_1
\equivwf
\Pi \AT{\ii}{\II}.G_2
}
\using\trule{WfLL}
\end{prooftree}
%\\ 
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash G_1 \gequivwf G_1'\quad 
%\Gamma \vdash
%{\G_2\subst{\jj}{\ii}\subst{G_2'\subst{\jj}{\ii}}{\xx}}
%\gequivwf
%\G_2'\subst{\jj}{\ii}\\[1mm]
%\termsize{\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}} \geq 
%\termsize{G_2'\subst{\jj}{\ii}} \quad \xx\not\in \ftv{(G_2')}
%\end{array}
%}
%\justifies
%{
%\Gamma \vdash
%\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_2}
%\equivwf
%\GR{\G_1'}{\AT{\ii}{\II}}{\xx}{\G_2'}
%}
%\using\trule{WfRecR}
%\end{prooftree}
%\\
%\\
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash G_1 \gequivwf G_1'\quad 
%\Gamma \vdash
%\G_2\subst{\jj}{\ii}
%\gequivwf
%{\G_2'\subst{\jj}{\ii}\subst{G_2\subst{\jj}{\ii}}{\xx}}
%\\[1mm]
%\termsize{\GR{\G_1'}{\AT{\ii}{\II}}{\xx}{\G_2'}} \geq 
%\termsize{G_2\subst{\jj}{\ii}} \quad \xx\not\in \ftv{(G_2)}
%\end{array}
%}
%\justifies
%{
%\Gamma \vdash
%\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_2}
%\equivwf
%\GR{\G_1'}{\AT{\ii}{\II}}{\xx}{\G_2'}
%}
%\using\trule{WfRecL}
%\end{prooftree}
%\\
%\\
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash G_1 \gequivwf G_2'\subst{0}{\ii}\quad 
%\Gamma \vdash
%{\G_2\subst{\jj}{\ii}\subst{G_2'\subst{\jj}{\ii}}{\xx}}
%\gequivwf
%\G_2'\subst{\jj}{\ii}\\[1mm]
%\termsize{\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}} \geq 
%\termsize{G_2'\subst{\jj}{\ii}} 
%\end{array}
%}
%\justifies
%{
%\Gamma \vdash
%\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_2}
%\equivwf
%\Pi \AT{\ii}{\II}.{G_2'}
%}
%\using\trule{WfRecR}
%\end{prooftree}
%\\
%\\
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash G_2'\subst{0}{\ii}\gequivwf G_1 \quad 
%\Gamma \vdash
%\G_2'\subst{\jj}{\ii}
%\gequivwf
%{\G_2\subst{\jj}{\ii}\subst{G_2'\subst{\jj}{\ii}}{\xx}}
%\\[1mm]
%\termsize{\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}} \geq 
%\termsize{G_2'\subst{\jj}{\ii}} 
%\end{array}
%}
%\justifies
%{
%\Gamma \vdash
%\Pi \AT{\ii}{\II}.{G_2'}
%\equivwf
%\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_2}
%}
%\using\trule{WfRecR}
%\end{prooftree}
\end{tabular}\\[2mm]
\caption{Global type weak head-normal form equivalence: Mathematical Induction rules} \label{fig:type-wf-recursion}
\end{figure}

%\begin{figure}
%\centering
%\begin{tabular}{c}
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash \U_1 \gequivwf \U_2 
%\quad 
%\Gamma \vdash \G_1 \gequivwf \G_2\\[1mm]
%\Gamma \vdash \GS{\p}{\p'}{\U_i}.\G_i \RHD \GType\\
%\end{array}
%}
%\justifies
%{\Gamma \vdash 
%\Gamma \vdash \GS{\p}{\p'}{\U_1}.\G_1\gequivwf 
%\Gamma \vdash \GS{\p}{\p'}{\U_2}.\G_2
%} \using\trule{CIO}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{
%\begin{array}{c}
%\forall i\in I.\ \Gamma \vdash \G_{1i} \gequivwf \G_{2i} \\[1mm]
%\Gamma \vdash 
%\TO{\p}{\q}\colon \{l_i: \G_{ji}\}_{i\in I}\RHD \GType \ 
%\ (j=1,2)
%\end{array}
%}
%\justifies
%{\Gamma \vdash \TO{\p}{\q}\colon \{l_i: \G_{1i}\}_{i\in I}\gequivwf  
%\TO{\p}{\q}\colon \{l_i: \G_{2i}\}_{i\in I}} 
%\using\trule{CBra}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \G_1 \gequivwf \G_2}
%\justifies
%{\Gamma \vdash \GM{\ty}{\G_1} \gequivwf \GM{\ty}{\G_2}}  
%\using\trule{WfRec}
%\end{prooftree}
%\\
% \\
%\begin{prooftree}
%{
%\begin{array}{c}
%\Gamma \vdash G_1 \gequivwf G_2
%\quad 
%\Gamma \vdash G_1' \gequivwf G_2'\\[1mm]
%\Gamma \vdash
%\GR{\G_i}{\AT{\ii}{\II}}{\xx}{\G_i'}\RHD \kappa 
%\quad (i=1,2)\\[1mm]
%\end{array}
%}
%\justifies
%{
%\Gamma \vdash
%\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
%\gequivwf
%\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}
%}
%\using\trule{Wf}
%\end{prooftree}
%\\
%\\
%\begin{prooftree}
%{\Gamma \vdash \Env}
%\justifies
%{\Gamma \vdash \ty \gequivwf \ty} \using\trule{WfTVar}
%\end{prooftree}
%\begin{prooftree}
%{\Gamma \vdash \Env}
%\justifies
%{\Gamma \vdash \xx \gequivwf \xx} \using\trule{WfRVar}
%\end{prooftree}
%\begin{prooftree}
%{\Gamma \vdash \Env}
%\justifies
%{\Gamma \vdash \End \gequivwf \End} \using\trule{WfEnd}
%\end{prooftree}\\
%\\
%\begin{prooftree}
%{\Gamma,\AT{\ii}{\II}\vdash \G_1\gequivwf \G_2}
%\justifies
%{\Gamma \vdash \Pi \AT{\ii}{\II}.\G_1\gequivwf \Pi \AT{\ii}{\II}.\G_2}
%\using\trule{WfProd}
%\end{prooftree}
%\begin{prooftree}
%{\begin{array}{c}
%\Gamma\vdash \G_1\gequivwf \G_2 \quad 
%\Gamma\models \ii_1:I = \ii_2:I\\[1mm]
%\Gamma\vdash \G_i\ii_i \RHD \kappa 
%\quad 
%(i=1,2)\\[1mm]
%\end{array}
%}
%\justifies
%{\Gamma \vdash \G_1 \ii_1 \gequivwf \G_2 \ii_2}
%\using\trule{WfApp}
%\end{prooftree}\\
%\\
%\end{tabular}
%\caption{Global type congruency rules} \label{fig:type-cong}
%\end{figure}




==> global_types.tex <==
\subsection{Global types}
\label{sec:globaltypes}
\noindent 
Global types allow the description
of the parameterised conversations of
multiparty sessions as a type signature.
%Our type syntax integrates
%three different formulations: (1) global types from
%\cite{BettiniCDLDY08LONG} to specify and type global multiparty interactions; (2)
%dependent types with primitive recursive combinators based on
%\cite{DBLP:conf/mfps/Nelson91} for their expressive power;
%and (3) parameterised dependent types 
%from a simplified Dependent ML % (DML)
%\cite{DBLP:conf/popl/XiP99,DependentBook} 
%as an effective base for constraining indices. 
Our type syntax integrates
elements from three different theories:
% three different formulations: 
(1) global types from
\cite{BettiniCDLDY08LONG}; (2)
dependent types with primitive recursive combinators based on
\cite{DBLP:conf/mfps/Nelson91};
and (3) parameterised dependent types 
from a simplified Dependent ML % (DML) 
\cite{DBLP:conf/popl/XiP99,DependentBook}.  

\input{fig_global}
% \input{fig_type_reduction}
 
%$G,G',\ldots$ range over \emph{Global types} 
%%$G,G',\ldots$ describe the whole conversation scenario of a
%%multiparty session as a type signature. 
%\emph{Local types } $\T,\T',\ldots$
%correspond to the behaviour of one of the session participants, which 
%will be explained \S~\ref{sec:typing}. 

The grammar of global types ($G,G',...$) is given in Figure~\ref{fig:global}.
%The key extension from \cite{BettiniCDLDY08LONG} is 
{\em Parameterised principals}, written $\p,\p',\q,\ldots$, % range over 
% $\p,\p',\q,..$. Principals $\pp$ are participant constants (\Alice, \Bob, ...)
can be indexed by one or more parameters, \eg $\Worker[5][\ii+1]$. Index
$\tii$ ranges over index variables $\ii,\jj,\nn$, naturals $\n$ or
arithmetic operations.  A global interaction can be a message exchange
($\GS{\p}{\p'}{\U}.\G$), where $\p,\p'$ denote the sending and receiving
principals, $\U$ the payload type of the message and $\G$ the subsequent
interaction.  Payload types $\U$ are either value types $\ST$ (which contain
base type $\Nat$ and session channel types $\mar{G}$), or 
{\em end-point types} $T$
(which correspond to the behaviour of one of the session participants and will
be explained in \S~\ref{sec:typing}) for
delegation. Branching ($\GB{\p}{\p'}$) allows the session to follow one of the different $\G_k$
paths in the interaction ($K$ is a ground and finite set of integers). 
$\GM{\xx}{\G}$ is a recursive type where   
type variable $\xx$ 
is guarded in the standard way 
(they only appear under some prefix)
 \cite{PierceBC:typsysfpl}.

The main novelty is the primitive recursive operator
$\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}$ from G\"odel's System
$\mathcal{T}$~\cite{GirardJY:protyp} 
% and the dependant global type $\Pi\AT{\ii}{\II}.\G$ from 
% \cite{DBLP:conf/mfps/Nelson91}.  
whose reduction semantics is given in Figure~\ref{fig:globalreduction}.  
% The primitive recursive operator takes as
Its parameters are a global type $\G$, an index variable
$\ii$ with range $\II$,
 a type variable for recursion $\xx$ and a recursion body
$\G'$.\footnote{We distinguish recursion and primitive recursion in order to get
  decidability results, see \S~\ref{sec:subjectreduction}. } 
% \footnote{A separation between the recursion and the recursor 
% is essential for decidability results in \S~\ref{sec:subjectreduction}. }  
When applied to an index $\tii$, its semantics corresponds to the
repetition $\tii$-times of the body $\G'$, with the index variable $\ii$ value
going down by one at each iteration, from $\tii-1$ to $0$. The final
behaviour is 
given by $\G$ when the index reaches $0$. 
% The
% dependent type $\Pi
% \AT{\ii}{\II}.\G$ also has a standard semantics: when applied to
% an index $\ii$, the index is simply substituted.  We assume a call-by value
%semantics so that the argument is evaluated first.  
The index sorts comprise the set of natural numbers and its restrictions by % sets
% % subset of index sorts, which are permitted only with respect
% of
predicates ($\PRED,\PRED',..$) that are, in our case, %.  In our case, these are
conjunctions of inequalities.  $\op$ represents first-order indices operators
(such as $+$, $-$, $\ast$,...). 
%are left as parameters to our theory. 
We often omit $\II$ and $\End$ in our examples. 
%$\Nat = \{ \nn \ | \ \nn\geq 0 \ \andl \ \nn \in \Int\}$.
 
% \noindent
Using $\mathbf{R}$, we define the product, composition, repetition and test
operators as syntactic sugar (seen in \S~\ref{sec:introduction}):
{\footnotesize
\[
\begin{array}{@{}l@{}c@{\,}l|@{\;\;}l@{}c@{\,}l}
\Pi \AT{\ii}{\II}.\G & = & \GR{\End}{\ii}{\xx}{\G\sub{\ii+1}{\ii}}
& \FOREACH{\ii}{\!<\!\jj}{G}& = &
 \GR{\End}{\ii}{\xx}{\G\sub{\xx}{\End}} \ \jj\\[1mm]
\MERGE{G_1;G_2} & = &
\GR{\G_2}{\ii}{\xx}{\G_1\sub{\xx}{\End}} \ 1 \ 
& \IF\ \jj \ \THEN\ \G_1 \ \ELSE \ \G_2 & = &
\GR{\G_2}{\ii}{\xx}{\G_1}\APP \jj
\end{array}
% \begin{array}{rcl}
% \Pi \ii.\G \ = \ \GR{\End}{\ii}{\xx}{\G\sub{\ii+1}{\ii}}
% & \quad &
% \MERGE{G_1;G_2} \ = \ 
% \GR{\G_2}{\ii}{\xx}{\G_1\sub{\xx}{\End}} \ 1\\[1mm]
% \FOREACH{\ii}{<\n}{G}& = &
%  \GR{\End}{\ii}{\xx}{\G\sub{\xx}{\End}} \ \n+1
% \\[1mm]
% \IF\ \n \ \THEN\ \G_1 \ \ELSE \ \G_2 & = &
% \GR{\G_2}{\ii}{\xx}{\G_1}\APP \n
% \end{array}
\]}

\noindent
where we assume that $\xx$ is not free in $G$ and $G_1$, and
that the leaves of the syntax trees of $G_1$ and $G$ are 
$\End$. 
%does not contain 
%terminate with $\End$, not recursive variables. 
These definitions rely on a special substitution of each ${\small\End}$ by ${\small\xx}$ (for example, 
${\small \TO{\p}{\p'}\{ l_1\!\!: !\ENCan{\Nat};\End, l_2\!\!:\!\End\}\sub{\xx}{\End}=
\TO{\p}{\p'}\{ l_1\!\!: !\ENCan{\Nat};\xx, l_2\!\!:\! \xx\}}$). 
The composition operator (which we usually write `$;$')
appends the execution of $G_2$ to $G_1$; the repetition operator above repeats
$\G$ $\jj$-times\footnote{
This version of $\mathtt{foreach}$ uses decreasing indices. One can write an
increasing version, see \S~\ref{sub:globalexample}.}; the boolean values are integers $0$
(\false) and $1$ (\true).
Similar syntactic sugar is defined for local types and processes. 

Note that composition and repetition do not necessarily impose 
sequentiality: only the order of the asynchronous messages and the 
possible dependencies~\cite{CHY07} between receivers and subsequent senders
controls the sequentiality. For example, a parallel version of 
the sequence example of
(\S~\ref{sec:introduction} (\ref{ex:sequence})) can be written in our
syntax as follows: 
% One can for example write a parallel version of the sequence example
% (\S~\ref{sec:introduction} (\ref{ex:sequence})) with:
\begin{eqnarray}\label{parallel_seq}
 \Pi n.(\FOREACH{\ii}{<n}{\GS{\W[n-\ii]}{\W[n-\ii-1]}{\Nat}})
\end{eqnarray}
where each worker $\W[\jj]$ sends asynchronously a value $v_j$ to its next 
worker $\W[\jj-1]$ without waiting for the message from $\W[\jj+1]$ to arrive
first (i.e.~each choice of $v_j$ is independent from the others). 

% {\footnotesize
% \begin{eqnarray}
% \label{ex:sequencepar}
% \!\!\!\Pi n.(\FOREACH{\ii}{<n}{\GS{\W[n-\ii+1]}{\W[n-\ii]}{\Nat}})
% %\Pi n.(\FOREACH{\ii}{<n}{\GS{\W[\ii+1]}{\W[\ii]}{\Nat}})
% %\Pi n.(\FOREACH{\ii}{<n}{\GS{\W[\ii+1]}{\W[\ii]}{\Nat}})
% \quad
% \begin{minipage}{10em}
% \xymatrix@C=15pt{
%   *+[F]{{\footnotesize \n}}\ar[r]
%   &*+[F]\txt{\footnotesize \n-1}\ar[r]
%   &{\ldots}\ar[r]
%   &*+[F]\txt{\footnotesize 0}}
% \end{minipage} 
% \end{eqnarray}}
% $${\small 
% \FOREACH{\ii}{<n}{\GS{\W[\ii+1]}{\W[\ii]}{\Nat}} \quad
% \FOREACH{\ii}{<n}{\GS{\W[\ii-n+1]}{\W[\ii-n]}{\Nat}}
% }$$
% \begin{center}
% \begin{tabular}{rclrrrclr}
% Global \quad 
%  $\G$ & ::= & $\e\rightarrow\e':\langle\U\rangle.{\G'}$  &\quad \quad \quad
% & Exchange \quad & $\UT$   & ::= & $\ptilde{S}\ |\ \T$
% \\
% %      & \sep & $\p\rightarrow\pset:\{l_i:\G_i\}_{i\in I}$ &

% & \sep & \RECSEQ{\G}{\n}{\x}{\G'} & & Sorts \quad &
    
%   $S$   & ::= & $\Bool\ |\ \Nat\ |\ G$ & \\
%    & \sep & $\Pi$n.\G  & \quad& Expressions \quad & $\e$   & ::= &$ \va \ \sep \x\ \sep \e+\e'\ $\\
%       & \sep & \x & \quad & \quad& & & $  \e-\e' $ \sep \e $\ast$ \e'\\ 
%       & \sep & \G\e & \quad& Values \quad & $\va$   & ::= &$ \Num$\\
%       & \sep & $\End$\\
      
% %      $\mu \ty.\G$  \sep $\ty$ \sep 
% \end{tabular}
% \end{center}

%\noindent
%We simplify the syntax in \cite{CHY07}
%by eliminating channels and parallel compositions,
%while preserving the original expressivity (see \S~\ref{sec:related}).\\
%\indent The global type $\Gv\p\p\U{\G'}$ says that participant
%$\p$ multicasts a message of type $\U$ to participants $\p_k$
%($\inpset{k}$) and then interactions described in $\G'$ take place.
%\emph{Exchange types} $\U,\U',...$ consist of {\em sorts} types
%$S, S', \ldots$ for values (either base types or global types),
%and {\em action} types $\T, \T', \ldots$  for channels (discussed
%in \S \ref{TypingSec}).
%Type $\p\rightarrow\pset:\{l_i:\G_i\}_{i\in I}$ says participant
%$\participant{p}$ multicasts one of the labels $l_i$ to
%participants $\participant{p}_k$ ($\kinpset$). If $l_j$ is sent,
%interactions described in $G_j$ take place. Type $\mu \ty.\G$ is a
%recursive type,
%assuming type variables
%($\ty, \ty', \dots$) are guarded in the standard way, i.e., type
%variables only appear under some prefix.  We take an
%\emph{equi-recursive} view of recursive types, not distinguishing
%between $\mu \ty.\G$ and its unfolding $G\subst{\mu
%\ty.\G}{\ty}$~\cite[\S 21.8]{PierceBC:typsysfpl}. We assume
%that $G$ in the grammar of sorts is closed, i.e., without free type
%variables. Type $\End$ represents the termination of the session. We
%often write $\participant{p}\to\participant{p}'$ for
%$\participant{p}\to\{\participant{p}'\}$.





==> initialization.tex <==
\paragraph{Initialisation}

The initialisation of a session does not necessarily require a multicast
request. It is possible to allow participants to join only when they start their
involvement in the session.

$$
\sa\Ia{\p_0..\p_\n}{\y}{\PP_0}\redsym 
(\nu \s)(\PP_{0}\sub{\si\s{\p_0}}{\y} \pc
 \s : \emptyset \pc \si{\Ia}{\p_1}:\s \pc ... \pc \si{\Ia}{\p_\n}:\s 
)
$$

$$
\si{\Ia}{\p_k}:\s \pc \sr\Ia{\p_k}{\y_k}{\PP_k} \redsym \PP_{k}\sub{\si\s {\p_k}}{\y_{k}}
$$

$$
\begin{prooftree}
{
\begin{array}{c}
\Gamma \vdash \Ia:\mar{\G}\quad
\Gamma \proves \pp\rhd \Nat \quad 
\Gamma \models \pp\in\pid(\G)\\[1mm] 
\end{array}
}
\justifies
{\Gamma \vdash \si{\Ia}{\pp}:\s \rhd \si{\s}{\pp}:\G \proj{\pp} } \using\trule{TAcc}
\end{prooftree}
$$

Another way is to have the first participant join the session the same way as
the others:
$$
\sa\Ia{\p_0..\p_\n}{\y}{\PP_0}\redsym 
(\nu \s)(\sr\Ia{\p_0}{\y}{\PP_0}\pc\s : \emptyset \pc \si{\Ia}{\p_0}:\s \pc ... \pc \si{\Ia}{\p_\n}:\s 
)
$$

==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\noindent
As the momentum around communications-based computing grows, the need
for effective frameworks to
% coordinate the interactions among distributed peers is
% pressing. Such coordination typically
globally {\em coordinate} and {\em structure} the application-level
interactions is pressing. % with respect to the
% sequences in which messages are transmitted
% and received, their compositions, choices and repetitions
% to form a larger composite, meaningful multiparty protocol.
%%For this purpose
The structures of interactions are naturally distilled as
{\em protocols}. Each protocol describes a bare skeleton of how
interactions should proceed, through e.g.
%% such operations as
sequencing, choices and repetitions.
% Built on
% the study on type structures for the $\pi$-calculus, the preceding
% studies have shown that such protocols can be captured as types for
% multiparty sessions~\cite{CHY07}. Just as an instance of a class
% should obey the type signature for method calls specified in that
% class,
In the theory of multiparty session types~\cite{CHY07,BC07,BettiniCDLDY08LONG},
such protocols can be captured as types for interactions,
% Participants engaged in an instance of a protocol, or a
% session, should follow the specified protocol structure.
%% Asf in other type theories,
and type checking can statically ensure runtime safety and fidelity
% interactions among endpoint programs
% will conform to
to a stipulated
protocol.

One of the particularly challenging aspects of protocol descriptions
is the fact that many actual communication protocols are
%% {\em dynamic}
highly {\em parametric}
in the sense that the number of participants  and
even the interaction structure itself are not fixed at design time.
% Rather, the number of participants
% involved in a protocol and how they are connected
% not only a protocol is parameterised,
% the actual endpoint programs
% themselves are parameterised, whose instantiations will only be
% determined at run-time.
Examples include parallel algorithms such as
the Fast  Fourier Transform % algorithm
(run on any number of
communication nodes depending on resource availability)
and Web
services such as business negotiation involving an
arbitrary number of sellers and buyers.
This nature is important, for instance,
for the programmer of a parallel algorithm
where the size or shape of the communication topology,
or the number of available threads might
be altered depending on the number
of available cores in the machine.
Another scenario is web services where the
participant sets may be known at design time,
or instantiated later.
%at runtime
This paper introduces a robust dependent type theory
which can statically ensure communication-safe, deadlock-free process
interactions which follow parameterised multiparty protocols.
% The
% underlying type structures can
% precisely capture a wide range of communication topologies.
% This
% parametrisation is made possible through by augmenting type structures from
% \cite{CHY07,GProgress08,esop09} with a classical construct in type
% theory, dependent types, combined with the recursor operator.
%
% This leads to the type theory where one parametric protocol can
% capture a family of infinite concrete protocols, with the
% corresponding typability ensuring safety and liveness for the
% execution of parametric communicating processes.
% The diverse applications
% that feature such dynamic protocols
% range over parallel algorithms
% %
% % want a single specification/implementation to support computations of arbitrary length and to be able to use different resource configurations, e.g. different number of cores.
% %
% %for scientific computing
% (\S~\ref{subsec:fft}) and
% %distributed
% Web service protocols (\S~\ref{sec:usecase}).
% %% as this paper
% %% shall illustrate.
% %
% % we of course connect to different parties at different places according to how the protocol proceeds. need extensibility to support modified/new participants without changing the main protocols every time.
% %

We illustrate the key ideas of our proposed parametric type structures
through examples. Let us first consider a simple protocol where
participant $\Alice$ sends a message of type $\Nat$ to participant
$\Bob$.  To develop the code for this protocol, we start by specifying
the global type, which can concisely and clearly describe a high-level
protocol for multiple participants
\cite{CHY07,BettiniCDLDY08LONG,esop09}, as follows ($\End$ denotes
protocol termination):
\[
\begin{array}{c}
G_1  \ = \ \GS{\Alice}{\Bob}{\Nat}.\End\\[-2ex]
\end{array}
\]
The flow of communication is indicated with the symbol $\rightarrow$ and
upon agreement on $G_1$ as a specification for $\Alice$ and $\Bob$,
each program can be implemented separately,
e.g. as $y!\ENCan{100}$ (output 100 to $y$) by $\Alice$ and
$y?(z);{\bf 0}$ (input at $y$) by $\Bob$.
For type-checking, $G_1$ is
{\em projected} into end-point session types:
one from $\Alice$'s point of view,
$!\ENCan{\Bob,\Nat}$ (output to $\Bob$ with $\Nat$-type),
and another from $\Bob$'s point of view, $?\ENCan{\Alice,\Nat}$
(input from $\Alice$ with $\Nat$-type), against which
the respective $\Alice$ and $\Bob$ programs are checked to be compliant.

The first step towards generalised type structures for multiparty
sessions is to allow modular specifications of protocols using
arbitrary compositions and repetitions of interaction units (this is a
standard requirement in multiparty contracts \cite{CDL}).  Consider
the type $G_2 \ = \ \GS{\Bob}{\Carol}{\Nat}.\End$.  The designer may
wish to compose sequentially $G_1$ and $G_2$ together to build a larger
protocol:
\[
\begin{array}{rclcl}
G_3
& = & \MERGE{G_1;G_2} %\\
& = & \GS{\Alice}{\Bob}{\Nat}.\GS{\Bob}{\Carol}{\Nat}.\End
\end{array}
\]
We may also want to iterate the composed protocols $\n$-times, which can be
written by $\FOREACH{i}{<\n}{\MERGE{G_1;G_2}}$, and moreover bind the number of
iteration $\n$ by a dependent product
% bind repetitions $j$-times by a dependent product type
to build a {\em family of global specifications}, as in
($\Pi n$ binds variable $n$):
\begin{eqnarray}
\label{alice-bob-carol}
\Pi n.\FOREACH{\ii}{<n}{\MERGE{G_1;G_2}}
%\Pi n.(\RECSEQ{\End}{i}{\xx}{}\GS{\Alice}{\Bob}{\Nat}.
%\GS{\Bob}{\Carol}{\Nat}.\xx \APP n)
\end{eqnarray}
%
%Now corresponding end-point types should be an indexed
%{\em session type sequence}. For example,
%\Alice\ would be typed by $\Pi j.\FOREACH{\ii}{<j}{!\ENCan{\Bob,\Nat};}$,
%which represents the length of sessions (the number of messages) is
%unfixed before
%executions. A process for \Alice\  should be also parameterised
%correctly, following (\ref{alice-bob-carol}).
%
%In order to support the type-based specification and programming of such idioms
%($\Pi$, $\mathtt{foreach}$, $\mathtt{comp}$),
%we use the primitive recursion operator ${\bf R}$ from G\"odel's System
%$\mathcal{T}$ \cite{GLT}.
%% To enable programming such idioms in the simplest and
%% the most canonical setting,
%% this paper adds a primitive recursive combinator ${\bf R}$ of
%% G\"odel's System $\mathcal{T}$ \cite{GLT}.
%The basic system
%of finite session types is thus extended to allow
%{\em primitive recursive formulations of session type
%sequences} from which dependent product types on natural
%numbers can be constructed. The following two reduction rules
%from System $\mathcal{T}$ are added to
%global program specifications:
%\begin{center}
%\footnotesize
%\begin{tabular}{rcl}
%$\GR{\G}{\ii}{\xx}{\G'}\APP 0$  & \redsym & \G \\[1mm]
%$\GR{\G}{\ii}{\xx}{\G'}\APP \n+1$ & \redsym &
%$\G'\sub{\n}{\ii}\sub{(\GR{\G}{\ii}{\xx}{\G'}\APP \n)}{\xx}$
%%$(\Pi \ii.\G)\APP \n$          & \redsym & \G\sub{\n}{\ii}\\[1mm]
%\end{tabular}
%\end{center}
%%
%% \input{fig_intro}
%
Beyond enabling a variable number of exchanges between a fixed set of
participants, the ability to parameterise {\em
  participant identities} can represent
%
% the framework is simple and intuitive, but when we
% {\em parameterise} participant identity, we can represent
%a great range of
a wide class of the communication topologies found in the literature.  For
example, the use of indexed participants $\W[i]$ (denoting the $i$-th
worker) % creates a parameterised family
% of workers, and we can
allows the specification of a family of session types such that
%  (when
% $G_0=\End$) as well as a simple ring topology
% (when $G_0=\GS{\W[0]}{\W[n]}{\Nat}$)
neither the number of participants nor
message exchanges are
known before the run-time instantiation of the parameters. The following type
and diagram both describe a sequence of messages from $\W[n]$ to $\W[0]$
(indices decrease in our $\mathtt{foreach}$, see \S~2):
%(as with ${\bf R}$,
% {\footnotesize
\begin{eqnarray}
\label{ex:sequence}
\Pi n.(\FOREACH{\ii}{<n}{\GS{\W[\ii+1]}{\W[\ii]}{\Nat}})
%\Pi n.(\FOREACH{\ii}{<n}{\GS{\W[\ii+1]}{\W[\ii]}{\Nat}})
\qquad
\begin{minipage}{10em}
\xymatrix@C=15pt{
  *+[F]{{\footnotesize \n}}\ar[r]
  &*+[F]\txt{\footnotesize \n-1}\ar[r]
  &{\ldots}\ar[r]
  &*+[F]\txt{\footnotesize 0}}
\end{minipage}
\end{eqnarray}% }
Here we face an immediate question:
%First
%{\em how expressive is this simple approach?}
%Can we program the representative communication
%topologies found across the literature and practice?
%Can we provide an efficient (decidable) typechecking
%which preserves the main properties the session types guarantee
%such as progress and communication-safety
%between non-fixed number of multiparty? Secondly,
{\em what is the underlying type structure for such parametrisation,
  and how can we type-check each (parametric) end-point program?}  The
type structure should allow the projection of a parameterised global
type to an end-point type {\em before} knowing the exact shape of the
concrete topology.

In (\ref{alice-bob-carol}), corresponding end-point
types are parameterised {\em families} of session types.
For example,
\Bob \ would be typed by $\Pi
j.\FOREACH{\ii}{<j}{?\ENCan{\Alice,\Nat};!\ENCan{\Carol,\Nat}}$, which
represents the product of session interactions with different lengths. The
choice is made when $j$ is instantiated, i.e. before execution.
The difficulty of the projection
% A more subtle problem of the projection
arises in
(\ref{ex:sequence}): if $\n\!\geq\! 2$, there are three
distinct {\em communication patterns} inhabiting this
specification: the initiator $\W[\n]$ (send only), the $\n-1$ middle workers
(receive then send), and the last worker $\W[0]$ (receive only). This is no
longer the case when $\n= 1$ (there is only the initiator and the last
worker) or when $\n= 0$ (no communication at all).  Can we provide a
decidable projection and static type-checking by which we
can preserve the main properties of the session types such as progress
and communication-safety in parameterised process topologies?  The key
technique proposed in this paper is a projection method from a
dependent global type onto a {\em generic end-point generator} which
exactly captures the interaction structures of parameterised end-points
and which can represent the class of all possible end-point
types.

The main contributions of this paper follow:
% \marginpar{changed}
 %(\S~\ref{subsec:endpoint}).
%\pagebreak
% Here we face a couple of immediate questions:
% \begin{itemize}
% \item
% {\em How expressive is this simple
% approach?} Are we able to we program the main communication
% topologies found across the literature for e.g. parallel algorithms and Web services?
% \item
% {\em How can we check program correctness?} More concretely,
% how can we project a parameterised global type to a local
% type even when we do not know the exact shape of the topology yet.
% \end{itemize}
% For example, in the sequencing topology of figure~\ref{fig:ex-intro},
% if $\n\geq 2$, then there are
% three different {\em roles} inhabiting this specification: the
% initiator, the $n-2$ middle workers, and the last worker, each of which
% engages in a distinct communication pattern. The number of
% roles is also variable; when $\n= 1$, there is only the initiator
% and the last worker; and when $\n= 0$, the session does not involve any
% communication.
%
% If we choose the
% ring topology, the situation is even more complex.
%
%There might be the two ways to implement the local process.
%\begin{enumerate}
%\item We build a local type from each end-point process
%and check whether it conforms to the general generator using $\equiv$.
%
%\item
%We first transform a general generator into an optimal local type,
%then write a process against that optimal local type.
%\end{itemize}
%We type FFT following the first approach in \S~\ref{sec:protocol}.
%The integration of dependent types and multiparty session types enables not only
%the precise description of the communication topology of agents and the scale of
%their interaction
%patterns, %
%it offers a powerful tool by which we can write down a \ny{generic}
%generator of end-point
%local types and implementations that follows the specified structure and can be statically type-checked. This means that whatever concrete topologies are formed by the generated code at runtime, the participants are always guaranteed to conform to the stipulated global topology and interaction
%patterns. The ability to treat the typed interactions among the arbitrary number of
%participants as a single multiparty session also leads to clearer prospects regarding
%resource usage by these agents.
%%since we have a rigorous description of communication topologies and patterns.
%
%\paragraph{\bf Contributions of this work}
\begin{itemize}
\item {\em A new expressive framework to globally specify and program}
  % programming global, distributed specifications
% which can elegantly and concisely
% describe
a wide range of
parametric communication protocols
(\S~\ref{sec:syntax_and_example}). We achieve this result by
combining dependent type theories derived from
G\"odel's System $\mathcal{T}$
\cite{DBLP:conf/mfps/Nelson91} (for expressiveness)
and indexed dependent types from \cite{DBLP:conf/popl/XiP99} (for parameter
control), with multiparty session types.

\item
{\em Decidable and flexible projection methods}
based on a generic end-point generator
and mergeability of branching types, enlarging the typability
(\S~\ref{subsec:endpoint}).

\item {\em A dependent typing system} that treats the full
multiparty session types integrated with dependent types (\S~\ref{sec:typing}).

\item {\em Properties of the dependent typing system}
which include
% based on  G\"odel's System $\mathcal{T}$.
%The resulting static typing system allows
decidability of
  type-checking.
The resulting static typing system also
guarantees type-safety and deadlock-freedom (progress) for
well-typed processes involved in parameterised multiparty communication
protocols (\S~\ref{sec:property}).

\item {\em Applications} featuring various process topologies
(\S~\ref{sec:syntax_and_example},\S~\ref{subsec:typingexample}),
  including the complex butterfly network of the parallel
  FFT algorithm
(\S~\ref{subsec:fft}, \S~\ref{subsec:fft:typing}).
As far as we know, this is the first time
such a complex protocol is %%described and
specified by
a single {\em type} and that its implementation can be automatically
type-checked
% (interactions among the arbitrary number of participants
% typed by it)
% and is automatically
% proved
to prove communication-safety and deadlock-freedom.
%for .
We also extend the calculus with a new asynchronous
primitive for session initialisation and apply it to web services usecases
%which requires a new participant can join to a sub-multiparty session
\cite{CDLRequirements} (\S~\ref{sec:applications}).
\end{itemize}

Section~\ref{sec:syntax_and_example} gives the definition of the parameterised
types and processes, with their semantics. Section~\ref{sec:typing} describes
the type system. The main properties of the type system are presented in
Section~\ref{sec:property}. Section~\ref{subsec:typingexample} shows typing
examples. Section~\ref{sec:related} concludes and discusses related work.

This article is a full version expanded from \cite{YDBH10}, with complete
definitions and additional results with detailed proofs.
It includes more examples with detailed explanations and verifications,
as well as expanded related work.
Some additional material related to implementations and programming
examples will be discussed in \S~\ref{sec:related}.



==> long_termination.tex <==
% Next we prove the termination for type-equality checking. 

\input{fig_size}

Proving the termination of type equality checking requires 
a detailed analysis 
since the premises of the mathematical induction 
rules compare the two types whose syntactic sizes are larger 
than those of their conclusions. 
The size of the judgements are defined 
in Figure \ref{fig:size}, 
using the following functions from \cite[\S~2.4.3]{DependentBook}, 
taking rule \trule{WfRecF} in Figure~\ref{fig:type-wf} into account. 
\begin{enumerate}
\item $\termsize{G}$ is the size of the structure of $G$ 
where we associate $\omega^2$-valued weight to each judgement 
to represent a possible reduction to a weak head normal form. 

\item $\inductiontermsize{G}$ is the size of the structure of $G$ 
where unfolding of recursors with finite index sets is considered,
taking \trule{WfRecF} in Figure~\ref{fig:type-wf} into account. 

\item $\reductionsize{\G}$ 
denotes an upper bound on the length of any 
$\redsym$ reduction sequence (see Figure~\ref{fig:globalreduction})  
starting from $G$ and its subterms.

\item $\inductionreductionsize{\G}$ 
denotes an upper bound on the length of any 
$\redsym$ reduction sequence (see Figure~\ref{fig:globalreduction})  
starting from $G$ and its subterms.  
It unfolds recursors with finite index sets. 
%the number of the head reductions from $G$. 
%\item $\reductionsize{G}$ is the number of the head reductions 
%from $G$ and its subterms. 
%\item $\inductionreductionsize{G}$ is the maximum number of 
%the head reductions from $G$ and its subterms. 
%This  includes the mathematical induction case 
%where the dependent applications with variables as the arguments. 
\end{enumerate}
The definition of the size of judgement 
$\judgementsize{\Gamma \proves G_1 \equivwf G_2}$ 
follows \cite[\S~2.4.3]{DependentBook}. 
We use $\inductionreductionsize{\G}$ and $\inductiontermsize{G}$ 
because of \trule{WfRecF} in Figure~\ref{fig:type-wf}. 
Note that $\termsize{G}$ corresponds to $\reductionsize{\G}$, 
 while $\inductiontermsize{G}$ corresponds to
$\inductionreductionsize{\G}$.  In $\inductionreductionsize{\G}$, 
we incorporate the number of reductions of unfolded 
recursors. Because the reduction of expressions 
strongly normalises, we choose the size of $e$ to be $1$ and 
the length of reductions of (closed) $e$ is assumed to be $0$.

The termination of type equality checking then is proved by the following main
lemma.  

\begin{LEM}[Size of equality judgements]\label{lem:size}
The weight of any premise of a rule is always 
less than the weight of the conclusion. 
\end{LEM}
\begin{proof}
Our proof is by induction on the length of reduction 
sequences and the size of terms. \\[1mm]
{\bf Case \trule{WfBase}.} The case $\WHNF{G_1}=G_1$ and 
$\WHNF{G_2}=G_2$ are obvious by definition. Hence we assume  
$\WHNF{G_1} \not = G_1$. Thus there exists at least one step reduction 
such that $G_1\redsym G_1'$. Hence by definition, 
$\inductionreductionsize{\WHNF{G_i}} < \inductionreductionsize{G_i}$ ($i=1,2$).
Similarly we have $\inductiontermsize{\WHNF{G_i}} \leq 
\inductiontermsize{G_i}$ by definition.  
Note that for any $G$, 
we have $\inductiontermsize{G}< \omega$. 
Hence we have 
\[
\begin{array}{lll}
  & 
\judgementsize{\Gamma \vdash \WHNF{G_1}\equivwf  \WHNF{G_2}}\\
= 
& \omega \cdot
\inductionreductionsize{\WHNF{G_1}} + \inductiontermsize{\WHNF{G_1}} + \omega \cdot
\inductionreductionsize{\WHNF{G_2}} + \inductiontermsize{\WHNF{G_2}} + 1\\ 
<  
& \omega \cdot \inductionreductionsize{G_1} + \inductiontermsize{G_1}+
  \omega \cdot \inductionreductionsize{G_2} + \inductiontermsize{G_2} + 2 \\
=& \judgementsize{\Gamma \vdash G_1\equiv  G_2}
\end{array}
\]
{\bf Case \trule{WfIO}.} Similar with \trule{WfBra} below.\\[1mm]
{\bf Case \trule{WfBra}.} 
\[
\begin{array}{ll}
& \Sigma_{k\in K}\judgementsize{\Gamma \vdash G_{1k}\equiv  G_{2k}}\\
= & 
\Sigma_{k\in K}(\judgementsize{\Gamma \vdash G_{1k}\equivwf G_{2k}}+1)\\
= & 
\Sigma_{k\in K}(
\omega\cdot(\inductionreductionsize{G_{1k}}+\inductionreductionsize{G_{2k}})+
\inductiontermsize{G_{1k}}+\inductiontermsize{G_{2k}}+2)\\
= & 
\Sigma_{k\in K}(
\omega\cdot(\reductionsize{G_{1k}}+\reductionsize{G_{2k}})+
\termsize{G_{1k}}+\termsize{G_{2k}}+2)\\
< & 
\Sigma_{k\in K}(
\omega\cdot(\reductionsize{G_{1k}}+\reductionsize{G_{2k}})+
\termsize{G_{1k}}+\termsize{G_{2k}}+2)+5\\
= & 
\judgementsize{
\Gamma \vdash \TO{\p}{\q}\colon \{l_k: \G_{1k}\}_{k\in K}\equivwf  
\TO{\p}{\q}\colon \{l_k: \G_{2k}\}_{k\in K}}
\end{array}
\] 
We note that $G_{1k}$ and $G_{2k}$ cannot 
be recursors 
since $\Gamma \proves G_{ik}\RHD \Type$ by the kinding rule, 
hence $\reductionsize{G_{ik}}=\inductionreductionsize{G_{ik}}$ and 
$\termsize{G_{ik}}=\inductiontermsize{G_{ik}}$ in 
the above third equation.  
\\[1mm]
{\bf Case \trule{WfPRec}.} Similar with \trule{WfBra} above. \\[1mm]
{\bf Cases \trule{WfRVar},\trule{WfEnd}.} By definition. \\[1mm]
{\bf Case \trule{WfRec}.} The case $I$ is infinite. 
{\small
\[
\begin{array}{ll}
& 
\judgementsize{\Gamma \vdash \G_1 \equiv \G_2} + 
\judgementsize{\Gamma,\AT{\ii}{\II} \vdash \G_1' \equiv \G_2'} \\
= & 
\judgementsize{\Gamma \proves G_1 \equivwf G_2}+1 + 
\judgementsize{\Gamma,\AT{\ii}{\II} \vdash \G_1' \equiv \G_2'}+1 \\
= & 
\omega\cdot(\inductionreductionsize{G_1}+\inductionreductionsize{G_2})+
\inductiontermsize{G_1}+\inductiontermsize{G_2}+2
 + 
\omega\cdot(\inductionreductionsize{G_1'}+\inductionreductionsize{G_2'})+
\inductiontermsize{G_1'}+\inductiontermsize{G_2'}+2\\
< & 
\omega\cdot(\inductionreductionsize{G_1}+\inductionreductionsize{G_2})+
\inductiontermsize{G_1}+\inductiontermsize{G_2}+4
 + 
\omega\cdot(\inductionreductionsize{G_1'}+\inductionreductionsize{G_2'})+
\inductiontermsize{G_1'}+\inductiontermsize{G_2'}+4 + 1\\
= & 
\judgementsize{
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
\equivwf
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}
}
\end{array}
\] 
}
The case $I$ is finite. 
{\small
\[
\begin{array}{ll}
& 
\judgementsize{\Gamma \vdash \G_1 \equiv \G_2} + 
\judgementsize{\Gamma,\AT{\ii}{\II} \vdash \G_1' \equiv \G_2'} \\
= & 
\omega\cdot(\inductionreductionsize{G_1}+\inductionreductionsize{G_2})+
\inductiontermsize{G_1}+\inductiontermsize{G_2}+2
 + 
\omega\cdot(\inductionreductionsize{G_1'}+\inductionreductionsize{G_2'})+
\inductiontermsize{G_1'}+\inductiontermsize{G_2'}+2\\
< & 
\Sigma_{n\in I}
(
\omega\cdot(m_{1n} + \inductionreductionsize{G_{1n}''} + 
m_{2n} + \inductionreductionsize{G_{2n}''}))\\
& +  \Sigma_{n\in I}
(
\omega \cdot 
(\inductionreductionsize{G_1}+\inductionreductionsize{G_2})+
\inductiontermsize{G_1}+\inductiontermsize{G_2}+4+2
)\\
&  +  
\Sigma_{n\in I}
(
\omega \cdot 
(\inductionreductionsize{G_1'}+\inductionreductionsize{G_2'})+
\inductiontermsize{G_1'}+\inductiontermsize{G_2'}+4+2
)+1\\
= & 
\judgementsize{
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
\equivwf
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}
}
\end{array}
\] 
}
where we assume ${m_{i\n}}$ is the length of the reduction 
sequence from  $\GR{\G_i}{\AT{\ii}{\II}}{\xx}{\G_i'}\, \n$ 
(in Figure~\ref{fig:globalreduction}), and 
$\GR{\G_i}{\AT{\ii}{\II}}{\xx}{\G_i'}\, \n 
 \redsym^\ast G_{i\n}'' \not\redsym$ for all $\n\in I$. 
\\[1mm]
{\bf Case \trule{WfRecF}.} Assume $I=[0,\ldots,\m]$. 
\[
\begin{array}{ll}
& 
\judgementsize{\Gamma \vdash G_1 \equiv  G_2} 
+ 
\Sigma_{1\leq \n \leq m}
\judgementsize{
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'} \n 
\equiv
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'} \n 
}\\
= & 
\omega\cdot \inductionreductionsize{G_1} 
+ \inductiontermsize{G_1}
+ \omega\cdot \inductionreductionsize{G_2} 
+ \inductiontermsize{G_2} + 2\\
& +  
\Sigma_{1\leq \n \leq m}
(\judgementsize{
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'} \n 
\equivwf 
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'} \n 
} + 1)
\\
= & 
\omega\cdot((m_{11}-1) + \inductionreductionsize{G_{11}''} + 
(m_{21}-1) + \inductionreductionsize{G_{21}''}))
+ \inductiontermsize{G_1} 
+ \inductiontermsize{G_2} + 2\\
& + \Sigma_{1\leq \n \leq m}
(
\omega\cdot(m_{1n} + \inductionreductionsize{G_{1n}''} + 
m_{2n} + \inductionreductionsize{G_{2n}''}))\\
& 
+ \Sigma_{1\leq \n \leq m}
(
\omega \cdot 
(\inductionreductionsize{G_1}+\inductionreductionsize{G_2})+
\inductiontermsize{G_1}+\inductiontermsize{G_2}+4+2
)\\
& +  
\Sigma_{1\leq \n \leq m}
(
\omega \cdot 
(\inductionreductionsize{G_1'}+\inductionreductionsize{G_2'})+
\inductiontermsize{G_1'}+\inductiontermsize{G_2'}+4+2
) \\
< & 
\Sigma_{n\in I}
(
\omega\cdot(m_{1n} + \inductionreductionsize{G_{1n}''} + 
m_{2n} + \inductionreductionsize{G_{2n}''}))\\
& 
+  \Sigma_{n\in I}
(
\omega \cdot 
(\inductionreductionsize{G_1}+\inductionreductionsize{G_2})+
\inductiontermsize{G_1}+\inductiontermsize{G_2}+4+2
)\\
& +  
\Sigma_{n\in I}
(
\omega \cdot 
(\inductionreductionsize{G_1'}+\inductionreductionsize{G_2'})+
\inductiontermsize{G_1'}+\inductiontermsize{G_2'}+4+2
) +1 \\
= & 
\judgementsize{
\Gamma \vdash
\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
\equivwf
\GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}
}
\end{array}
\] 
where we assume ${m_{i\n}}$ is the length of the reduction 
sequence from  $\GR{\G_i}{\AT{\ii}{\II}}{\xx}{\G_i'}\, \n$ 
(in Figure~\ref{fig:globalreduction}), and 
$\GR{\G_i}{\AT{\ii}{\II}}{\xx}{\G_i'}\, \n 
 \redsym^\ast G_{i\n}'' \not\redsym$ for all $\n\in I$. 

\noindent{\bf Case \trule{WfApp}} First, 
since \trule{WfApp} has a lower priority than \trule{WfBase}, 
we have $G_i\tii_i\not\redsym$.  
Hence
$\inductionreductionsize{G_i \tii_i}=\inductionreductionsize{G_i}$. 
We also note that:
\begin{enumerate}
\item 
If $G_i$ is not recursor, then 
$\inductiontermsize{G_i}=\termsize{G_i}$; and  

\item 
If $G_i$ is a recursor, then $\tii_i$ contains free variables (since 
\trule{WfApp} has a lower priority than \trule{WfBase}, if $\tii_i$ is
closed, it reduces to $\m$ for some $\m$), 
hence 
$\inductiontermsize{G_i\, \tii_i}=\inductiontermsize{G_i}+2$. 
\end{enumerate} 
There is no case such that $G_i$ is a recursor 
and $\tii_i$ is some natural number $\n$ since, if so, we 
can apply \trule{WfBase}. Thus, by (1,2), 
$\inductiontermsize{G_i\, \tii_i}=\inductiontermsize{G_i}+2$. 
Hence we have: 
\[
\begin{array}{lll}
  & \judgementsize{\Gamma \vdash \G_1\equivwf \G_2}\\
= & \omega \cdot 
(\inductionreductionsize{G_1}+\inductionreductionsize{G_2})+
\inductiontermsize{G_1}+\inductiontermsize{G_2}+1\\
< & 
\omega \cdot 
(\inductionreductionsize{G_1}+\inductionreductionsize{G_2})+
\inductiontermsize{G_1}+\inductiontermsize{G_2}+4+1\\
= & \judgementsize{\Gamma \vdash \G_1 \tii_1 \equivwf \G_2 \tii_2}
\end{array}
\] 
as required.
\end{proof}



==> old_fig_size.tex <==
\begin{figure}
\centering
\begin{tabular}{l@{\ }l@{\ }l@{\quad}l}
{\bf Judgements} &  
\ 
$\judgementsize{\Gamma \proves G_1 \equivwf G_2}=
\omega\cdot\reductionsize{G_1}+
\omega\cdot\reductionsize{G_2}+
\termsize{G_1}+\termsize{G_2}+1$\\[1mm]
& \ 
$\judgementsize{\Gamma \proves G_1 \gequivwf G_2}=
\judgementsize{\Gamma \proves G_1 \equivwf G_2}+1$
\\[1mm]
{\bf Types} \\[2mm]
Value \quad& $\termsize{\Bool}={\Nat}=1$, 
             $\termsize{\mar\G}= \termsize{G}+1$\\[1mm]
Global \quad & $\termsize{\GS{\p}{\p'}{\U}.\G}=
   2+\termsize{\U}+\termsize{\G}$,\quad 
  $\termsize{\GB{\p}{\p'}}=2+\Sigma_{k\in K} (1+ \termsize{G_k})$\\[1mm]
& $\termsize{\GM{\xx}{\G}}=\termsize{\G}+1$, \quad 
  $\termsize{\xx}=\termsize{\End}=1$\\[1mm]
&  
%$\termsize{\Pi \AT{\ii}{\II}.\G}=1+\termsize{G}$, \quad   
 $\termsize{\G\APP \tii}=\termsize{G}+1$, \quad 
$\termsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}=
   4+\termsize{G}+\termsize{G'}$\\[1mm]
Local\quad &
  $\termsize{\Lout{\p}{\U}{\T}}=3+\termsize{\U}+\termsize{\T}$, 
  \quad 
  $\termsize{\Lin{\p}{\U}{\T}}=3+\termsize{\U}+\termsize{\T}$\\[1mm] 
  & $\termsize{\Lsel{\p}{\T_k}}= \termsize{\Lbranch{\p}{\T_k}}
     =2+\Sigma_{k\in K}(1+\termsize{T_k})$\\ 
   & $\termsize{\LM{\xx}{\T}} =\termsize{\T}+1$, 
\quad $\termsize{\xx}=\termsize{\End}=1$\\[1mm]
& %$\termsize{\Pi \AT{\ii}{\II}.\T}=1+\termsize{T}$, \quad   
  $\termsize{\T\APP \tii}=\termsize{T}+1$,\quad 
$\termsize{\GR{\T}{\AT{\ii}{\II}}{\xx}{\T'}}=
   4+\termsize{T}+\termsize{T'}$\\[1mm]
Principals & 
$\termsize{\Pi\AT{\ii}{\II}.{U_p}}= 1 + \termsize{U_p}$\\[1mm]
Processes  & 
$\termsize{\emptyset}=0$, 
$\termsize{\Delta,\AT{c}{\T}}=\termsize{\Delta}+\termsize{\T}+1$,
$\termsize{\Pi\AT{\ii}{\II}.\tau}= 1 + \termsize{\tau}$ 
%$\termsize{\tau\APP \tii}= 1 + \termsize{\tau}$ 
\\[1mm]
\end{tabular}\\[2mm]
\caption{Size of types and judgements} \label{fig:size}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{l@{\ }l@{\ }l@{\quad}l}
$\reductionsize{\GS{\p}{\p'}{\U}.\G}=
\reductionsize{\U}+\reductionsize{\G}$,\quad 
   $\reductionsize{\GB{\p}{\p'}}=\Sigma_{k\in K}
    \reductionsize{G_k}$\\[1mm]
$\reductionsize{\GM{\ty}{\G}}=\reductionsize{\G}$, \quad 
$\reductionsize{\ty}=\reductionsize{\xx}=\reductionsize{\End}=0$\\[1mm]
%$\reductionsize{\Pi \AT{\ii}{\II}.\G}=\reductionsize{G}$\\[1mm]
$\reductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}=
\reductionsize{G}+\reductionsize{G'}$\\[1mm]
$\reductionsize{G\APP\m}=
\headreductionsize{G \APP \m}+\reductionsize{\WHNF{G \APP \m}}$\\[1mm]
$\reductionsize{G\APP\ii}=\inductionreductionsize{G}$\\[1mm]
%$\inductionreductionsize{\Pi \AT{\ii}{\II}.\G}=\Sigma_{0\leq \tjj\leq \n+1}
% \ (\reductionsize{G\APP \tjj}+1)+1$ \quad ($\II=[0..\n]$)\\[1mm] 
%$\inductionreductionsize{\Pi \AT{\ii}{\II}.\G}=
%\reductionsize{\Pi \AT{\ii}{\II}.\G}$ \quad ($\II=\Nat$)\\[1mm] 
$\inductionreductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}
=\Sigma_{0\leq \tjj\leq \n+1}
\ (\reductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}{\tjj}}+1)+1$ 
\quad ($\II=[0..\n]$)\\[1mm] 
$\inductionreductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}
=\reductionsize{\GR{\G}{\AT{\ii}{\II}}{\xx}{\G'}}$ 
\quad ($\II=\Nat$)\\[1mm]
$\headreductionsize{\G}=\nn \quad \text{if}\    \G\redsym^\nn G'\not\redsym$
\end{tabular}\\[2mm]

\caption{Number of reductions} \label{fig:reduction-size}
\end{figure}



==> process_example.tex <==
\subsection{Processes for parameterised multiparty protocols}
\label{subsec:processexample}
\noindent 
We give here the processes corresponding to the interactions described in
\S~\ref{sec:introduction} and \S~\ref{subsec:examples}, then introduce a
parallel implementation of the Fast Fourier Transform algorithm.
There are various ways to implement end-point 
processes from a single global type, and we show one instance for each example
below.

\paragraph{\bf Repetition}
A concrete definition for the protocol (\ref{alice-bob-carol}) in \S~1 
is:
\[
\begin{array}{l}
\Pi n.(\RECSEQ{\End}{i}{\xx}{}\GS{\Alice}{\Bob}{\Nat}.
\GS{\Bob}{\Carol}{\Nat}.\xx \APP n)
\end{array}
\]
Then $\Alice$ and $\Bob$ 
can be implemented
with recursors as follows (we abbreviate 
\Alice~by $\participant{a}$, \Bob~by $\participant{b}$ and 
\Carol~by $\participant{c}$). 
\[
\begin{array}{lll}
\Alice(\nn) = \sr{a}{\participant{a},\participant{b},\participant{c}}
\y(\RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\participant{b},\e[i]}}\X\APP n)\\[1mm]
\Bob(\nn) = \ssa{a}{\participant{b}}
\y(\RECSEQP{\inact}{\ii}{\X}{\inpS{y}{\participant{a},z}\outS{\y}{\participant{c},\z}}\X\APP
n)\\[1mm]
\Carol(\nn) = \ssa{a}{\participant{c}}
\y(\RECSEQP{\inact}{\ii}{\X}{\inpS{\y}{\participant{b},z}}\X\APP n)
\end{array}
\]
% %% \[
% %% \begin{array}{lll}
% %% \Alice(\nn) = \sr{a}{\Alice,\Bob,\Carol}
% %% \y(\RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\e[i]}}\X\APP n)\\[1mm]
% %% \Bob(\nn) = \ssa{a}{\Bob}
% %% \y(\RECSEQP{\inact}{\ii}{\X}{\inpS{y}{z}\outS{\y}\z}\X\APP n)\\[1mm]
% %% \end{array}
% %% \]
% We omit $\Carol$, which is also implemented using a recursor.
$\Alice$ repeatedly sends a message $e[i]$ to $\Bob$ $n$-times.
Then $\nn$ can be bound by $\lambda$-abstraction, allowing 
the user to dynamically assign the number of the repetitions.  
\begin{center}
{\small
$
\begin{array}{l}
\lambda \nn.(\nuc{\Ia}{(\Alice(\nn) \pc \Bob(\nn) \pc
\Carol(\nn))}) \ 1000
\end{array}
$}
\end{center}
%%\noindent We give process representations for parametric protocols.
\paragraph{\bf Sequence from \S~\ref{sec:introduction} (\ref{ex:sequence})}
%Ring topology - figure~\ref{fig:examples}(a)}
%This topology features three distinct participant roles (when $n\!\geq 2$).
% because of the inia
% workers $\W[\nn]$ and $\W[0]$. The rest of the workers first
% receive a value and then send a value to the next worker. 
The process below generates all participants using a recursor:
%
{\small
\[
\begin{array}{llrlll}
\Pi \nn.(\Pifthenelse{\nn=0 & }{ & \inact & \\
& }{ &(\mathbf{R} &
(\sr{a}{\W[\nn],..,\W[0]}{y}{\outS{\y}{\W[\nn-1],v}\inact}
\\[1mm]
& & & \pc \ssa{a}{\W[0]}{y}{\inpS{y}{\W[1],z}{\inact}})\\[1mm]
& & & \lambda {\ii}.\lambda{\X}.(
\ssa{a}{\W[\ii+1]}{y}{\inpS{y}{\W[\ii+2],z}\outS{\y}{\W[\ii],z}\inact \pc X}) {\quad \nn-1})}
\end{array}
\]}
\noindent When $n=0$ no message is exchanged. In the other case, the recursor
creates the $n-1$ workers through the main loop and finishes by spawning the initial and final ones.

As an illustration of the semantics, we show the reduction of the above process
for $n=2$. After several applications of the [SuccR] and [ZeroR] rules, we have:
{\small
\[
\begin{array}{l}
\sr{a}{\W[2],\W[1],\W[0]}{y}{\outS{\y}{\W[1],v}}\inact \pc
\ssa{a}{\W[0]}{y}{\inpS{y}{\W[1],z}}\inact \pc
\ssa{a}{\W[1]}{y}{\inpS{y}{\W[2],z}\outS{\y}{\W[0],z}}\inact
\end{array}
\]
} which, with [Init], [Join], [Send], [Recv], gives:
%(the $\inact$ process is omitted):
{\small
\[
\begin{array}{ll}
\red{}{} &(\nu \s)(s : \qbot \pc \outS{\si\s {\W[2]}}{\W[1],v}\inact \pc \sj{\Ia}{\W[1]}{\s}\pc \sj{\Ia}{\W[0]}{\s}\pc \\
 & \qquad
\ssa{a}{\W[0]}{y}{\inpS{y}{\W[1],z}}\inact \pc \ssa{a}{\W[1]}{y}{\inpS{y}{\W[2],z}\outS{\y}{\W[0],z}}\inact)\\
\red{}{} & (\nu \s)(s : \qbot \pc \outS{\si\s {\W[2]}}{\W[1],v}\inact \pc \sj{\Ia}{\W[1]}{\s}\pc\\
 &  \qquad %\sj{\Ia}{\W[0]}{\s}\pc 
\inpS{\si\s {\W[0]}}{\W[1],z}\inact \pc
\ssa{a}{\W[1]}{y}{\inpS{y}{\W[2],z}\outS{\y}{\W[0],z}}\inact)\\
\red{}{}^* & (\nu \s)(s : \qbot \pc \outS{\si\s {\W[2]}}{\W[1],v}\inact \pc %\sj{\Ia}{\W[1]}{\s}\pc \sj{\Ia}{\W[0]}{\s}\pc 
\inpS{\si\s {\W[0]}}{\W[1],z}\inact \pc
\inpS{\si\s {\W[1]}}{\W[2],z}\outS{\si\s {\W[1]}}{\W[0],z}\inact)\\
\red{}{}^* &
(\nu \s)(s :  \qbot \pc \inpS{\si\s {\W[0]}}{\W[1],z}\inact \pc
\outS{\si\s {\W[1]}}{\W[0],v}\inact) \\
\red{}{}^* & \equiv \inact
\end{array}
\]
}


% {\small
% \[
% \begin{array}{lllll}
% \mathbf{R} &
% (\sr{a}{\W[\nn]..\W[0]}{y}{\outS{\y}{\W[\nn-1],v}\inpS{y}{\W[0],z}P}
% \ | \ 
% \ssa{a}{\W[0]}{y}{\inpS{y}{\W[1],z}{\outS{\y}{\W[\nn],z}Q}})\\[1mm]
% & \quad \lambda {\ii}.\lambda{\X}.(
% \Pifthenelse{i\not = 0}%
% {\ssa{a}{\W[\ii]}{y}{\inpS{y}{\W[\ii-1],z}\outS{\y}{\W[\ii+1],z}}{}}%
% {\inact}{\pc X}) {\quad \nn} 
% \end{array}
% \]
% }
% Note that $\nn\geq 1$ can be ensured by typing.

% \paragraph{Tree topology - figure~\ref{fig:examples}(c)}
% There are the three roles represented in this protocol --
% the root, the nodes and the leaves. We give a process for each of them:
% {\small 
% \[
% \begin{array}{rcl}
% P_{\text{root}} & = & \sr{a}{\W[0][0]..\W[\n][\n]}{y}{\inpS{\y}{\x_1}\inpS{y}{\x_2}{\PP}}\\[1mm]
% P_{\text{node}[i][j]} & = & \ssa{a}{\W[i][j]}{y}{\inpS{\y}{\x_1}\inpS{\y}{\x_2}\outS{y}{\x_1+\x_2}{\inact}}\\[1mm]
% P_{\text{leaf}[j]} & = & \ssa{a}{\W[\n][j]}{y}{\outS{\y}{\z_j}{\inact}}\\[1mm]
% \end{array}
% \]
% } %
% where we omit the participant annotations from sending and receiving. Here the
% processes compute the sum of a number of values that are known to the leaves. A
% process $\PP$ is left abstract to represent the root's actions using this sum.
% We can generate all the processes using a recursor in a similar way to the
% previous example.

\paragraph{\bf Ring - Figure \ref{fig:examples}(a)}
The process that generates all the
roles using a recursor is as follows:
{\small
\[
\begin{array}{lllll}
\Pi \nn.(\mathbf{R} &
\sr{a}{\W[0], ..., \W[\nn]}{y}{\outS{\y}{\W[1],v}\inpS{y}{\W[\nn],z}P}\\[1mm]
& \ssa{a}{\W[\nn]}{y}{\inpS{y}{\W[\nn-1],z}{\outS{\y}{\W[0],z}Q}}\\[1mm]
& \quad \lambda {\ii}.\lambda{\X}.(
\ssa{a}{\W[\ii+1]}{y}{\inpS{y}{\W[\ii],z}\outS{\y}{\W[\ii+2],z} \pc X}) {\quad \nn-1} )
\end{array}
\]
}
We take the range of $\nn$ to be $\nn\geq 2$.


\paragraph{\bf Mesh - Figure~\ref{fig:examples} (c)}
In this example, 
% The mesh example is more complex:
when \n~and \m~are bigger than $2$, there are
9 distinct patterns of communication.  

We write below these processes. We assume the existence of a function
$f(z_1,z_2,i,j)$ which computes from $z_1$ and $z_2$ the value to be transmitted
to $\W[\ii][\jj]$. We then designates the processes based on their position in
the mesh. The initiator $\W[\nn][\mm]$ is in the top-left corner of the mesh and
is implemented by $\PP_{\text{top-left}}$. The workers that are living in the
other corners are implemented by $\PP_{\text{top-right}}$ for $\W[\nn][0]$,
$\PP_{\text{bottom-left}}$ for $\W[0][\mm]$ and $\PP_{\text{bottom-right}}$ for
the final worker $\W[0][0]$. The processes $\PP_{\text{top}}$,
$\PP_{\text{left}}$, $\PP_{\text{bottom}}$ and $\PP_{\text{right}}$ respectively
implement the workers from the top row, the leftmost column, the bottom row and
the rightmost column. The workers that are in the central part of the mesh are
played by the $\PP_{\text{center}}(\ii, \jj)$ processes.\\[2mm]
% $\PP_{\text{start}}$ corresponds to the top-left
% worker $\W[\nn][\mm]$ who initiates the protocol.
% The process that implements a parameterised mesh communication pattern is
% defined as follows. The processes having as second name  
% ``middle" define the elements in the middle of rows and columns, which
% place is defined  by the first name.
% For example,  the centre workers $\W[i][j]$ ($0\!<\! i\!<\!n$,
%  $0\!<\! j\!<\!m$) who are connected in all four directions, 
% the initiator $\W[n][m]$ from the top-left corner, and 
% the workers $\W[0][j]$ ($1\!<\! j\!<\!m$) from the middle of the
% bottom row. Below, $f(i,j)$ represents the
% expression computed at the $(i,j)$-th element.  \\
{\small
$\begin{array}{ll}
\PP_{\text{top-left}}(z_1,z_2,\nn, \mm)  & =  \sr{a}{\W[\nn][\mm], ..., \W[0][0]}{y}{
\outS{y}{\W[n-1][m], f(z_1,z_2,n-1,m)}}\\
 & ~~~\outS{y}{\W[n][m-1], f(z_1,z_2,n,m-1)}{\inact}\\[1mm]
\PP_{\text{top-right}}(z_2,\nn) & = \ssa{a}{\W[n][0]}{y}{\inpS{y}{\W[n][1], z_1}\outS{y}{\W[n-1][0], f(z_1,z_2,n-1,0)}\inact}\\[1mm]
\PP_{\text{bottom-left}}(z_1,\mm) & =  \ssa{a}{\W[0][m]}{y}{\inpS{y}{\W[1][m], z_2}\outS{y}{\W[0][m-1], f(z_1,z_2,0,m-1)}\inact}\\[1mm]
\PP_{\text{bottom-right}}(\mm) & =   \ssa{a}{\W[0][0]}{y}{\inpS{y}{\W[1][0], z_1}\inpS{y}{\participant{\W[0][1]}, z_2}\inact}\\[1mm]
\PP_{\text{top}}(z_2,\nn, \kk) & = 
\ssa{a}{\W[n][k+1]}{y}{\inpS{y}{\W[n][k+2], z_1}}\\
 & ~~~ \outS{y}{\W[n-1][k+1], f(z_1,z_2,n-1,k+1)}\outS{y}{{\W[n][k]}, f(z_1,z_2,n,k)}\inact\\[1mm] 
\PP_{\text{bottom}}(\kk) & = \ssa{a}{\W[0][k+1]}{y}{\inpS{y}{\W[1][k+1], z_1}\inpS{y}{\W[0][k+2], z_2}}\\
& ~~~ \outS{y}{\W[0][k], f(z_1,z_2,0,k)}\inact\\[1mm]
\PP_{\text{left}}(z_1,\mm, \ii) & = \ssa{a}{\W[i+1][m]}{y}{\inpS{y}{{\W[i+2][m]}, z_2}\outS{y}{{\W[i][m]}, f(z_1,z_2,i,m)}}\\
& ~~~ \outS{y}{{\W[i+1][m-1]}, f(z_1,z_2,i+1,m-1)}\\[1mm] 
\PP_{\text{right}}(\ii) & =  \ssa{a}{\W[i+1][0]}{y}{\inpS{y}{{\W[i+2][0]}, z_1}\inpS{y}{{\W[i+1][1]}, z_2}}\\
& ~~~ \outS{y}{{\W[i][0]}, f(z_1,z_2,i,0)}\inact\\[1mm]
\PP_{\text{center}}(\ii, \jj) & = \ssa{a}{\W[i+1][j+1]}{y}{\inpS{\y}{\W[i+2][j+1], z_1} \inpS{\y}{\W[i+1][j+2], z_2}}\\
 &~~~ \outS{y}{\W[i][j+1], f(z_1,z_2,i,j+1)}\outS{y}{\W[i+1][j], f(z_1,z_2,i+1,j)}\inact\\[1mm]
\end{array}$
}

The complete implementation can be generated using the following process:

{\small
\[
\begin{array}{l}
\Pi \nn.\Pi \mm.(\mathbf{R} ~(\mathbf{R}~ 
\PP_{\text{top-left}}(z_1,z_2,\nn, \mm) | \PP_{\text{bottom-right}}(\mm)  | \PP_{\text{top-right}}(z_2,\nn)  | \PP_{\text{bottom-left}}(z_1,\mm))\\
\qquad\qquad\qquad \lambda \kk.\lambda Z.(\PP_{\text{top}}(z_2,\nn, \kk) | \PP_{\text{bottom}}(\kk) | Z)\\
\qquad\qquad\quad m-1)\\
\qquad\qquad~~\lambda \ii.\lambda \X. (\mathbf{R}~ \PP_{\text{left}}(z_1,\mm, \ii) | \PP_{\text{right}}(\ii) | \X \\[1mm]
\qquad\qquad\qquad\qquad~~  \lambda \jj.\lambda \Y.(\PP_{\text{center}}(\ii, \jj) | \Y)\\
\qquad\qquad\qquad\qquad \mm-1)\\
\qquad\qquad \nn-1)\\
\end{array}
\]
}


%% {\small
%% \[
%% \begin{array}{l@{\;}c@{\;}l}
%% P_{\text{centre}}(i,j) & = & \ssa{a}{\W[i][j]}{y}{\inpS{\y}{\W[i+1][j], z_1}
%% \inpS{\y}{\W[i][j+1], z_2}}\\
%% &&  \qquad\qquad\quad~ \outS{y}{\W[i-1][j], f(i-1,j)}
%% \outS{y}{\W[i][j-1], f(i,j-1)}\inact \\[1mm]
%% P_{\text{start}}(n,m) & = & \sr{a}{\W[0][0]..\W[n][m]}{y}
%% {\outS{y}{\W[n-1][m], f(n-1,m)}} %\\
%% % &&  \qquad\qquad\quad~ 
%% % \outS{y}{\W[n][m-1], f(n,m-1)}\inact}\\[1mm]
%% % P_{\text{bot\_middle}}(n,m) & = & \ssa{a}{\W[0][j]}{y}
%% % {\inpS{y}{\W[1][j], x}{\inpS{y}{\W[0][j+1], z}
%% % \outS{y}{\W[0][j-1], f(0,j)}\inact}}\\[1mm]
%% %P_{RTC} & = & \ssa{a}{\W[3][0]}{y}{\inpS{y}{\W[3][1], z}\\
%% %& & \qquad\qquad\quad~~\outS{y}{\W[2][0], e(2,0)}\inact}\\[1mm]
%% %P_{LBC} & = & \ssa{a}{\W[0][3]}{y}{\inpS{y}{\W[1][3], z}\\
%% %& & \qquad\qquad\quad~~\outS{y}{\W[0][2], e(0,2)}\inact}\\[1mm]
%% %P_{RBC} & = & \ssa{a}{\W[0][0]}{y}{\inpS{y}{\W[1][0], z_1}\\
%% %& & \qquad\qquad\quad~~\inpS{y}{\participant{\W[0][1]}, z_2}\inact}\\[1mm]
%% %P_{TR[2..1]} & = & \ssa{a}{\W[3][j]}{y}{\inpS{y}{\participant{\W[3][j+1]}, z_1}\\
%% %& & \qquad\qquad\quad~\outS{y}{\participant{\W[2][j]}, e(2,j)}}\\
%% %& & \qquad\qquad\quad~\outS{y}{\participant{\W[3][j-1]}, e(3,j-1)}\inact\\[1mm]
%% %P_{\text{bottom}}(j) & = & \ssa{a}{\W[0][j]}{y}{\inpS{y}{\W[1][j], z_1}\inpS{y}{\W[0][j+1], z_2}}\\
%% %& & \qquad\qquad\quad~\outS{y}{\W[0][j-1], e(0,j-1)}\inact\\[1mm]
%% %P_{\text{bottom}}(j) & = & \ssa{a}{\W[0][j]}{y}{\inpS{y}{\W[1][j], z_1}\inpS{y}{\W[0][j+1], z_2}}\\
%% %& & \qquad\qquad\quad~\outS{y}{\W[0][j-1], f(0,j-1)}\inact\\[1mm]
%% %P_{LC[2..1]} & = & \ssa{a}{\W[i][3]}{y}{\inpS{y}{\participant{\W[i+1][3]}, z_1}\\
%% %& & \qquad\qquad\quad~\outS{y}{\participant{\W[i-1][3]}, e(i-1,3)}}\\
%% %& & \qquad\qquad\quad~\outS{y}{\participant{\W[i][2]}, e(i,2)}\inact\\[1mm]
%% %P_{RC[2..1]} & = & \ssa{a}{\W[i][j]}{y}{\inpS{y}{\participant{\W[i+1][0]}, z_1}\\
%% %& & \qquad\qquad\quad~\inpS{y}{\participant{\W[i][1]}, z_2}}\\
%% %& & \qquad\qquad\quad~\outS{y}{\participant{\W[i-1][0]}, e(i-1,0)}\inact\\[1mm]
%% \end{array}
%% \]
%% }
%% %  Note that, for the sequence and mesh examples, a parallel version of the
%% % \texttt{foreach} would be ideal to help the programmer spawn all processes.







==> projection_algorithm.tex <==
%\subsection{Role-type Projection.}
\paragraph{Role-type projection}
\label{subsec:roletype}
%
%As an alternative to the type-equality approach introduced in this paper, we 
%%plan to 
%investigated a role-based approach for checking the conformance of processes against global %type specifications. 
\noindent 
%\ny{In the programming method introduced in this paper, 
%each user writes his own local program directly 
%against given a global type or  (or its diagram), 
%and checks its correctness via the type equality
%between its own local type and the generic generator of the global type.} 
As we discussed in the ring example in \S~\ref{subsec:processexample},  
we have also investigated an alternative 
{\em role-based approach}, for checking the
conformance of processes against global type specifications.
Although this method currently works only if all participants are parameterised
and without index multiplication, we can generate role-types for
participants directly without using the type equality, dispensing with
recursors. 
The projection algorithm returns the distinct sets of role-types that are possible for a given global type,
%later used to type-check
which are then used to type-check
the processes. 
Taking the example of the ring topology defined in \S \ref{subsec:typingexample} (figure~4a), one set of role-types generated by the projection has 
%Starter ($\W[n]$), Middle and Final ($\W[0]$) workers:\\
the following:
\[\begin{array}{rcl}
\text{Starter}& \triangleq & \Lout{\W[n-1]}{\Nat}{\Lin{\W[0]}{\Nat}}{\End}@\W[n],\\
\text{Middle}& \triangleq & \Lin{\W[i+1]}{\Nat}{\Lout{\W[i-1]}{\Nat}}{\End}@\W[i], \\
\text{Final}& \triangleq & \Lin{\W[1]}{\Nat}{\Lout{\W[n]}{\Nat}}{\End}@\W[0], \\
\end{array}
\]
where $1 \leq i \leq n-1$ and $T@\W[\tii]$ denotes role-type $T$ assigned to participant \W[\tii]. The projection algorithm also returns an (in)equality on $n$ for which each role-type set is valid, e.g. the above role-types are valid for $n \geq 2$. For $n=1$, the role-types generated are only Starter (which becomes $\W[1]$) and Final.
%where $n$ is instantiated by 1.
%$\Lout{\W[0]}{\Nat}{\Lin{\W[0]}{\Nat}}{\End}@\W[1]$, Master instantiated for $n=1$, and $\Lin{\W[1]}{\Nat}{\Lout{\W[1]}{\Nat}}{\End}@\W[0]$, LastWorker instantiated for $n=1$.
For $n=0$, the single role-type generated is $\Lout{\W[0]}{\Nat}{\Lin{\W[0]}{\Nat}}{\End}@\W[0]$,
%which corresponds to
a different role to the ones defined above. Briefly, this projection algorithm works over 4 stages: calculation of the participant ranges for each reference to $i$-indexed participants, intersection of these ranges, arrangement of actions in a role-type, and concatenation of the role-types for
$i=n$ and $i=0$.
%$i \in \{0, n\}$.
%$i = n, 0$.
For the Middle role of the ring example, the range of $\W[i]$ is [$\W[n-1]..\W[0]$] since $0 \leq i \leq n-1$ from the definition of \textbf{R};
%$i$ ranges between [$n-1..0$]
the intersection of the ranges between $\W[i]$ and $\W[i+1]$, i.e. [$\W[n-1]..\W[1]$], is defined for $n \geq 2$ and denotes the
%non-index
participants that will perform the actions defined for both $\W[i]$ and $\W[i+1]$; the actions $\Linn{\W[i+1]}{\Nat}$ and $\Loutt{\W[i-1]}{\Nat}$ are arranged in this order as determined from the global type;
%to $\Linn{\W[i+1]}{\Nat}{\Loutt{\W[i-1]}{\Nat}}{x}$;
%and the last stage obtains $\End$ by projecting participants [$\W[n-1]..\W[1]$] onto the global type for $i = 0$, substituting it for $\xx$.
and finally $\xx$ is substituted by the case for $i = 0$.
%The projection algorithm return also the role-types for StarterWorker and FinalWorker, and the role-types for $n=1$ and $n=0$.
Similarly for Starter and Final, and the role-types for $n=1$ and $n=0$. 
%(see \cite{fullversion}).

%typing theory to the system presented throughout this paper, we plan to investigate
%The typing strategy proposed in this paper uses a type-equality definition to check the conformance of the behaviour of processes with
%Another alternative of typing evolving communication topologies would be to have a role-based projection of the global types and then typecheck the processes against the role-types that they implement.

%This paragraph describes the algorithm of end-point types generation
%for parameterised-participants in primitive recursive global
%types. The algorithm takes as input a parameterised global type and
%returns a list of pairs, where the first element of a pair is an equality or disequality and the second element is a list of end-point types of all participants. The relation between the first and second element of a pair is a satisfaction relation, where the equality or disequality defines the range of values of the parameter for which the end-point types are valid. We will introduce the algorithm following the example of
%the ring topology presented in Section \ref{subsec:typingexample}:
%
%{\small\begin{align*}
%      \Pi n.(& \RECSEQ{\GS{\W[0]}{\W[n]}{\Nat}.\End\\
%        &\quad }{i}{\xx}{\GS{\W[i+1]}{\W[i]}{\Nat}.\xx}\APP \\
%      &n)
%    \end{align*}
%    }
%
%\noindent For $n=0$, we have $\GS{\W[0]}{\W[n]}{\Nat}.\End \proj \pp$ otherwise for $n \geq 1$:
%
%\begin{enumerate}
%
%\item the algorithm calculates the range of participants for each parameterised-participant indexed by $i$ knowing that $n-1 \geq i \geq 0$; for the ring topology, we have ${\W[n-1]} \geq {\W[i]} \geq {\W[0]}$ and  $\W[n] \geq \W[i+1] \geq  \W[1]$.
%
%\item the algorithm computes the intersection of the ranges for all parameterised-participants to obtain the list of actions a participant will perform. In the ring, the intersection of participants ranges from $\W[1]..\W[n-1]$ and those participants will perform both receiving and sending actions, whilst participant $\W[0]$ will perform only a receive and participant $\W[n]$ will perform only a send. The actions in a list are rearranged to preserve the order specified in the global types. In the ring example, the rearrangement of actions returns the list $\Lin{\W[i+1]}{\Nat}{\Lout{\W[i]}{\Nat}}{}$ for participants $\W[1]..\W[n-1]$. The rearrangement of actions is defined as a total order between the parameterised-participants who perform those actions. The total ordering between parameterised-participants is defined on the mathematical expressions that denote those participants. Depending on the index sign, an order has an increasing or decreasing sense, respectively for negative and positive. To make ordering decidable, we have restricted the definition of it to mathematical expressions without multiplication between indexes. Rearrangement is defined as follows: in the case of a decreasing order, the actions that are defined by smaller parameterised-participants than others are placed before, whilst in the case of increasing order, actions defined by greater parameterised-participant are placed before.
%
%%
%%the algorithm concatenates the actions of the parameterized-participants and then rearranges the elements of the actions list to preserve the order of messages specified in the global type.  The rearrangement of actions in the actions list is defined when a total order can be defined between the participants
%
%%participants that fall in the intersection of the ranges of two or more parameterized-participants will perform all the actions specified by the late ones. The concatenation of these actions is done in a way that preserves the order of messages specified in global types. The ordering of actions is defined for two cases, when all the parameterized participants define ranges that are all increasing or all decreasing. In the case when all ranges are decreasing, the actions that are defined by parameterized-participants with smaller range than the other are placed before, whilst for increasing ranges, actions defined by parameterized-participant of greater ranges are placed before. The intuition that stands in these two rules is that, for participants that will perform all the actions, they will perform as first action the one that is defined by the smallest range in case when the ranges are decreasing or the biggest when the ranges are increasing. In the ring topology the order of actions is arranged to $\Lin{\W[i+1]}{\Nat}{\Lout{\W[i]}{\Nat}}{}$ for participants that perform both actions, $\W[1]..\W[n-1]$, where the ranges of parameterized-participants is decreasing and the action performed by $\W[i]$ is placed before the action performed by $\W[i+1]$.
%
%\item the algorithm eliminates \xx \ from the end-point types by replacing it with the end-point obtained by $\GS{\W[0]}{\W[n]}{\Nat}.\End \proj \pp$.
%
%\end{enumerate}
%
%\noindent The intuition that holds rearrangement in the decreasing order is that the first occurrence of a participant in a global type would appear in the smallest parameterized-participant and as the index decreases then the participant would appear in the position of greater parameterised-participants. A symmetric intuition holds for increasing order. The algorithm assumes that parameterised-participants are one-dimension (\W[\tii]) and that \tii ~is defined without using multiplication between indexes. As future work, we plan to build a projection algorithm for every kind of participant, parameterised or constant, and to extend the strategy of this algorithm for n-dimension parameterised-participant. 


==> proofs.tex <==
\section{Proofs of the lemmas and theorems}

%We study the two main properties of the typing system: one is the
%termination of type-checking and another is type-soundness. The proofs
%require a careful analysis due to the subtle interplay between
%dependent types, recursors, recursive types and branching types.
\subsection{Basic properties}
\label{sec:basic}
%\noindent 
\noindent We prove here a series of consistency lemmas concerning permutations
and weakening
of judgements follow.
They are invariably deduced by induction on the derivations in the
standard manner.  

We use the following additional notations: $\Ga
\subseteq \Ga'$ iff $\AT{u}{S}\in \Ga$ implies $\AT{u}{S}\in \Ga'$ and
similarly for other mappings. In other words, $\Ga \subseteq \Ga'$
means that $\Ga'$ is a permutation of an extension of $\Gamma$.

\begin{LEM} \label{lem:basic}
\begin{enumerate}
\item (Permutation and Weakening)\ 
\label{lem:per}
Suppose $\Ga \subseteq \Ga'$ and $\Ga'\proves \Env$. Then 
$\Gamma \proves \judg$ 
implies
$\Gamma' \proves \judg$.  

\item (Strengthening)\ 
\label{lem:st}
$\Gamma,\AT{u}{U},\Gamma' \proves \judg$ 
and $u\not\in \fv(\Gamma', \judg)\cup \fn(\Gamma', \judg)$. Then $\Gamma,\Gamma' \proves \judg$.
Similarly for other mapping. 

\item (Agreement)
\label{lem:agree}
\begin{enumerate}
\item 
\label{lem:agreeEnv}
$\Gamma \proves J$ implies $\Gamma \proves \Env$. 
\item 
\label{lem:agreeK}
$\Gamma \proves \G \RHD \K$ implies 
$\Gamma \proves \K$. Similarly for other judgements. 

\item 
\label{lem:agreeEq}
$\Gamma \proves \G \equiv \G'$ implies 
$\Gamma \proves G \RHD \K$. Similarly for other judgements. 

\item 
\label{lem:agreeTy}
$\Gamma \proves P \rhd \Ty$ implies $\Gamma \proves \Ty \RHD \K$.
Similarly for other judgements. 
\end{enumerate}
\item (Exchange) 
\label{lem:agreeEx}
\begin{enumerate} 
\item 
\label{lem:ExT}
$\Gamma,\AT{u}{U},\Gamma' \proves \judg$ and $\Gamma \proves U\equiv
U'$. Then $\Gamma,\AT{u}{U'},\Gamma' \proves \judg$. 
Similarly for other mappings. 
\item 
\label{lem:ExI}
$\Gamma,\AT{\ii}{\II},\Gamma' \proves \judg$ and $\Gamma\models
\AT{\ii}{\II}=
\AT{\ii}{\II'}$. Then 
$\Gamma,\AT{\ii}{\II'},\Gamma' \proves \judg$. 

\item 
\label{lem:ExP}
$\Gamma,\PRED,\Gamma' \proves \judg$ and $\Gamma\models
\PRED=\PRED'$. Then 
$\Gamma,\PRED',\Gamma' \proves \judg$. 
\end{enumerate}
\end{enumerate}
\end{LEM}
The next 
lemma will be important in the proof of Subject Reduction.
The following lemma which states that well-typedness is
preserved by substitution of appropriate values for variables, is the
key result underlying Subject Reduction. This also guarantees that 
the substitution for the index which affects to a shared environment and
a type of a term, and the substitution for a process variable are
always well-defined.  

\begin{LEM}[Substitution Lemma]\label{lem:substitution}

\begin{enumerate}
\item \labelx{subs01} 
If ${\Ga,\ptilde{\ii}:\II,\Ga'}\proves {\judg}$ and 
$\Ga\models \n: \II$, then 
${\Ga,(\Ga'\subst{\n}{\ii})}\proves \judg\subst{\n}{\ii}$.
%If \der{\Ga,\ptilde{\ii}:\II,\Ga'}{\PP}{\Ty} and 
%\de\Ga{\n}{\Nat} with $\Ga\models \n: \II$, then 
%\der{\Ga,\Ga'\subst{\n}{\ii}}{\PP\subst{\n}{\ii}}{\Ty\subst{\n}{\ii}}.
\item \labelx{subs02} 
If \der{\Ga,\ptilde{\X}:\ptilde{\D_0}}{\PP}{\Ty} and 
\de\Ga{\ptilde{\QQ}}{\D_0}, then
\der{\Ga}{\PP\subst{\QQ}{\ptilde{X}}}{\Ty}.
\item \label{subs1} 
If \der{\Ga,\ptilde{\x}:\ptilde{\ST}}{\PP}{\D} and \de\Ga{\ptilde{v}}{\ptilde{\ST}}, then
\der{\Ga}{\PP\subst{\ptilde{\va}}{\ptilde{\x}}}{\D}.
\item \labelx{subs2} If
\der{\Ga}{\PP}{\D,\y:\T}, then
\der{\Ga}{\PP\sub{\si\s \pv}{\y}}{\D,\si\s \pv:\T}.
\end{enumerate}
\end{LEM}
Note that 
%shows that, under certain circumstances, a variable can be replaced
%% by an index or a term throughout a judgement, although this
%% 
substitutions may change session types and environments in the index case.
The application of (1) to process judgements is especially useful for the
Subject Reduction Theorem:  
if \der{\Ga,\ptilde{\ii}:\II,\Ga'}{\PP}{\Ty} and 
\der{\Ga}{\n}{\Nat} with $\Ga\models \n: \II$, then 
$\der{\Ga,(\Ga'\subst{\n}{\ii})}{\PP\subst{\n}{\ii}}{\Ty\subst{\n}{\ii}}$. 

%We also use the following lemma for the branching 
%local types whose projections are extended by the mergeability operator  
%$\mergeop$. Below, $\subT$ denotes the standard 
%branching subtyping \cite{GH05,CHY07} 
%(the full definitions can be found in Appendix).   
%%congruwith the 
%%selection rule and its dual branching rules:
%\begin{center}
%{\small
%$
%\begin{array}{llll}
%\begin{prooftree}
%{\forall \ii\in I\subseteq J,\ \Gamma \vdash \T_\ii \subT \T_\ii'}
%\justifies
%{ \Gamma \vdash \LselI{\p}{\T_\ii'}{\ii}{I}\subT  \LselI{\p}{\T_\jj'}{\jj}{J}} \using\using\trule{Sel${}_\subT$}
%\end{prooftree}\\
%%\\
%%\begin{prooftree}
%%{\forall \ii\in J\subseteq I,\ \Gamma \vdash \T_\ii \subT \T_\ii'}
%%\justifies
%%{ \Gamma \vdash \LbranchI{\p}{\T_\ii'}{\ii}{I} \subT \LbranchI{\p}{\T_\jj'}{\jj}{J}} \using\trule{Bra${}_\subT$}
%%\end{prooftree}\\
%\end{array}
%$
%}
%\end{center} 
%%whose typability is extended by mergeability. 


\subsection{Proofs for Propositions, Lemmas and Theorems in the main sections}
\label{app:proofs}

\begin{PROP}[Termination and Confluence]
(restatement of \ref{prop:SNconfluent})
The head relation $\redsym$ on global and end-point types 
(i.e. $\G\redsym \G'$
and $\T\redsym \T'$ for closed types in Figure 2) 
are strong normalising and confluent on well-formed kindings. 
Similarly 
the relation $\redsym$ on global and end-point types 
(i.e. $\G\redsym \G'$
and $\T\redsym \T'$ for open types which reduce under 
recursive prefixes, abstractions and recursors) 
are strong normalising and confluent on well-formed kindings. 
\end{PROP}
\begin{proof}
By strong normalisation of System $\mathcal{T}$ \cite{GirardJY:protyp}. 
For the confluence, we first prove that the relation $\redsym$ 
is locally confluent, i.e. if  $\G\redsym \G_i$ ($i=1,2$) then 
$\G_i\redsym^\ast \G'$. Then we achieve the result
by Newman's Lemma. $\square$
\end{proof}


\begin{PROP}[Termination for Type-Equality Checking]
(cf. \ref{pro:equiv-termination})
Assuming that proving the 
judgements $\Gamma\models \judg$ appearing in type equality derivations 
is decidable 
(e.g.~in $\trule{KProj}$),
then type-equality checking of $\Gamma\proves \alpha \equiv \beta$ 
terminates. 
\end{PROP}

\input{../FIG/fig_size}

\noindent 

To prove termination of the second equality requires 
a careful analysis 
since the premises of the mathematical induction 
rules compare the two types whose sizes are lager 
than those of the conclusions. 
These rules correspond to the contextual congruence.  
The size of the judgements are carefully defined 
using the following four functions 
(figures \ref{fig:size} and \ref{fig:reduction-size}). 
\begin{enumerate}
\item $\termsize{G}$ is the size of (the structure of) $G$ 
\item $\headreductionsize{\G}$ is the number of the head reductions 
from $G$. 
\item $\reductionsize{G}$ is the number of the head reductions 
from $G$ and its subterms. 

\item $\inductionreductionsize{G}$ is the maximum number of 
the head reductions from $G$ and its subterms. 
This  includes the mathematical induction case 
where the dependent applications with variables as the arguments. 
\end{enumerate}

The termination then is proved by the following lemma. 

\begin{LEM}[Size of Equality Judgements]\label{lem:size}
The weight of any premise of a rule is always 
less than the weight of the conclusion. 
\end{LEM}
We argue by induction of the length of reduction 
sequences and the size of terms. This is obvious for 
the rules in figure \ref{fig:type-wf-context}. 
The rule \trule{WfBase} is by definition. 
Other rules use the definition of $\mu^\star$ directly. 


\begin{LEM}[Soundness of mergeability]
(restatement of \ref{lem:mergeability})
Suppose $G_1\proj{\p} \mergeop G_2\proj{\p}$ and 
$\Gamma \proves G_i$. Then there exists $G$ such that 
$G\proj{\p}=\sqcap \{T\ | \ T \subT G_i\proj{\p} \ (i=1,2)\}$
where $\sqcap$ denotes the maximum element with respect to $\subT$. 
\end{LEM}
\begin{proof}
The only interesting case is $G_1\proj{\p}$ and $G_2\proj{\p}$ take 
a form of the branching type. Suppose 
$G_1 = \TO{\p'}{\p}\colon\! \indexed{l}{{\G'}}{i}{I}$
and 
$G_2 = \TO{\p'}{\p}\colon\! \indexed{l}{{\G''}}{j}{J}$
with $G_1\proj{\p} \mergeop G_2\proj{\p}$. 
Let $\G'_{i}\proj{\p}=T_{i}$ and 
$\G''_{j}\proj{\p}=T_{j}'$. 
Then by the definition of $\mergeop$ in \S~\ref{subsec:endpoint}, 
we have $G_1\proj{\p}=\LbranchI{\p'}{T_{i}}{i}{I}$ 
and
$G_2\proj{\p}=\&\langle\p',\{l_j:T_{j}'\}_{j\in J}\rangle$ 
with 
${\forall i\in (I \cap J). T_i\mergeop T_j' \quad 
\forall i\in (I \setminus J)\cup (J \setminus I).l_i \not = l_j}$. 
By the assumption and inductive hypothesis on $T_i\mergeop T_j'$, 
we can set 
\[
T=\&\langle\p',\{l_k:T''_{k}\}_{k\in K}\rangle
\] 
such that $K=I \cup J$; and (1) if $k\in I \cap J$, then  
$T''_{k}=T_{k}\sqcap T'_{k}$; (2) if $k\in I, k\not\in J$, then  
$T''_{k}=T_{k}$; and (3)
if $k\in J, k\not\in I$, then  
$T''_{k}=T'_{k}$. Set 
$G_{0k}\proj{\p}=T''_k$. Then we can obtain 
\[ 
G=\TO{\p'}{\p}\colon\! \indexed{k}{{\G_{0}}}{k}{K}
\]
which satisfies 
$G\proj{\p}=\sqcap \{T\ | \ T \subT G_i\proj{\p} \ (i=1,2)\}$, 
as desired. 
\end{proof}

\begin{THM}[Subject Congruence and Reduction]
(cf \ref{thm:sr})\mbox{}\\[-3ex]
\begin{itemize}
\item
If $\derqq\Ga{}\PP\D$ and $\PP\equiv{\PP'}$, then
\derqq\Ga{}{\PP'}{\D}. 
\item 
If \derqq\Ga{}\PP\Ty\ and \redM\PP{\PP'}, then
\derqq\Ga{}{\PP'}{\Ty'}\ for some $\Ty'$ such that
$\seredstar\Ty\Ty'$.
\end{itemize}
\end{THM}
\begin{proof} 
  We only list the crucial cases of the proof of subject reduction: the recursor
  (where mathematical induction is required) and the initialisation. Our proof
  works by induction on the length of the derivation \redM\PP{\PP'}. The base
  case is trivial. We then proceed by a case analysis on the reduction
  \red\PP{\PP'}. We omit the hat from principal values for readability.
% The most interesting case 
% is the recursor where we use
% mathematical induction in addition to induction on the derivation. 
% Also the initialisation uses the mergeability lemma. 
%We omit 
%$\Sigma$ from the turnstile since it is fixed for these cases. 
%The session initialisation uses the property of the subtyping 
%for the mergeability. 
%\\[1mm]
%{\bf Case Beta:}  Suppose 
%$\derqq\Ga{}{(\lambda \ii.\PP)\n}{\Ty}$  
%and $\red{(\lambda \ii.\PP)\n}{\PP\subst{\n}{\ii}}$. 
%Then there exists $\Ty'$ such that 
%$\derqq\Ga{}{\lambda \ii.\PP}{\Pi\AT{\ii}{\II}.\Ty'}$ 
%and $\Ty \equiv (\Pi\AT{\ii}{\II}.\Ty') \n \equiv \Ty'\subst{\n}{\ii}$
%and $\Ga{\models}{n: \II}$. The first judgement must have been 
%derived with \trule{TApp}, thus we have the derivations such that 
%$\Gamma, \AT{\ii}{\II}\vdash \PP\rhd \Ty'$. By applying the
%Substitution Lemma (Lemma \ref{lem:substitution} (\ref{subs01})), we obtain
%$\Gamma\vdash \PP\subst{\n}{\ii}\rhd \Ty'\subst{\n}{\ii}$, 
%as required. 
\\[1mm]
{\bf Case ZeroR:}  Trivial. \\[1mm]
{\bf Case SuccR:}  Suppose 
$\derqq\Ga{}{\GR{P}{\ii}{X}{Q}\APP \n+1}{\tau}$
and 
$\red{\GR{P}{\ii}{X}{Q}\APP \n+1}
{P\sub{\n}{\ii}\sub{\GR{P}{\ii}{X}{Q}\APP \n}{X}}$. 
Then there exists $\Ty'$ such that 
\begin{eqnarray}
& 
\label{eq:rec1}
\Gamma, \ii : \minus{\II},\X:\Ty\sub{\ii}{\jj}  \vdash \QQ  \rhd
  \Ty'\sub{\ii+1}{\jj} \\
& 
\label{eq:rec2}
\derqq\Ga{}{P}{\Ty'\subst{0}{\ii}}\\ 
& 
\label{eq:rec3}
\Gamma\vdash \Pi \AT{\jj}{\II}.\Ty \RHD \Pi\AT{\jj}{\II}.\K
\end{eqnarray}
with 
$\Ty \equiv (\Pi\AT{\ii}{\II}.\Ty') \n+1 \equiv \Ty'\subst{\n+1}{\ii}$
and $\Ga{\models}{\n+1:\II}$. 
By Substitution Lemma (Lemma \ref{lem:substitution} (\ref{subs01})), 
noting $\Ga{\models}{\n: \minus{\II}}$,  
we have: 
$\Gamma, \X:\Ty\sub{\ii}{\jj}\sub{\n}{\ii}  \vdash \QQ\sub{\n}{\ii}  \rhd
  \Ty'\sub{\ii+1}{\jj}\sub{\n}{\ii}$, 
which means that 
\begin{eqnarray}
\label{eq:subs}
\Gamma, \X:\Ty\sub{\n}{\jj}  \vdash \QQ\sub{\n}{\ii}  \rhd
  \Ty'\sub{\n+1}{\jj} 
\end{eqnarray}
Then there are two cases. \\[1mm]
{\em Base Case $\n=0$:} 
By applying Substitution Lemma (Lemma \ref{lem:substitution}
(\ref{subs02})) to  (\ref{eq:subs}) with (\ref{eq:rec2}), we have 
$\Gamma  \vdash \QQ\sub{1}{\ii}\sub{P}{X}  \rhd
  \Ty'\sub{1}{\jj}$.  \\[1mm]
{\em Inductive Case $\n\geq 1$:} 
By the inductive hypothesis on $\n$, 
we assume: 
$\derqq\Ga{}{\GR{P}{\ii}{X}{Q}\APP \n}{\Ty'\sub{\n}{\jj}}$. 
Then by applying Substitution Lemma (Lemma \ref{lem:substitution}) to
(\ref{eq:subs}) with this hypothesis, 
we obtain
$\Gamma\vdash \QQ\sub{\n}{\ii}\sub{\GR{P}{\ii}{X}{Q}\ \n}{X}  \rhd
 \Ty'\sub{\n+1}{\jj}$. \\[1mm]
\\[1mm]
{\bf Case [Init]}
$$
\sr\Ia{\p_0,..,\p_\n}{\y}{\PP}\redsym (\nu \s)(
        \PP\sub{\si\s {\p_0}}{\y} \pc s : \qbot \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
        \sj{\Ia}{\p_\n}{\s})
$$
We assume that
$\derqq{\Ga}{\emptyset}{\sr\Ia{\p_0,..,\p_\n}{\y}{\PP}}{\D}$. Inversion of
\trule{TInit} and \trule{TSub} gives that $\D'\leq\D$ and:
\begin{eqnarray}
& \forall i\neq 0, & \Gamma \proves \p_i\rhd \Nat\label{case-pi}\\
& & \Gamma \vdash \Ia:\mar{\G} \label{case-Ia}\\
& & \Gamma \models \pid(\G)=\{\p_0..\p_\n\} \label{case-pid}\\
& & \Gamma \vdash \PP \rhd \D', \y:\G \proj{\p_0} \label{case-PP}\\
\text{From~(\ref{case-PP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}),}
& & \derqq{\Ga}{}{\PP\sub{\si\s {\p_0}}{\y}}{\D, \si\s {\p_0}:\G \proj{\p_0}} \label{case-sub}\\
\text{\hspace{-3ex}From Lemma~\ref{lem:basic}~(\ref{lem:agreeEnv}) and \trule{QInit},}
& & \derqq{\Ga}{s}{s : \qbot}{\emptyset} \label{case-sbot}\\
\text{From (\ref{case-pi}), (\ref{case-Ia}), (\ref{case-pid}) and
  \trule{TReq},}
& \forall i\neq 0, & \Gamma \vdash \sj{\Ia}{\pp_i}{\s} \rhd \s[\pp_i]:\G \proj{\pp_i} \label{case-sppi}
\end{eqnarray}

% From~(\ref{case-PP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}), we have
% $\derqq{\Ga}{}{\PP\sub{\si\s {\p_0}}{\y}}{\D, \si\s {\p_0}:\G \proj{\p_0}}$ 

% From Lemma~\ref{lem:basic}~(\ref{lem:agreeEnv}) and \trule{QInit}, we
% have $\derqq{\Ga}{s}{s : \qbot}{\emptyset}$.

% From (\ref{case-pi}) and (\ref{case-Ia}) and (\ref{case-pid}), \trule{TJoin}
% gives us $\Gamma \vdash \sj{\Ia}{\pp_i}{\s} \rhd \s[\pp_i]:\G \proj{\pp_i}$ for
% $i$ between $1$ and $n$. 

Then \trule{TPar} on (\ref{case-sub}), (\ref{case-sbot}) and (\ref{case-sppi}) gives:
$$\Gamma \vdash \PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} %
\rhd \D', \s[\pp_0]:\G \proj{\pp_0}, ... , \s[\pp_n]:\G
\proj{\pp_n}
$$
From \trule{GInit} and \trule{GPar}, we have:
$$\Gamma \vdash _ s \PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} \pc s : \qbot%
\rhd \D', \s[\pp_0]:\G \proj{\pp_0}, ... , \s[\pp_n]:\G
\proj{\pp_n}
$$
From Lemma \ref{lem:mergeability} we know that $\coe{(\s[\pp_0]:\G \proj{\pp_0},
  ... , \s[\pp_n]:\G\proj{\pp_n})}{\s}$. We can then use \trule{GSRes} to get:
$$\Gamma \vdash _ \emptyset (\nu \s)(\PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} \pc s : \qbot) \rhd \D'
$$
We conclude from % \trule{GInit}, \trule{GPar}, \trule{GSRes} and 
\trule{TSub}.
\\[1mm]
{\bf Case [Join]} 
$$
\sj{\Ia}{\pp}{\s} \pc \sa\Ia{\pp}{\y}{\PP}\redsym 
        \PP\sub{\si \s {\p}}{\y}
$$
We assume that $\Gamma \vdash _{} \sj{\Ia}{\p}{\s} \pc \sa\Ia{\p}{\y}{\PP}\rhd
\D$. Inversion of \trule{TPar} and \trule{TSub} gives that $\D=\D',\s[\pp]:\T$ and :
\begin{eqnarray}
& & \Gamma \vdash \sj{\Ia}{\pp}{\s} \rhd \s[\pp]:\G \proj{\pp}\label{case-Join-spp}\\
& & \T\geq\G\proj{\pp}\label{case-Join-subt}\\
& & \Gamma \vdash \sa\uu\pp\y\PP \rhd \D'\label{case-Join-PP}\\
\text{By inversion of \trule{TAcc} from~(\ref{case-Join-PP})}
& & \Gamma \vdash \PP \rhd \D', \y:\G \proj{\pp}\label{case-Join-projPP}\\
\text{From~(\ref{case-Join-projPP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}),}
& & \derqq{\Ga}{}{\PP\sub{\si\s {\p}}{\y}}{\D', \si\s {\p}:\G \proj{\p}} \label{case-Join-sub}
\end{eqnarray}

We conclude by \trule{TSub} from (\ref{case-Join-sub}) and (\ref{case-Join-subt}).
% \\[1mm]
% {\bf Case [Branch]} 

% $$\lbranch{\sii}{\q} \Par \qpop{\labheap{l_{i_0
%     }}{\p}{\q}} \redsym \PP_{i_0 } \Par \mqueue{\s}{\queue} \quad (i_0
%   \in I)
% $$
% We assume $\Gamma \vdash _{}\lbranch{\sii}{\q} \Par
% \qpop{\labheap{l_{i_0}}{\p}{\q}}\rhd \D $. Inversion of \trule{TPar} and
% \trule{TSub} gives that $\D=(\D',\s[\pp]:\T_\pp) \Dcomp (\D'',\s[\qq]:\T_\qq)$ and :
% \begin{eqnarray}
% & & \Gamma \vdash \Pbranch{\si\s {\p}}{\q}\rhd \D',\si\s{\p}:\LbranchI{\q}{\T_i}{i}{I}
% \label{case-Branch-bra}\\
% & & \T_\pp\geq\LbranchI{\q}{\T_i}{i}{I}\label{case-Branch-bra-sub}\\
% & & \derq{\Ga}{\qpop{\labheap{l_{i_0}}{\p}{\q}}}{\D'',\siq :\LselI{\p}{\T'_j}{j}{J}}\label{case-Branch-sel}\\
% & & \T_\qq\geq\LselI{\p}{\T'_j}{j}{J}\label{case-Branch-sel-sub}\\
% \text{From \ref{}}
% \end{eqnarray}


% We use Lemma \ref{lem:mergeability} to get the existence of a global type
% $G$ such that $\Gamma \vdash T_i\geq\G \proj{\pp_i}$ and $\coe{(\D,
%   \s[\pp_0]:\T_o, ... , \s[\pp_n]:\T_n)}{\s}$. 



% \mbox{} \\[1mm]
% {\bf Case Link} We omit the hat from principals for a readability. 
% {\small
% \begin{center}
%          $\sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}
%         \pc..\pc\sa\Ia{\p_1}{\y_1}{\PP_1}
%          \redsym (\nu \s)(\PP_{0}\sub{\si\s {\p_0}}{\y_{0}} \pc ...\pc
%         \PP_\n\sub{\si \s {\p_\n}}{\y_\n}\pc s : \emptyset)$.  
% \end{center}
% }
% \noindent Assume
% $\derqq{\Ga}{\Sigma}{
% \sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}\pc
% \sa\Ia{\p_1}{\y_1}{\PP_1}\pc...\pc\sa\Ia{\p_\n}{\y_\n}{\PP_\n}}{\D}$,
% then $\Sigma=\emptyset$ and
% \begin{eqnarray}
% & \der{\Ga}{\sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}}{\D_0'}\\
% & \der{\Ga}{\sr\Ia {\p_i}{\y_i}{\PP_i}}{\D_i'}\quad (1\leq i\leq \n)
% \label{L3}
% \end{eqnarray}
% where $\D =\bigcup_{i=0}^{\n} \D_i$ with $\D_i\geq \D_i'$.
% Then we have, by Lemma \ref{lem:mergeability}, 
% \begin{eqnarray}
% & & \nonumber \de\Ga \Ia{\an \G}\label{L4}\\
% & & \der{\Ga}{\PP_0}{\D_0',\y_0:T_0\quad \quad T_0\subT \pro{\G}{\p_0}\label{L5}}	
% \end{eqnarray}
% and  $\Gamma\proves \pid(G)=\{\p_0,...,\p_\n\}$.
% Next we have, again by Lemma \ref{lem:mergeability},  
% \begin{eqnarray}
% & & \nonumber \de\Ga \Ia{\an \G}\label{L6}\\
% & & \der\Ga{\PP_i}{\D_i',\y_i\ins T_i} \quad \quad T_i \leq \pro{\G}{\p_i} 
% \quad \quad (1\leq i\leq \n). 
% \label{L7}\end{eqnarray}
% Using Substation Lemma (Lemma \ref{lem:substitution} (4)) on (\ref{L5}) and (\ref{L7})
% \begin{eqnarray}
% \derq\Ga{\PP_i\sub{\si\s i}{\y_i}}{\D_i',\si{\s}{i}:T_i} \quad (1\leq
% i\leq n). \label{L8}\end{eqnarray}
% Using \trule{Conc} more times on (\ref{L8}) we have
% \begin{eqnarray}
% \der{\Ga}{\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}}{\bigcup_{i=0}^{\n} (\D_i',\si{\s}{i}:T_i
%         )}.\label{L9}\end{eqnarray}
% Note that
% \begin{eqnarray*}
% \bigcup_{i=0}^{\n} (\D'_i,\si{\s}{i}\ins T_i) \leq \D,\si{\s}{0}\ins\pro{\G}{\p_0},\ldots,\si{\s}{n}\ins\pro{\G}{\p_\n}\end{eqnarray*}
% Using \trule{GInit}, \trule{QInit}, \trule{GPar} and \trule{Subs} on (\ref{L9}) we have
% \begin{eqnarray}
% \derqq{\Ga}{\{\s\}}{\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}\pc s :
% \eq}{\D,\si{\s}{1}\ins\pro{\G}{\p_0},
% \ldots,\si{\s}{\n}\ins\pro{\G}{\p_\n}} \quad \quad \label{L10}
% \end{eqnarray}
% Using \trule{QScope} on (\ref{L10}) we have
% \begin{eqnarray}
% \derqq{\Ga}{\emptyset}{(\nu \s)(\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}\pc s : \eq)}{\D}\label{L11}
% \end{eqnarray}
% since 
% \[
% (\D,\si{\s}{0}\ins\pro{\G}{\p_0},\ldots,\si{\s}{\n}\ins
% \pro{\G}{\p_{\n}})\setminus {\s} = \D. 
% \]
%The proof of the communication rules uses the subtyping relation
%and the Substitution Lemma (\ref{lem:substitution} (\ref{subs1}),
%(\ref{subs2})), together with the subtyping rule for the extended mergeability
%(Lemma \ref{lem:mergeability}).
\end{proof}

The proof of the progress is a corollary from this theorem. 
The detailed definitions (simple and well-linked) can be found in a full version 
of \cite{CHY07}. 


==> protocol.tex <==
\subsection{Web Service} %  Choreography and FFT}
\label{sec:applications}
\noindent 
This section demonstrates the expressiveness of our type theory. We % first
program and type a real-world Web service usecase: Quote Request (C-U-002) is the most complex scenario 
described in \cite{CDLRequirements}, the
public document authored by the W3C Choreography Description Language Working
Group \cite{CDL}. % We then conclude by 
% typing our implementation of the FFT algorithm and prove its correctness. 

%This protocol which includes growing multiparty 
%topologies treats the most complex interactive structure 
%among the CDL requirements.      
%it is  know as challenging to program this specification 
%since it includes dynamically growing global multiparty interactions. 
%We show that 
%the key requirements listed in that document are 
%guaranteed by our dependent type theory, 
%and a group of multiple peers implemented following our global
%dependent type can
%automatically ensuring the type- and communication safety and
%deadlock-freedom. 

% \subsection{Choreography of Interactions in Web Services}
% \label{subsec:cdl}

%This section demonstrates an expressiveness of our type theory
%throughout programming and typing a real world Web services usecase
%(C-U-002 Quote Request, the most complex one in \cite{CDLRequirements}), extracted from the
%public document authored by the W3C Choreography Description Language Working
%Group \cite{CDL}. 
%%This protocol which includes growing multiparty 
%%topologies treats the most complex interactive structure 
%%among the CDL requirements.      
%%it is  know as challenging to program this specification 
%%since it includes dynamically growing global multiparty interactions. 
%%We show that 
%%the key requirements listed in that document are 
%%guaranteed by our dependent type theory, 
%%and a group of multiple peers implemented following our global
%%dependent type can
%%automatically ensuring the type- and communication safety and
%%deadlock-freedom. 

\begin{figure}[ht]
%\centerline{\includegraphics[width=0.3\textwidth]{quote-request2.eps}}
\begin{center}
\begin{tabular}{c}
\xymatrix@C=25pt@R=1pt{
 & *+[F] {\Supp[0]}\ar@{<->}[r]\ar@{<->}[ddr]
 &  *+[F] {\Manu[0]}\ar@{}[r]|\equiv & \txt{\Manu[0][0]} \\
 &  &  \\
  *+[F]{\Buyer} \ar@{<->}[r]\ar@{<->}[uur]\ar@{<->}[ddr]
&  *+[F]{\Supp[1]} \ar@{<->}[ddr]
&  *+[F] {\Manu[1]}\ar@{}[r]|\equiv & \txt{\Manu[0][1]\\ \Manu[2][1]}\\
 &  &   \\
&  *+[F]{\Supp[2]} \ar@{<->}[r]\ar@{<->}[uur]
&  *+[F] {\Manu[2]}\ar@{}[r]|\equiv & \txt{\Manu[1][2]\\ \Manu[2][2]}\\
 & {:} & {:}  \\
}\\
\end{tabular}
\end{center}
\caption{The Quote Request usecase (C-U-002) \cite{CDLRequirements} \label{fig:CDL}}
%\vspace{1mm}
\end{figure}

\paragraph{\bf Quote Request usecase}
The usecase is described below (as published in \cite{CDLRequirements}). 
A buyer interacts with multiple suppliers who in turn
interact with multiple manufacturers in order to obtain quotes for some
goods or services. 
%A concrete example can be a company that
%wishes to purchase a fleet of cars from various automobile suppliers which in
%turn request quotes for specific items and materials from the
%component manufacturers. 
The steps of the interaction are: 
\begin{enumerate}
\item A buyer requests a quote from a set of suppliers.
All suppliers receive the request for quote and send requests
for a bill of material items to their respective manufacturers.

\item 
The suppliers interact with their manufacturers to build their quotes
for the buyer. The eventual quote is sent back to the buyer. 

\item EITHER
\begin{enumerate}
\item The buyer agrees with one or more of the quotes and places the order or orders. OR 
\item The buyer responds to one or more of the quotes by modifying 
and sending them back to the relevant suppliers.
\end{enumerate}
\item EITHER
\begin{enumerate}
\item The suppliers respond to a modified quote 
by agreeing to it and sending a confirmation message back to the buyer. OR

\item The supplier responds by modifying the quote and sending it back
to the buyer and the buyer goes back to STEP 3. OR 

\item 
The supplier responds to the buyer rejecting the modified quote. OR 

\item 
The quotes from the manufacturers need to be renegotiated by the supplier. Go to STEP 2. 
\end{enumerate}
\end{enumerate}
%
%The usecase is depicted in figure~\ref{fig:CDL}. 
%
%\paragraph{Requirements}
The usecase, depicted in figure~\ref{fig:CDL}, may seem simple, 
but it contains many challenges. 
The Requirements 
in Section 3.1.2.2 of \cite{CDLRequirements} include:  
{\bf [R1]} the ability to repeat the same set of interactions 
between different parties using a single definition
%for the interactions, 
and to compose them;
%%and compose them;   
{\bf [R2]} 
the number of participants 
may be bounded at design time or at runtime; and  
{\bf [R3]} 
the ability to {\em reference a global description from within a
global description} to support {\em recursive behaviour} as 
denoted in {\sc Step} 4(b, d).   
%%4b and 4d.
The following works through a parameterised 
global type specification that satisfies these requirements.   
%%Below we list them by replacing  a term ``choreography''
%%by a global specification. 

%\begin{description}
%\item[R1] {\em Needs the ability to repeat the same set of interactions
%and compose them.} 
%The interactions between supplier and manufacturers need only be defined
%once and then repeated for each relevant supplier manufacturer
%pairing. 

%\item[R2]
%{\em Needs participant sets (i.e. the number of participants) 
%that may be bounded at design time or at the runtime.} 
%For instance, the set of suppliers may be
%determined when the global description is designed or when some parameter is
%instantiated dynamically as the interaction progresses. 

%\item[R3] 
%Needs to be able to {\em reference a global description from within a
%global description} to support {\em recursive behaviour} such as a manufacturer
%placing an order with its supplier ({\sc Step} 4(b,d)).   
%\end{description}
%For the first and third points, we propose 
%{\em programming idioms} for repeating and 
%composing types to make a larger type.  The second point 
%is naturally represented by our dependent types. The third point 
%requires a complex combination with recursive and branching types
%with recursors.   

%\paragraph{Programming idioms}
%For {\bf R1}, 
%the first step is defining two simple idioms for 
%merging and repeating global specifications. 
%\[
%\begin{array}{rcll}
%\MERGE{G_1,G_2} & \!\!= \!\!& 
%\GR{\G_2}{\ii}{\xx}{\G_1\sub{\xx}{\End}} \ 1
%\\[1mm]
%\FOREACH{\ii}{[0..\jj]}{G}& \!\!= \!\!&
% \GR{\End}{\AT{\ii}{[0..\jj]}}{\xx}{\G\sub{\xx}{\End}} \ \jj+1
%\end{array}
%\]
%where we assume $\xx\not\in G_1,G$, and $G_1$ and $G$ end 
%with $\End$. In the encodings, $\End$ is replaced by $\xx$. 
%The first composes two 
%global types and the second repeats $G$ $j+1$-times. 

\paragraph{\bf Modular programming using global types}
We develop the specification of the usecase program modularly, 
starting from smaller global types. Here, 
$\texttt{Buyer}$ stands for the buyer, 
$\texttt{Supp}[\ii]$ for a supplier, 
and $\texttt{Manu}[\jj]$ for a manufacturer. Then we alias manufacturers by $\texttt{Manu}[\ii][\jj]$ to identify that $\texttt{Manu}[\jj]$ 
is connected to  $\texttt{Supp}[\ii]$ (so a single $\texttt{Manu}[\jj]$ can have multiple
aliases $\texttt{Manu}[\ii'][\jj]$, see figure~\ref{fig:CDL}). Then, using the idioms presented in \S~1, {\sc Step} 1 
is defined as:
\[ 
\begin{array}{lll}
\G_1 = 
\FOREACH{\ii}{\II}{
\GS{\texttt{Buyer}}{\texttt{Supp}[\ii]}{\mathsf{Quote}}.\End}
\end{array}
\]
For {\sc Step} 2, we compose a nested loop and the subsequent action
within the main loop ($J_i$ gives all $\texttt{Manu}[\jj]$ connected
to $\texttt{Supp}[\ii]$):  
{\small
\[ 
\begin{array}{ll}
\multicolumn{2}{l}{G_2 = \mathtt{foreach}({\ii}:{\II})\{
\MERGE{G_2[i],\
\GS{\texttt{Supp}[i]}{\texttt{Buyer}}{\mathsf{Quote}}.\End}\}} \\[1mm]
%\end{array}
%\]
%%\[
%%\begin{array}{ll}
%%G_2[i]=\\[1mm]
%%\mathtt{foreach}({\jj}:{J_i})\{&
%%\GS{\texttt{Supp}[\ii]}{\texttt{Manu}[\ii][\jj]}{\mathsf{Item}}.\\
%%&\GS{\texttt{Manu}[\ii][\jj]}{\texttt{Supp}[\ii]}{\mathsf{Quote}}.\End\}
%%\end{array}
%%\]
%\[
%\begin{array}{ll}
G_2[i]= \mathtt{foreach}({\jj}:{J_i})\{ & 
\GS{\texttt{Supp}[\ii]}{\texttt{Manu}[\ii][\jj]}{\mathsf{Item}}.\\
& \GS{\texttt{Manu}[\ii][\jj]}{\texttt{Supp}[\ii]}{\mathsf{Quote}}.\End\}
\end{array}
\]
}
%\[ 
%\begin{array}{ll}
%G_2 = \mathtt{foreach}({\ii}:{\II})\{\\
%\qquad\qquad \MERGE{G_2[i],\
%\GS{\texttt{Supp}[i]}{\texttt{Buyer}}{\mathsf{Quote}}.\End}\} \\[1mm]
%%\end{array}
%%\]
%%%\[
%%%\begin{array}{ll}
%%%G_2[i]=\\[1mm]
%%%\mathtt{foreach}({\jj}:{J_i})\{&
%%%\GS{\texttt{Supp}[\ii]}{\texttt{Manu}[\ii][\jj]}{\mathsf{Item}}.\\
%%%&\GS{\texttt{Manu}[\ii][\jj]}{\texttt{Supp}[\ii]}{\mathsf{Quote}}.\End\}
%%%\end{array}
%%%\]
%%\[
%%\begin{array}{ll}
%G_2[i]= \mathtt{foreach}({\jj}:{J_i})\{ \\
%\qquad\qquad \GS{\texttt{Supp}[\ii]}{\texttt{Manu}[\ii][\jj]}{\mathsf{Item}}.\\
%\qquad\qquad \GS{\texttt{Manu}[\ii][\jj]}{\texttt{Supp}[\ii]}{\mathsf{Quote}}.\End\}
%\end{array}
%\]
%
%The G[i] is not quite right because J_i can be discontinuous (according to the Usecase spec.), but foreach assumes continuous.
%

\noindent
$G_2[i]$ represents the second loop between the $i$-th supplier and its
manufacturers.  
Regarding {\sc Step} 3,  
the specification involves buyer preference for certain suppliers.  
%with respect to the received quotes. 
Since this can be encoded using dependent types 
(like the encoding of $\mathsf{if}$),
%in the case of $I$ and $J$ range over finite numbers,  
%or by naturally extending the dependent types
%for values of {\sf Quote}. 
we omit this part and assume 
the preference is given by the (reverse) ordering of $\II$ in order to focus on the
description of the
interaction structure.
%\[
%\begin{array}{llll}
%G_3 =
%\GR{\ \ty\ }{i}{\yy}{}\\
%\quad \TO{\texttt{Buyer}}{\texttt{Supp}[i]}.\\
%\quad \{ \mathsf{ok}: \End\\
%\quad  \mathsf{modify}: 
%\GS{\texttt{Buyer}}{\texttt{Supp}[i]}{\mathsf{Quote}}\\
%\ \quad \ \quad \  \ \
%\begin{array}{ll}
%\TO{\texttt{Supp}[i]}{\texttt{Buyer}}\\
%\\ 
%\\
%\end{array}
%\begin{array}{ll}
%\{
%\mathsf{ok}: & \End \\
%\mathsf{retryStep3}: & \yy\\
%\mathsf{reject}: & \End\}\}\ \ii
%\end{array}
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \ 
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\ \ \quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \mathsf{reject}:\End\}
%\end{array}
%\]
\[
\begin{array}{rcl}
G_3 & = & \GR{\ \ty\ }{i}{\yy}{} \TO{\texttt{Buyer}}{\texttt{Supp}[i]} : \{ \\
& & \quad \begin{array}{llll}
\mathsf{ok}: & \End \\
\mathsf{modify}: & \multicolumn{3}{l}{\GS{\texttt{Buyer}}{\texttt{Supp}[i]}{\mathsf{Quote}}} \\
& \TO{\texttt{Supp}[i]}{\texttt{Buyer}}: \{
&  \mathsf{ok}: & \End \\
&& \mathsf{retryStep3}: & \yy\\
&&  \mathsf{reject}: & \End\}\}\ \ii
\end{array}
\end{array}
\]
In the innermost branch, $\mathsf{ok}$, $\mathsf{retryStep3}$ and 
$\mathsf{reject}$ correspond to {\sc Step} 4(a), (b) and (c)
respectively. Type variable $\ty$ is for (d). 
We can now compose all these subprotocols together. Taking
%\[ 
$G_{23}\ =\ \GM{\ty}{\MERGE{G_2,\ G_3}}$ 
%\]
%If we wish to repeat it some finite number of times ($m$), we can write 
%\[ 
%G_{23}\ =\ \FOREACH{k}{[0..m]}{\MERGE{G_2,\ G_3}}
%\]
and assuming $\II=[0..i]$, the full global type is 
\[
\lambda i.\lambda \VEC{J}.\MERGE{G_1,G_{23}} 
\]
where we have $i$ suppliers, and $\VEC{J}$ gives the $J_i$ (continuous) index sets of the $\texttt{Manu}[\jj]$s connected with each $\texttt{Supp}[\ii]$. 

\paragraph{End-point types}
We show the end-point type for suppliers, who engage in
the most complex interaction structures among the participants.  
The projections corresponding to 
$G_1$ and $G_2$ are 
straightforward:
%\[
%\begin{array}{lllll}
%G_1\proj{\texttt{Supp}[\n]} 
%=  \Lin{\texttt{Buyer}}{\mathsf{Quote}}{}\\[1mm]
%G_2\proj{\texttt{Supp}[\n]} 
%=\\ 
%\quad \mathtt{foreach}({\jj}:{J_i})\{
%\Lout{\texttt{Manu}[\n][\jj]}{\mathsf{Item}}
%{\Lin{\texttt{Manu}[\n][\jj]}{\mathsf{Quote}}{}\}\\
%\quad\quad {\Lout{\texttt{Buyer}}{\mathsf{Quote}}{}}}
%\end{array}
%\]
\[
\begin{array}{lllll}
G_1\proj{\texttt{Supp}[\n]} = \Linn{\texttt{Buyer}}{\mathsf{Quote}} \\[1mm]
G_2\proj{\texttt{Supp}[\n]} = \mathtt{foreach}({\jj}:{J_i})\{ \Loutt{\texttt{Manu}[\n][\jj]}{\mathsf{Item}}; \\
\qquad\qquad\qquad\qquad {\Linn{\texttt{Manu}[\n][\jj]}{\mathsf{Quote}}\}; {\Loutt{\texttt{Buyer}}{\mathsf{Quote}}}}
\end{array}
\]
For $G_3\proj{\texttt{Supp}[\n]}$, 
we use the branching injection and 
mergeability theory developed in 
\S~\ref{subsec:endpoint}. 
%
After the relevant application of \trule{TEq}, we can obtain 
the following projection:
%\[
%\begin{array}{llll}
%\&\langle\texttt{Buyer}, 
%\{ \mathsf{ok}: \End\\
%\quad\quad\quad\quad\quad  \mathsf{modify}: 
%\Lin{\texttt{Buyer}}{\mathsf{Quote}}{}\\
%\quad\quad\quad\quad\ \quad \ \quad \  \ \ \quad
%\begin{array}{ll}
%\oplus\langle\texttt{Buyer}
%\\
%\\
%\\
%\end{array}
%\begin{array}{ll}
%\{
%\mathsf{ok}: & \End \\
%\mathsf{retryStep3}: & T\\
%\mathsf{reject}: & \End\}\rangle\\
%\end{array}
%\end{array}
%\]
\[
\begin{array}{l}
\begin{array}{l}
\&\langle\texttt{Buyer}, \{ \\
\\
\\
\\
\\
\end{array}
\begin{array}{ll}
\mathsf{ok}: & \End\\
\mathsf{modify}: & \Lin{\texttt{Buyer}}{\mathsf{Quote}}{} \oplus\langle\texttt{Buyer}, \{ \\
& \begin{array}{ll}
\qquad \mathsf{ok}: & \End \\
\qquad \mathsf{retryStep3}: & T\\
\qquad \mathsf{reject}: & \End\}\rangle\}\rangle\\
\end{array}
\end{array}
\end{array}
\]
where $T$ is a type for the invocation 
from $\texttt{Buyer}$: 
\[
\begin{array}{l}
\IF \ \n\leq i \ \THEN \ \&\langle \texttt{Buyer}, \{ \mathsf{closed}:\End, 
\ \mathsf{retryStep3}:\ty \} \rangle \\ 
\ELSE\IF \ i=\n \ \THEN \ \ty
\end{array}
\]
%
To tell the other suppliers whether the loop is being reiterated 
or if it is finished, 
we can simply insert the following closing notification
$\FOREACH{\jj}{\II\setminus \ii}
{\TO{\texttt{Buyer}}{\texttt{Supp}[j]}:\{\mathsf{close}:\}}
$
before each $\End$, 
and a similar retry notification (with label $\mathsf{retryStep3}$) before $\ty$.
%\[
%\begin{array}{lll}
%\FOREACH{\jj}{\II\setminus \ii}
%{\TO{\texttt{Buyer}}{\texttt{Supp}[j]}:\{\mathsf{close}:\}}\\
%\FOREACH{\jj}{\II\setminus \ii}{
%\TO{\texttt{Buyer}}{\texttt{Supp}[j]}:\{\mathsf{retryStep3	}:\}}
%\end{array}
%\] 
%
Finally, each end-point type is formed by the following composition: 
\[ 
\begin{array}{l}
\MERGE{G_1\proj{\texttt{Supp}[\n]}, 
{\GM{\ty}{\MERGE{G_2\proj{\texttt{Supp}[\n]},\ G_3\proj{\texttt{Supp}[\n]}}}}})
\end{array}
\]
Following this specification, the projections can be implemented in various
end-point languages (such as CDL or BPEL).  
%% We have implemented this usecase \cite{fullversion} (with the number of participants bound at runtime) in SJ \cite{HU07TYPE-SAFE}. 
%see \cite{} for further notes on
%implementation experience.  

%We implemented
%and tested this usecase in SJ (Java with session types
%\cite{HU07TYPE-SAFE})
%\cite{Emmanuel09} where the number of suppliers and 
%manufactures can be specified as the parameters 
%by the user, following the specification. 

%The local code 
%since it can be implemented by 
%different end-point languages \cite{CDL} 
%and a working code is large \cite{Emmanuel09}, see \S~\ref{sec:conclusion}.  
%%We had implemented this usecase in SJ \cite{} where 
%%the end-point code is roughly following this end-point code 
%%and they can be complied taking 
%%the parameters . 



%\quad \mathsf{else} 
%\ \&\ \langle\mathtt{Buyer}, 
%\{\mathsf{closed:}\End, \mathsf{retryStep3}:\yy\}
%\rangle
%) \ \ii
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \ 
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\ \ \quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \mathsf{reject}:\End\}
%Then three end points are merged as the global type.  
%It is kind of $\mathtt{Buyer}$ to let other suppliers if he 
%finishes the interaction with one of the supplier in order to safely 
%close the connection. Hence $G_3$ is modified as follows: 
%\[
%\begin{array}{llll}
%G_{3}' =
%\GR{\End}{i}{\yy}{}\\
%\quad \TO{\texttt{Buyer}}{\texttt{Supp}[i]}.\\
%\quad \{ \mathsf{ok}: \mathit{Closed}\\
%\quad  \mathsf{modify}: 
%\GS{\texttt{Buyer}}{\texttt{Supp}[i]}{\mathsf{Quote}}\\
%\ \quad \ \quad \  \ \
%\begin{array}{ll}
%\TO{\texttt{Supp}[i]}{\texttt{Buyer}}\\
%\\ 
%\\
%\end{array}
%\begin{array}{ll}
%\{
%\mathsf{ok}: & \mathit{Closed} \\
%\mathsf{retryStep3}: & \mathit{Retry};\yy\\
%\mathsf{reject}: & \mathit{Closed}\}\ \ii
%\end{array}
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \ 
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\ \ \quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \mathsf{reject}:\End\}
%\end{array}
%\]
%$\mathit{Closed}$ is a closed protocol 
%defined as: $\mathit{Closed}=
%\FOREACH{\jj}{\II\setminus \ii}{
%\TO{\texttt{Buyer}}{\texttt{Supp}[j]}\{\mathsf{closed}:\}}$. 
%Similarly 
%$\mathit{Retry}=
%\FOREACH{\jj}{\II\setminus \ii}{
%\TO{\texttt{Buyer}}{\texttt{Supp}[j]}\{\mathsf{retryStep3	}:\}}$. 
%Then the end-point type 
%$G_{3}'\proj{\texttt{Supp}[\n]}$ 
%is given as: 
%\[
%\begin{array}{llll}
%\GR{\End}{i}{\yy}{}\\
%\quad \mathsf{if}\ i=\n \ \mathsf{then} \ 
%\&\langle\texttt{Buyer}, \\
%\quad \{ \mathsf{ok}: \End\\
%\quad  \mathsf{modify}: 
%\Lin{\texttt{Buyer}}{\mathsf{Quote}}{}\\
%\ \quad \ \quad \  \ \ \quad
%\begin{array}{ll}
%\oplus\langle\texttt{Buyer}
%\\
%\\
%\\
%\end{array}
%\begin{array}{ll}
%\{
%\mathsf{ok}: & \End \\
%\mathsf{retryStep3}: & \yy\\
%\mathsf{reject}: & \End\}\rangle\\
%\end{array}\\
%\quad \mathsf{else} 
%\ \&\ \langle\mathtt{Buyer}, 
%\{\mathsf{closed:}\End, \mathsf{retryStep3}:\yy\}
%\rangle
%) \ \ii
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \ 
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\ \ \quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \mathsf{reject}:\End\}
%\end{array}
%\]
%Then three end points are merged as the global type.  
%We omit the local code 
%since it can be implemented by 
%different end-point languages \cite{CDL} 
%and a working code is large \cite{Emmanuel09}, see \S~\ref{sec:conclusion}.  
%%We had implemented this usecase in SJ \cite{} where 
%%the end-point code is roughly following this end-point code 
%%and they can be complied taking 
%%the parameters . 

%The main three of four requirements 
%listed in 3.1.2.2 in \cite{CDLRequrements} follow. 

%\begin{enumerate}
%\item 
%The ability to {\em repeat the same set of interactions} is needed. The
%interactions between supplier and manufacturers need only be defined
%once and then repeated for each relevant supplier manufacturer
%pairing.

%\item 
%Needs participant sets that may be bounded at design time, at the
%runtime or not at all. 
%For instance, the set of suppliers may be
%determined when the global description is designed or when it is
%instantiated, or may be completely dynamic.

%\item 
%Needs to be able to reference a global description from within a
%global description to support recursive behaviour such as a manufacturer
%placing an order with its supplier.
%\end{enumerate}
%We do not treat the forth requirement about a transaction recovery.  
%To make clear, we replaced a term ``choreography'' by a global description
%(i.e. global dependent type) in the above requirements, but the rest 
%is the same as in \cite{CDLRequrements}. 
%The second requirement is less clearer but we believe 
%In summary, we illustrate our theory offers:  
%\begin{itemize}
%\item {\em\bf Merging global scenarios:} 
%We can develop a large specification from small pieces 
%of independent specifications using dependent types 
%(cf.~\S~1) ({\bf Part I}).
 
%\item {\em\bf Repeating actions:} 
%We can describe looping and broadcasting 
%easily using the parameterised dependent session types.  

%\item {\em\bf Flexibility by nested recursors:} 
%We can write expressive specifications 
%as nested dependent global types, combining 
%with branching types and recursions with enlarged 
%projectability (cf.~Defition \ref{def:}). 
%\end{itemize}


==> ring_mesh.tex <==
%Author: Andi Bejleri
\section{Ring and mesh communication patterns}
\label{app:ring_mesh}

We present some programming examples of global types 
which make use of typical communication patterns that can be found in classical
parallel algorithms textbooks.

\begin{figure*}[h!]
\centering
\begin{tabular}{c@{}c}
%{\bf \textsf (a) Ring pattern} & {\bf \textsf (b) Mesh pattern} \\
\begin{tabular}{c}
{\bf \textsf (a) Ring pattern}\\[3ex]
\xymatrix@C=15pt{
  *+[F]{\small 0}\ar[r]
  &*+[F]\txt{\small 1}\ar[r]
  &{\ldots}\ar[r]
  &*+[F]\txt{\small \n}\ar@/^1.5pc/[lll]}\\[4ex]
\begin{minipage}{10em}{\small\begin{align*}
      & \Pi n:I.\\
      & \quad (\RECSEQ{\GS{\W[n]}{\W[0]}{U}.\End\\
        &\qquad }{i}{\xx}{\GS{\W[n-i-1]}{\W[n-i]}{U}.\xx}\APP \\
      &n)\\
    \end{align*}}
\end{minipage}\\

\end{tabular}
&
\begin{tabular}{c}
{\bf \textsf (b) Mesh pattern}\\
\xymatrix@C=10pt@R=10pt{
  *[F]{\hole} \ar[r]\ar[d]
  &*[F]{\hole}\ar[r]\ar[d]
  &{\ldots}\ar[r]
  &*[F]{\hole}\ar[d]\\
  *[F]{\hole}\ar[r]\ar[d]
  &*[F]{\hole}\ar[r]\ar[d]
  &{\ldots}\ar[r]
  &*[F]{\hole}\ar[d]\\
  {:}\ar[d]
  &{:}\ar[d]
  &{\ddots}
  &{:}\ar[d]
  \\
  *[F]{\hole}\ar[r]
  &*[F]{\hole}\ar[r]
  &{\ldots}\ar[r]
  &*[F]{\hole}
}\\
\begin{minipage}{10em}{\small\begin{align*}
      &\Pi n.\Pi m. \\
      &\ (\RECSEQ{ \\
    & \quad (\RECSEQ{\End}{k}{\zz}{\GS{\W[0][k+1]}{\W[0][k]}{\Nat}.\zz}\APP m)\\
    & \quad }{i}{\xx}{ \\
      & \qquad (\RECSEQ{(\GS{\W[i+1][0]}{\W[i][0]}{\Nat}.\xx)\\
        & \quad \qquad  }{j}{\yy}{ \\
        & \qquad \qquad  \GS{\W[i+1][j+1]}{\W[i][j+1]}{\Nat}.\\
        & \qquad \qquad  \GS{\W[i+1][j+1]}{\W[i+1][j]}{\Nat}.\yy} \\
      & \qquad \APP m}) \\
    & \quad \APP n) 
   \end{align*}}
\end{minipage}
\end{tabular}

\end{tabular}
\ \\[-3mm]
\label{fig:examples-appendix}
\end{figure*}

\paragraph{Ring} The ring pattern consists of $\n+1$ workers (named by $\W$) that each has exactly
two neighbours: the worker $\W[\ii]$ communicates with the worker $\W[\ii-1]$
and $\W[\ii+1]$ ($1\leq\ii\leq\n-1)$, with the exception of $\W[0]$ and $\W[\n]$
who share a direct link. The non-uniformity of linking between the workers in the ring gives 
three distinct roles: Starter, represented by $\W[0]$, 
Middle, represented by $\W[\ii]$ for $1\leq\ii\leq\n-1$, and  Last, represented by $\W[\n]$. 
The type specifies that the first message is sent by $\W[0]$ to $\W[1]$, and the last one is sent from $\W[\n]$ back 
to $\W[0]$. To ensure the presence of all three roles in the workers of this topology, the parameter domain
is set to $\n \geq 2$. The process that generates all the
roles using a recursor is as follows:

%\subsection{Processes}
%\paragraph{Ring-Figure \ref{fig:examples}(a)}

%\noindent \ensuremath{\text{def}~\tilde{\pp} =  \RECSEQ{\emptyset}{\ii}{\X}{\W[\ii+1], \X} ~\nn-1}\\
{\small
\[
\begin{array}{lllll}
\Pi \nn.(\mathbf{R} &
\sr{a}{\W[0], ..., \W[\nn]}{y}{\outS{\y}{\W[1],v}\inpS{y}{\W[\nn],z}P}\\[1mm]
& \sa{a}{\W[\nn]}{y}{\inpS{y}{\W[\nn-1],z}{\outS{\y}{\W[0],z}Q}}\\[1mm]
& \quad \lambda {\ii}.\lambda{\X}.(
\sa{a}{\W[\ii+1]}{y}{\inpS{y}{\W[\ii],z}\outS{\y}{\W[\ii+2],z} \pc X}) {\quad \nn-1} )
\end{array}
\]
}

\paragraph{Mesh}

The session from figure~\ref{fig:examples}(c) describes communication over a
two dimensional mesh pattern. The participants in the first and last rows and columns, 
except the corners which have two neighbors, have three neighbors. The other participants 
have four neighbors. The roles of the mesh are defined by the communication behavior of each
participant and by the links the participants have with their neighbors. From the figure, it is easy to 
identify the nine roles present in the pattern. %The roles will be discussed in Section~ \ref{subsec:processexample}.
Our session
takes two parameters $n$ and $m$ which represent the number of rows and the
number of columns. Then we have two iterators that repeat
$\GS{\W[\ii+1][\jj+1]}{\W[\ii][\jj+1]}{\Nat}$ and 
$\GS{\W[\ii+1][\jj+1]}{\W[\ii+1][\jj]}{\Nat}$ for all $\ii$ and $\jj$. These two messages
specify the fact that each worker not situated on the last row or last column
sends a message to his neighbors situated below and on its right. The types
$\GS{\W[\ii+1][0]}{\W[\ii][0]}{\Nat}$ and
$\RECSEQ{\End}{k}{\zz}{\GS{\W[0][k+1]}{\W[0][k]}{\Nat}.\zz}\APP m$ deal with, 
respectively, the last column and the last row. %As in the tree example, the
%messages converge towards $\W[0][0]$. 
Variants of this pattern include toric meshes and hypercubes. To ensure the presence of all three roles in the workers of this 
topology, the parameter domain is set to $\n, \m \geq 2$.

%{\small
%\noindent \ensuremath{\begin{array}{l}
%\text{def}~ \tilde{\pp} = \mathbf{R~}(\mathbf{R~}{\emptyset}~{\lambda \kk}.{\lambda Z}.{\W[\nn][\kk]}~ \mm-1)\\[1mm]
%\qquad\qquad~~ \lambda \ii.\lambda \X.\mathbf{R}~ \X\\[1mm]
%\qquad\qquad\qquad\qquad~~ \lambda \jj.\lambda \Y.\W[\ii][\jj], \Y\\[1mm]
%\qquad\qquad\qquad\qquad \mm+1\\
%\qquad\qquad \nn\\
%\end{array}}
%}

The process that implements a parameterised mesh communication pattern is defined as follows. The processes having as second name 
``middle" define the elements in the middle of rows and columns, which place is defined  by the first name.\\

{\small
$\begin{array}{ll}
\PP_{\text{start}}(\nn, \mm)  & =  \sr{a}{\W[\nn][\mm], ..., \W[0][0]}{y}{
\outS{y}{\W[n-1][m], f(n-1,m)}}\\
 & ~~~\outS{y}{\W[n][m-1], f(n,m-1)}{\inact}\\[1mm]
\PP_{\text{top\_right\_corner}}(\nn) & = \sa{a}{\W[n][0]}{y}{\inpS{y}{\W[n][1], z}\outS{y}{\W[n-1][0], f(n-1,0)}\inact}\\[1mm]
\PP_{\text{bottom\_left\_corner}}(\mm) & =  \sa{a}{\W[0][m]}{y}{\inpS{y}{\W[1][m], z}\outS{y}{\W[0][m-1], f(0,m-1)}\inact}\\[1mm]
\PP_{\text{bottom\_right\_corner}}(\mm) & =   \sa{a}{\W[0][0]}{y}{\inpS{y}{\W[1][0], z_1}\inpS{y}{\participant{\W[0][1]}, z_2}\inact}\\[1mm]
\PP_{\text{top\_middle}}(\nn, \kk) & = \sa{a}{\W[n][k+1]}{y}{\inpS{y}{\participant{\W[n][k+2]}, z_1}}\\
 & ~~~ \outS{y}{\participant{\W[n-1][k+1]}, f(n-1,k+1)}\outS{y}{{\W[n][k]}, f(n,k)}\inact\\[1mm] 
\PP_{\text{bottom\_middle}}(\kk) & = \sa{a}{\W[0][k+1]}{y}{\inpS{y}{\W[1][k+1], z_1}\inpS{y}{\W[0][k+2], z_2}}\\
& ~~~ \outS{y}{\W[0][k], f(0,k)}\inact\\[1mm]
\PP_{\text{left\_middle}}(\mm, \ii) & = \sa{a}{\W[i+1][m]}{y}{\inpS{y}{{\W[i+2][m]}, z_1}\outS{y}{{\W[i][m]}, f(i,m)}}\\
& ~~~ \outS{y}{{\W[i+1][m-1]}, f(i+1,m-1)}\\[1mm] 
\PP_{\text{right\_middle}}(\ii) & =  \sa{a}{\W[i+1][0]}{y}{\inpS{y}{{\W[i+2][0]}, z_1}\inpS{y}{{\W[i+1][1]}, z_2}}\\
& ~~~ \outS{y}{{\W[i][0]}, f(i,0)}\inact\\[1mm]
\PP_{\text{center}}(\ii, \jj) & = \sa{a}{\W[i+1][j+1]}{y}{\inpS{\y}{\W[i+2][j+1], z_1} \inpS{\y}{\W[i+1][j+2], z_2}}\\
 &~~~ \outS{y}{\W[i][j+1], f(i,j+1)}\outS{y}{\W[i+1][j], f(i+1,j)}\inact\\[1mm]
\end{array}$
}
\\

{\small
\[
\begin{array}{l}
\Pi \nn.\Pi \mm.(\mathbf{R} ~(\mathbf{R}~ 
\PP_{\text{start}}(\nn, \mm) | \PP_{\text{bottom\_right\_corner}}(\mm)  | \PP_{\text{top\_right\_corner}}(\nn)  | \PP_{\text{bottom\_left\_corner}}(\mm))\\
\qquad\qquad\qquad \lambda \kk.\lambda Z.(\PP_{\text{top\_row}}(\nn, \kk) | \PP_{\text{bottom\_middle}}(\kk) | Z)\\
\qquad\qquad\quad m-1)\\
\qquad\qquad~~\lambda \ii.\lambda \X. (\mathbf{R}~ \PP_{\text{left\_middle}}(\mm, \ii) | \PP_{\text{right\_middle}}(\ii) | \X \\[1mm]
\qquad\qquad\qquad\qquad~~  \lambda \jj.\lambda \Y.(\PP_{\text{center}}(\ii, \jj) | \Y)\\
\qquad\qquad\qquad\qquad \mm-1)\\
\qquad\qquad \nn-1)\\
\end{array}
\]
}

\subsection{Typing}
\paragraph{Ring pattern - figure~\ref{fig:examples}(a)}

The typing of the ring pattern is similar to the one of sequence.
%The highlight of this example is
%a type-equality
%between the general end-point generator and a {\em role-based}
%local type (called {\em role-types}).
%The role-type groups the participants who inhabit
%in the same parameterised protocol as a single role.
%We observe the ring topology consists of the three roles (when $n\geq
%1$): one
%is the starter $\W[n]$ who sends the message first and
%receives the final message from the final worker $\W[0]$,
%and others are the middle workers  who receive a data and
%send back to the next worker. The transformation starts
%from 
The general generator of this pattern is 
{\small
\[
\begin{array}{lll}
   \RECSEQ{(\GS{\W[\nn]}{\W[0]}{\Nat}.\End)\proj \pp\\
   \quad }{i}{\xx}{ \IF\ \pp=\W[\nn-i-1]\ \THEN \ \Lout{\W[\nn-\ii]}{\Nat}\xx\\
  \quad \quad\quad\quad\quad \ \ELSE\IF\ \ \pp=\W[\nn-\ii]\ \THEN \ \Lin{\W[\n-\ii-1]}{\Nat}\xx \\
 \quad \quad\quad\quad\quad\ \ELSE\IF\ \ \xx \ } & n
\end{array}
\]
}

and

%First we note the kinding rules \trule{KRcr} and
%\trule{KApp} ensure $\nn\geq 1$.
%From
%the figure~\ref{fig:examples}(a),
the user would design the end-point type as follows:
{\small\[
\begin{array}{lll}
\IF \ &
\p=\W[0] \ \THEN \ \Lout{\W[1]}{\Nat}{\Lin{\W[n]}{\Nat}{}}\\
\ELSE\IF &
\p=\W[n]  \ \THEN \ \Lin{\W[n-1]}{\Nat}{\Lout{\W[0]}{\Nat}{}}\\
\ELSE\IF & 1 \leq i+1 \leq n-1  \ \mathsf{and}\ \p=\W[\ii+1]\\
& \THEN \  {\Lin{\W[i]}{\Nat}{}}{\Lout{\W[i+2]}{\Nat}{}}
\end{array}
\]}
The first case denotes the protocol of the initiator;
the second one corresponds to the last worker, while
the third one to one of the middle workers.

The type equality is the same as the sequence:
%The type equality is easily 
proved by the case analysis
by the induction of the recursor using the inductive rules in a
version of the end-point types following in 
figure~\ref{fig:type-wf-recursion} (\trule{WfBase,WfLL,WfRecF}), 
combining the $\beta$-reductions 
over two end-point types. 
%Let $T[\p][n]$ for the first original type and $T'[\p][n]$ for the
%second role type. We can check for all $\n\geq 1$ and $\p$, we have:
%\begin{center}
%$(\prod n.T[\p][n] )\n \redsym^\ast T_\n\not\redsym$ iff 
%$(\prod n.T'[\p][n] )\n \redsym^\ast T_\n\not\redsym$. 
%\end{center}
%Hence $\prod n.T[\p][n]\gequivwf \prod n.T'[\p][n]$. 
%For example, when $\p=\W[0]$, then 
%$(\prod n.T[\W[0]][n] )\n \redsym^\ast
%{\Lout{\W[1]}{\Nat}{}}\Lin{\W[\n]}{\Nat}{}$ 
%and 
%$(\prod n.T'[\W[0]][n] )\n \redsym^\ast
%{\Lout{\W[1]}{\Nat}{}}\Lin{\W[\n]}{\Nat}{}$. 
%Similarly for  the case $\p=\W[n]$ and 
%$\p=\W[i+1]$ with $1\leq i+1 \leq n-1$. 
%Note that for all $\n$, the $\beta$-reduction terminates, 
%so that the equality checking terminates. 

From these types, the ring processes are straightforwardly
typable using ${\bf R}$. 
%Recall the implementation of this ring protocol from \S~\ref{subsec:processexample}: 

%{\small
%\[
%\begin{array}{lllll}
%P_{\text{ring}} \ = \ \mathbf{R} &
%\sr{a}{\W[0], \W[\n], \tilde{\pp}}{y}{\outS{\y}{\W[1],v}\inpS{y}{\W[\nn],z}P}\\[1mm]
%& \sa{a}{\W[\nn]}{y}{\inpS{y}{\W[\nn-1],z}{\outS{\y}{\W[0],z}Q}}\\[1mm]
%& \quad \lambda {\ii}.\lambda{\X}.(
%\sa{a}{\W[\ii+1]}{y}{\inpS{y}{\W[\ii],z}\outS{\y}{\W[\ii+2],z} \pc X}) {\quad \nn-1} 
%\end{array}
%\]
%}
%%{\small
%%\[
%%\begin{array}{lllll}
%%P_{\text{ring}} \ = \ 
%%\mathbf{R} &
%%\sr{a}{\W[\nn]..\W[0]}{y}{\outS{\y}{\W[\nn-1],v}\inpS{y}{\W[0],z}P}\\[1mm]
%%& \sa{a}{\W[0]}{y}{\inpS{y}{\W[1],z}{\outS{\y}{\W[\nn],z}Q}}\\[1mm]
%%& \quad \lambda {\ii}.\lambda{\X}.(
%%\ifthenelse{i\not = 0}%
%%{\sa{a}{\W[\ii]}{y}{\inpS{y}{\W[\ii-1],z}\outS{\y}{\W[\ii+1],z}}{}}%
%%{\inact}\\[1mm]
%%& {\quad\quad\quad\quad\quad\quad \pc X}) {\quad \nn} 
%%\end{array}
%%\]
%%}
Let us define: 
\[ 
\begin{array}{lllll}
P_0 & = &  
\sr{a}{\W[0],.., \W[\n]}{y}{\outS{\y}{\W[1],v}\inpS{y}{\W[\nn],z}P}\\[1mm]
P_n & = &  
\sa{a}{\W[\nn]}{y}{\inpS{y}{\W[\nn-1],z}{\outS{\y}{\W[0],z}Q}}\\[1mm]
P_{\ii+1} & = &  
\sa{a}{\W[\ii+1]}{y}{\inpS{y}{\W[\ii],z}\outS{\y}{\W[\ii+2],z}}
& 1 \leq i+1 \leq n-1 \\[1mm]
%P_{\text{body}} & = &  \ifthenelse{i\not = 0}{P_{\ii}}{\inact}
\end{array}
\]
Assume 
\[ 
\emptyset \vdash P \rhd \D_0
\]
By \trule{TOut, TIn}, we have: 
\[ 
a:\mar{\G} \vdash 
\outS{\y}{\W[1],v}\inpS{y}{\W[n],z}P  \rhd \D_n,\y:\G \proj{\p_0}
\]
where $\G \proj{\p_0}$ is obtained from the role type above. 
Hence, by \trule{TInit},  noting $\p_0=\W[0]$,  
\[ 
a:\mar{\G} \vdash P_0 \rhd \D_0
\]
Similarly, using \trule{TAcc}  with $\p_n=\W[n]$,     
we have: 
\[ 
a:\mar{\G} \vdash P_n \rhd \D_n
\]
Hence we have 
\[
a:\mar{\G} \vdash P_0\Par P_n \rhd \D 
\]
with $\D=\D_0,\D_n$. 
Similarly, we can type: 
\[ 
a:\mar{\G}, \ii:\II^-, 1 \leq i+1  \vdash P_{i+1} \rhd \emptyset
\]
with $\II=[0..n-1]$. 
Also we have: 
%\[ 
%a:\mar{\G}  \vdash \inact \rhd \emptyset 
%\]
%and 
\[ 
a:\mar{\G},\ii:\II^-,X:\tau\subst{i}{j}  \vdash X \rhd \tau\subst{i+1}{j} 
\]
where $\tau\subst{i}{j}=\D$ for all $i$. 
Hence by strengthing and \trule{TPar}, we have: 
\[ 
a:\mar{\G},\ii:\II^-,X:\tau\subst{i}{j}  \vdash P_{i+1} | X \rhd \tau\subst{i+1}{j} 
\]
Hence applying \trule{TPRec},  
we can type the ring  process as: 
\[
a:\mar{\G}  \vdash  P_{\text{ring}} \rhd \D 
\]
as required. 
%%We also discuss an algorithm for the automatic 
%%generation of role-types in \S~\ref{subsec:roletype}.

\paragraph{Mesh pattern - figure~\ref{fig:examples}(b)} 
The highlight of this example is
a type-equality
between the general end-point generator and a {\em role-based}
end-point type (called {\em role-types}).
The role-type groups the participants who inhabit
in the same parameterised protocol as a single role. 
We observe the mesh pattern consists of the nine roles (when $n,m\geq
2$). The participants in the first and last rows and columns, 
except the corners which have two neighbors, have three neighbors. The other participants 
have four neighbors. The roles of the mesh are defined by the communication behavior of each
participant and by the links the participants have with their neighbors. The transformation starts 
from the general generator of this topology given below. 

{\small
\[
\begin{array}{lll}
\RECSEQ{  ~~ (\RECSEQ{\End\proj \pp}{k}{\zz}{
    \IF \ \pp=\W[0][k+1]\ \THEN \ \Lout{\W[0][k]}{\Nat}\zz\\
     \qquad\qquad\quad \quad\quad\quad\quad~~ \ \ELSE\IF\ \ \pp=\W[0][k]\ \THEN \ \Lin{\W[0][k+1]}{\Nat}\zz \\
 \qquad\qquad\quad \quad\quad\quad\quad~~\ \ELSE\ \ \zz \ })  m\\
     \quad }{i}{\xx}{ \\
       \qquad (\RECSEQ{~( \IF \ \pp=\W[i+1][0]\ \THEN \ \Lout{\W[i][0]}{\Nat}\xx\\
     \quad \quad\quad\quad \ \ELSE\IF\ \ \pp=\W[i][0]\ \THEN \ \Lin{\W[i+1][0]}{\Nat}\xx \\
 \quad \quad\quad\quad \ \ELSE\ \ \xx \ )\\       
           \quad \qquad  }{j}{\yy}{ \\         
          \qquad \qquad  ~\IF \ \pp=\W[i+1][j+1]\ \THEN \ \Lout{\W[i][j+1]}{\Nat}\\
          \qquad\qquad\qquad \IF \ \pp=\W[i+1][j+1]\ \THEN \ \Lout{\W[i+1][j]}{\Nat} \yy\\
          \qquad\qquad\qquad  \ELSE\IF\ \ \pp=\W[i+1][j]\ \THEN \ \Lin{\W[i+1][j+1]}{\Nat}\yy \\
                    \qquad\qquad\qquad \ELSE\ \yy\\
     \quad \quad\quad\quad \ \ELSE\IF\ \ \pp=\W[i][j+1]\ \THEN \ \Lin{\W[i+1][j+1]}{\Nat}\yy \\
      \qquad\qquad\qquad \IF \ \pp=\W[i+1][j+1]\ \THEN \ \Lout{\W[i+1][j]}{\Nat} \yy\\
          \qquad\qquad\qquad  \ELSE\IF\ \ \pp=\W[i+1][j]\ \THEN \ \Lin{\W[i+1][j+1]}{\Nat}\yy \\
                    \qquad\qquad\qquad \ELSE \ \yy\\
        \qquad\qquad \ELSE\IF \ \pp=\W[i+1][j+1]\ \THEN \ \Lout{\W[i+1][j]}{\Nat} \yy\\
          \qquad\qquad  \ELSE\IF\ \ \pp=\W[i+1][j]\ \THEN \ \Lin{\W[i+1][j+1]}{\Nat}\yy \\
            \qquad\qquad  \ELSE \ \yy}\\
       \qquad  m) \\
     \quad n} 
\end{array}
\]
}

From the figure~\ref{fig:examples}(b),
the user would design the end-point type as follows:
{\small\[
\begin{array}{lll}
\IF \ &
\p=\W[n][m] \ \THEN \ \Lout{\W[n-1][m]}{\Nat}{\Lout{\W[n][m-1]} {\Nat}{}}\\
\ELSE\IF &
\p=\W[n][0]  \ \THEN \ \Lin{\W[n][1]}{\Nat}{\Lout{\W[n-1][0]}{\Nat}{}}\\
\ELSE\IF &
\p=\W[0][m]  \ \THEN \ \Lin{\W[1][m]}{\Nat}{\Lout{\W[0][m-1]}{\Nat}{}}\\
\ELSE\IF &
\p=\W[0][0]  \ \THEN \ \Lin{\W[1][0]}{\Nat}{\Lin{\W[0][1]}{\Nat}{}}\\
\ELSE\IF &
 1 \leq k+1 \leq m-1 ~ \mathsf{and}\ \p=\W[n][k+1]\\
 & \THEN \ \Lin{\W[n][k+2]}{\Nat}{\Lout{\W[n-1][k+1]}{\Nat}{\Lout{\W[n][k]}{\Nat}}}\\ 
\ELSE\IF &
 1 \leq k+1 \leq m-1 ~ \mathsf{and}\ \p=\W[0][k+1]\\
 & \THEN \ \Lin{\W[1][k+1]}{\Nat}{\Lin{\W[0][k+2]}{\Nat}\Lout{\W[0][k]}{\Nat}}\\ 
\ELSE\IF &
 1 \leq i+1 \leq n-1  ~\mathsf{and}\ \p=\W[i+1][m]\\
 & \THEN \ \Lin{\W[i+2][m]}{\Nat}{\Lout{\W[i][m]}{\Nat}{\Lout{\W[i+1][m-1]}{\Nat}}}\\ 
\ELSE\IF &
 1 \leq i+1 \leq n-1  ~\mathsf{and}\ \p=\W[i+1][0]\\
 & \THEN \ \Lin{\W[i+2][0]}{\Nat}{\Lin{\W[i+1][1]}{\Nat}{\Lout{\W[i][0]}{\Nat}}}\\ 
 \ELSE\IF &
 1 \leq i+1 \leq n-1  ~\mathsf{and}\ 1 \leq j+1 \leq m-1 ~\mathsf{and}~ \p=\W[i+1][j+1]\\
 & \THEN \ \Lin{\W[i+2][j+1]}{\Nat}{\Lin{\W[i+1][j+2]}{\Nat}{\Lout{\W[i][j+1]}{\Nat}{\Lout{\W[i+1][j]}{\Nat}}}}\\ 
\end{array}
\]}

Each case denotes a role in the mesh pattern. Role names are given in process definition. We will present the typing
of the two roles left-top-corner and bottom-row to give an idea of how our system types the mesh pattern. The other cases
are left to the reader. 

Let $T[\p][n][m]$ for the first original type and $T'[\p][n][m]$ for the
second role type. We can check for all $\n, \m \geq 2$ and $\p$, we have:
\begin{center}
$(\prod n.\prod m.T[\p][n][m])\n \m \redsym^\ast T_{\n, \m}\not\redsym$ iff 
$(\prod n.\prod m.T'[\p][n][m]) \n \m \redsym^\ast T_{\n, \m}\not\redsym$. 
\end{center}

For $\p=\W[n][m]$, which implements the left top corner role, the generator type reduces to one step and gives the end-point type 
$\Lout{\W[\n-1][\m]}{\Nat}{\Lout{\W[\n][\m-1]} {\Nat}{}}$, which is the same to the one returned by the case analysis of the role-type built 
by the programmer. For $\p=\W[0][k+1]$, we analyze the case when $\n =2$ and $\m=2$, where $1 \leq k+1 \leq \m-1$. The generator 
type returns the end-point type \Lin{\W[1][k+2]}{\Nat}{\Lin{\W[0][k+2]}{\Nat}\Lout{\W[0][k]}{\Nat}} where the first action comes from the 
case in line number 13, the second action comes from the case in line 2 and the third action comes from case in line 1. One can observe that 
the end-point type returned for $\p=\W[0][k+1]$ in the role-type of the programmer is the same as the one returned by the generator. Similarly for all
the other cases. Note that for all $\n, \m$, the $\beta$-reduction terminates, 
so that the equality checking terminates. 

By \trule{TOut, TIn}, we have: 
\[ 
a:\mar{\G} \vdash \outS{y}{\W[n-1][m], f(n-1,m)}\outS{y}{\W[n][m-1], f(n,m-1)}{\inact}
  \rhd \D,\y:\G \proj{\p_{\text{start}}}
  \]
  \[
a:\mar{\G} \vdash \inpS{y}{\W[1][k+1], z_1}\inpS{y}{\W[0][k+2], z_2}\outS{y}{\W[0][k], f(0,k)}\inact \rhd \D', \y :\G \proj{\p_{\text{bottom\_row}}}\\
\]
where $\G \proj{\p}$ is obtained from the role type above. 

The primitive recursive process is typed similarly as for the one of the sequence pattern.


==> semantics.tex <==
%\input{fig_runtime_syntax}

\subsection{Semantics}
%\noindent 
\label{subsec:semantics}
%% Following \cite{BettiniCDLDY08LONG},  user-defined processes equipped with global
%% types are executed through a translation into runtime processes given
%% in figure~\ref{fig:runtime-syntax}.  
% The basis of our process semantics comes from~\cite{BettiniCDLDY08LONG} to which we add
% the indices evaluation and the reduction of the recursion operator,
% from the evaluation of indices and 
% The key departure from \cite{BettiniCDLDY08LONG} is 
% that the principals' indices should be evaluated during 
% execution. 

\input{fig_semantics}

\input{fig_evaluationcontext}

%\paragraph{\bf Semantics}
The semantics is defined by the reduction relation $\red{}{}$ presented in
Figure~\ref{fig:reduction}. The standard definition of evaluation contexts (that
allow 
e.g. $\W[3+1]$ to be reduced to $\W[4]$) is in Figure~\ref{fig:context}.
%The evaluation order (here call-by-value) is
% enforced through evaluation context whose standard definition we omit
% here (for example, they allow $\W[3+1]$ to be reduced to $\W[4]$).
 % Some of the run-time syntax is detailed in figure~\ref{fig:syntax}.
The metavariables $\pv,\qv,..$ range over principal values (where all indices
have been evaluated).
% to integers (such as $\W[3][5]$).
%
% The reduction rules feature $\beta$-reduction and recursors. Note that our
% $\beta$-reduction does not take higher-order values but {\em only numerals}.
% We omit integer and boolean operations.  
Rules [ZeroR] and [SuccR] are standard and
identical to their global type counterparts.  Rule [Init] describes the
initialisation of a session by its first participant
$\sr\Ia{\p_0,..,\p_\n}{\y_0}{\PP_0}$. It spawns asynchronous requests
$\sj{\Ia}{\pv_k}{\s}$ that allow delayed acceptance by the other session
participants (rule [Join]).  After the connection, the participants share the
private session name \s, and the queue associated to \s~(which is initially
empty by rule [Init]).  The variables $\y_\p$ in each participant $\p$ are then
replaced with the corresponding session channel, $\si{\s}{\p}$. An equivalent,
but symmetric, version of [Init] (where any participant can start the session, 
not only $\p_0$) can be also used. Rule [Init] would then be replaced by the
following:
$$
\bar{\Ia}[\pv_0,..,\pv_\n] \redsym (\nu \s)(
        s : \qbot \pc \sj{\Ia}{\pv_0}{\s} \pc ...\pc
        \sj{\Ia}{\pv_\n}{\s})
$$
% could also be used~\cite{fullversion}.
% The most important rule is [Link], which describes the
% initiation of a new session among $\n$ participants that synchronise over a
% service name \Ia. The first participant $\sr\Ia{\p_0..\p_\n}{\y_0}{\PP_0}$ is
% distinguished by the overbar on the service name. His role is to specify the set
% of participants, which would be dynamically determined during execution.
% 

%\input{fig_evaluationcontext}

% We use evaluation contexts % defined in figure \ref{fig:context}
% to ensure the evaluation of indices
% before session reductions (such as $\sa\Ia{\_}{\y}{\PP}$) and the evaluation of
% expressions (e.g. $\_\op\_$).
% %defined in figure~\ref{fig:context} in Appendix. 
% For example, 
% $\sr\Ia{\W[0],\W[3+1],\W[2+2]}{\y_0}{\PP_0}$
% %$\sr\Ia{\W[0],\W[3+1]}{\y_0}{\PP_0}$
% becomes 
% $\sr\Ia{\W[0],\W[4]}{\y_0}{\PP_0}$ 
% before [Link] is applied. 
% This facility, in combination with the [Beta] reduction, makes it possible to
% determine the participant number of a multiparty session at runtime (see
% e.g. the sequence example of figure~\ref{fig:ex-intro}).  


\noindent  The rest of the session reductions are standard \cite{BettiniCDLDY08LONG,CHY07}.  The
output rules [Send] 
and [Label] push values, channels and labels into the queue of the session
\s{}.  Rules [Recv] 
and [Branch] perform the complementary operations.  Note that these operations
check that the sender and receiver match.
% (in particular, for [Recv], we need to remove the receiving
%participant from the set of the receivers in order to avoid reading the same
%message more than once).
Processes are considered modulo structural equivalence, denoted
by $\equiv$ (in particular, we note 
$\mu X.P \equiv P\subst{\mu X.P}{X}$),  
whose definition is found in Figure~\ref{tab:structcong}.  
Besides the standard rules
\cite{MilnerR:commspc}, we have
a rule for rearranging messages when the senders or the receivers
are different, and a rule for the garbage-collection of unused and empty
queues. 

\input{fig_process_congruence}

%(Table~\ref{tab:structcong}); 



==> shortprotocol.tex <==
\paragraph{\bf Web Service example - Figure~\ref{fig:CDL-short}} %  Choreography and FFT}
\label{sec:webservice}
\label{sec:usecase}
\noindent 
We program and type a real-world Web service use case: Quote Request (C-U-002) is
the most complex scenario described in \cite{CDLRequirements}, the
public document authored by the W3C Choreography Description Language Working
Group \cite{CDL}. 
%
\begin{figure}[t]
%\centerline{\includegraphics[width=0.3\textwidth]{quote-request2.eps}}
\begin{tabular}{@{}l@{}l@{}}
\begin{minipage}{0.35\textwidth}
{\scriptsize
\begin{tabular}{c}
\xymatrix@C=15pt@R=1pt{
 & *+[F] {\Supp[0]\!}\ar@{<->}[r]\ar@{<->}[ddr]
 &  *+[F] {\Manu[0][0]\!} \\
 &  &  \\
  *+[F]{\Buyer\!} \ar@{<->}[r]\ar@{<->}[uur]\ar@{<->}[ddr]
&  *+[F]{\Supp[1]\!} \ar@{<->}[ddr]
&  *+[F] \txt{\Manu[0][1]\!\\\Manu[2][1]\!}\\
 &  &   \\
&  *+[F]{\Supp[2]\!} \ar@{<->}[r]\ar@{<->}[uur]
&  *+[F] \txt{\Manu[1][2]\!\\\Manu[2][2]\!}\\
 & {:} & {:}  \\
}\\
\end{tabular}
}
\end{minipage}
& %\\
\begin{minipage}{0.65\textwidth}
{\footnotesize
\begin{enumerate}
\item[{\bf 1.}] A buyer requests a quote from a set of suppliers.\\
$G_1=\FOREACH{\ii}{<n}{\GS{\mathtt{Buyer}}{\mathtt{Supp}[\ii]}{\mathsf{Quote}}}$
\item[{\bf 2.}] All suppliers receive the request to ask their respective manufacturers
for a bill of material items.
% \item[{\bf 3.}]
The suppliers interact with their manufacturers to build their quotes
for the buyer.\\
$\begin{array}{l@{}l}
\!G_2(i)\!=\! \FOREACH{\jj\!}{:\! J_i\!}{&\GS{\mathtt{Supp}[\ii]}{\mathtt{Manu}[\ii][\jj]}{\mathsf{Item}}.\\
& \GS{\mathtt{Manu}[\ii][\jj]\!}{\!\mathtt{Supp}[\ii]}{\mathsf{Quote}}}
\end{array}$\\
 The eventual quote is sent back to the buyer.\\
%\hspace{\fill} 
$G_2 \!=\!\FOREACH{\ii}{\!:\!\II}{G_2(i) ;
  \GS{\mathtt{Supp}[i]\!}{\mathtt{Buyer}}{\mathsf{Quote}}}$ 
\end{enumerate}
}
\end{minipage}
\end{tabular}

%\vspace{-1ex}
\begin{minipage}{\textwidth}
{\footnotesize
\begin{enumerate} 
% \item[{\bf 1.}] A buyer requests a quote from a set of suppliers.\\
% $G_1=\FOREACH{\ii}{<n}{\GS{\mathtt{Buyer}}{\mathtt{Supp}[\ii]}{\mathsf{Quote}}.\End}$
% \item[{\bf 2.}] All suppliers receive the request and ask their respective manufacturers
% for a bill of material items.\\
% $G_2[i]\!=\! \FOREACH{\ii}{:J_i}{\GS{\mathtt{Supp}[\ii]}{\mathtt{Manu}[\ii][\jj]}{\mathsf{Item}}.
% \GS{\mathtt{Manu}[\ii][\jj]}{\mathtt{Supp}[\ii]}{\mathsf{Quote }}}$
% % \item[{\bf 3.}]
% The suppliers interact with their manufacturers to build their quotes
% for the buyer. The eventual quote is sent back to the buyer. 
\item[{\bf 3.}] EITHER
\begin{enumerate}
\item The buyer agrees with one or more of the quotes and places the order(s). OR 
\item The buyer responds to one or more of the quotes by modifying 
and sending them back to the relevant suppliers.
\end{enumerate}
\item[{\bf 4.}] EITHER
\begin{enumerate}
\item The suppliers respond to a modified quote 
by agreeing to it and sending a confirmation message back to the buyer. OR

\item The supplier responds by modifying the quote and sending it back
to the buyer and the buyer goes back to STEP 3. OR 

\item 
The supplier responds to the buyer rejecting the modified quote. OR 

\item 
The quotes from the manufacturers need to be renegotiated by the supplier. Go to STEP 2. 
\end{enumerate}
\end{enumerate}
}
\end{minipage}

\[
\begin{array}{@{}c|c}
\begin{array}{@{}l}
G_3 = \GR{\ \ty\ }{i}{\yy}{ %\\
} \TO{\mathtt{Buyer}}{\mathtt{Supp}[i]} : \{ \\
%& & 
\ \begin{array}{l@{}l@{}ll}
\mathsf{ok}: & \End \\
\mathsf{modify}: & \multicolumn{3}{l}{\GS{\mathtt{Buyer}}{\mathtt{Supp}[i]}{\mathsf{Quote}}.} \\
& \TO{\mathtt{Supp}[i]}{\mathtt{Buyer}}: \{
&  \mathsf{ok}: & \End \\
&& \mathsf{retryStep3}: & \yy\\
&&  \mathsf{reject}: & \End\}\}\ \ii
\end{array}
\end{array}
& 
\begin{array}{l}
\begin{array}{l}
% \begin{array}{l}
% \&\langle\mathtt{Buyer}, \{ \\
% \\
% \\
% \\
% \\
% \end{array}
\begin{array}{ll}
\multicolumn{2}{l}{G_3\proj{\mathtt{Supp}[\n]}=\&\langle\mathtt{Buyer}, \{}\\
\ \mathsf{ok}\!: & \!\End\\
\ \mathsf{modify}\!: & \!\Lin{\mathtt{Buyer}}{\mathsf{Quote}}{} \oplus\langle\mathtt{Buyer},\!\{\! \\
& \begin{array}{ll}
\qquad \mathsf{ok}: & \End \\
\qquad \mathsf{retryStep3}: & \yy \\
\qquad \mathsf{reject}: & \End\}\rangle\}\rangle
\end{array}
\end{array}
\end{array}
\end{array}
\end{array}
\]
\caption{The Quote Request use case (C-U-002) \cite{CDLRequirements} with the
  corresponding global types\label{fig:CDL-short}}
%\vspace{1mm}
\end{figure}
%
% The use case is
As described in Figure~\ref{fig:CDL-short}, % (as published in \cite{CDLRequirements}). 
a buyer interacts with multiple suppliers who in turn
interact with multiple manufacturers in order to obtain quotes for some
goods or services. %The steps of the interaction are: 
%A concrete example can be a company that
%wishes to purchase a fleet of cars from various automobile suppliers which in
%turn request quotes for specific items and materials from the
%component manufacturers. 
%
%The usecase is depicted in figure~\ref{fig:CDL}. 
%
%\paragraph{Requirements}
% The use case %, depicted in figure~\ref{fig:CDL}, 
% contains many challenges. 
% For example,
The Requirements 
from Section 3.1.2.2 of \cite{CDLRequirements} include
the ability to {\em reference a global description from within a
global description} to support {\em recursive behaviour} as 
denoted in {\sc Step} 4(b, d): this can be achieved by parameterised
multiparty session types.
% The following works through
% This can be achieved by \ny{a parameterised global type
%   specification}. 
% that satisfies these requirements.


%\begin{description}
%\item[R1] {\em Needs the ability to repeat the same set of interactions
%and compose them.} 
%The interactions between supplier and manufacturers need only be defined
%once and then repeated for each relevant supplier manufacturer
%pairing. 

%\item[R2]
%{\em Needs participant sets (i.e. the number of participants) 
%that may be bounded at design time or at the runtime.} 
%For instance, the set of suppliers may be
%determined when the global description is designed or when some parameter is
%instantiated dynamically as the interaction progresses. 

%\item[R3] 
%Needs to be able to {\em reference a global description from within a
%global description} to support {\em recursive behaviour} such as a manufacturer
%placing an order with its supplier ({\sc Step} 4(b,d)).   
%\end{description}
%For the first and third points, we propose 
%{\em programming idioms} for repeating and 
%composing types to make a larger type.  The second point 
%is naturally represented by our dependent types. The third point 
%requires a complex combination with recursive and branching types
%with recursors.   

%\paragraph{Programming idioms}
%For {\bf R1}, 
%the first step is defining two simple idioms for 
%merging and repeating global specifications. 
%\[
%\begin{array}{rcll}
%\MERGE{G_1,G_2} & \!\!= \!\!& 
%\GR{\G_2}{\ii}{\xx}{\G_1\sub{\xx}{\End}} \ 1
%\\[1mm]
%\FOREACH{\ii}{[0..\jj]}{G}& \!\!= \!\!&
% \GR{\End}{\AT{\ii}{[0..\jj]}}{\xx}{\G\sub{\xx}{\End}} \ \jj+1
%\end{array}
%\]
%where we assume $\xx\not\in G_1,G$, and $G_1$ and $G$ end 
%with $\End$. In the encodings, $\End$ is replaced by $\xx$. 
%The first composes two 
%global types and the second repeats $G$ $j+1$-times. 

%\paragraph{Modular programming using global types}

We write the specification of the usecase program modularly, starting from the
first steps of the informal description above. Here, $\mathtt{Buyer}$ stands for
the buyer, $\mathtt{Supp}[\ii]$ for a supplier, and $\mathtt{Manu}[\jj]$ for a
manufacturer. We alias manufacturers by $\mathtt{Manu}[\ii][\jj]$ to express the
fact that $\mathtt{Manu}[\jj]$ is connected to $\mathtt{Supp}[\ii]$ (a single
$\mathtt{Manu}[\jj]$ can have multiple aliases $\mathtt{Manu}[\ii'][\jj]$, see
figure~\ref{fig:CDL-short}).  Then, we can write global types for each of the
steps. {\sc Step} 1 is a simple {\em multicast} (type $G_1$). 
%  {\sc Step} 1
% is defined as $G_1$ below.
%$$
%%\begin{array}{lll}
%$\G_1 = 
%\FOREACH{\ii}{\II}{
%\GS{\mathtt{Buyer}}{\mathtt{Supp}[\ii]}{\mathsf{Quote}}.\End}
%$
%\end{array}
%$$
For {\sc Step} 2, we write first $G_2(i)$, the nested interaction loop between the $i$-th
supplier and its manufacturers ($J_i$ gives all $\mathtt{Manu}[\jj]$ connected
to $\mathtt{Supp}[\ii]$). Then $G_2$ can describe the subsequent action within
the main loop. 
% {\small
% \[ 
% \begin{array}{ll}
% \G_1 = 
% \FOREACH{\ii}{\II}{
% \GS{\mathtt{Buyer}}{\mathtt{Supp}[\ii]}{\mathsf{Quote}}.\End}\\[1mm]
% G_2 = \mathtt{foreach}({\ii}:{\II})\{
% \MERGE{G_2[i] \, ; \,
% \GS{\mathtt{Supp}[i]}{\mathtt{Buyer}}{\mathsf{Quote}}.\End}\} \\[1mm]
% %\end{array}
% %\]
% %%\[
% %%\begin{array}{ll}
% %%G_2[i]=\\[1mm]
% %%\mathtt{foreach}({\jj}:{J_i})\{&
% %%\GS{\mathtt{Supp}[\ii]}{\mathtt{Manu}[\ii][\jj]}{\mathsf{Item}}.\\
% %%&\GS{\mathtt{Manu}[\ii][\jj]}{\mathtt{Supp}[\ii]}{\mathsf{Quote}}.\End\}
% %%\end{array}
% %%\]
% %\[
% %\begin{array}{ll}
% G_2[i]= \mathtt{foreach}({\jj}:{J_i})\{  
% \GS{\mathtt{Supp}[\ii]}{\mathtt{Manu}[\ii][\jj]}{\mathsf{Item}}.
% \GS{\mathtt{Manu}[\ii][\jj]}{\mathtt{Supp}[\ii]}{\mathsf{Quote}}.\End\}
% \end{array}
% \]
% }
%\[ 
%\begin{array}{ll}
%G_2 = \mathtt{foreach}({\ii}:{\II})\{\\
%\qquad\qquad \MERGE{G_2[i]\, ; \,
%\GS{\mathtt{Supp}[i]}{\mathtt{Buyer}}{\mathsf{Quote}}.\End}\} \\[1mm]
%%\end{array}
%%\]
%%%\[
%%%\begin{array}{ll}
%%%G_2[i]=\\[1mm]
%%%\mathtt{foreach}({\jj}:{J_i})\{&
%%%\GS{\mathtt{Supp}[\ii]}{\mathtt{Manu}[\ii][\jj]}{\mathsf{Item}}.\\
%%%&\GS{\mathtt{Manu}[\ii][\jj]}{\mathtt{Supp}[\ii]}{\mathsf{Quote}}.\End\}
%%%\end{array}
%%%\]
%%\[
%%\begin{array}{ll}
%G_2[i]= \mathtt{foreach}({\jj}:{J_i})\{ \\
%\qquad\qquad \GS{\mathtt{Supp}[\ii]}{\mathtt{Manu}[\ii][\jj]}{\mathsf{Item}}.\\
%\qquad\qquad \GS{\mathtt{Manu}[\ii][\jj]}{\mathtt{Supp}[\ii]}{\mathsf{Quote}}.\End\}
%\end{array}
%\]
%
%The G[i] is not quite right because J_i can be discontinuous (according to the
%Usecase spec.), but foreach assumes continuous. 
%  
%the specification involves buyer preference for certain suppliers.  
%%with respect to the received quotes. 
%\ny{Since this can be encoded using dependent types 
%(like the encoding of $\mathsf{if}$),
%%in the case of $I$ and $J$ range over finite numbers,  
%%or by naturally extending the dependent types
%%for values of {\sf Quote}. 
%we omit this part and assume 
%the preference is given by the (reverse) ordering of $\II$ in order to focus on the
%description of the
%interaction structure. }
%\[
%\begin{array}{llll}
%G_3 =
%\GR{\ \ty\ }{i}{\yy}{}\\
%\quad \TO{\mathtt{Buyer}}{\mathtt{Supp}[i]}.\\
%\quad \{ \mathsf{ok}: \End\\
%\quad  \mathsf{modify}: 
%\GS{\mathtt{Buyer}}{\mathtt{Supp}[i]}{\mathsf{Quote}}\\
%\ \quad \ \quad \  \ \
%\begin{array}{ll}
%\TO{\mathtt{Supp}[i]}{\mathtt{Buyer}}\\
%\\ 
%\\
%\end{array}
%\begin{array}{ll}
%\{
%\mathsf{ok}: & \End \\
%\mathsf{retryStep3}: & \yy\\
%\mathsf{reject}: & \End\}\}\ \ii
%\end{array}
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \ 
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\ \ \quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \mathsf{reject}:\End\}
%\end{array}
%\]
For {\sc Step} 3, for simplicity we assume the preference is given by the
(reverse) ordering of $\II$. 
% $G_3$ is given in Figure~\ref{fig:CDL-G3} (a).
The first choice of $G_3$ corresponds to the two cases of {\sc Step} 3.  In the
innermost branch of $G_3$, the branches $\mathsf{ok}$, $\mathsf{retryStep3}$ and
$\mathsf{reject}$ correspond to {\sc Step} 4(a), (b) and (c) respectively, while
the type variable $\ty$ models {\sc Step} 4(d).  We can now compose these
subprotocols together. % Taking
%\[ 
% $G_{23} = \GM{\ty}{\MERGE{(G_2\, ; \, G_3)}}$ 
%\]
%If we wish to repeat it some finite number of times ($m$), we can write 
%\[ 
%G_{23}\ =\ \FOREACH{k}{[0..m]}{\MERGE{G_2\, ; \, G_3}}
%\]
% and assuming $\II=[0..i]$
The full global type is then
$
\G = \Pi i.\Pi \VEC{J}.(\MERGE{G_1\, ; \,\GM{\ty}{\MERGE{(G_2\, ; \, G_3)}}}) 
$
where we have $i$ suppliers, and $\VEC{J}$ gives the index sets $J_i$ of the
$\mathtt{Manu}[\jj]$s connected with each $\mathtt{Supp}[\ii]$.  

For the end-point projection, 
we focus on the suppliers' case.
%%\paragraph{End-point types}
%We show the local type for suppliers, who engage in
%the most complex interaction structures among the participants.  
The projections of $G_1$ and $G_2$ are straightforward.
%%\[
%%\begin{array}{lllll}
%%G_1\proj{\mathtt{Supp}[\n]} 
%%=  \Lin{\mathtt{Buyer}}{\mathsf{Quote}}{}\\[1mm]
%%G_2\proj{\mathtt{Supp}[\n]} 
%%=\\ 
%%\quad \mathtt{foreach}({\jj}:{J_i})\{
%%\Lout{\mathtt{Manu}[\n][\jj]}{\mathsf{Item}}
%%{\Lin{\mathtt{Manu}[\n][\jj]}{\mathsf{Quote}}{}\}\\
%%\quad\quad {\Lout{\mathtt{Buyer}}{\mathsf{Quote}}{}}}
%%\end{array}
%%\]
%\[
%\begin{array}{lllll}
%G_1\proj{\mathtt{Supp}[\n]} = \Linn{\mathtt{Buyer}}{\mathsf{Quote}} \\[1mm]
%G_2\proj{\mathtt{Supp}[\n]} = \mathtt{foreach}({\jj}:{J_i})\{ \Loutt{\mathtt{Manu}[\n][\jj]}{\mathsf{Item}}; \\
%\qquad\qquad\qquad\qquad {\Linn{\mathtt{Manu}[\n][\jj]}{\mathsf{Quote}}\}; {\Loutt{\mathtt{Buyer}}{\mathsf{Quote}}}}
%\end{array}
%\]
For $G_3\proj{\mathtt{Supp}[\n]}$, 
we use the branching injection and 
mergeability theory developed in 
\S~\ref{subsec:endpoint}. 
%
After the relevant application of \trule{TEq}, we can obtain 
%the following projection:
the projection written in Figure~\ref{fig:CDL-short}. % {\bf (b)}. 
% where $T$ is a type for the invocation 
% from $\mathtt{Buyer}$.  
%%\[
%%\begin{array}{llll}
%%\&\langle\mathtt{Buyer}, 
%%\{ \mathsf{ok}: \End\\
%%\quad\quad\quad\quad\quad  \mathsf{modify}: 
%%\Lin{\mathtt{Buyer}}{\mathsf{Quote}}{}\\
%%\quad\quad\quad\quad\ \quad \ \quad \  \ \ \quad
%%\begin{array}{ll}
%%\oplus\langle\mathtt{Buyer}
%%\\
%%\\
%%\\
%%\end{array}
%%\begin{array}{ll}
%%\{
%%\mathsf{ok}: & \End \\
%%\mathsf{retryStep3}: & T\\
%%\mathsf{reject}: & \End\}\rangle\\
%%\end{array}
%%\end{array}
%%\]
%\[
%\begin{array}{l}
%\begin{array}{l}
%\&\langle\mathtt{Buyer}, \{ \\
%\\
%\\
%\\
%\\
%\end{array}
%\begin{array}{ll}
%\mathsf{ok}: & \End\\
%\mathsf{modify}: & \Lin{\mathtt{Buyer}}{\mathsf{Quote}}{} \oplus\langle\mathtt{Buyer}, \{ \\
%& \begin{array}{ll}
%\qquad \mathsf{ok}: & \End \\
%\qquad \mathsf{retryStep3}: & T\\
%\qquad \mathsf{reject}: & \End\}\rangle\}\rangle\\
%\end{array}
%\end{array}
%\end{array}
%\]
%\[
%\begin{array}{l}
%\IF \ \n\leq i \ \THEN \ \&\langle \mathtt{Buyer}, \{ \mathsf{closed}:\End, 
%\ \mathsf{retryStep3}:\ty \} \rangle \\ 
%\ELSE\IF \ i=\n \ \THEN \ \ty
%\end{array}
%\]
%%
To tell the other suppliers whether the loop is being reiterated 
or if it is finished, 
\ny{we can simply insert the following closing notification
${\small\FOREACH{\jj}{\in\II\setminus \ii}
{\TO{\mathtt{Buyer}}{\mathtt{Supp}[j]}:\{\mathsf{close}:\}}}
$
before each ${\small\End}$, 
and a similar retry notification 
(with label $\mathsf{retryStep3}$) before $\xx$.} 
%\[
%\begin{array}{lll}
%\FOREACH{\jj}{\II\setminus \ii}
%{\TO{\mathtt{Buyer}}{\mathtt{Supp}[j]}:\{\mathsf{close}:\}}\\
%\FOREACH{\jj}{\II\setminus \ii}{
%\TO{\mathtt{Buyer}}{\mathtt{Supp}[j]}:\{\mathsf{retryStep3	}:\}}
%\end{array}
%\] 
%
Finally, each end-point type is formed by 
%\[ 
$
%\begin{array}{l}
(\MERGE{G_1\proj{\mathtt{Supp}[\n]}\, ; \,
  {\GM{\xx}{\MERGE{G_2\proj{\mathtt{Supp}[\n]}\, ; \,\
        G_3\proj{\mathtt{Supp}[\n]}}}}}). 
%\end{array}
$
While the global types look sequential, actual typed processes 
can asynchronously join a session and be executed in parallel (e.g.,
at {\sc Step} 1-2, no synchronisation is needed between $\Supp[i]$).  
% thanks for our join operator,
%\]
%Following this specification, the local projections can be implemented in various end-point languages (such as CDL or BPEL). 
%We have implemented this usecase \cite{fullversion} (with the number of participants bound at runtime) in SJ \cite{HU07TYPE-SAFE}; 
%see \S~\ref{subsec:bmarks} for further notes on
%implementation experience.  

%We implemented
%and tested this usecase in SJ (Java with session types
%\cite{HU07TYPE-SAFE})
%\cite{Emmanuel09} where the number of suppliers and 
%manufactures can be specified as the parameters 
%by the user, following the specification. 

%The local code 
%since it can be implemented by 
%different end-point languages \cite{CDL} 
%and a working code is large \cite{Emmanuel09}, see \S~\ref{sec:conclusion}.  
%%We had implemented this usecase in SJ \cite{} where 
%%the end-point code is roughly following this end-point code 
%%and they can be complied taking 
%%the parameters . 



%\quad \mathsf{else} 
%\ \&\ \langle\mathtt{Buyer}, 
%\{\mathsf{closed:}\End, \mathsf{retryStep3}:\yy\}
%\rangle
%) \ \ii
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \ 
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\ \ \quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \mathsf{reject}:\End\}
%Then three end points are merged as the global type.  
%It is kind of $\mathtt{Buyer}$ to let other suppliers if he 
%finishes the interaction with one of the supplier in order to safely 
%close the connection. Hence $G_3$ is modified as follows: 
%\[
%\begin{array}{llll}
%G_{3}' =
%\GR{\End}{i}{\yy}{}\\
%\quad \TO{\mathtt{Buyer}}{\mathtt{Supp}[i]}.\\
%\quad \{ \mathsf{ok}: \mathit{Closed}\\
%\quad  \mathsf{modify}: 
%\GS{\mathtt{Buyer}}{\mathtt{Supp}[i]}{\mathsf{Quote}}\\
%\ \quad \ \quad \  \ \
%\begin{array}{ll}
%\TO{\mathtt{Supp}[i]}{\mathtt{Buyer}}\\
%\\ 
%\\
%\end{array}
%\begin{array}{ll}
%\{
%\mathsf{ok}: & \mathit{Closed} \\
%\mathsf{retryStep3}: & \mathit{Retry};\yy\\
%\mathsf{reject}: & \mathit{Closed}\}\ \ii
%\end{array}
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \ 
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\ \ \quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \mathsf{reject}:\End\}
%\end{array}
%\]
%$\mathit{Closed}$ is a closed protocol 
%defined as: $\mathit{Closed}=
%\FOREACH{\jj}{\II\setminus \ii}{
%\TO{\mathtt{Buyer}}{\mathtt{Supp}[j]}\{\mathsf{closed}:\}}$. 
%Similarly 
%$\mathit{Retry}=
%\FOREACH{\jj}{\II\setminus \ii}{
%\TO{\mathtt{Buyer}}{\mathtt{Supp}[j]}\{\mathsf{retryStep3	}:\}}$. 
%Then the end-point type 
%$G_{3}'\proj{\mathtt{Supp}[\n]}$ 
%is given as: 
%\[
%\begin{array}{llll}
%\GR{\End}{i}{\yy}{}\\
%\quad \mathsf{if}\ i=\n \ \mathsf{then} \ 
%\&\langle\mathtt{Buyer}, \\
%\quad \{ \mathsf{ok}: \End\\
%\quad  \mathsf{modify}: 
%\Lin{\mathtt{Buyer}}{\mathsf{Quote}}{}\\
%\ \quad \ \quad \  \ \ \quad
%\begin{array}{ll}
%\oplus\langle\mathtt{Buyer}
%\\
%\\
%\\
%\end{array}
%\begin{array}{ll}
%\{
%\mathsf{ok}: & \End \\
%\mathsf{retryStep3}: & \yy\\
%\mathsf{reject}: & \End\}\rangle\\
%\end{array}\\
%\quad \mathsf{else} 
%\ \&\ \langle\mathtt{Buyer}, 
%\{\mathsf{closed:}\End, \mathsf{retryStep3}:\yy\}
%\rangle
%) \ \ii
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \ 
%%\ \quad \ \quad \ \quad \ \ \quad \ \quad \
%%\ \ \quad \quad \  \ \ \ \quad \ \quad \ \quad \  \ \mathsf{reject}:\End\}
%\end{array}
%\]
%Then three end points are merged as the global type.  
%We omit the local code 
%since it can be implemented by 
%different end-point languages \cite{CDL} 
%and a working code is large \cite{Emmanuel09}, see \S~\ref{sec:conclusion}.  
%%We had implemented this usecase in SJ \cite{} where 
%%the end-point code is roughly following this end-point code 
%%and they can be complied taking 
%%the parameters . 

%The main three of four requirements 
%listed in 3.1.2.2 in \cite{CDLRequrements} follow. 

%\begin{enumerate}
%\item 
%The ability to {\em repeat the same set of interactions} is needed. The
%interactions between supplier and manufacturers need only be defined
%once and then repeated for each relevant supplier manufacturer
%pairing.

%\item 
%Needs participant sets that may be bounded at design time, at the
%runtime or not at all. 
%For instance, the set of suppliers may be
%determined when the global description is designed or when it is
%instantiated, or may be completely dynamic.

%\item 
%Needs to be able to reference a global description from within a
%global description to support recursive behaviour such as a manufacturer
%placing an order with its supplier.
%\end{enumerate}
%We do not treat the forth requirement about a transaction recovery.  
%To make clear, we replaced a term ``choreography'' by a global description
%(i.e. global dependent type) in the above requirements, but the rest 
%is the same as in \cite{CDLRequrements}. 
%The second requirement is less clearer but we believe 
%In summary, we illustrate our theory offers:  
%\begin{itemize}
%\item {\em\bf Merging global scenarios:} 
%We can develop a large specification from small pieces 
%of independent specifications using dependent types 
%(cf.~\S~1) ({\bf Part I}).
 
%\item {\em\bf Repeating actions:} 
%We can describe looping and broadcasting 
%easily using the parameterised dependent session types.  

%\item {\em\bf Flexibility by nested recursors:} 
%We can write expressive specifications 
%as nested dependent global types, combining 
%with branching types and recursions with enlarged 
%projectability (cf.~Defition \ref{def:}). 
%\end{itemize}



==> simple_termination.tex <==
Next we prove the termination for type-equality checking. 

To prove termination of the second equality requires 
a detailed analysis 
since the premises of the mathematical induction 
rules compare the two types whose syntactic sizes are lager 
than those of the conclusions. 
The size of the judgements are defined 
in Figure \ref{fig:size}, 
using the following two functions from \cite[\S~2.4.3]{DependentBook}.
\begin{enumerate}
\item $\termsize{G}$ is the size of the structure of $G$ 
where we associate $\omega^2$-valued weight to each judgement 
to represent a possible reduction to a weak head normal form. 
\item $\reductionsize{\G}$ 
denotes an upper bound on the length of any 
$\redsym$ reduction sequence starting from $G$ and its subterms. 
%the number of the head reductions from $G$. 
%\item $\reductionsize{G}$ is the number of the head reductions 
%from $G$ and its subterms. 
%\item $\inductionreductionsize{G}$ is the maximum number of 
%the head reductions from $G$ and its subterms. 
%This  includes the mathematical induction case 
%where the dependent applications with variables as the arguments. 
\end{enumerate}
The first case of the size of the judgement 
$\judgementsize{\Gamma \proves G_1 \equivwf G_2}$ 
corresponds to 
\trule{WfRecF} in Figure~\ref{fig:type-wf} 
(recursors with the finite index set). 
The second case is 
corresponds to 
\trule{WfRec} (recursors with the infinite index set).  
Other definitions are from \cite[\S~2.4.3]{DependentBook}.  

The termination then is proved by the following main lemma. 

\begin{LEM}[Size of Equality Judgements]\label{lem:size}
The weight of any premise of a rule is always 
less than the weight of the conclusion. 
\end{LEM}
\begin{proof}
We argue by induction of the length of reduction 
sequences and the size of terms. \\[1mm]
{\bf Case \trule{WfBase}} The case $\WHNF{G_1}=G_1$ and 
$\WHNF{G_2}=G_2$ are obvious by definition. Hence we assume  
$\WHNF{G_1} \not = G_1$. Thus there exists at least one step reduction 
such that $G_1\redsym G_1'$. Note that for any $G$, 
we have $\termsize{G}< \omega$. 
Hence we have 
\[
\begin{array}{lll}
  & 
\judgementsize{\Gamma \vdash \WHNF{G_1}\equivwf  \WHNF{G_2}}\\
= 
& \omega \cdot
\reductionsize{\WHNF{G_1}} + \termsize{\WHNF{G_1}} + \omega \cdot
\reductionsize{\WHNF{G_2}} + \termsize{\WHNF{G_2}} + 1\\ 
<  
& \omega \cdot \reductionsize{G_1} + \termsize{G_1}+
  \omega \cdot \reductionsize{G_2} + \termsize{G_2} + 2 \\
=& \judgementsize{\Gamma \vdash G_1\equiv  G_2}
\end{array}
\]
{\bf Case \trule{WfIO}} Similar with \trule{WfBra} below.\\[1mm]
{\bf Case \trule{WfBra}} 
\[
\begin{array}{ll}
& \Sigma_{k\in K}\judgementsize{\Gamma \vdash G_{1k}\equiv  G_{2k}}\\
= & 
\Sigma_{k\in K}(\judgementsize{\Gamma \vdash G_{1k}\equivwf G_{2k}}+1)\\
= & 
\Sigma_{k\in K}(
\omega\cdot(\reductionsize{G_{1k}}+\reductionsize{G_{2k}})+
\termsize{G_{1k}}+\termsize{G_{2k}}+2)\\
< & 
\Sigma_{k\in K}(
\omega\cdot(\reductionsize{G_{1k}}+\reductionsize{G_{2k}})+
\termsize{G_{1k}}+\termsize{G_{2k}}+2)+4\\
= & 
\judgementsize{
\Gamma \vdash \TO{\p}{\q}\colon \{l_k: \G_{1k}\}_{k\in K}\equivwf  
\TO{\p}{\q}\colon \{l_k: \G_{2k}\}_{k\in K}}
\end{array}
\] 
In the third equation, we note that $G_{1k}$ and $G_{2k}$ cannot 
be recursors since $\Gamma \proves G_{ik}\RHD \Type$ by the kinding rule.\\[1mm]
{\bf Case \trule{WfPRec}} Similar with \trule{WfBra} above. \\[1mm]
{\bf Case \trule{WfRVar},\trule{WfEnd},\trule{WfRec},\trule{WfRecF},\trule{WfApp}} 
By definitions. %\\[1mm]
%{\bf Case \trule{WfApp}} 
%Note that $\Gamma \vdash G_{1}\equivwf G_{2}$ in the premise does not match 
%\trule{WfRecF} by the side condition
%hence it matches either the second or third cases of 
%$\judgementsize{\Gamma \vdash G_{1}\equivwf G_{2}}$. \\[1mm]
%(2) The third case: 
%\[
%\begin{array}{ll}
%&  \judgementsize{\Gamma \vdash G_{1}\equivwf G_{2}}\\[1mm]
%= & 
%\omega\cdot(\reductionsize{G_{1}}+\reductionsize{G_{2}})+
%\termsize{G_{1}}+\termsize{G_{2}}+1\\[1mm]
%< & 
%\omega\cdot(\reductionsize{G_{1} \tii_1}+
%            \reductionsize{G_{2} \tii_2})+ 
%            \termsize{G_{1} \tii_1}+\termsize{G_{2} \tii_2}+1\\[1mm]
%= & 
%\judgementsize{\Gamma \vdash G_{1}\tii_1\equivwf G_{2}\tii_2}
%\end{array}
%\]
\qed 
\end{proof}

\input{fig_simple_size}



==> subjectreduction.tex <==

\subsection{Type soundness and progress}
%\label{sec:subjred}
\noindent 

\noindent The following lemma states that mergeability is sound 
with respect to the branching subtyping 
%We also use the following lemma for the branching 
%local types whose projections are extended by the mergeability operator  
%$\mergeop$. 
$\subT$. 
By this, we can safely replace the third clause 
$\sqcup_{k\in K}  \G_k\proj{\qq}$ of the branching case from the projection definition by 
$\sqcap \{T\ | \ \forall k\in K.T \subT (G_k\proj{\qq}) \}$.  
This allows us to prove subject reduction by including subsumption 
as done in \cite{CHY07}. 


\begin{LEM}[Soundness of mergeability]
\label{lem:mergeability}
Suppose $G_1\proj{\p} \mergeop G_2\proj{\p}$ and 
$\Gamma \proves G_i$. Then there exists $G$ such that 
$G\proj{\p}=\sqcap \{T\ | \ T \subT G_i\proj{\p} \ (i=1,2)\}$
where $\sqcap$ denotes the maximum element with respect to $\subT$. 
\end{LEM}
\begin{proof}
The only interesting case is when $G_1\proj{\p}$ and $G_2\proj{\p}$ take 
a form of the branching type. Suppose 
$G_1 = \TO{\p'}{\p}\colon\! \indexed{l}{{\G'}}{k}{K}$
and 
$G_2 = \TO{\p'}{\p}\colon\! \indexed{l}{{\G''}}{j}{J}$
with $G_1\proj{\p} \mergeop G_2\proj{\p}$. 
Let $\G'_{k}\proj{\p}=T_{k}$ and 
$\G''_{j}\proj{\p}=T_{j}'$. 
Then by the definition of $\mergeop$ in \S~\ref{subsec:endpoint}, 
we have $G_1\proj{\p}= \langle\p',\{l_k:T_{k}\}_{k\in K}\rangle$ 
and
$G_2\proj{\p}=\&\langle\p',\{l_j:T_{j}'\}_{j\in J}\rangle$ 
with 
$\forall i\in (K \cap J). T_i\mergeop T_i'$ and
$\forall k\in (K \setminus J),\forall j\in (J \setminus K).l_k \not = l_j$. 
By the assumption and inductive hypothesis on $T_k\mergeop T_j'$, 
we can set 
\[
T=\&\langle\p',\{l_k:T''_{i}\}_{i\in I}\rangle
\] 
such that $I=K \cup J$; and (1) if $i\in K \cap J$, then  
$T''_{i}=T_{i}\sqcap T'_{i}$; (2) if $i\in K, i\not\in J$, then  
$T''_{i}=T_{i}$; and (3)
if $i\in J, i\not\in K$, then  
$T''_{i}=T'_{i}$. Set 
$G_{0i}\proj{\p}=T''_i$. Then we can obtain 
\[ 
G=\TO{\p'}{\p}\colon\! \indexed{l}{{\G_{0}}}{i}{I}
\]
which satisfies 
$G\proj{\p}=\sqcap \{T\ | \ T \subT G_i\proj{\p} \ (i=1,2)\}$, 
as desired. 
\end{proof}

\noindent
As session environments record channel states, they evolve when communications proceed.
% Since session environments represent the effect of 
% natural number instantiations by dependent types and the forthcoming
% communications, during reductions, session environments can
% change. 
This can be formalised by introducing
a notion of session environments reduction. These rules are formalised below
modulo $\equiv$. 
%with with [Context] in figure~\ref{fig:reduction}:
{\small
\begin{itemize}
\item
$\sered{\set{\si{\s}{\pv}:\Lout{\qv}{\U}{\T},\si{\s}{\qv}:\Lin{\pv}{\U}{\T'}}}{\!\set{\si\s\pv: \T, \si\s{\qv}:\T'}}$
\item
$\sered{\set{\si{\s}{\pv}:\Lout{\pv}{\U}{\Lin{\pv}{\U}{\T'}}}}
{\!\set{\si\s\pv: \T'}}$
\item
$\sered{\set{\si\s\pv:\Lsel{\qv}{\T_k}}}{\set{\si\s\pv:\LselSingle{\qv}{l_j};T_j}}$
\item
$\sered{\set{\si\s\pv:\LselSingle{\qv}{l_j};T,
\si\s{\qv}:\branchtype}}{\set{\si\s\pv:\T, \si\s{\qv}:\T_j}}$
%\quad if $l=l_i$
%\item
%$\sered{\set{\si\s\pv:\oT\UT{\emptyset};\ \T}}{\set{\si\s\pv:\T}}$
%\qquad
%$\sered{\set{\si\s\pv:\oplus\langle\emptyset,l\rangle;\T}}{\set{\si\s\pv:\T}}$
\item
$\sered{\D\cup\D''}{\D'\cup\D''}$ if $\sered{\D}{\D'}$. 
\end{itemize}
}
%The first rule corresponds to the reductions for the recursor and 
%the lambda-abstraction, while 
\noindent
The first rule corresponds to the reception of
a value or channel by the participant $\qv$; 
the second rule formalises 
the reception of a value or channel sent by itself $\pv$;
the third rule 
treats the case of the choice of label $l_j$ while the forth rule
propagate these choices to the receiver (participant $\qv$). 

For the subject reduction theorem, we need to define 
{\em the coherence of the session 
environment \D}, which means that each end-point type is dual with
other end-point types.  

\begin{DEFINITION}\label{cd}
A session environment \D\ is {\em coherent for the session \s}
(notation \coe{\D}{\s}) if $ \sii:\T\in\Delta$ and
$\pro{\T}\q\not=\End$ imply $ \siq:\T'\in\Delta$ and
$\dual{\pro{\T}\q}{\pro{\T'}\p}$.  A session environment \D\ is
{\em coherent} if it is coherent for all sessions 
which occur in it.
\end{DEFINITION}
The definitions for $\pro{\T}\q$ and $\dual{}{}$ are defined in
Appendix~\ref{app:runtime}. Intuitively, $\pro{\T}\q$ is a projection
of $T$ onto $\q$ which is similarly defined as $\pro{\G}\q$; and 
$\dual{\pro{\T}\q}{\pro{\T'}\p}$ means actions in $\T$ onto 
$\q$ and actions in $\T'$ onto $\p$ are dual (i.e. input matches 
output, and branching matches with selections, and vice versa). 
Note that two projections of a same global type are always dual: 
let $\G$ a global type and $\p,\q \in \G$
with $\p \neq \q$. Then
$\dual{\pro{(\pro{\G}{\p})}{\q}}{\pro{(\pro{\G}{\q})}{\p}}$, 
i.e. session environments corresponding to global
type are always coherent.


Using the above notion we can state type preservation under reductions
as follows:
%% \begin{THM}[Subject Congruence and Reduction]\label{thm:sr}
%% If \derqq\Ga{}\PP\Ty\ and \redM\PP{\PP'} with \Ty coherent, then
%% \derqq\Ga{}{\PP'}{\Ty'}\ for some $\Ty'$ such that
%% $\seredstar\Ty\Ty'$ with $\Ty'$ coherent.
%% \end{THM}
\begin{THM}[Subject Congruence and
  Reduction]\label{thm:sr}\mbox{\;}

\begin{enumerate}
\item
If $\derqq\Ga{\Sigma}\PP\D$ and $\PP\equiv{\PP'}$, then
\derqq\Ga{\Sigma}{\PP'}{\D}. 
\item 
If \derqq\Ga{\Sigma}\PP\Ty\ and \redM\PP{\PP'} with 
\Ty\ coherent, then
\derqq\Ga{\Sigma}{\PP'}{\Ty'}\ for some $\Ty'$ such that
$\seredstar\Ty\Ty'$ with $\Ty'$ coherent.
\end{enumerate}
\end{THM}
\begin{proof}
  We only list the crucial cases of the proof of subject reduction: the recursor
  (where mathematical induction is required), the initialisation, the input and
  the output.  The proof of subject congruence is essentially as the same as
  that in \cite{CHY07,BettiniCDLDY08LONG}.  Our proof for (2) works by induction
  on the length of the derivation \redM\PP{\PP'}. The base case is trivial. We
  then proceed by a case analysis on the first reduction step
  \red\PP{\PP''}\redM{}{\PP'}. We omit the hat from principal values and
  $\Sigma$ for readability.
% The most interesting case 
% is the recursor where we use
% mathematical induction in addition to induction on the derivation. 
% Also the initialisation uses the mergeability lemma. 
%We omit 
%$\Sigma$ from the turnstile since it is fixed for these cases. 
%The session initialisation uses the property of the subtyping 
%for the mergeability. 
%\\[1mm]
%{\bf Case Beta:}  Suppose 
%$\derqq\Ga{}{(\lambda \ii.\PP)\n}{\Ty}$  
%and $\red{(\lambda \ii.\PP)\n}{\PP\subst{\n}{\ii}}$. 
%Then there exists $\Ty'$ such that 
%$\derqq\Ga{}{\lambda \ii.\PP}{\Pi\AT{\ii}{\II}.\Ty'}$ 
%and $\Ty \equiv (\Pi\AT{\ii}{\II}.\Ty') \n \equiv \Ty'\subst{\n}{\ii}$
%and $\Ga{\models}{n: \II}$. The first judgement must have been 
%derived with \trule{TApp}, thus we have the derivations such that 
%$\Gamma, \AT{\ii}{\II}\vdash \PP\rhd \Ty'$. By applying the
%Substitution Lemma (Lemma \ref{lem:substitution} (\ref{subs01})), we obtain
%$\Gamma\vdash \PP\subst{\n}{\ii}\rhd \Ty'\subst{\n}{\ii}$, 
%as required. 
\\[1mm]
{\bf Case [ZeroR].}  Trivial. \\[1mm]
{\bf Case [SuccR].}  Suppose 
that we have
$\derqq\Ga{}{\GR{P}{\ii}{X}{Q}\APP \n+1}{\tau}$
and 
$\red{\GR{P}{\ii}{X}{Q}\APP \n+1}
{Q\sub{\n}{\ii}\sub{\GR{P}{\ii}{X}{Q}\APP \n}{X}}$. 
Then there exists $\Ty'$ such that 
\begin{eqnarray}
& 
\label{eq:rec1}
\Gamma, \ii : \minus{\II},\X:\Ty'\sub{\ii}{\jj}  \vdash \QQ  \rhd
  \Ty'\sub{\ii+1}{\jj} \\
& 
\label{eq:rec2}
\derqq\Ga{}{P}{\Ty'\subst{0}{\ii}}\\ 
& 
\label{eq:rec3}
\Gamma\vdash \Pi \AT{\jj}{\II}.\Ty \RHD \Pi\AT{\jj}{\II}.\K
\end{eqnarray}
with 
$\Ty \equiv (\Pi\AT{\jj}{\II}.\Ty') \n+1 \equiv \Ty'\subst{\n+1}{\jj}$
and $\Ga{\models}{\n+1:\II}$. 
By Substitution Lemma (Lemma \ref{lem:substitution} (\ref{subs01})), 
noting $\Ga{\models}{\n: \minus{\II}}$,  
we have: 
$\Gamma, \X:\Ty'\sub{\ii}{\jj}\sub{\n}{\ii}  \vdash \QQ\sub{\n}{\ii}  \rhd
  \Ty'\sub{\ii+1}{\jj}\sub{\n}{\ii}$, 
which means that 
\begin{eqnarray}
\label{eq:subs}
\Gamma, \X:\Ty'\sub{\n}{\jj}  \vdash \QQ\sub{\n}{\ii}  \rhd
  \Ty'\sub{\n+1}{\jj} 
\end{eqnarray}
Then we use an induction on $\n$. \\[1mm]
{\em Base Case $\n=0$:} 
By applying Substitution Lemma (Lemma \ref{lem:substitution}
(\ref{subs02})) to  (\ref{eq:subs}) with (\ref{eq:rec2}), we have 
$\Gamma  \vdash \QQ\sub{1}{\ii}\sub{P}{X}  \rhd
  \Ty'\sub{1}{\jj}$.  \\[1mm]
{\em Inductive Case $\n\geq 1$:} 
By the inductive hypothesis on $\n$, 
we assume: 
$\derqq\Ga{}{\GR{P}{\ii}{X}{Q}\APP \n}{\Ty'\sub{\n}{\jj}}$. 
Then by applying Substitution Lemma (Lemma \ref{lem:substitution}) to
(\ref{eq:subs}) with this hypothesis, 
we obtain
$\Gamma\vdash \QQ\sub{\n}{\ii}\sub{\GR{P}{\ii}{X}{Q}\ \n}{X}  \rhd
 \Ty'\sub{\n+1}{\jj}$. \\[1mm]
\\[1mm]
{\bf Case [Init].}
$$
\sr\Ia{\p_0,..,\p_\n}{\y}{\PP}\redsym (\nu \s)(
        \PP\sub{\si\s {\p_0}}{\y} \pc s : \qbot \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
        \sj{\Ia}{\p_\n}{\s})
$$
We assume that
$\derqq{\Ga}{\emptyset}{\sr\Ia{\p_0,..,\p_\n}{\y}{\PP}}{\D}$. Inversion of
\tftrule{TInit} and \tftrule{TSub} gives that $\D'\leq\D$ and:
{\small
\begin{eqnarray}
& \forall i\neq 0, & \Gamma \proves \p_i\rhd \Nat\label{case-pi}\\
& & \Gamma \vdash \Ia:\mar{\G} \label{case-Ia}\\
& & \Gamma \models \pid(\G)=\{\p_0..\p_\n\} \label{case-pid}\\
& & \Gamma \vdash \PP \rhd \D', \y:\G \proj{\p_0} \label{case-PP}\\
\text{From~(\ref{case-PP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}),}
& & \derqq{\Ga}{}{\PP\sub{\si\s {\p_0}}{\y}}{\D', \si\s {\p_0}:\G \proj{\p_0}} \label{case-sub}\\
\text{\hspace{-3ex}From Lemma~\ref{lem:basic}~(\ref{lem:agreeEnv}) and \trule{QInit},}
& & \derqq{\Ga}{s}{s : \qbot}{\emptyset} \label{case-sbot}\\
\text{From (\ref{case-pi}), (\ref{case-Ia}), (\ref{case-pid}) and
  \tftrule{TReq},}
& \forall i\neq 0, & \Gamma \vdash \sj{\Ia}{\pp_i}{\s} \rhd \s[\pp_i]:\G \proj{\pp_i} \label{case-sppi}
\end{eqnarray}
}
% From~(\ref{case-PP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}), we have
% $\derqq{\Ga}{}{\PP\sub{\si\s {\p_0}}{\y}}{\D, \si\s {\p_0}:\G \proj{\p_0}}$ 

% From Lemma~\ref{lem:basic}~(\ref{lem:agreeEnv}) and \tftrule{QInit}, we
% have $\derqq{\Ga}{s}{s : \qbot}{\emptyset}$.

% From (\ref{case-pi}) and (\ref{case-Ia}) and (\ref{case-pid}), \tftrule{TJoin}
% gives us $\Gamma \vdash \sj{\Ia}{\pp_i}{\s} \rhd \s[\pp_i]:\G \proj{\pp_i}$ for
% $i$ between $1$ and $n$. 

Then \tftrule{TPar} on (\ref{case-sub}), (\ref{case-sbot}) and (\ref{case-sppi}) gives:
$$\Gamma \vdash \PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} %
\rhd \D', \s[\pp_0]:\G \proj{\pp_0}, ... , \s[\pp_n]:\G
\proj{\pp_n}
$$
From \trule{GInit} and \trule{GPar}, we have:
$$\Gamma \vdash _ s \PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} \pc s : \qbot%
\rhd \D', \s[\pp_0]:\G \proj{\pp_0}, ... , \s[\pp_n]:\G
\proj{\pp_n}
$$
From Lemma \ref{lem:mergeability} we know that $\coe{(\s[\pp_0]:\G \proj{\pp_0},
  ... , \s[\pp_n]:\G\proj{\pp_n})}{\s}$. We can then use \trule{GSRes} to get:
$$\Gamma \vdash _ \emptyset (\nu \s)(\PP\sub{\si\s {\p_0}}{\y} \pc \sj{\Ia}{\p_1}{\s} \pc ...\pc
\sj{\Ia}{\p_\n}{\s} \pc s : \qbot) \rhd \D'
$$
We conclude from % \trule{GInit}, \trule{GPar}, \trule{GSRes} and 
\tftrule{TSub}.
\\[1mm]
{\bf Case [Join].} 
$$
\sj{\Ia}{\pp}{\s} \pc \ssa\Ia{\pp}{\y}{\PP}\redsym 
        \PP\sub{\si \s {\p}}{\y}
$$
We assume that $\Gamma \vdash _{} \sj{\Ia}{\p}{\s} \pc \ssa\Ia{\p}{\y}{\PP}\rhd
\D$. Inversion of \tftrule{TPar} and \tftrule{TSub} gives that $\D=\D',\s[\pp]:\T$ and :
\begin{eqnarray}
& & \Gamma \vdash \sj{\Ia}{\pp}{\s} \rhd \s[\pp]:\G \proj{\pp}\label{case-Join-spp}\\
& & \T\geq\G\proj{\pp}\label{case-Join-subt}\\
& & \Gamma \vdash \ssa\uu\pp\y\PP \rhd \D'\label{case-Join-PP}\\
\text{By inversion of \tftrule{TAcc} from~(\ref{case-Join-PP})}
& & \Gamma \vdash \PP \rhd \D', \y:\G \proj{\pp}\label{case-Join-projPP}\\
\text{From~(\ref{case-Join-projPP}) and Lemma~\ref{lem:substitution}~(\ref{subs2}),}
& & \derqq{\Ga}{}{\PP\sub{\si\s {\p}}{\y}}{\D', \si\s {\p}:\G \proj{\p}} \label{case-Join-sub}
\end{eqnarray}

We conclude by \tftrule{TSub} from (\ref{case-Join-sub}) and
(\ref{case-Join-subt}).
\smallskip

\noindent{\bf Case [Send].} 
\[\red{\out{\si{\s}{\q}}{\va}{\p}{\PP} \Par \mqueue{\s}{\queue}}
    {\PP \Par \mqueue{\s}{\qtail{\valheap{\va}{\p}{\q}}}}\]
By inductive hypothesis, 
$\derqq{\Ga}{\Sigma}{\out{\si{\s}{\q}}{\e}{\p}{\PP} \Par
\mqueue{\s}{\queue}}{\D}$ with  
$\Sigma=\set{\s}$. Since this is derived by [GPar], we have:
\begin{eqnarray}
\der{\Ga}{\out{\si{\s}{\q}}{\va}{\p}{\PP}}{\D_1}\label{L21}\\
\derqq{\Ga}{\{s\}}{\mqueue{\s}{\queue}}{\D_2}\label{L22}
\end{eqnarray}
where $\D=\D_2\Dcomp\D_1$.
  From (\ref{L21}), we have
\begin{eqnarray}
\nonumber \D_1=\D_1',\si{\s}{\q}:\oT{\ptilde{\ST}}{\p};\T\label{L23}\\
\de\Ga{\va}{\ST}\label{L24}\\
\der\Ga\PP{\D_1',\si{\s}{\q}:\T}.\label{L25}
\end{eqnarray}
Using \trule{QSend} on (\ref{L22}) and (\ref{L24}) we derive
\begin{eqnarray}
\derqq{\Ga}{\{s\}}{ \mqueue{\s}{\qtail{
\valheap{\va}{\p}{\q}}}}{\D_2\Tcomp\set{ \si{\s}{\q} :
\oT{\SST}{\p}}}.\label{L26}
\end{eqnarray}
Using \trule{GInit} on (\ref{L25}) we derive
{\begin{eqnarray}
\derqq\Ga{\emptyset}\PP{\D_1',\si{\s}{\q}:\T}\label{L251}
\end{eqnarray}}
and then using \trule{GPar} on (\ref{L251}) and (\ref{L26}), we conclude
\begin{eqnarray*}
\derqq{\Ga}{\{\s\}}{\PP\pc\mqueue{\s}{\qtail{
\valheap{\va}{\q}{\p}}}}{(\D_2\Tcomp\set{\si{\s}{\q} :
\oT{\SST}{\p}})\Dcomp (\D_1',\si{\s}{\q}:\T)}.\label{L27}
\end{eqnarray*}

Note that $(\D_2\Tcomp\set{ \si{\s}{\q} : \oT{\SST}{\p}})\Dcomp
(\D_1',\si{\s}{\q}:\T){=}\D_2\Dcomp( \D_{1}',\si{\s}{\q} : \oT{\SST}{\p};\T).$

\medskip

\noindent{\bf Case [Recv].} 
\[ \inp{\sii}{\x}{\q}{\PP} \Par
\qpop{\valheaps{\va}{\set\p}{\q}} \redsym
\PP\subst{\ptilde{\va}}{\ptilde{\x}} \Par \s:\h\]
By inductive hypothesis, $\derqq{\Ga}{\Sigma}{\inp{\sii}{\x}{\q}{\PP} \Par
\qpop{\valheaps{\va}{\set\p}{\q}} }{\D}$ with $\Sigma=\set\s$.   
Since this is derived by [GPar], we have: 
\begin{eqnarray}
\der{\Ga}{\inp{\sii}{\x}{\q}{\PP}}{\D_1}\label{L31}\\
\derqq{\Ga}{\{\s\}}{\qpop{\valheaps{\va}{\p}{\q}}}{\D_2}\label{L32}
\end{eqnarray}
 
where $\D=\D_2\Dcomp\D_1$. From (\ref{L31}) we have
\begin{eqnarray}
\nonumber \D_1=\D_1',\si\s\p:\iT{\ptilde{\ST}}\q;\T\label{L33}\\
\der{\Ga,\ptilde{\x}:\ptilde{\ST}}\PP{\D_1',\si{\s}{\p}:\T}\label{L34}
\end{eqnarray}
From (\ref{L32}) we have
\begin{eqnarray}
\nonumber \D_2=\set{\siq :\oT{\SST'}{\p}}\Dcomp
 \D_2'\label{L36}\\
\derq{\Ga}{\stdqueue}{\D_2'}\label{L37}\\
 \de{\Ga}{\values}{\SST'}.\label{L38}
\end{eqnarray}
The coherence of $\D$ implies $\SST=\SST'$.
From (\ref{L34}) and (\ref{L38}), together with Substitution lemma, we obtain
$\der{\Ga}{\PP\subst{\ptilde{\va}}{\ptilde{\x}}}{\D_1',\si{\s}{\p}:\T}$, which implies by rule \trule{GInit}
\begin{eqnarray}
\derqq{\Ga}{\emptyset}{\PP\subst{\ptilde{\va}}{\ptilde{\x}}}{\D_1',\si{\s}{\p}:\T}.\label{L35}
\end{eqnarray}
Using rule \trule{GPar} on (\ref{L35}) and (\ref{L37}) we conclude
\begin{eqnarray*}
\derqq{\Ga}{\{\s\}}{\PP\subst{\ptilde{\va}}{\ptilde{\x}}\pc
\s:\h}{
 \D_2'\Dcomp(\D_1',\si{s}{\p}:\T}).\end
{eqnarray*}
Note that
${(\set{\siq :\oT{\SST}{\p}}\Dcomp
 \D_2')\Dcomp(\D_1',\s [\p]:\iT{\ptilde{\ST}}\q;\T)}~\Rightarrow{
 \D_2'\Dcomp(\D_1',\si{\s}{\p}:\T)}.$ 
% \\[1mm]
% {\bf Case [Branch]} 

% $$\lbranch{\sii}{\q} \Par \qpop{\labheap{l_{i_0
%     }}{\p}{\q}} \redsym \PP_{i_0 } \Par \mqueue{\s}{\queue} \quad (i_0
%   \in I)
% $$
% We assume $\Gamma \vdash _{}\lbranch{\sii}{\q} \Par
% \qpop{\labheap{l_{i_0}}{\p}{\q}}\rhd \D $. Inversion of \tftrule{TPar} and
% \trule{TSub} gives that $\D=(\D',\s[\pp]:\T_\pp) \Dcomp (\D'',\s[\qq]:\T_\qq)$ and :
% \begin{eqnarray}
% & & \Gamma \vdash \Pbranch{\si\s {\p}}{\q}\rhd \D',\si\s{\p}:\LbranchI{\q}{\T_i}{i}{I}
% \label{case-Branch-bra}\\
% & & \T_\pp\geq\LbranchI{\q}{\T_i}{i}{I}\label{case-Branch-bra-sub}\\
% & & \derq{\Ga}{\qpop{\labheap{l_{i_0}}{\p}{\q}}}{\D'',\siq :\LselI{\p}{\T'_j}{j}{J}}\label{case-Branch-sel}\\
% & & \T_\qq\geq\LselI{\p}{\T'_j}{j}{J}\label{case-Branch-sel-sub}\\
% \text{From \ref{}}
% \end{eqnarray}


% We use Lemma \ref{lem:mergeability} to get the existence of a global type
% $G$ such that $\Gamma \vdash T_i\geq\G \proj{\pp_i}$ and $\coe{(\D,
%   \s[\pp_0]:\T_o, ... , \s[\pp_n]:\T_n)}{\s}$. 



% \mbox{} \\[1mm]
% {\bf Case Link} We omit the hat from principals for a readability. 
% {\small
% \begin{center}
%          $\sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}
%         \pc..\pc\ssa\Ia{\p_1}{\y_1}{\PP_1}
%          \redsym (\nu \s)(\PP_{0}\sub{\si\s {\p_0}}{\y_{0}} \pc ...\pc
%         \PP_\n\sub{\si \s {\p_\n}}{\y_\n}\pc s : \emptyset)$.  
% \end{center}
% }
% \noindent Assume
% $\derqq{\Ga}{\Sigma}{
% \sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}\pc
% \ssa\Ia{\p_1}{\y_1}{\PP_1}\pc...\pc\ssa\Ia{\p_\n}{\y_\n}{\PP_\n}}{\D}$,
% then $\Sigma=\emptyset$ and
% \begin{eqnarray}
% & \der{\Ga}{\sr\Ia {\p_0..\p_\n}{\y_0}{\PP_0}}{\D_0'}\\
% & \der{\Ga}{\sr\Ia {\p_i}{\y_i}{\PP_i}}{\D_i'}\quad (1\leq i\leq \n)
% \label{L3}
% \end{eqnarray}
% where $\D =\bigcup_{i=0}^{\n} \D_i$ with $\D_i\geq \D_i'$.
% Then we have, by Lemma \ref{lem:mergeability}, 
% \begin{eqnarray}
% & & \nonumber \de\Ga \Ia{\an \G}\label{L4}\\
% & & \der{\Ga}{\PP_0}{\D_0',\y_0:T_0\quad \quad T_0\subT \pro{\G}{\p_0}\label{L5}}	
% \end{eqnarray}
% and  $\Gamma\proves \pid(G)=\{\p_0,...,\p_\n\}$.
% Next we have, again by Lemma \ref{lem:mergeability},  
% \begin{eqnarray}
% & & \nonumber \de\Ga \Ia{\an \G}\label{L6}\\
% & & \der\Ga{\PP_i}{\D_i',\y_i\ins T_i} \quad \quad T_i \leq \pro{\G}{\p_i} 
% \quad \quad (1\leq i\leq \n). 
% \label{L7}\end{eqnarray}
% Using Substation Lemma (Lemma \ref{lem:substitution} (4)) on (\ref{L5}) and (\ref{L7})
% \begin{eqnarray}
% \derq\Ga{\PP_i\sub{\si\s i}{\y_i}}{\D_i',\si{\s}{i}:T_i} \quad (1\leq
% i\leq n). \label{L8}\end{eqnarray}
% Using \trule{Conc} more times on (\ref{L8}) we have
% \begin{eqnarray}
% \der{\Ga}{\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}}{\bigcup_{i=0}^{\n} (\D_i',\si{\s}{i}:T_i
%         )}.\label{L9}\end{eqnarray}
% Note that
% \begin{eqnarray*}
% \bigcup_{i=0}^{\n} (\D'_i,\si{\s}{i}\ins T_i) \leq \D,\si{\s}{0}\ins\pro{\G}{\p_0},\ldots,\si{\s}{n}\ins\pro{\G}{\p_\n}\end{eqnarray*}
% Using \trule{GInit}, \trule{QInit}, \trule{GPar} and \trule{Subs} on (\ref{L9}) we have
% \begin{eqnarray}
% \derqq{\Ga}{\{\s\}}{\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}\pc s :
% \eq}{\D,\si{\s}{1}\ins\pro{\G}{\p_0},
% \ldots,\si{\s}{\n}\ins\pro{\G}{\p_\n}} \quad \quad \label{L10}
% \end{eqnarray}
% Using \trule{QScope} on (\ref{L10}) we have
% \begin{eqnarray}
% \derqq{\Ga}{\emptyset}{(\nu \s)(\PP_0\sub{\si\s 0}{\y_0} | ... |
%         \PP_\n\sub{\si\s \n}{\y_\n}\pc s : \eq)}{\D}\label{L11}
% \end{eqnarray}
% since 
% \[
% (\D,\si{\s}{0}\ins\pro{\G}{\p_0},\ldots,\si{\s}{\n}\ins
% \pro{\G}{\p_{\n}})\setminus {\s} = \D. 
% \]
%The proof of the communication rules uses the subtyping relation
%and the Substitution Lemma (\ref{lem:substitution} (\ref{subs1}),
%(\ref{subs2})), together with the subtyping rule for the extended mergeability
%(Lemma \ref{lem:mergeability}).
\end{proof}
\noindent 
Note that communication safety~\cite[Theorem 5.5]{CHY07}
and session fidelity~\cite[Corollary 5.6]{CHY07} 
are corollaries of the above theorem.  

A notable fact is,  
in the presence of the asynchronous initiation primitive, we can still obtain 
{\em progress} in a single multiparty session as in \cite[Theorem
5.12]{CHY07}, i.e.~if a program $P$ starts from one session, 
the reductions at session channels do not get a stuck.
Formally 
\begin{enumerate}
\item 
We say $P$ is {\em simple} if 
$P$ is typable and derived by  
$\Gamma \proves^\star P \rhd \Delta$ 
where the session typing in the premise and
the conclusion of each prefix rule
is restricted to at most a singleton. 
More concretely, (1) we eliminate $\Delta$ from 
\tfrule{TInit}, \tfrule{TAcc}, \tfrule{TOut}, \tfrule{TIn},
\tfrule{TSel} and \tfrule{TBra}, (2) we delete 
\tfrule{TDeleg} and \tfrule{TRecep}, 
(3) we restrict $\tau$ and $\Delta$ in 
\tfrule{TPRec}, \tfrule{TEq}, \tfrule{TApp}, \tfrule{TRec} and \tfrule{TVar}
contain at most only one session typing, and 
(4) we set $\Delta=\emptyset$  and $\Delta'$ contains 
at most only one session typing; or vice-versa in \tfrule{TPar}. 
\item 
We say $P$ is {\em well-linked} when for
each $P \redsym^\ast Q$, whenever $Q$ has an active prefix whose subject is
a (free or bound) shared channels, then it is always reducible. 
This condition eliminates the element 
which can hinder progress is when interactions
at shared channels cannot proceed. See \cite[\S~5]{CHY07} more detailed
definitions. 
\end{enumerate}
The proof of the following theorem 
is essentially identical with \cite[Theorem 5.12]{CHY07}.

\begin{THM}[Progress]
\label{thm:progress}
If $P$ is well-linked and without any
element from the runtime syntax and 
	$\Gamma \vdash^\star P \rhd \emptyset$. 
Then for all $P\redsym^\ast Q$, either $Q\equiv \inact$ or 
$Q\redsym R$ for some $R$. 
\end{THM}

%% \paragraph{\bf Another formulation of progress}
%% The well-linkedness condition for progress can be replaced 
%% by the following definition (from \cite{BettiniCDLDY08LONG}) 
%% if we assume processes have no shared name restrictions.
%% The alternative definition of a progress below says that a process has
%% the progress property if it can never reach a deadlock state,
%% i.e., if it never reduces to a process which contains open sessions
%% (this amounts to containing session channels) and which is
%% irreducible in any inactive context (represented by another
%% inactive process running in parallel).

%% \begin{DEFINITION}{\rm (Progress)}\ 
%% We say process $P$ has the {\em progress property} if 
%% $P\redsym^\ast P'$ implies that either (1) 
%% $P'$ does not contain open session channels or
%% (2) $P'|Q$ for some $Q$ 
%% such that $P'|Q$ is well-typed and $Q\not \redsym$. 
%% \end{DEFINITION}
%% If we consider processes without shared name restriction, 
%% this alternative progress definition 
%% works since we can always compose external init or accept processes ($Q$ in 
%% the above definition). 
%% The following alternative progress theorem can then be 
%% proved as in the above theorem.   

%% \begin{THM} {\rm (Progress)}\ 
%% Suppose $\Gamma \proves^\star P \rhd \Delta$. Assume $P$ does 
%% not contain shared name restrictions. 
%% Then $P$ satisfies the progress property. 
%% \end{THM}
%% These constranits (for $\proves^\star$ and no shared name restriction) 
%% can be deleted if we introduce the interaction typing system in
%% \cite{BettiniCDLDY08LONG}:  
%% we believe a stronger 
%% progress property for interleaved multiparty sessions 
%% ensured by the interaction typing in \cite{BettiniCDLDY08LONG} 
%% can be obtained in this framework, too (since our
%% typing system is an extension from 
%% the communication system in \cite{BettiniCDLDY08LONG}).

%% %can be also obtained by a similar method as the one found in~\cite{CHY07}.



==> syntax.tex <==
\section{Types and processes for parameterised multiparty sessions}
\label{sec:syntax_and_example}
\input{global_types}

\input{examples}

\input{all_syntax}

\input{semantics}

\input{process_example}

% FFT over a butterfly network
\input{fft}




==> termination.tex <==
%\section{Formal results}
\label{sec:subjectreduction}
\subsection{Termination of equality checking and type checking} 
\label{subsec:termination}
This subsection proves the termination of the type-checking 
(we assume that we use the type equality rules in Figure~\ref{fig:type-wf}).  
%This subsection proves the termination of the type-checking. 
%First we prove the termination of the type-checking. 
\noindent Ensuring termination of type-checking with dependent types is not an
easy task since type equivalences are often derived from term equivalences.  We
rely on the strong normalisation of System $\mathcal{T}$
\cite{GirardJY:protyp} for the termination proof.
 
\begin{PROP}[Termination and confluence]
\label{prop:SNconfluent}
The reduction relation $\redsym$ on global and end-point types 
(i.e. $\G\redsym \G'$
and $\T\redsym \T'$ for closed types in Figure \ref{fig:globalreduction}) 
are strong normalising and confluent on well-formed kindings. 
More precisely, 
if $\Gamma\proves G \RHD \K$, then there exists a unique term 
$G'= \WHNF{G}$ such that $G \redsym^\ast G'\not\redsym$. 
%Similarly 
%the relation $\redsym$ on global and end-point types 
%(i.e. $\G\redsym \G'$
%and $\T\redsym \T'$ for open types which reduce under 
%recursive prefixes, abstractions and recursors) 
%are strong normalising and confluent on well-formed kindings. 
%
%\item (Terms) \ Suppose the syntax does not include the definition agents. 
%Then the relation $\redsym$ on the 
%processes are strong normalising on well-formed types. 
%\end{itemize}
\end{PROP}
\begin{proof}
By strong normalisation of System $\mathcal{T}$ \cite{GirardJY:protyp}. 
For the confluence, we first note that the reduction relation on 
global types defined in Figure~\ref{fig:globalreduction} 
and on expressions with the first-order operators in the types 
is {\em deterministic}, i.e. if $\G\redsym \G_i$  
by rules in Figure~\ref{fig:globalreduction}, then $\G_1=\G_2$. 
Hence it is locally confluent, i.e. if  $\G\redsym \G_i$ ($i=1,2$) then 
$\G_i\redsym^\ast \G'$. Then we achieve the result
by Newman's Lemma. The second clause is a direct consequence 
from the fact that $\redsym$ coincides with the head reduction.
\end{proof}

%\input{simple_termination}
\input{long_termination}

\begin{PROP}[Termination for type equality checking]
\label{pro:equiv-termination}
Assuming that proving \\
the predicates 
$\Gamma\models \PRED$ 
appearing in type equality derivations is decidable,  
then type-equality checking of $\Gamma\proves G \equiv G'$
terminates. 
Similarly for other types. 
\end{PROP}
\begin{proof} 
By Lemma \ref{lem:size} and termination 
of kinding and well-formed environment checking.
\end{proof}

%Note that we do not require to prove the termination of 
%process reduction since term (process) equivalence is 
%not used in our typing rules (cf.~\cite{DBLP:conf/popl/XiP99}). 

We first formally define annotated processes which are processes 
with explicit type annotations for bound names and variables (see \S~\ref{par:annotated}). 
\begin{center}
\begin{tabular}{rcl}
 \PP  & ::= & \sr\uu{\p_0,..,\p_\n} {\AT{\y}{T}}\PP   
      \sep  \ssa\uu\p{\AT{\y}{T}}\PP   
      \sep  \Pin{\ccc}{\p}{\AT{\x}{T}}{\PP} 
      \sep  \nuc{\AT{a}{\ENCan{G}}}\PP\\[1mm]
      & \sep & $\mu \AT{X}{\tau}.\PP$ 
      \sep  $\RECSEQP{\PP}{\AT{\ii}{\II}}{\X}{\QQ}$ 
      \sep  $\X^\tau$ \\
\end{tabular}
\end{center}

\begin{THM}[Termination of type checking]
\label{thm:termination}
Assuming that proving the 
predicates $\Gamma\models \PRED$ appearing in kinding, 
equality, projection and typing derivations  
is decidable, 
then type-checking of annotated process $P$, i.e. 
$\Gamma\proves P\rhd \emptyset$ terminates. 
\end{THM}
\begin{proof} 
First, it is straightforward to show that 
kinding checking, well-formed environment checking and 
projection are decidable 
as long as deciding the predicates
$\Gamma\models \PRED$ appearing in the rules 
is possible. 

Secondly, we note that by the standard argument from indexed dependent types 
\cite{DependentBook,DBLP:conf/popl/XiP99}, 
for the dependent $\lambda$-applications (\tftrule{TApp} in Figure~\ref{fig:process-typing1}), we do not require 
equality of terms (i.e.~we only need the equality 
of the indices by the semantic consequence judgements). 

Thirdly, by the result from \cite[Corollary 2, page 217]{GH05}, 
the type isomorphic checking $\tau \WB \tau'$ terminates so that 
the type isomorphic checking 
in $\tftrule{Tvar}$ in Figure~\ref{fig:process-typing1} 
(between $\tau$ in the environment and 
$\tau'$ of $X^{\tau'}$) always terminates. 

Forth, it is known that type checking for annotated 
terms with session types terminates with subtyping 
\cite[\S~5.2]{GH05} and multiparty session types \cite{CHY07}. 

Hence the rest of the proof consists in eliminating the type equality rule
$\tftrule{Teq}$ in order to make the rules syntax-directed.    
We include the type equality check into 
$\tftrule{TInit,TReq,TAcc}$ 
(between the global type and its projected session
type), the input rules $\tftrule{TIn,TRecep}$ (between the session type 
and the type annotating $x$), 
$\tftrule{TRec}$ 
(between the session type and the type annotating $X$),   
and 
$\tftrule{TRec}$ 
(between the session type and the type annotating $X$ in $\Gamma$).  
We show the four syntax-directed rules. 
The first rule is the initialisation. 
\[ 
\begin{prooftree}
{
\begin{array}{@{}c@{}}
\Gamma \vdash \uu:\mar{\G} \quad 
\Gamma \vdash \PP \rhd \D, \y:T
\quad \Gamma \vdash \G \proj{\p_0} \equiv T\\[1mm]
\Gamma \proves \p_i\rhd \Nat \quad 
\Gamma \models \pid(\G)=\{\p_0..\p_\n\}\\[1mm]
\end{array}
}
\justifies
{\Gamma \vdash \sr\uu{\p_0,..,\p_\n} \y\PP \rhd \D} 
\using\tfrule{TInit}
\end{prooftree}
\]
Then it is straightforward to check 
$\Gamma \vdash \uu:\mar{\G}$ terminates.  
Checking $\Gamma \vdash \PP \rhd \D, \y:T$ also terminates by inductive
hypothesis. 
Checking $\Gamma \vdash \G \proj{\p_0} \equiv T$ terminates 
since the projection terminates and 
checking $\alpha \equiv \beta$ (for any type $\alpha$ and $\beta$) 
terminates by Lemma \ref{lem:size}.
Checking $\Gamma \proves \p_i\rhd \Nat$ terminates since 
the kinding checking terminates. Finally 
checking $\Gamma \models \pid(\G)=\{\p_0..\p_\n\}$ terminates 
by assumption. 

The second rule is the session input. 
\[
\begin{prooftree}
{\Gamma \vdash \PP\rhd \D,\ccc:\T,\y:\T' \quad 
\Gamma\proves T_0\equiv \T'}
\justifies
{\Gamma \vdash \Pin{\ccc}{\p}{\AT{\y}{T_0}}{\PP}\rhd \D,\ccc:\Lin{\p}{\T'}{\T}}
\using\tfrule{TRecep}
\end{prooftree}
\]
Then checking $\Gamma \vdash \PP\rhd \D,\ccc:\T,\y:\T'$ terminates by 
inductive hypothesis and checking $\Gamma\proves T_0\equiv \T'$ 
terminates by Lemma \ref{lem:size}.

The third and forth rules are recursions. 
\[
\begin{prooftree}
{\Gamma, \X:\Ty \vdash P \rhd \Ty' \quad \Gamma\proves \Ty \equiv \Ty'}
\justifies
{\Gamma \vdash \mu{\AT{\X}{\Ty}}.P \rhd \Ty'} \using\tfrule{TRec}
\end{prooftree}
\begin{prooftree}
{\Gamma, \X:\Ty \vdash \Env \quad \Gamma\vdash \Ty \WB \Ty' \quad 
\Gamma\vdash \Ty' \equiv \Ty_0}
\justifies
{\Gamma, \X:\Ty \vdash \X^{\Ty'} \rhd \Ty_0} 
\using\tfrule{TVar}
\end{prooftree}
\]
In \tftrule{TRec}, we assume $P\not = X$ (such a term is meaningless). 
Then \tftrule{TRec} terminates by inductive hypothesis 
and Lemma \ref{lem:size}, while \tftrule{TVar} terminates 
by termination of isomorphic checking (as said above) 
and Lemma \ref{lem:size}. 

Other rules are similar, hence we conclude the proof. 
\end{proof}
% Notice that the projection of $G$ on $\participant{p}$ is always 
% decidable if the equality on principals is decidable. 
To ensure the termination of $\Gamma\models \PRED$, possible solutions include
the restriction of predicates to linear equalities over natural numbers without
multiplication (or to other decidable arithmetic subsets) or the restriction of
indices to finite domains, cf.~\cite{DBLP:conf/popl/XiP99}.


==> typing.tex <==
\section{Typing parameterised multiparty interactions}
\label{sec:typing}
\noindent 
This section introduces the type system, by which we can statically type
parameterised global specifications.

\subsection{End-point types and end-point projections}
\label{subsec:endpoint}
\input{fig_local}
\noindent 
A global type is projected to an {\em end-point type} according to each
participant's viewpoint.
%The first key challenge is to define a projection 
%from a global type to the end-point types 
%of individual participants, whose identities and numbers 
%might only be known at runtime. 
The syntax of end-point types is given in 
Figure~\ref{fig:local}. 
{\rm Output} expresses the sending to
$\p$ of a value or channel
of type \UT, followed by the interactions \T.
{\rm Selection} represents the transmission to 
$\p$ of a label $l_k$ chosen in $\{l_k\}_{k\in K}$ 
followed by $\T_k$. 
{\rm Input} and {\rm branching} are their dual counterparts.
The other types are similar to their global versions.
% We use the following macro encoded by a recursor. 
% \[ 
% \begin{array}{rcl}
% (\IF\ \tii \ \THEN\ \T_1 \ \ELSE \ \T_2) \quad =
% \quad \GR{T_1}{\ii}{\xx}{T_2}{\ \tii}
% \end{array}
% \]
% where $\ii$ and $\xx$ are not free in $T_2$. \true is encoded by $0$ and \false
% by any other integer. 

\paragraph{\bf End-point projection: a generic projection}
The relation between end-point types and global types is formalised by the projection
relation. 
Since the actual participant characteristics might only be determined at
runtime, we cannot straightforwardly use the definition
from~\cite{CHY07,BettiniCDLDY08LONG}.  %
Instead, we rely on the expressive power of the primitive recursive operator:
{\em a generic end-point projection of \G\ onto \q}, written \pro\G\q,
represents the family of all the possible end-point types that a principal $\q$ can
satisfy at run-time. %
% Intuitively, we wish to ensure:
% \begin{quote}
% if $T$ is semantically equivalent up to the generic
% end-point generator, 
% and if $P$ conforms to $T$, then $P$ is type-safe. 
% \end{quote}
% where semantically equivalent might be 
% the $\beta$-equality or some form of contextual congruence 
% (the equivalence relation is defined formally in \S~\ref{subsec:teq}). 

\input{fig_projection}

The general endpoint generator is defined in Figure~\ref{fig:projection} using
the derived condition construct $\Pifthenelse{\_}{\_}{\_}$.  The projection
$\GS{\p}{\p'}{\U}.\G\proj{\qq}$ leads to a case analysis: if the participant
$\q$ is equal to $\p$, then the end-point type of $\q$ is an output of type $\U$
to $\p'$; if participant $\q$ is $\p'$ then $\q$ inputs $U$ from $\p'$; else we
skip the prefix. The first case corresponds to the possibility for the sender
and receiver to be identical.  
Projecting the branching global type is similarly
defined, but for the operator $\sqcup$ explained below. For the other cases (as
well as for our derived operators), the projection is homomorphic.
We also identify $\mu \xx.\xx$ as $\End$ ($\mu \xx.\xx$
is generated when a target participant is not included 
under the recursion, for example, $\GS{\p}{\p'}{\U}.\mu
\xx.\GS{\q}{\q'}{\U}.\xx\proj{\p}=\Lout{\p}{\U}{\mu \xx.\xx}$) 
and $\mu \xx.T$ as $T$ if $\xx\not\in \ftv({T})$.

\paragraph{\bf Mergeability of branching types} 
We first recall the example from~\cite{CHY07}, which explains that
na\"ive branching projection leads to inconsistent end-point types. 

{\small
$$
\begin{array}{lll}
\TO{\W[0]}{\W[1]}: & \{\mathsf{ok}:\TO{\W[1]}{\W[2]}:\ENCan{\Bool}, %\\
                     & \ \mathsf{quit}:\TO{\W[1]}{\W[2]}:\ENCan{\Nat}\}
\end{array}
$$}

% The usual projection of the following global type is {\em undefined}.
We cannot project the above type onto $\W[2]$ because, while the branches behave
differently, $\W[0]$ makes a choice without informing $\W[2]$ who thus cannot
know the type of the expected value. 
% , regardless of the choice made
% by $\W[0]$, $\W[2]$ does not know its outcome while the branches do not behave in the same way while $\W[2]$ is not
% aware of the chosen branch and thus cannot know the type of the expected value.
A solution is to define projection only when the branches are identical, i.e. we change the above $\Nat$ to
$\Bool$ in our example above. % , the
% projection of $\W[2]$ would then work and be defined as
% $\Lin{\W[2]}{\Bool}{\End}$.
% have all the branches be identical.
% This illustrates the fact that the projection of all branches is required to be
% identical.
% except for the principals involved (which do
% not appear in end-point types)
% (i.e.~$G_0\proj{\qq}=G_j\proj{\qq}$ for the case of $\qq\not=\p,\p'$ as defined
% in \cite{CHY07,BettiniCDLDY08LONG}).

In our framework, this restriction is too strong since each branch may contain
different parametric interaction patterns.  To overcome this, below we propose
a method called {\em mergeability} of branching types.\footnote{The idea of mergeability is introduced informally 
in the tutorial paper  \cite{Tutorial09}.}
\begin{DEFINITION}[Mergeability] \rm
\label{def:mergeability}
%Formally, 
The mergeability relation $\mergeop$ is the smallest congruence relation over 
end-point types such that:% ; the present paper states the 
% formal properties and proofs
% if 
%$\forall i\in (K \cap J). T_k\mergeop T_j'$ and 
%$\forall i\in (K \setminus J)\cup (J \setminus K).l_k \not = l_j$, 
%then 
%${\Lbranch{\p}{\T_k}\mergeop 
%\&\langle\p,\{l_j:T_j'\}_{j\in J}\rangle}$.
%\end{prooftree}
$$
\begin{prooftree}
{\forall i\in (K \cap J). T_i\mergeop T_i' \quad 
\forall k\in (K \setminus J), \forall j.(J \setminus K).l_k \not = l_j
}
\justifies 
{\langle\p,\{l_k:T_k\}_{k\in K}\mergeop 
\&\langle\p,\{l_j:T_j'\}_{j\in J}\rangle
}
\end{prooftree}
$$
When $T_1\mergeop T_2$ is defined, 
we define the operation $\mergecup$ as a partial commutative 
operator over two  types such that $T\mergecup T=T$ for all types and that:
\[
\begin{array}{lll}
\Lbranch{\p}{\T_k}\mergecup 
\&\langle\p,\{l_j:T_j'\}_{j\in J}\rangle \ = \\ 
\quad \&\langle\p,\{l_i:T_i\mergecup T_i'\}_{i\in K\cap J}
\cup \{l_k:T_k\}_{k\in K\setminus J}
\cup \{l_j:T_j'\}_{j\in J\setminus K}\rangle\\[1mm]
\end{array}
\]
and homomorphic for other types (i.e. 
$\mathcal{C}[T_1] \sqcup \mathcal{C}[T_2]=\mathcal{C}[T_1\sqcup
T_2]$ where $\mathcal{C}$ is a context for local types). 
\end{DEFINITION}
The mergeability relation states that two types are identical up to their
branching types where only branches with distinct labels are allowed to be
different.  By this extended typing condition, we can modify our previous global
type example to add $\mathsf{ok}$ and $\mathsf{quit}$ labels to notify
$\W[2]$. We get:

{\small\[
\begin{array}{llll}
\TO{\W[0]}{\W[1]}:& \{\mathsf{ok}:\TO{\W[1]}{\W[2]}:
\{ \mathsf{ok}:\TO{\W[1]}{\W[2]}\ENCan{\Bool} \ \}, \\
&\
\mathsf{quit}:\TO{\W[1]}{\W[2]}:\{\mathsf{quit}:\TO{\W[1]}{\W[2]}\ENCan{\Nat}\}\}\}
\end{array}
\]}

%where $l:\ENCan{U}$ means 
%$l:\TO{\W[1]}{\W[2]}\ENCan{U}$ above.  
Then $\W[2]$ can have the type $\&\ENCan{\W[1], \ \{
  \mathsf{ok}:\ENCan{\W[1],\Bool}, \ \mathsf{quit}:\ENCan{\W[1],\Nat} \}}$ which
could not be obtained through the original projection rule
in~\cite{CHY07,BettiniCDLDY08LONG}.
%
This projection is sound 
%consistent up to subtyping between
up to branching subtyping 
(it will be proved in Lemma \ref{lem:mergeability} later).
%and use this fact to prove type-safety. 

\subsection{Type system (1): environments, judgements and kinding}
\noindent 
This subsection introduces the environments and kinding systems. 
Because free indices appear both in terms (e.g.
participants in session initialisation) and in types, the formal definition of
what constitutes a valid term and a valid type are interdependent and
both in turn require a careful definition of a valid global type.
%Although some techniques developed for
%the $\lambda$-calculus are useful, 
% Other contributions include typing a recursor and session initialisations with 
% a general end-point generator for growing topologies. 

\paragraph{\bf Environments}
One of the main differences with previous session type systems is that session
environments $\Delta$ % can now be applied to indices and
can contain dependent {\em process types}.  The grammar of environments, process
types and kinds are given below.
\begin{center}
\small
\begin{tabular}{ll}
\begin{tabular}{rcl@{\quad}l}
\D & ::= & $\emptyset$ \sep \D, \ccc:\T\\[1mm]  
%\Ty & ::= & \D \sep $\GR{\Ty}{\AT{\ii}{\II}}{\xx}{\Ty'}\sep \Pi
%\AT{\ii}{\II}.\Ty \sep \Ty\APP\tii \sep \xx$\\[1mm]
%%\Ty & ::= & \D \sep $\Pi \AT{\ii}{\II}.\Ty  $\\[1mm] % \sep \Ty\APP\tii
\end{tabular}
&
\begin{tabular}{rcl@{\quad}l}
$\Gamma$ & ::= & $\emptyset \sep\Gamma, \PRED \sep \Gamma, u:\ST \sep 
\Gamma, \ii:\II \sep \Gamma, \X:\Ty$
\quad 
$\Ty \ ::= \ \D \sep \Pi \AT{\ii}{\II}.\Ty$\\
%\K & ::= &  \GType \sep \SType \sep \PRType  \sep  \LType \sep \PType 
%\sep  $\Pi\AT{\ii}{\II}.\K$ 
\end{tabular}
\end{tabular}
\end{center}
$\D$ is the {\em session environment} 
which associates
channels to session types. 
$\Ga$ is the {\em standard environment}
which contains predicates and which associates variables to sort types, service names to global
types, indices to index sets and process variables 
to session types. 
$\Ty$ is a {\em process type} which 
is either a session environment or a 
%recursor,\footnote{The extended
%abstract has omitted the recursor for simplicity: the examples 
%are typable without recursors for the process types} 
dependent type. 
%$\K$ denotes {\em kinding} which includes the kind of proper
%types for global, value, principal, end-point and process types, or the kind of type
%families.  
We write $\Ga,\uu:S$ only if $\uu\not\in\dom{\Gamma}$ 
where
$\dom{\Gamma}$ denotes the domain of $\Gamma$.  
We use the same convention for others.

\begin{figure*}
\center
\begin{tabular}{lllllllll}
$\Ga \proves \Env$ & \quad\quad & well-formed environments\\%[1mm] 
$\Ga \proves \kappa$ & \quad \quad& well-formed kindings\\%[1mm]
$\Ga \proves \alpha\RHD \kappa$ & \quad\quad & well-formed types\\%[1mm]
$\Ga \proves \alpha\equiv \beta$ & \quad\quad & type
equivalence\\%[1mm]
\end{tabular}\quad 
\begin{tabular}{lllllllll}
$\Ga \proves \alpha\WB \beta$ & \quad\quad & type isomorphism\\%[1mm]
$\Ga \proves \e \rhd U$ & \quad\quad & expression\\%[1mm]
$\Ga \proves \p \rhd \ParT$ & \quad\quad & participant \\%[1mm]
$\Ga \proves \PP \rhd \tau$ & \quad\quad & processes\\%[1mm]
\end{tabular}
\caption{Judgements ($\alpha,\beta,...$ range over any types)}\label{fig:judgements}
\end{figure*}

% \begin{center}
% \begin{tabular}{llllll}
% $\Ga \models \PRED$ & \quad \quad& predicate $\PRED$ is a consequence of $\Gamma$\\
% $\Ga \models \tii : I$ & \quad\quad & $\tii : I$ follows from the assumptions 
% of $\Ga$ 
% \end{tabular}
% \end{center}
% \noindent 
\paragraph{\bf Judgements}
Our type system uses the judgements listed in
Figure~\ref{fig:judgements}.

Following \cite{DBLP:conf/popl/XiP99},  we assume given in the typing rules two
semantically defined judgements: $\Ga \models \PRED$ (predicate $\PRED$ is a
consequence of $\Gamma$) and $\Ga \models \tii : I$ ($\tii : I$ follows from the
assumptions of $\Ga$).

We write $\Gamma \proves \judg$ for arbitrary judgements and 
write $\Gamma \proves \judg,\judg'$ to stand for both 
$\Gamma \proves \judg$ and $\Gamma \proves \judg'$. 
In addition, we use two additional judgements for 
the runtime systems (one for queues $\derq{\Ga}{\stdqueue}{\D}$ and one for 
runtime processes $\derqq{\Ga}{\Sigma}{\PP}{\D}$) which are similar with those 
in \cite{BettiniCDLDY08LONG} and listed in the Appendix. 
We often omit $\Sigma$ from $\derqq{\Ga}{\Sigma}{\PP}{\D}$ if it is
not important.
% ; they are not the main focus 
% of this paper, hence are omitted. 
%The full rules are listed in the Appendix. 
%
% \begin{figure}
% \center
% \begin{tabular}{lllllllll}
% $\Ga \proves \Env$ & \quad\quad & well-formed environments\\%[1mm] 
% $\Ga \proves \kappa$ & \quad \quad& well-formed kindings\\%[1mm]
% $\Ga \proves \alpha\RHD \kappa$ & \quad\quad & well-formed types\\%[1mm]
% $\Ga \proves \alpha\equiv \beta$ & \quad\quad & type equivalence\\%[1mm]
% $\Ga \proves \alpha\WB \beta$ & \quad\quad & type isomorphism\\%[1mm]
% $\Ga \proves \e \rhd U$ & \quad\quad & expression\\%[1mm]
% $\Ga \proves \p \rhd \ParT$ & \quad\quad & participant with 
% $\ParT :: = \Nat \sep \Pi\AT{\ii}{\II}.{U_p}$\\%[1mm]
% $\Ga \proves \PP \rhd \tau$ & \quad\quad & processes\\%[1mm]
% \end{tabular}
% \caption{Judgements ($\alpha,\beta,...$ range over any end-point or global type)}\label{fig:judgements}
% \end{figure}
%
%%\paragraph{Kinding}
%A term $\tii$ in the index syntax is well-formed 
%in $\Gamma$ if the set of free index variables in $\tii$ is 
%a subset of the set of the index variables in $\Gamma$. 
%For contexts, we assume that no variable is bound 
%more than once and that the free index variables appearing in 
%$\ii:\II$ and $\PRED$ are declared earlier in the context. 

\paragraph{\bf Kinding}
%\label{app:kind}
The definition of kinds is given below: 
\[
\begin{array}{l}
\kappa ::= \Pi \jj:I.\kappa \sep \Type 
\quad \quad \quad 
%\sep \SType \sep \PRType \sep \LType \sep \PType\quad 
\ParT :: = \Nat \sep \Pi\AT{\ii}{\II}.{U_p}\\
\end{array}
\]
We inductively define well-formed types using a 
kind system. The judgement $\Gamma\vdash \alpha \!\RHD\!
\kappa$ means type $\alpha$ has kind $\kappa$.  Kinds include
%% $\K$ denotes {\em kinding} which includes the kind of 
proper types for global, value, principal, end-point and process types (denoted
by $\Type$), and the kind of type families, written by $\Pi\AT{\ii}{\II}.\K$.
%\begin{figure}[h!]
%\center
%\caption{Kinds}\label{fig:kindsgrammar}
%\end{figure}
%
The kinding rules are defined in 
Figure~\ref{fig:kindsystembase} 
and Figure~\ref{fig:kind_all} 
in this section and 
Figure~\ref{fig:localkindsystem} in the Appendix.
The environment well-formedness rules are in Figure
\ref{fig:wellformed_env}. 

The kinding rules for types, value types, principals, index sets and
process types are listed in  Figure~\ref{fig:kind_all}.  
In \trule{KMar} in the value types, $\ftv(G)$ denotes a set of 
free type variables in $G$. The condition $\ftv(G)=\emptyset$ 
means that shared channel types are always closed. 
Rule \trule{KIndex} forms the index 
sort which contains only natural number (by the condition $0\leq i$). 
Other rules in Figure~\ref{fig:kind_all} and the rules in 
Figure~\ref{fig:wellformed_env} are standard.   

We next explain the global type kinding rules from
Figure~\ref{fig:kindsystembase}. 
The local type kinding in Figure~\ref{fig:localkindsystem}
in Appendix is similar. 

Rule \trule{KIO} states that if both participants have $\Nat$-type,  
that the carried type $\U$ and the rest of the global type $\G'$ 
are kinded by $\Type$, and that $\U$ does not contain any free type variables, 
then the resulting type is well-formed. This prevents these types from being
dependent. The rule \trule{KBra} is similar, while rules \trule{KRec,KTVar} are
standard.  

Dependent types are introduced when kinding recursors
in \trule{KRcr}.  
% and abstractions in \trule{Kpi}. 
In \trule{KRcr}, we need an updated index range for $\ii$ in the premise $\Gamma,
\ii:\II^- \vdash \G' \RHD \Type$ since the index substitution uses the
predecessor of $\ii$. We define $\minus\II$ using the abbreviation 
$[0..\tjj]  =  \CONSTRAINT{\ii}{\Nat}{\ii\leq \tjj}$:
\begin{center}
${}\qquad \qquad \qquad \minus{[0..0]}  =  \emptyset 
\quad \text{and}\quad \minus{[0..\tii]}  = [0..\tii-1] 
$
\end{center}
Note that the second argument ($\lambda {\AT{\ii}{\II^-}}.\lambda
{\xx}.{\G'}$) is closed (i.e. it does not contain 
free type variables).
We use \trule{KApp} for both index applications. 
Note that \trule{KApp} checks whether the argument $\tii$ satisfies 
the index set $\II$.
Other rules are similarly understood including those 
for process types (noting $\Delta$ is a well-formed environment 
if it only contains types $T$ of kind $\PType$). 

\input{fig_kind_system}

\input{fig_kind_global}

\subsection{Type system (2): type equivalence}
Since our types include dependent types and recursors, 
we need a notion of type equivalence. 
We extend the standard method of \cite[\S2]{DependentBook} with the
recursor. 
The rules are found in Figure~\ref{fig:type-wf} and applied 
following the order appeared in Figure~\ref{fig:type-wf}.   
For example, % \trule{WfBase} has a higher priority than 
% \trule{WfApp}, and
\trule{WfRec} has a higher priority than 
\trule{WfRecF}. 
We only define the rules for $G$.   
The same set of rules can be applied to $T$ and $\tau$. 

Rule \trule{WfBase} 
is the main rule defining $\G_1\equiv\G_2$ and relies on the
existence of a common weak head normal form  for the two types. 

Rules \trule{WfIO} and \trule{WfBra} say if 
subterms are equated and each type satisfies the kinding rule, 
then the resulting global types are equated. 

Rule \trule{WfPRec} says the two recursive types 
are equated only if the bodies are equated. 
Note that we do not check whether unfolded recursive types are 
equated or not. 

Rule \trule{WfRVar} and \trule{WfEnd} are the base cases. 

Two recursors are equated if either (1) 
each global type subexpression is equated by $\equiv$ 
(rule \trule{WfRec}), or if not, 
(2) they reduce to the same normal forms when applied to a finite
number of indices (rule \trule{WfRecF}). 
Note that rule \trule{WfRec} has a higher priority 
than rule \trule{WfRecF} (since it is more efficient without 
reducing recursors). If $\GR{\G_1}{\AT{\ii}{\II}}{\xx}{\G_1'}
\equivwf \GR{\G_2}{\AT{\ii}{\II}}{\xx}{\G_2'}$ 
is derived by applying \trule{WfRec} under finite $I$, 
then the same equation can be derived using \trule{WfRecF}. 
Thus, when the index range is finite, 
\trule{WfRec} subsumes \trule{WfRecF}. On the other hand, 
\trule{WfRec} can be used for infinite index sets. 

Similarly, \trule{WfBase} is staged with \trule{WfApp} to ensure that 
the premise of \trule{WfRecF} always matches with \trule{WfBase}, 
not with \trule{WfApp} 
(it avoids 
the infinite application of rules \trule{WfRecF} and \trule{WfApp}).  
A use of these rules are given in the examples later. 
Other rules are standard. 

\input{fig_type_wf} 
\input{fig_meta}

\paragraph{\bf Type equivalence with meta-logic reasoning}
The set of rules in Figure~\ref{fig:type-wf} are designed with algorithmic
checking in mind (see \S~\ref{subsec:termination}). In some examples, in order
to type processes with types that are not syntactically close, it is
interesting to extend the equivalence classes on types, at the price of the
decidability of type checking.

We propose in Figure~\ref{fig:meta-equivalence} an additional equivalence rule
that removes from rule \trule{WfRecF} the finiteness assumption on $\II$. It
allows to prove the equivalence of two recursor-based types if it is possible to
prove meta-logically that they are extensionally equivalent. This technique can
be used to type several of our examples (see \S~\ref{subsec:typingexample}).

\subsection{Typing processes}
\input{fig_process_typing}

We explain here (Figure~\ref{fig:process-typing1}) the 
typing rules for the initial processes. 
Rules \tftrule{TNat} and \tftrule{TVari} are
standard. Judgement $\Gamma\proves \Env$ (defined in Figure
\ref{fig:wellformed_env}) in the premise 
means that $\Gamma$ is well-formed. 
For participants, we check their typing by \tftrule{TId} and \tftrule{TP}
in a similar way as~\cite{DBLP:conf/popl/XiP99}.  
Rule \tftrule{TPRec} deals with the
changed index range within the recursor body. More precisely, we first check
$\tau$'s kind.  Then we verify for the base case ($\jj = 0$) that $P$ has type
$\Ty\sub{0}{\jj}$. Last, we check the more complex inductive case: $Q$ should
have type $\Ty\sub{\ii+1}{\jj}$ under the environment $\Gamma,
\ii\!\!:\!\!\minus{\II},\X\!\!:\!\!\Ty\sub{\ii}{\jj}$ where $\Ty\sub{\ii}{\jj}$
of $X$ means that $X$ satisfies the predecessor's type (induction
hypothesis). Rule \tftrule{TApp} is the elimination rule for dependent types. 

Rule \tftrule{TEq} states that typing works up to type
equivalence where $\equiv$ is defined in the previous subsection.
Recursion \tftrule{TRec} rule is standard. 
In rule \tftrule{TVar}, $\Delta\WB \Delta'$ denotes 
the standard isomorphism rules for recursive types 
(i.e.~we identify $\LM{\xx}{\T}$ and $T\sub{\LM{\xx}{\T}}{\xx}$), 
see Appendix \ref{app:kind}. Note that 
we apply isomorphic rules 
only when recursive variables are introduced. This way, we can separate 
type isomorphism for recursive types and type equalities 
with recursors. 

Rule \tftrule{TInit} types a session initialisation on shared channel \uu, binding
channel \y\ and 
requiring participants $\{\pp_0,..,\pp_n\}$. 
The premise verifies that the type of \y\
is the first projection of the global type \G\ of \uu\ and that the participants
in \G\ (denoted by $\mathtt{pid}(\G)$) can be semantically derived as
$\{\p_0,..,\p_\n\}$. % Note that the position of $\p_0$ is fixed, but others can be

Rule \tftrule{TAcc} allows to type the \p-th participant to the session initiated on
\uu. The typing rule checks that the type of \y\ is the \p-th projection of the
global type \G\ of \uu\ and that \G\ is fully
instantiated.   
% Note that not only the participant's name, but also
% $\G$ itself can contain the free index, permitting the number of repetitions or
% the total number of participants to be variable.
The kind rule ensures that $\G$ 
 is fully instantiated (i.e. $G'$'s kind is $\Type$).
Rule \tftrule{TReq} types the process that waits for an accept from a
participant: its 
type corresponds to the end-point projection of $G$. 
 
The next four rules are associate the input/output processes with the
input/output types, and delegation input/output processes to 
session input/output types. 
Then the next two rules are branching/selection rules. 

Rule \tftrule{TNull} checks that $\Delta$ is well-formed and only contains
$\End$-type for weakening (the condition $\Delta\ \End\text{ only}$ means $\forall c \in \dom{\Delta}.\Delta(c)=\End$). Rule \tftrule{TPar} puts in parallel two processes
only if their sessions environments have disjoint domains. 
Other rules are standard. 
%(\tftrule{TOut}), input, delegation,  
%(\trule{TDeleg}, \trule{TRecep}), 
%inaction, branching/selection and the expression typing rules as well as the typing rules
%for queues are similar to those in \cite{CHY07,BettiniCDLDY08LONG}.

% \input{typing_examples}



















 








==> typing_examples.tex <==
\section{Typing examples}
\label{subsec:typingexample}
 \noindent
In this section, we give examples of typing derivations for the protocols
mentioned in
%  We type the process representation for communication topologies from
\S~\ref{sec:introduction} and \S~\ref{subsec:examples}.

\subsection{Repetition example - \S~\ref{sec:introduction}
  (\ref{alice-bob-carol})} 
This example illustrates the repetition of a message
pattern. The global type for this protocol is 
$G(n)=\FOREACH{\ii}{<n}{\GS{\Alice}{\Bob}{\Nat}.\GS{\Bob}{\Carol}{\Nat}}$. % this
% example illustrates the use of recursors to express a varying number of
% repetitions. Let the type in (\ref{alice-bob-carol}) in the introduction as
% $\Pi n.G(n)$.  We type \Alice.
Following the projection from Figure~\ref{fig:projection}, \Alice 's end-point
projection of $G(n)$ has the following form:
% \footnote{For readability, in the following examples, we
%   omit from the nested conditionals the impossible cases such as
%   $\Alice=\Bob$.}
{\small
\[
\begin{array}{rcll}
  G(n)\!\proj\! \Alice & = & \RECSEQ{& \End\\
    & & &}{i}{\xx}{\IF\ \Alice\!=\!\Alice\!=\!\Bob\ \THEN\ 
    (\ldots) \\
    & & & \ELSE\ \IF\ \Alice\!=\!\Alice\ \THEN\ ({\Lout{\Bob}{\Nat}{\IF\
        \Alice\!=\!\Bob\!=\!\Carol\ \THEN\ \ldots}}) \\
    & & & \ELSE\ \IF\ \Alice=\Bob\ \THEN\ \ldots \\
    & & & \ELSE\ \ldots} \APP n
\end{array}
\]}

For readability, we omit from our examples the impossible cases created by
the projection algorithm. The number of cases can be automatically trimmed to
only keep the ones whose resolutions depend on free variables.

In this case, the projection yields the following local type:
{\small
$$
G(n)\proj \Alice=
%\FOREACH{\ii}{<n}{\Lout{\Bob}{\Nat}{}}
\RECSEQ{\End}{i}{\xx}{\Lout{\Bob}{\Nat}{\xx}} \APP n
$$
}
\noindent Before typing, we first define some abbreviations:
{\small
\[
\begin{array}{rcl}
\Alice(n)& =& \sr{a}{\Alice,\Bob,\Carol}{y}{(\RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\Bob,\e[i]}}
  \X \APP n)}\\
\Delta(n) & = & \{y:(G(n)\proj \Alice) \}\\
\Gamma & = & \AT{n}{\Nat}, \AT{a}{\ENCan{G(n)}}
\end{array}
\]}
% $\Alice(n)=\sr{a}{\Alice,\Bob,\Carol}{y}{(\RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\Bob,\e[i]}}
%   \X \APP n)}$ and let $ \Delta(n) = \{
% % y:(\RECSEQ{\End}{i}{\xx}{\Lout{\Bob}{\Nat}{\xx}} \APP n)
% y:(G(n)\proj \Alice) \} $ and $\Gamma = \AT{n}{\Nat},
% \AT{a}{\ENCan{G}}$.  
Our goal is to prove the typing judgement 
\[ \Gamma \proves \Alice(n) \rhd \emptyset
\]
We start from the leafs.
\[
\begin{prooftree}
{
\begin{prooftree}
{
\begin{prooftree}
{\Gamma, \ii : \minus{\II},\X:\Delta(\ii)  \vdash \Env }
\justifies
{\Gamma, \ii : \minus{\II},\X:\Delta(\ii)  \vdash \X  \rhd
y:\Delta(\ii)}\using\tftrule{TVar}
\end{prooftree}
}
\justifies
{\Gamma, \ii : \minus{\II},\X:\Delta(\ii)  \vdash \outS{\y}{\Bob,\e[i]}\X  \rhd
y:\Lout{\Bob}{\Nat}{\Delta(\ii)}
}\using\tftrule{TOut}
\end{prooftree}}
\justifies
{\Gamma, \ii : \minus{\II},\X:\Delta(\ii)  \vdash \outS{\y}{\Bob,\e[i]}\X  \rhd
\Delta(\ii+1)
}\using\tftrule{TEq}
\end{prooftree}
\]
% The application of the \tftrule{TEq} rule is justified by the fact that the
The \tftrule{TEq} rule can be used because
types $\Delta(\ii+1)$ and
$y:\!\Lout{\Bob}{\Nat}{(\RECSEQ{\End}{j}{\xx}{\Lout{\Bob}{\Nat}{\xx}} \APP \ii)}$
are equivalent: they have the same weak-head normal form (we use the rule
\trule{WfBase}).

% \[
% \begin{prooftree}
% {\Gamma, n : \minus{\II},\X:\Delta(n)  \vdash \outS{\y}{\Bob,\e[i]}\X  \rhd
% y:\Lout{\Bob}{\Nat}{
% (\RECSEQ{\End}{j}{\xx}{\Lout{\Bob}{\Nat}{\xx}} \APP n)}
% }
% \justifies
% {\Gamma, n : \minus{\II},\X:\Delta(n)  \vdash \outS{\y}{\Bob,\e[i]}\X  \rhd
% \Delta(n+1)}
% \end{prooftree}
% \]

Since we have the trivial $\Gamma\vdash \inact  \rhd \Delta(0)$, we can apply
the rules \tftrule{TApp} and \tftrule{TPRec}.
\[
\begin{prooftree}
{\begin{prooftree}
{\begin{array}{c}
\Gamma, \ii : \minus{\II},\X:\Delta(\ii)  \vdash \outS{\y}{\Bob,\e[i]}\X  \rhd
 \Delta(\ii+1) \\
\Gamma\vdash \inact  \rhd \Delta(0) \quad \Gamma,\AT{\ii}{\II}\vdash \Delta(\ii) \RHD \K
\end{array}
}
\justifies
{\Gamma \vdash (\RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\Bob,\e[i]}}
  \X)\rhd \Pi \AT{\ii}{\II}.\Delta(\ii)}\using\tftrule{TPRec}
\end{prooftree}
}\justifies
{\Gamma \vdash (\RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\Bob,\e[i]}}
  \X \APP n)\rhd \Delta(n)}\using\tftrule{TApp}
\end{prooftree}
\]
We conclude with \tftrule{TInit}.
\[
\begin{prooftree}
{
\begin{array}{@{}c@{}}
\Gamma \vdash a:\mar{\G(n)} \quad 
\Gamma \vdash (\RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\Bob,\e[i]}}
  \X \APP n)\rhd \Delta(n)
\end{array}
}
\justifies
{\Gamma \vdash \Alice(n) \rhd \emptyset} 
\using\tftrule{TInit}
\end{prooftree}
\]
% We then rely on \tftrule{TApp} and \tftrule{TPRec}.



% We
% can prove that 
% \[ \Gamma \proves \Alice(n) \rhd \emptyset
% \]
% from \tftrule{TInit} if we
% have $\Gamma \proves \RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\Bob,\e[i]}}\X \APP n
% \rhd \Delta(\nn)$. 
% This, in turn, is given by \tftrule{TPRec} and \tftrule{TApp}
% from $\Gamma, \ii:\II^-, X:\Delta(\ii) \proves y!\ENCan{\Bob,e[\ii]};X\rhd
% \Delta(\ii+1)$ and the trivial $\Gamma\proves \inact\rhd y:\End$. 

% From \tftrule{TVar}, we have $\Gamma, n:\II^-, X:\Delta(n) \proves X\rhd
% \Delta(n)$. 
% We conclude by \tftrule{TOut} and, using the weak head normal form
% \trule{WF}, we can use the rule \trule{WF} to prove the equivalence of the
% types $\Delta(n+1)$ and $y:\Lout{\Bob}{\Nat}{
% (\RECSEQ{\End}{j}{\xx}{\Lout{\Bob}{\Nat}{\xx}} \APP n)}$.

% \marginpar{I do not understand how it is derived. Also footnote. I
%   think it is better no omission as the first example.}

$\Bob(n)$ and $\Carol(n)$ can be similarly typed.

% First we note $\Gamma \proves \Pi j:I.\Delta(j) \RHD \Pi j:I.\Type$ by renaming
% with $\II =[0..n+1]$.  For the base case, we have: $\Gamma\proves \inact\rhd
% y:\End$ by \tftrule{TNull} (in \cite{fullversion}).  For the inductive case, first
% we derive, by \tftrule{TVar}, $\Gamma, \ii:\II^-, X:\Delta(\ii) \proves X\rhd
% \Delta(\ii)$.  From this judgement, using \tftrule{TOut}, we have:
% \[\Gamma, \ii:\II^-, X:\Delta(\ii) \proves
%  y!\ENCan{\Bob,e[\ii]};X\rhd \Delta(\ii+1)\]
% From \tftrule{TPRec} and
% \tftrule{TApp},
% $\Gamma \proves \RECSEQP{\inact}{\ii}{\X}{\outS{\y}{\Bob,\e[i]}}\X \APP n
% \rhd \Delta(\nn)$. Now we can apply \tftrule{TInit} to obtain
% $\Gamma \proves \Alice(n) \rhd \emptyset$. 
% Similarly for
% Finally we can compose by \tftrule{Par},
% $\AT{n}{\Nat}, \AT{a}{\ENCan{G}}
% \proves \Alice(n)\sep \Bob(n)\sep \Carol(n)\rhd \emptyset$.  Applying
% \trule{TNu} and \tftrule{TPRec}, we have:
% \[\emptyset \proves
% \Pi n.(\nu a)(\Alice(n)\sep \Bob(n)\sep \Carol(n))\rhd
% \Pi n:\Nat.\emptyset
% \]




\subsection{Sequence example - \S~\ref{sec:introduction}
  (\ref{ex:sequence})}
% The highlight of this example is
% a type-equality
% between the general end-point generator and a {\em role-based}
% local type (called {\em role-types}).
% The role-type groups the participants who inhabit
% in the same parameterised protocol as a single role.
% We observe t
The sequence example consists of $n$ participants organised in the following way
(when $n\geq 2$): the starter $\W[n]$ sends the first message, the final worker
$\W[0]$ receives the final message and the middle workers first receive a
message and then send another to the next worker. We write below the result of
the projection for a participant $\W[\pp]$ (left) and the end-point type that
naturally types the processes (right):
% generic
% projection for participant $\W[\pp]$ (left) and the end-point type that
% naturally types the processes (right):
{\small
\[
\begin{array}{l|l}
\begin{array}{llll}
   \RECSEQ{\End }{i}{\xx}{\\
%     \IF\ \pp=\W[i+1]=\W[i]\ \THEN \ \Lout{\W[i]}{\Nat}{\Lin{\W[i+1]}{\Nat}\xx}\\
  % \quad \quad\quad\quad\quad
 \ \IF\ \ \pp=\W[i+1]\ \THEN \ \Lout{\W[i]}{\Nat}\xx \\
 % \quad \quad\quad\quad\quad
 \ \ELSE\ \IF\ \ \pp=\W[i]\ \THEN \ \Lin{\W[i+1]}{\Nat}\xx \\
 % \quad \quad\quad\quad\quad
 \ \ELSE\ \xx \ } \\
 n
\end{array}
&
\begin{array}{lll}
\IF \ &
\p=\W[n]  \ \THEN \ \Lout{\W[n-1]}{\Nat}{}\ELSE\\
\IF &
\p=\W[0] \ \THEN \ {\Lin{\W[1]}{\Nat}{}}\ELSE\\
\IF & \p=\W[\ii]\  \THEN \  {\Lin{\W[i+1]}{\Nat}{}}{\Lout{\W[i-1]}{\Nat}{\!}}
\end{array}
\end{array}
\]
} %

\noindent
This example illustrates the main challenge faced by the type checking algorithm.
In order to type this example, we need to prove the equivalence
of these two types. For any concrete instantiation of $\p$ and $\n$, the standard weak
head normal form equivalence rule \trule{WfBase} is sufficient.  Proving the
equivalence for all $\p$ and $\n$ requires either (a) to bound the domain $\II$
in which they live, and check all instantiations within this finite domain using
rule \trule{WfRecF}; or (b) to prove the equivalence through the meta-logic
rule \trule{WfRecExt}.  In case (a), type checking terminates, while case (b)
allows to prove stronger properties about a protocol's implementation. 

% {\small
% \[
% \begin{array}{lll}
%    \RECSEQ{\End }{i}{\xx}{ \IF\ \pp=\W[i+1]=\W[i]\ \THEN \ \Lout{\W[i]}{\Nat}{\Lin{\W[i+1]}{\Nat}\xx}\\
%   \quad \quad\quad\quad\quad \ \ELSE\IF\ \ \pp=\W[i+1]\ \THEN \ \Lout{\W[i]}{\Nat}\xx \\
%  \quad \quad\quad\quad\quad\ \ELSE\IF\ \ \pp=\W[i]\ \THEN \ \Lin{\W[i+1]}{\Nat}\xx \\
%  \quad \quad\quad\quad\quad\ \ELSE\IF\ \ \xx \ } & n
% \end{array}
% \]
% }
% {\small
% \[
% \begin{array}{lll}
%    \RECSEQ{(\GS{\W[0]}{\W[n]}{\Nat}.\End)\proj \pp\\
%    \quad }{i}{\xx}{ \IF\ \pp=\W[i+1]\ \THEN \ \Lout{\W[i]}{\Nat}\xx\\
%   \quad \quad\quad\quad\quad \ \ELSE\IF\ \ \pp=\W[i]\ \THEN \ \Lin{\W[i+1]}{\Nat}\xx \\
%  \quad \quad\quad\quad\quad\ \ELSE\IF\ \ \xx \ } & n
% \end{array}
% \]
% }
% First we note the kinding rules \tftrule{KRcr} and
% \tftrule{KApp} ensure $\nn\geq 1$.
% From
% the figure~\ref{fig:examples}(a),
% the user would design the end-point type as follows:
% {\small\[
% \begin{array}{lll}
% \IF \ &
% \p=\W[n]  \ \THEN \ \Lout{\W[n-1]}{\Nat}{}\\
% \ELSE\IF &
% \p=\W[0] \ \THEN \ {\Lin{\W[1]}{\Nat}{}}\\
% \ELSE\IF & \p=\W[\ii] \THEN \  {\Lin{\W[i+1]}{\Nat}{}}{\Lout{\W[i-1]}{\Nat}{}}
% \end{array}
% \]}
% {\small\[
% \begin{array}{lll}
% \IF \ &
% \p=\W[n]  \ \THEN \ \Lout{\W[n-1]}{\Nat}{\Lin{\W[0]}{\Nat}{}}\\
% \ELSE\IF &
% \p=\W[0] \ \THEN \ {\Lin{\W[1]}{\Nat}{}}\Lout{\W[n]}{\Nat}{}\\
% \ELSE\IF & 1 \leq i \leq n-1  \ \mathsf{and}\ \p=\W[\ii]\\
% & \THEN \  {\Lin{\W[i+1]}{\Nat}{}}{\Lout{\W[i-1]}{\Nat}{}}
% \end{array}
% \]}

% The first case denotes the protocol of the initiator;
% the second one corresponds to the last worker, while
% the third one to one of the middle workers.
% The type equality is easily proved by the case analysis
% by the induction of the recursor using the inductive rules in a
% version of the end-point types following in 
% figure~\ref{fig:type-wf-recursion} (\trule{WfBase,WfLL,WfRecF}), 
% combining the $\beta$-reductions 
% over two end-point types. 
% Let $T[\p][n]$ for the first original type and $T'[\p][n]$ for the
% second role type. We can check for all $\n\geq 1$ and $\p$, we have:
% \begin{center}
% $(\prod n.T[\p][n] )\n \redsym^\ast T_\n\not\redsym$ iff 
% $(\prod n.T'[\p][n] )\n \redsym^\ast T_\n\not\redsym$. 
% \end{center}
% Hence $\prod n.T[\p][n]\gequivwf \prod n.T'[\p][n]$. 
% For example, when $\p=\W[0]$, then 
% $(\prod n.T[\W[0]][n] )\n \redsym^\ast
% {\Lin{\W[1]}{\Nat}{}}\Lout{\W[\n]}{\Nat}{}$ 
% and 
% $(\prod n.T'[\W[0]][n] )\n \redsym^\ast
% {\Lin{\W[1]}{\Nat}{}}\Lout{\W[\n]}{\Nat}{}$. 
% Similarly for  the case $\p=\W[n]$ and 
% $\p=\W[i]$ with $1\leq i \leq n-1$. 
% Note that for all $\n$, the $\beta$-reduction terminates, 
% so that the equality checking terminates. 

% From these types, the ring processes are straightforwardly
% implemented and typable using ${\bf R}$. 
% Recall the implementation of this ring protocol from \S~\ref{subsec:processexample}: 
% {\small
% \[
% \begin{array}{lllll}
% P_{\text{ring}} \ = \ 
% \mathbf{R} &
% \sr{a}{\W[\nn]..\W[0]}{y}{\outS{\y}{\W[\nn-1],v}\inpS{y}{\W[0],z}P}\\[1mm]
% & \sa{a}{\W[0]}{y}{\inpS{y}{\W[1],z}{\outS{\y}{\W[\nn],z}Q}}\\[1mm]
% & \quad \lambda {\ii}.\lambda{\X}.(
% \ifthenelse{i\not = 0}%
% {\sa{a}{\W[\ii]}{y}{\inpS{y}{\W[\ii-1],z}\outS{\y}{\W[\ii+1],z}}{}}%
% {\inact}\\[1mm]
% & {\quad\quad\quad\quad\quad\quad \pc X}) {\quad \nn} 
% \end{array}
% \]
% }
% Let us define: 
% \[ 
% \begin{array}{lllll}
% P_n & = &  
% \sr{a}{\W[\nn]..\W[0]}{y}{\outS{\y}{\W[\nn-1],v}\inpS{y}{\W[0],z}P}\\[1mm]
% P_0 & = &  
% \sa{a}{\W[0]}{y}{\inpS{y}{\W[1],z}{\outS{\y}{\W[\nn],z}Q}}\\[1mm]
% P_{\ii} & = &  
% {\sa{a}{\W[\ii]}{y}{\inpS{y}{\W[\ii-1],z}\outS{\y}{\W[\ii+1],z}}{}}
% & 1 \leq i \leq n-1 \\[1mm]
% P_{\text{body}} & = &  \ifthenelse{i\not = 0}{P_{\ii}}{\inact}
% \end{array}
% \]
% Assume 
% \[ 
% \emptyset \vdash P \rhd \D_n
% \]
% By \tftrule{TOut, TIn}, we have: 
% \[ 
% a:\mar{\G} \vdash 
% \outS{\y}{\W[\nn-1],v}\inpS{y}{\W[0],z}P  \rhd \D_n,\y:\G \proj{\p_0}
% \]
% where $\G \proj{\p_0}$ is obtained from the role type above. 
% Hence, by \tftrule{TInit} ,  noting $\p_0=n$,  
% \[ 
% a:\mar{\G} \vdash P_0 \rhd \D_n
% \]
% Similarly, using \tftrule{TAcc}  with $\p_n=0$,     
% we have: 
% \[ 
% a:\mar{\G} \vdash P_0 \rhd \D_0
% \]
% Hence we have 
% \[
% a:\mar{\G} \vdash P_n\Par P_0 \rhd \D 
% \]
% with $\D=\D_0,\D_n$. 
% Similarly, we can type: 
% \[ 
% a:\mar{\G}, \ii:\II^-, 1 \leq i  \vdash P_i \rhd \emptyset 
% \]
% with $\II=[0..n]$. 
% Also we have: 
% \[ 
% a:\mar{\G}  \vdash \inact \rhd \emptyset 
% \]
% and 
% \[ 
% a:\mar{\G},\ii:\II^-,X:\tau\subst{i}{j}  \vdash X \rhd \tau\subst{i+1}{j} 
% \]
% where $\tau\subst{i}{j}=\D$ for all $i$. 
% Hence by strenghting, \tftrule{TIf} and \tftrule{TPar}, we have: 
% \[ 
% a:\mar{\G},\ii:\II^-,X:\tau\subst{i}{j}  \vdash P_{\text{body}} \rhd \tau\subst{i+1}{j} 
% \]
% Hence applying \tftrule{TPRec} and \tftrule{TPar},  
% we can type the ring  process as: 
% \[
% a:\mar{\G}  \vdash  P_{\text{ring}} \rhd \D 
% \]
% as required. 
% We also discuss an algorithm for the automatic 
% generation of role-types in \S~\ref{subsec:roletype}.

%The highlight of this example is
%a transformation from the general end-point generator to a {\em role-based}
%local type using the type equality.
%The role-based end-point type groups the participants who inhabit
%in the same parameterised protocol as a single role.
%We observe the ring topology consists of the two roles: one
%is an initiator who sends the message first and
%receives the final message from $\W[0]$; and others
%are the middle workers  who receive a data and
%send back to the next worker. The transformation starts
%from the general generator of this topology given below.
%{\small
%\[
%\begin{array}{lll}
%   \RECSEQ{(\GS{\W[0]}{\W[n]}{\Nat}.\End)\proj \pp\\
%   \quad }{i}{\xx}{ \IF\ \pp=\W[i+1]\ \THEN \ \Lout{\W[i]}{\Nat}.\xx\\
%  \quad \quad\quad\quad\quad \ \ELSE\IF\ \pp=\W[i]\ \THEN \ \Lin{\W[i+1]}{\Nat}.\xx \\
% \quad \quad\quad\quad\quad\ \ELSE\IF\ \xx \ } & n
%\end{array}
%\]
%}
%Let the above type as $G$ and $G_0=\GS{\W[0]}{\W[n]}{\Nat}.\End$.
%This is transformated to the most optimal local type as:
%\[
%\begin{array}{lll}
%\IF \ & n=0 &\!\!\THEN \ \Lout{\W[0]}{\Nat}{\Lin{\W[0]}{\Nat}{}}\\
%\ELSE\IF & 1\leq n\ \mathsf{and}\ \p=\W[n]
%& \!\!\THEN \ \Lout{\W[n-1]}{\Nat}{\Lin{\W[0]}{\Nat}{}}\\
%\ELSE\IF & 1 \leq i \leq n-1  \ \mathsf{and}\ & \hspace{-0.3cm}\p=\W[\ii]\\
%& &\hspace{-0.5cm}\THEN \  {\Lin{\W[i+1]}{\Nat}{}}{\Lin{\W[i-1]}{\Nat}{}}
%\end{array}
%\]
%The first conditional means the special case where the
%initiator is the receiver, too.
%The second one denotes the protocol of the initiator,
%while the third one corresponds the protocol of the middle workers.
%The first line is subsumed in the second line when $n=1$.
%The type equality is easily proved by the case analysis
%since $i$'s range is fixed from $1$ to $n-1$ in the recursor.
%We shall discuss an algorithm for the automatic transformation
%and its implementation in \S~\ref{subsec:implemenation}.
%From these types, the ring processes are straightforwardly
%implemented and typable using ${\bf R}$: the whole process
%has type $\Delta$ where $\Delta$ is
%types for the free sessions of the initiator
%$\sr{a}{\W[0]..\W[\n]}{y}{\outS{\y}{v}\inpS{y}{z}P}$
%(note the $i$-th process
%$(\sa{a}{\W[\ii]}{y}{\inpS{y}{z}\outS{\y}{z}})$
%under the recursion should contain no free sessions).

%The rest of the workers might be generated by a recursor.
%\[
%\begin{array}{lllll}
%\mathbf{R} &
%\sr{a}{\W[0]..\W[\n]}{y}{\outS{\y}{v}\inpS{y}{z}P}\\[1mm]
%& \quad \quad \lambda {\ii}.\lambda{\X}.(
%\sa{a}{\W[\ii]}{y}{\inpS{y}{z}\outS{\y}{z}} \pc X)
%{\quad \n}
%\end{array}
%\]
%$\n$ can be bound by the $\lambda$-abstraction as the previous
%example.
%Note this includes the case $\n=0$.
%We omit the multicast.


\subsection{Ring - Figure~\ref{fig:examples}(a)}

The typing of the ring pattern is similar to the one of the sequence.
%The highlight of this example is
%a type-equality
%between the general end-point generator and a {\em role-based}
%local type (called {\em role-types}).
%The role-type groups the participants who inhabit
%in the same parameterised protocol as a single role.
%We observe the ring topology consists of the three roles (when $n\geq
%1$): one
%is the starter $\W[n]$ who sends the message first and
%receives the final message from the final worker $\W[0]$,
%and others are the middle workers  who receive a data and
%send back to the next worker. The transformation starts
%from 
The projection of this global session type for $\W[\pp]$ gives the following
local type: 
{\small
\[
\begin{array}{lll}
   \RECSEQ{(\GS{\W[\nn]}{\W[0]}{\Nat}.\End)\proj \W[\pp]\\
   \quad }{i}{\xx}{ \IF\ \pp=\W[\nn-i-1]\ \THEN \ \Lout{\W[\nn-\ii]}{\Nat}\xx\\
  \quad \quad\quad\quad\quad \ \ELSE\IF\ \ \pp=\W[\nn-\ii]\ \THEN \ \Lin{\W[\nn-\ii-1]}{\Nat}\xx \\
 \quad \quad\quad\quad\quad\ \ELSE\IF\ \ \xx \ } & n
\end{array}
\]
}

On the other hand, user processes can be easily type-checked with an end-point
type of the following form:
%First we note the kinding rules \trule{KRcr} and
%\trule{KApp} ensure $\nn\geq 1$.
%From
%the figure~\ref{fig:examples}(a),
% the user would design the end-point type as follows:
{\small
\[
\begin{array}{lll}
\IF \ &
\p=\W[0] \ \THEN \ \Lout{\W[1]}{\Nat}{\Lin{\W[n]}{\Nat}{}}\\
\ELSE\IF &
\p=\W[n]  \ \THEN \ \Lin{\W[n-1]}{\Nat}{\Lout{\W[0]}{\Nat}{}}\\
\ELSE\IF & 1 \leq i+1 \leq n-1  \ \mathsf{and}\ \p=\W[\ii+1]\\
& \THEN \  {\Lin{\W[i]}{\Nat}{}}{\Lout{\W[i+2]}{\Nat}{}}
\end{array}
\]}

\noindent
% In this typeThe first case denotes the protocol of the initiator;
% the second one corresponds to the last worker, while
% the third one to one of the middle workers.
Proving the equivalence between these types is similar as the one the sequence:
%The type equality is easily proved by the case analysis
we rely on rules \trule{WfBase} and \trule{WfRecF} when the domain of $n$ is
bounded, or on the meta-logic rule \trule{WfRecExt}.

% by the induction of the recursor using the inductive rules in a
% version of the end-point types following in 
% Figure~\ref{fig:type-wf} (\trule{WfBase,WfRecF}), 
% combining the $\beta$-reductions 
% over two end-point types. 

%Let $T[\p][n]$ for the first original type and $T'[\p][n]$ for the
%second role type. We can check for all $\n\geq 1$ and $\p$, we have:
%\begin{center}
%$(\prod n.T[\p][n] )\n \redsym^\ast T_\n\not\redsym$ iff 
%$(\prod n.T'[\p][n] )\n \redsym^\ast T_\n\not\redsym$. 
%\end{center}
%Hence $\prod n.T[\p][n]\gequivwf \prod n.T'[\p][n]$. 
%For example, when $\p=\W[0]$, then 
%$(\prod n.T[\W[0]][n] )\n \redsym^\ast
%{\Lout{\W[1]}{\Nat}{}}\Lin{\W[\n]}{\Nat}{}$ 
%and 
%$(\prod n.T'[\W[0]][n] )\n \redsym^\ast
%{\Lout{\W[1]}{\Nat}{}}\Lin{\W[\n]}{\Nat}{}$. 
%Similarly for  the case $\p=\W[n]$ and 
%$\p=\W[i+1]$ with $1\leq i+1 \leq n-1$. 
%Note that for all $\n$, the $\beta$-reduction terminates, 
%so that the equality checking terminates. 

% From these types, the ring processes are straightforwardly
% typable using ${\bf R}$. 
%Recall the implementation of this ring protocol from \S~\ref{subsec:processexample}: 

%{\small
%\[
%\begin{array}{lllll}
%P_{\text{ring}} \ = \ \mathbf{R} &
%\sr{a}{\W[0], \W[\n], \tilde{\pp}}{y}{\outS{\y}{\W[1],v}\inpS{y}{\W[\nn],z}P}\\[1mm]
%& \sa{a}{\W[\nn]}{y}{\inpS{y}{\W[\nn-1],z}{\outS{\y}{\W[0],z}Q}}\\[1mm]
%& \quad \lambda {\ii}.\lambda{\X}.(
%\sa{a}{\W[\ii+1]}{y}{\inpS{y}{\W[\ii],z}\outS{\y}{\W[\ii+2],z} \pc X}) {\quad \nn-1} 
%\end{array}
%\]
%}
%%{\small
%%\[
%%\begin{array}{lllll}
%%P_{\text{ring}} \ = \ 
%%\mathbf{R} &
%%\sr{a}{\W[\nn]..\W[0]}{y}{\outS{\y}{\W[\nn-1],v}\inpS{y}{\W[0],z}P}\\[1mm]
%%& \sa{a}{\W[0]}{y}{\inpS{y}{\W[1],z}{\outS{\y}{\W[\nn],z}Q}}\\[1mm]
%%& \quad \lambda {\ii}.\lambda{\X}.(
%%\ifthenelse{i\not = 0}%
%%{\sa{a}{\W[\ii]}{y}{\inpS{y}{\W[\ii-1],z}\outS{\y}{\W[\ii+1],z}}{}}%
%%{\inact}\\[1mm]
%%& {\quad\quad\quad\quad\quad\quad \pc X}) {\quad \nn} 
%%\end{array}
%%\]
%%}
% More precisely, we define: 
% {\small
% \[ 
% \begin{array}{lllll}
% P_0 & = &  
% \sr{a}{\W[0],.., \W[\n]}{y}{\outS{\y}{\W[1],v}\inpS{y}{\W[\nn],z}P}\\[1mm]
% P_n & = &  
% \sa{a}{\W[\nn]}{y}{\inpS{y}{\W[\nn-1],z}{\outS{\y}{\W[0],z}Q}}\\[1mm]
% P_{\ii+1} & = &  
% \sa{a}{\W[\ii+1]}{y}{\inpS{y}{\W[\ii],z}\outS{\y}{\W[\ii+2],z}}
% & 1 \leq i+1 \leq n-1 \\[1mm]
% %P_{\text{body}} & = &  \ifthenelse{i\not = 0}{P_{\ii}}{\inact}
% \end{array}
% \]
% }
% Assume $\emptyset \vdash P \rhd \D_0$. 
% By \tftrule{TOut, TIn}, we have: 
% $a:\mar{\G} \vdash 
% \outS{\y}{\W[1],v}\inpS{y}{\W[n],z}P  \rhd \D_n,\y:\G \proj{\p_0}$ 
% where $\G \proj{\p_0}$ is obtained from the local type above. 
% Hence, by \trule{TInit},  writing $\p_0=\W[0]$,  
% we have: $a:\mar{\G} \vdash P_0 \rhd \D_0$. 
% Similarly, using \trule{TAcc}  with $\p_n=\W[n]$,     
% we have: 
% $a:\mar{\G} \vdash P_n \rhd \D_n$. 
% Hence we derive: 
% $a:\mar{\G} \vdash P_0\Par P_n \rhd \D $ 
% with $\D=\D_0,\D_n$. 
% Similarly, we can type: 
% $a:\mar{\G}, \ii:\II^-, 1 \leq i+1  \vdash P_{i+1} \rhd \emptyset$ 
% with $\II=[0..n-1]$. 
% Also we have: 
% %\[ 
% %a:\mar{\G}  \vdash \inact \rhd \emptyset 
% %\]
% %and 
% $a:\mar{\G},\ii:\II^-,X:\tau\subst{i}{j}  \vdash X \rhd
% \tau\subst{i+1}{j}$ 
% where $\tau\subst{i}{j}=\D$ for all $i$. 
% Hence by strengthening and \trule{TPar}, we have: 
% $a:\mar{\G},\ii:\II^-,X:\tau\subst{i}{j}  \vdash P_{i+1} | X \rhd
% \tau\subst{i+1}{j}$.    
% Hence applying \trule{TPRec},  
% we can type the ring  process as: 
% $a:\mar{\G}  \vdash  P_{\text{ring}} \rhd \D$,  
% as required. 
% %%We also discuss an algorithm for the automatic 
% %%generation of role-types in \S~\ref{subsec:roletype}.

\subsection{Mesh pattern - Figure~\ref{fig:examples}(b)} 
%% The highlight of this example is
%% a type-equality
%% between the general end-point generator and a {\em role-based}
%% end-point type (called {\em role-types}).
%% The role-type groups the participants who inhabit
%% in the same parameterised protocol as a single role. 
The mesh example describes nine different participants behaviours (when
$n,m\geq 2$). The participants in the first and last rows and columns, except
the corners which have two neighbours, have three neighbours. The other
participants have four neighbours. The specifications of the mesh are defined by
the communication behaviour of each participant and by the links the
participants have with their neighbours. 
% 
The term below is the result of the projection of the global type for
participant $\pp$% The transformation starts from the
% general generator of this topology given below.

{\small
\[
\begin{array}{lll}
\RECSEQ{  ~~ (\RECSEQ{\End\proj \pp}{k}{\zz}{
    \IF \ \pp=\W[0][k+1]\ \THEN \ \Lout{\W[0][k]}{\Nat}\zz\\
     \qquad\qquad\quad \quad\quad\quad\quad~~ \ \ELSE\IF\ \ \pp=\W[0][k]\ \THEN \ \Lin{\W[0][k+1]}{\Nat}\zz \\
 \qquad\qquad\quad \quad\quad\quad\quad~~\ \ELSE\ \ \zz \ })  m\\
     \quad }{i}{\xx}{ \\
       \qquad (\RECSEQ{~( \IF \ \pp=\W[i+1][0]\ \THEN \ \Lout{\W[i][0]}{\Nat}\xx\\
     \quad \quad\quad\quad \ \ELSE\IF\ \ \pp=\W[i][0]\ \THEN \ \Lin{\W[i+1][0]}{\Nat}\xx \\
 \quad \quad\quad\quad \ \ELSE\ \ \xx \ )\\       
           \quad \qquad  }{j}{\yy}{ \\         
          \qquad \qquad  ~\IF \ \pp=\W[i+1][j+1]\ \THEN \ \Lout{\W[i][j+1]}{\Nat}\\
          \qquad\qquad\qquad \IF \ \pp=\W[i+1][j+1]\ \THEN \ \Lout{\W[i+1][j]}{\Nat} \yy\\
          \qquad\qquad\qquad  \ELSE\IF\ \ \pp=\W[i+1][j]\ \THEN \ \Lin{\W[i+1][j+1]}{\Nat}\yy \\
                    \qquad\qquad\qquad \ELSE\ \yy\\
     \quad \quad\quad\quad \ \ELSE\IF\ \ \pp=\W[i][j+1]\ \THEN \ \Lin{\W[i+1][j+1]}{\Nat}\yy \\
      \qquad\qquad\qquad \IF \ \pp=\W[i+1][j+1]\ \THEN \ \Lout{\W[i+1][j]}{\Nat} \yy\\
          \qquad\qquad\qquad  \ELSE\IF\ \ \pp=\W[i+1][j]\ \THEN \ \Lin{\W[i+1][j+1]}{\Nat}\yy \\
                    \qquad\qquad\qquad \ELSE \ \yy\\
        \qquad\qquad \ELSE\IF \ \pp=\W[i+1][j+1]\ \THEN \ \Lout{\W[i+1][j]}{\Nat} \yy\\
          \qquad\qquad  \ELSE\IF\ \ \pp=\W[i+1][j]\ \THEN \ \Lin{\W[i+1][j+1]}{\Nat}\yy \\
            \qquad\qquad  \ELSE \ \yy}\\
       \qquad  m) \\
     \quad n} 
\end{array}
\]
}

From Figure~\ref{fig:examples}(c),
the user would design the end-point type as follows:
{\small\[
\begin{array}{lll}
\IF \ &
\p=\W[n][m] \ \THEN \ \Lout{\W[n-1][m]}{\Nat}{\Lout{\W[n][m-1]} {\Nat}{}}\\
\ELSE\IF &
\p=\W[n][0]  \ \THEN \ \Lin{\W[n][1]}{\Nat}{\Lout{\W[n-1][0]}{\Nat}{}}\\
\ELSE\IF &
\p=\W[0][m]  \ \THEN \ \Lin{\W[1][m]}{\Nat}{\Lout{\W[0][m-1]}{\Nat}{}}\\
\ELSE\IF &
\p=\W[0][0]  \ \THEN \ \Lin{\W[1][0]}{\Nat}{\Lin{\W[0][1]}{\Nat}{}}\\
\ELSE\IF &
 1 \leq k+1 \leq m-1 ~ \mathsf{and}\ \p=\W[n][k+1]\\
 & \THEN \ \Lin{\W[n][k+2]}{\Nat}{\Lout{\W[n-1][k+1]}{\Nat}{\Lout{\W[n][k]}{\Nat}}}\\ 
\ELSE\IF &
 1 \leq k+1 \leq m-1 ~ \mathsf{and}\ \p=\W[0][k+1]\\
 & \THEN \ \Lin{\W[1][k+1]}{\Nat}{\Lin{\W[0][k+2]}{\Nat}\Lout{\W[0][k]}{\Nat}}\\ 
\ELSE\IF &
 1 \leq i+1 \leq n-1  ~\mathsf{and}\ \p=\W[i+1][m]\\
 & \THEN \ \Lin{\W[i+2][m]}{\Nat}{\Lout{\W[i][m]}{\Nat}{\Lout{\W[i+1][m-1]}{\Nat}}}\\ 
\ELSE\IF &
 1 \leq i+1 \leq n-1  ~\mathsf{and}\ \p=\W[i+1][0]\\
 & \THEN \ \Lin{\W[i+2][0]}{\Nat}{\Lin{\W[i+1][1]}{\Nat}{\Lout{\W[i][0]}{\Nat}}}\\ 
 \ELSE\IF &
 1 \leq i+1 \leq n-1  ~\mathsf{and}\ 1 \leq j+1 \leq m-1 ~\mathsf{and}~ \p=\W[i+1][j+1]\\
 & \THEN \ \Lin{\W[i+2][j+1]}{\Nat}{\Lin{\W[i+1][j+2]}{\Nat}{\Lout{\W[i][j+1]}{\Nat}{\Lout{\W[i+1][j]}{\Nat}}}}\\ 
\end{array}
\]}

Each case denotes a different local behaviour in the mesh pattern. % Names are
% given in process definition.
We present the following meta-logic proof of the typing equivalence through
\trule{WfRecExt} in the two cases of the 
top-left corner and bottom row, in order to demonstrate how our
system types the mesh session. The other cases are left to the reader. 

Let $T[\p][n][m]$ designate the first original type and $T'[\p][n][m]$ the
second type. To prove the type equivalence, we want to check that for all $\n,
\m \geq 2$ and $\p$, we have: 
\begin{center}
\small
$(\prod n.\prod m.T[\p][n][m])\n \m \redsym^\ast T_{\n, \m}\not\redsym$ iff 
$(\prod n.\prod m.T'[\p][n][m]) \n \m \redsym^\ast T_{\n, \m}\not\redsym$. 
\end{center}

For $\p=\W[n][m]$, which implements the top-left corner, the generator type
reduces several steps and gives the end-point type
$\Lout{\W[\n-1][\m]}{\Nat}{\Lout{\W[\n][\m-1]} {\Nat}{\inact}}$, which is the same to
the one returned in one step by the case analysis of the type built by the
programmer. For $\p=\W[0][k+1]$, we analyse the case % when $\n =2$ and $\m=2$,
where $1 \leq k+1 \leq \m-1$. The generator type returns the end-point type
\Lin{\W[1][k+2]}{\Nat}{\Lin{\W[0][k+2]}{\Nat}\Lout{\W[0][k]}{\Nat}}.%  where the
% first action comes from the case in line number 13, the second action comes from
% the case in line 2 and the third action comes from case in line 1
One can observe that the end-point type returned for $\p=\W[0][k+1]$ in the type of the
programmer is the same as the one returned by the generator. Similarly for all
the other cases. %  Note that for all $\n, \m$, the $\beta$-reduction terminates,
% so that the equality checking terminates.

By \tftrule{TOut, TIn}, we have: 
{\small
\[ 
a:\mar{\G} \vdash \outS{y}{\W[n-1][m], f(n-1,m)}\outS{y}{\W[n][m-1], f(n,m-1)}{\inact}
  \rhd \D,\y:\G \proj{\p_{\text{top-left}}}
  \]
  \[
a:\mar{\G} \vdash \inpS{y}{\W[1][k+1], z_1}\inpS{y}{\W[0][k+2], z_2}\outS{y}{\W[0][k], f(0,k)}\inact \rhd \D', \y :\G \proj{\p_{\text{bottom}}}\\
\]
}
where $\G \proj{\p}$ is obtained from the type above. 

% The primitive recursive process is typed similarly as for the one of the sequence pattern.

\subsection{FFT example - Figure~\ref{fig:fft}}
\noindent 
\label{subsec:fft:typing}
We prove
type-safety and deadlock-freedom for the FFT processes.  
Let $P_{\text{fft}}$ be the following process:
{\small
\[
\begin{array}{lll}
%P_{\text{fft}}=& 
\Pi n.(\nu a)(
\mathbf{R} \ \sr{a}{\p_0..\p_{2^n-1}}{y}{P(2^n-1,\p_0,x_{\overline{\p_0}},y,r_{\p_0})}\\[1mm]
%& 
\quad \lambda{\ii}.\lambda {\Y}.
{(\sr{a}{\p_{\ii+1}}{y}{P({\ii+1},\p_{\ii+1},x_{\overline{\p_{\ii+1}}},y,r_{\p_{\ii+1}})}
\sep \Y)}\APP 2^n-1)
\end{array}
\] 
}

\noindent
As we reasoned above, each $P(n,\p,x_{\overline{\p}},y,r_\pp)$ is
straightforwardly typable by an end-point type which can be proven to be
equivalent with the one projected from the global type $G$ from
Figure~\ref{fig:fft}(c). Automatically checking the equivalence for all $n$ is
not easy though: we need to rely on the finite domain restriction using
\trule{WfRecF} or to rely on a meta-logic proof through \trule{WfRecExt}.
The following theorem says once $P_{\text{fft}}$ is applied 
to a natural number $\m$, its evaluation always 
terminates with the answer at $r_\pp$.
% Then
% $P_{\text{fft}}$ is typable by 
% the same reasoning as the example in \S~\ref{subsec:typingexample}. 
% as indices strictly
% decrease at each recursor application
%and the typing equivalence can be proved
%by \trule{WF}. 

\begin{THM}[Type safety and deadlock-freedom of FFT]
\label{theorem:fft}
For all $\m$, $\emptyset \proves P_{\text{fft}} \APP \m\rhd \emptyset$;  
and if $P_{\text{fft}} \APP  \m \longrightarrow^\ast Q$, then $Q\longrightarrow^\ast
(\Poutend{r_0}{0}{\X_0}\pc\ldots\pc\Poutend{r_{2^\m-1}}{0}{\X_{2^\m-1}})$
where the $\Poutend{r_\pp}{0}{\X_\pp}$ are the actions sending the
final values $\X_\pp$ on external channels $r_\pp$. 
\end{THM}
\begin{proof}
For the proof, we first show 
$P_{\text{fft}} \APP  \m$ 
is typable by a single, multiparty dependent session
(except the answering channel at $r_\pp$).  
Then the result is immediate as a corollary
of progress (Theorem \ref{thm:progress}). 

To prove that 
the processes
are typable against the given global type,  
we start from the end-point projection. 

We assume index $n$ to be a parameter as in Figure~\ref{fig:fft}. 
The main loop is an iteration over the $n$ steps of the
algorithm. Forgetting for now the content of the main loop, the generic
projection for machine $\pp$ has the following skeleton:\\[1mm]
{\small
$\begin{array}{ll}
& \Pi n.(\RECSEQ{(\RECSEQ{\End}{l}{\xx}{(\ldots)}\APP n) \\
& }{k}{\uuu}{\\
& \quad \Pifthenelse{\pp=k}{\Lout{k}{\U}{\Lin{k}{\U}{\uuu}}}{\uuu}})\\
& ~ 2^n\\
\end{array}$} 
\\[1mm]
A simple induction gives us through \trule{WfRecExt} the equivalent type:\\[1mm]
{\small
$\begin{array}{ll}
& \Pi n.\Lout{\pp}{\U}{\Lin{\pp}{\U}{(\RECSEQ{\End}{l}{\xx}{(\ldots)}\APP n)}} \APP 2^n\\
\end{array}$} 
\\[1mm]
We now consider the inner loops. The generic projection gives:\\[1mm]
{\small
$\begin{array}{@{}l@{}l}
& \ldots \\
& \quad (\RECSEQ{\xx}{i}{\yy}{ \\
    & \qquad (\RECSEQ{\yy}{j}{\zz}{ \\
          & \quad \qquad \Pifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j=i*2^{n-l}+j}{\ldots\\
          & \quad \qquad }{\Pifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j}{\Lout{i*2^{n-l}+j}{\U}{\ldots}\\
          & \quad \qquad }{\Pifthenelse{\pp=i*2^{n-l}+j}{\Lin{i*2^{n-l}+2^{n-l-1}+j}{\U}{\ldots}\\
          & \quad \qquad }{\Pifthenelse{\ldots}{\ldots}{\ldots}}}}}\\
    & \qquad)\APP  2^{n-l-1}} \\
  & \quad) \APP 2^l \\
& \ldots \\
\end{array}$}
\\[1mm]
An induction over $\pp$ and some simple arithmetic over binary numbers gives us
through \trule{WfRecExt} the only two branches that can be taken:\\[1mm]
{\small
$\begin{array}{@{}l@{}l}
& \ldots \\
&\Pifthenelse{\bit{n-l}(\pp)=0 \\
& }{\Lin{\pp+2^{n-l-1}}{\U}{\Lout{\pp+2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\Lin{\pp}\U{\xx}}}}\\
& }{\Lout{\pp-2^{n-l-1}}{\U}{\Lin{\pp-2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\Lin{\pp}\U{\xx}}}}}\\
% & \quad (\RECSEQ{\xx}{i}{\yy}{ \\
%     & \qquad (\RECSEQ{\yy}{j}{\zz}{ \\
%           & \quad \qquad \Pifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j=i*2^{n-l}+j}{\ldots\\
%           & \quad \qquad }{\Pifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j}{\Lout{i*2^{n-l}+j}{\U}{\ldots}\\
%           & \quad \qquad }{\Pifthenelse{\pp=i*2^{n-l}+j}{\Lin{i*2^{n-l}+2^{n-l-1}+j}{\U}{\ldots}\\
%           & \quad \qquad }{\Pifthenelse{\ldots}{\ldots}{\ldots}}}}\\
% %          & \quad \qquad \GS{i*2^{n-l}+2^{n-l-1}+j}{i*2^{n-l}+j}{\Nat}.\\
% %          & \quad \qquad \GS{i*2^{n-l}+j}{i*2^{n-l}+2^{n-l-1}+j}{\Nat}.\\
% %          & \quad \qquad \GS{i*2^{n-l}+2^{n-l-1}+j}{i*2^{n-l}+2^{n-l-1}+j}{\Nat}.\\
% %          & \quad \qquad \GS{i*2^{n-l}+j}{i*2^{n-l}+j}{\Nat}.\zz}\\
%     & \qquad)\APP  2^{n-l-1}} \\
%   & \quad) \APP 2^l \\
& \ldots \\
\end{array}$} 
\\[1mm]
The first branch corresponds to the upper part of the butterfly while the second
one corresponds to the lower part.
% The natural projection would be:\\[1mm]
% {\small
% $
% \begin{array}{lll}
% \Pi n.\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{}} \\[1mm]
%   \ (\LR{\End}{\l}{\xx} {\\[1mm]
%     \ 
%    \Pifthenelse{\bit{n-l}(\pp)=0\\
%       \ } {\Lin{\pp+2^{n-l-1}}{\Nat}{\Lout{\pp+2^{n-l-1}}{\Nat}{
%           \Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}\\[1mm]
%       \ } {\Lout{\pp-2^{n-l-1}}{\Nat}{\Lin{\pp-2^{n-l-1}}{\Nat}{
%          \Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}}}) \APP n
% \end{array}
% $
% } 
% \\[1mm]
% The test $\bit{n-l}(\pp)=0$ corresponds to testing the value of
% the $k$ and $k'$ index from the global type. 
% Each of the branches of the test
% have the two sends and two receives corresponding to the butterfly pattern.  
For programming reasons (as seen in the processes, the natural implementation
include sending a first initialisation message with the $x_k$ value), we want to
shift the self-receive $\Lin{\pp}\U{}$ from the initialisation to the beginning
of the loop iteration at the price of adding the last self-receive to the end:
$\Lin{\pp}\U{\End}$. 
The resulting equivalent type up to $\equiv$ is: \\[2mm]
{\small
$
\begin{array}{ll}
\Pi n.\Lout{\pp}{\U}{} \\
 \ (\LR{\Lin{\pp}\U{\End}}{l}{\xx} {\\[1mm]
 \  \Pifthenelse{\bit{n-l}(\pp)=0\\[1mm]
    \ } {\Lin{\pp}\U{\Lin{\pp+2^{n-l-1}}{\U}{\Lout{\pp+2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\xx}}}}\\[1mm]
    \ } {\Lin{\pp}\U{\Lout{\pp-2^{n-l-1}}{\U}{\Lin{\pp-2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\xx}}}}}}) \APP n
\end{array}
$
}\\[1mm]
From this end-point type, it is straightforward to type 
and implement the processes defined in 
Figure~\ref{fig:fft}(d) in \S~\ref{subsec:fft}. 
Hence we conclude the proof. 
\end{proof}


%\subsection{Correctness of FFT processes}
%\noindent 
%\label{subsec:fft:typing}
%%Figure~\ref{fig:fft}(d) gives the local type that each of the machines has to
%%satisfy in order to comply with the global type. 
%We prove here that the processes given in the FFT example in \S~\ref{subsec:fft}
%are typable against the given global type. Their termination
%(i.e.~deadlock-freedom) is then obtained as a corollary.
%We assume index $n$ to be a parameter as in figure~\ref{fig:fft}. 
%The main loop is an iteration over the $n$ steps of the
%algorithm. Forgetting for now the content of the main loop, the generic
%projection for machine $\pp$ has the following skeleton:\\[1mm]
%{\small
%$\begin{array}{ll}
%& \Pi n.(\RECSEQ{(\RECSEQ{\End}{l}{\xx}{(\ldots)}\APP n) \\
%& }{k}{\uuu}{\\
%& \quad \Pifthenelse{\pp=k}{\Lout{k}{\U}{\Lin{k}{\U}{\uuu}}}{\uuu}})\\
%& ~ 2^n\\
%\end{array}$} 
%\\[1mm]
%A simple induction gives us the equivalent type:\\[1mm]
%{\small
%$\begin{array}{ll}
%& \Pi n.\Lout{\pp}{\U}{\Lin{\pp}{\U}{(\RECSEQ{\End}{l}{\xx}{(\ldots)}\APP n)}} \APP 2^n\\
%\end{array}$} 
%\\[1mm]
%We now consider the inner loops. The generic projection gives:\\[1mm]
%{\small
%$\begin{array}{@{}l@{}l}
%& \ldots \\
%& \quad (\RECSEQ{\xx}{i}{\yy}{ \\
%    & \qquad (\RECSEQ{\yy}{j}{\zz}{ \\
%          & \quad \qquad \Pifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j=i*2^{n-l}+j}{\ldots\\
%          & \quad \qquad }{\Pifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j}{\Lout{i*2^{n-l}+j}{\U}{\ldots}\\
%          & \quad \qquad }{\Pifthenelse{\pp=i*2^{n-l}+j}{\Lin{i*2^{n-l}+2^{n-l-1}+j}{\U}{\ldots}\\
%          & \quad \qquad }{\Pifthenelse{\ldots}{\ldots}{\ldots}}}}}\\
%    & \qquad)\APP  2^{n-l-1}} \\
%  & \quad) \APP 2^l \\
%& \ldots \\
%\end{array}$}
%\\[1mm]
%An induction over $\pp$ and some simple arithmetic over binary numbers gives us
%the only two branches that can be taken:\\[1mm]
%{\small
%$\begin{array}{@{}l@{}l}
%& \ldots \\
%&\Pifthenelse{\bit{n-l}(\pp)=0 \\
%& }{\Lin{\pp+2^{n-l-1}}{\U}{\Lout{\pp+2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\Lin{\pp}\U{\xx}}}}\\
%& }{\Lout{\pp-2^{n-l-1}}{\U}{\Lin{\pp-2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\Lin{\pp}\U{\xx}}}}}\\
%% & \quad (\RECSEQ{\xx}{i}{\yy}{ \\
%%     & \qquad (\RECSEQ{\yy}{j}{\zz}{ \\
%%           & \quad \qquad \Pifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j=i*2^{n-l}+j}{\ldots\\
%%           & \quad \qquad }{\Pifthenelse{\pp=i*2^{n-l}+2^{n-l-1}+j}{\Lout{i*2^{n-l}+j}{\U}{\ldots}\\
%%           & \quad \qquad }{\Pifthenelse{\pp=i*2^{n-l}+j}{\Lin{i*2^{n-l}+2^{n-l-1}+j}{\U}{\ldots}\\
%%           & \quad \qquad }{\Pifthenelse{\ldots}{\ldots}{\ldots}}}}\\
%% %          & \quad \qquad \GS{i*2^{n-l}+2^{n-l-1}+j}{i*2^{n-l}+j}{\Nat}.\\
%% %          & \quad \qquad \GS{i*2^{n-l}+j}{i*2^{n-l}+2^{n-l-1}+j}{\Nat}.\\
%% %          & \quad \qquad \GS{i*2^{n-l}+2^{n-l-1}+j}{i*2^{n-l}+2^{n-l-1}+j}{\Nat}.\\
%% %          & \quad \qquad \GS{i*2^{n-l}+j}{i*2^{n-l}+j}{\Nat}.\zz}\\
%%     & \qquad)\APP  2^{n-l-1}} \\
%%   & \quad) \APP 2^l \\
%& \ldots \\
%\end{array}$} 
%\\[1mm]
%The first branch corresponds to the upper part of the butterfly while the second
%one corresponds to the lower part.
%% The natural projection would be:\\[1mm]
%% {\small
%% $
%% \begin{array}{lll}
%% \Pi n.\Lout{\pp}{\Nat}{\Lin{\pp}\Nat{}} \\[1mm]
%%   \ (\LR{\End}{\l}{\xx} {\\[1mm]
%%     \ 
%%    \Pifthenelse{\bit{n-l}(\pp)=0\\
%%       \ } {\Lin{\pp+2^{n-l-1}}{\Nat}{\Lout{\pp+2^{n-l-1}}{\Nat}{
%%           \Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}\\[1mm]
%%       \ } {\Lout{\pp-2^{n-l-1}}{\Nat}{\Lin{\pp-2^{n-l-1}}{\Nat}{
%%          \Lout{\pp}{\Nat}{\Lin{\pp}\Nat{\xx}}}}}}) \APP n
%% \end{array}
%% $
%% } 
%% \\[1mm]
%% The test $\bit{n-l}(\pp)=0$ corresponds to testing the value of
%% the $k$ and $k'$ index from the global type. 
%% Each of the branches of the test
%% have the two sends and two receives corresponding to the butterfly pattern.  
%For programming reasons (as seen in the processes, the natural implementation
%include sending a first initialisation message with the $x_k$ value), we want to
%shift the self-receive $\Lin{\pp}\U{}$ from the initialisation to the beginning
%of the loop iteration at the price of adding the last self-receive to the end:
%$\Lin{\pp}\U{\End}$. 
%The resulting equivalent type up to $\equiv$ is: \\[2mm]
%{\small
%$
%\begin{array}{ll}
%\Pi n.\Lout{\pp}{\U}{} \\
% \ (\LR{\Lin{\pp}\U{\End}}{\l}{\xx} {\\[1mm]
% \  \Pifthenelse{\bit{n-l}(\pp)=0\\[1mm]
%    \ } {\Lin{\pp}\U{\Lin{\pp+2^{n-l-1}}{\U}{\Lout{\pp+2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\xx}}}}\\[1mm]
%    \ } {\Lin{\pp}\U{\Lout{\pp-2^{n-l-1}}{\U}{\Lin{\pp-2^{n-l-1}}{\U}{\Lout{\pp}{\U}{\xx}}}}}}) \APP n
%\end{array}
%$
%}\\[1mm]
%From this local type, it is straightforward to type and implement the processes defined in 
%figure~\ref{fig:fft}(d) in \S~\ref{subsec:fft}. 

%Finally we prove
%type-safety and deadlock-freedom for the FFT processes.  
%Below we let: 
%\[
%\begin{array}{lll}
%P_{\text{fft}}=& \lambda n.(\nu a)(
%\mathbf{R} \ \sr{a}{\p_0..\p_n}{y}{P(n,\p_0,x_{\overline{\p_0}},y)}\\[1mm]
%& \quad \lambda{\ii}.\lambda {\Y}.
%{(\sr{a}{\p_{\ii+1}}{y}{P({\ii+1},\p_{\ii+1},x_{\overline{\p_{\ii+1}}},y)}
%\sep \Y)}\APP n)
%\end{array}
%\] 
%As we reasoned above, each 
%$P(n,\p,x_{\overline{\p}},y)$ is straightforwardly typable 
%by the local type which is equivalent 
%with one  projected from $G$ up to $\equiv$ listed above. Then
%$P_{\text{fft}}$ is typable by 
%the same reasoning as the example in \S~\ref{ex:typingexample}. 
%We also note that once $P_{\text{fft}}$ is applied by any natural
%number $\m$, it eventually terminates 
%since $\m$ strictly decreasing by the definition of the recursor. Hence
%we finally arrive at: 

% \begin{THM}[Type Safety and Deadlock-freedom of FFT]
% \label{theorem:fft}
% For all $\m$, $\emptyset \proves P_{\text{fft}} \APP \m\rhd \emptyset$;  
% and for all $Q$ such that 
% $P_{\text{fft}} \APP  \m \longrightarrow^\ast Q$, we have $Q\longrightarrow^\ast \inact$. 
% \end{THM}

